ECFA Higgs, electroweak, and top Factory Study

The ECFA Higgs, electroweak, and top Factory Study ran between 2021 and 2025 as a broad effort across the experimental and theoretical particle physics communities, bringing together participants from many different proposed future collider projects. Activities across three main working groups advanced the joint development of tools and analysis techniques, fostered new considerations of detector design and optimisation, and led to a new set of studies resulting in improved projected sensitivities across a wide physics programme. This report demonstrates the significant expansion in the state-of-the-art understanding of the physics potential of future e+e- Higgs, electroweak, and top factories, and has been submitted as input to the 2025 European Strategy for Particle Physics Update.

==> ecfa_acknowledgements.tex <==
\noindent {\Large{Acknowledgements}}

\vspace*{5mm}
\noindent This work was supported 
% EU
by the European Research Council, the European Union's Horizon 2020 Research and Innovation programme, and the European Union's NextGenerationEU programme; 
% CERN
by the CERN Strategic Programme on Technologies for Future Experiments (EP-R\&D); 
% Australia 
by the Australian Research Council;
% Belgium
by the Fonds de la Recherche Scientifique (FNRS) and the Research Foundation Flanders (FWO), Belgium;
% Canada
by the Natural Sciences and Engineering Research Council of Canada; 
% China
by the National Natural Science Foundation of China; 
% Croatia
by the Croatian Science Foundation (HRZZ); 
%France
by the CNRS/IN2P3, France;
%Germany
by the Deutsche Forschungsgemeinschaft (DFG, German Research Foundation), the Helmholtz-Gemeinschaft Deutscher Forschungszentren (HGF,  Helmholtz Association of German Research Centres), and the Bundesministerium für Bildung und Forschung (BMBF, German Federal Ministry of Education and Research); 
%Israel
by the ISF and BSF, Israel; 
%Italy
by the INFN and the Italian Ministry of Universities and Research (MUR), Italy;
%Netherlands 
by the NWO, Netherlands; 
%Poland
by the National Science Centre, Poland; 
%Spain
by the Spanish Ministry of Science, Innovation and Universities, 
the Generalitat Valenciana,
the Severo Ochao excellence program, and
the Comunidad Aut\'onoma de Madrid, Spain;
%Serbia
% Serbia
by the Science Fund of the Republic of Serbia; 
%Sweden 
by the Swedish Research Council and the Carl Trygger Foundation, Sweden; 
%Switzerland
by the Swiss National Science Foundation;
%UK
by the Science and Technology Facilities Council, the Leverhulme Trust, and the Royal Society, United Kingdom;
%USA
and by the Department of Energy and
the National Science Foundation, United States.


==> ecfa_authors_p3_YR2format_250213d.tex <==
% Author list for 'ECFA Higgs/top/electroweak Factory Study Report' in YR2 format
% automatically generated on 2025-02-13 at 10:02:50 UTC
% via https://www.ppe.gla.ac.uk

%Australia, University of Adelaide
\addauthor{
A.~Desai$^{0}$\\
\emph{The University of Adelaide, Adelaide, SA 5005, Australia}
}

%Belgium, Ghent University
\addauthor{
K.~Skovpen\\
\emph{Ghent University, Proeftuinstraat 86, 9000 Gent, Belgium}
}

%Belgium, Université catholique de Louvain
\addauthor{
M. ~Drewes,
G.~Durieux,
Y.~Georis,
Y.~Ma\\
\emph{Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, 1348 Louvain-la-Neuve, Belgium}
}

%Belgium, Vrije Universiteit Brussel
\addauthor{
A.~De Moor,
K.~Gautam$^{1}$,
E.~Ploerer$^{1}$\\
\emph{Vrije Universiteit Brussel,
Bd de la Plaine 2, 1050 Ixelles, Belgium}
}

%Brazil, Universidade do Estado do Rio de Janeiro
\addauthor{
K.~Mota~Amarilo\\
\emph{Universidade do Estado do Rio de Janeiro, Rio de Janeiro, Brazil}
}

%Canada, TRIUMF
\addauthor{
M.J.~Basso$^{2}$\\
\emph{TRIUMF, Wesbrook Mall, Vancouver, Canada}
}

%China, Hefei University of Technology
\addauthor{
Y.~Zhang\\
\emph{School of Physics, Hefei University of Technology, Hefei 230601, China}
}

%China, Institute of High Energy Physics, Chinese Academy of Sciences
\addauthor{
X.-H.~Jiang$^{3}$,
Bin Yan\\
\emph{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
}

%China, Peking University
\addauthor{
Xin-Kai Wen\\
\emph{School of Physics, Peking University, Beijing 100871, China}
}

%China, Sun Yat-sen University
\addauthor{
J.~Liao\\
\emph{School of Physics, Sun Yat-sen University, Guangzhou, 510275, China}
}

%China, Sun Yat-sen University (Shenzhen)
\addauthor{
C.~Li\\
\emph{Sun Yat-sen University (SYSU), Shenzhen, 518107, China}
}

%Croatia, Rudjer Boskovic Institute
\addauthor{
T.~Robens\\
\emph{Rudjer Boskovic Institute, Bijenicka cesta 54, 10000 Zagreb, Croatia}
}

%Denmark, Niels Bohr Institute, Copenhagen University
\addauthor{
M.~Dam\\
\emph{Niels Bohr Institute, Copenhagen University, Jagtvej 155, 2200 Copenhagen, Denmark}
}

%France, APC, Laboratoire AstroParticule et Cosmologie, Paris
\addauthor{
G.~Bernardi,
K.~Dewyspelaere,
A.~Maloizel,
G.~Marchiori\\
\emph{APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, Paris, France}
}

%France, Institut de Physique des 2 Infinis de Lyon IN2P3-CNRS/Université Claude Bernard Lyon 1
\addauthor{
S.~Gascon-Shotkin,
E.~Jourd'huy,
C.~Verollet,
J.~Xiao\\
\emph{Institut de Physique des 2 Infinis de Lyon IN2P3-CNRS, rue Enrico Fermi
69622 Villeurbanne Cedex, France}
}

%France, Institut Polytechnique des Sciences Avancées
\addauthor{
R.~Perez-Ramos$^{4}$\\
\emph{DRII-IPSA, 94200 Ivry-sur-Seine, France}
}

%France, Laboratoire de Physique de Clermont Auvergne, Université Clermont Auvergne, CNRS/IN2P3
\addauthor{
R.~Madar,
T.~Miralles,
S.~Monteil\\
\emph{LPCA, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand, France}
}

%France, Laboratoire de physique des 2 infinis Irène Joliot-Curie
\addauthor{
I.~Combes,
N.~Morange,
R.~P\"oschl,
F.~Richard\\
\emph{IJCLab, Universit\'e Paris-Saclay, CNRS/IN2P3, 91405 Orsay, France}
}

%France, Laboratoire de Physique Théorique et Hautes Energies
\addauthor{
G.~Cacciapaglia\\
\emph{Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), Sorbonne Universit\'e et CNRS, 75252 Paris, France}
}

%France, LAPP, Université Savoie Mont Blanc, CNRS/IN2P3, Annecy
\addauthor{
O.~Arnaez,
M.~Delmastro,
H.~Taibi,
Z.~Wu\\
\emph{LAPP, 9 Chem. de Bellevue, 74940 Annecy, France}
}

%Germany, Albert-Ludwigs-Universität Freiburg
\addauthor{
M.G.~Gabelmann\\
\emph{Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany}
}

%Germany, CNRS Helmholtz Dark Matter Lab
\addauthor{
D.~Zerwas\\
\emph{DMLab, Deutsches Elektronen-Synchrotron DESY, CNRS/IN2P3, Hamburg, Germany}
}

%Germany, DESY Hamburg
\addauthor{
J.~Alimena,
M.~Berggren,
F.~Blekman,
B.~Bliewert,
J.~Braathen,
A.~Filipe Silva,
F.~Gaede,
C.~Grojean,
J.~List,
T.~Madlener,
A.B.~Meyer,
M.T.~N\'u\~nez Pardo de Vera,
K.~Radchenko Serdula,
J.~Reuter,
F.~Sefkow,
J.~Torndal,
A.~Verduras Schaeidt,
G.~Weiglein\\
\emph{DESY, Hamburg, Germany}
}

%Germany, II. Physikalisches Institut, Georg-August-Universität Göttingen
\addauthor{
K.~K\"oneke\\
\emph{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"ottingen, G\"ottingen, Friedrich-Hund-Platz 1, 37077 G\"ottingen, Germany}
}

%Germany, Johannes Gutenberg Universität Mainz
\addauthor{
F.~Yu\\
\emph{PRISMA+ Cluster of Excellence and Mainz Institute for Theoretical Physics, Johannes Gutenberg University, 55099 Mainz, Germany}
}

%Germany, Karlsruhe Institute of Technology
\addauthor{
S.~Alshamaily,
G.~Brodbek,
U.~Einhaus,
S.~Giappichini,
P.~Goldenzweig,
S.~Keilbach,
J.~Kieseler,
M.~Klute,
M.~Presilla,
F.~Simon,
A.~Wiedl,
X.~Zuo\\
\emph{Karlsruhe Institute of Technology, Karlsruhe, Germany}
}

%Germany, Max-Planck-Institut für Physik
\addauthor{
P.~Lo Chiatto$^{5}$\\
\emph{Max-Planck-Institut f{\"u}r Physik, Boltzmannstra{\ss}e 8, 85748 Garching bei M{\"u}nchen, Germany}
}

%Germany, Rheinische Friedrich-Wilhems-Universität Bonn
\addauthor{
P.~Bechtle,
M.~Vellasco\\
\emph{University of Bonn, Physikalisches Institute, Nussallee 12, 53115 Bonn, Germany}
}

%Germany, TU Dortmund University
\addauthor{
J.~Albrecht,
K.~Kr\"oninger,
L.~R\"ohrig$^{6}$\\
\emph{Department of Physics, Otto-Hahn-Str. 4a, 44225 Dortmund, Germany}
}

%Germany, Universität Heidelberg
\addauthor{
H.~Bahl\\
\emph{Universit\"at Heidelberg, Heidelberg, Germany}
}

%Germany, University of Hamburg
\addauthor{
A.~Grohsjean,
G.~Moortgat-Pick\\
\emph{University of Hamburg, Hamburg, Germany}
}

%Iran, Institute for Research in Fundamental Sciences
\addauthor{
M.~Mohammadi Najafabadi,
M.~Nourbakhsh,
S. ~Tizchang$^{7}$\\
\emph{School of Particles and Accelerators, Institute for Research in Fundamental Sciences (IPM), Artesh Highway, Tehran 1956836681, Iran}
}

%Iran, Isfahan University of Technology
\addauthor{
Z.~Baharyioon,
A.~Jafari\\
\emph{Department of Physics, Isfahan University of Technology, Isfahan, 84156-83111, Iran}
}

%Iran, University of Tehran
\addauthor{
A.~Amiri$^{8}$,
K.~Azizi$^{9}$,
F.~Fatehi,
R.~Jafariseyedabad$^{8}$,
M. ~Malekhosseini,
S. ~Rostami\\
\emph{Department of Physics, University of Tehran, North Karegar Avenue, Tehran 14395-547, Iran}
}

%Ireland, Dublin Institute for Advanced Studies
\addauthor{
V.~Keus\\
\emph{Dublin Institute of Advanced Studies (DIAS), 10 Burlington Road, Dublin 4, Ireland}
}

%Israel, Technion – Israel Institute of Technology
\addauthor{
Y.~Soreq\\
\emph{Physics Department, Technion - Israel Institute of Technology, Haifa 3200003, Israel}
}

%Italy, INFN Laboratori Nazionali di Frascati
\addauthor{
E.~Bagnaschi,
F.~Mescia\\
\emph{INFN, Laboratori Nazionali di Frascati, Via E. Fermi 40, 00044 Frascati, Italy}
}

%Italy, INFN Milan
\addauthor{
A.~Andreazza$^{10}$,
C.~Meroni$^{10}$,
F.~Sabatini,
R.~Zanzottera$^{10}$,
M.~Zaro$^{11}$\\
\emph{INFN Sezione di Milano, Via Celoria 16, 20133 Milano, Italy}
}

%Italy, INFN Sezione di Bologna
\addauthor{
G.L.~Alberghi,
L.~Bellagamba\\
\emph{Viale Carlo Berti Pichat 6/2, 40127 Bologna, Italy}
}

%Italy, INFN Sezione di Firenze
\addauthor{
M.~Tammaro\\
\emph{INFN Sezione di Firenze, Via G. Sansone 1, 50019 Sesto Fiorentino, Italy}
}

%ITALY, INFN Sezione di Lecce
\addauthor{
E.G.~Gorini,
F.G.~Grancagnolo,
M.P.~Primavera\\
\emph{INFN Sezione di Lecce, Lecce, Italy}
}

%Italy, INFN Sezione di Padova
\addauthor{
P.~Azzi,
A. ~De Vita,
N.~Selimovi\'c\\
\emph{INFN Sezione di Padova, Via Marzolo 8, 35100 Padova, Italy}
}

%Italy, INFN Sezione di Pavia
\addauthor{
C.~Carloni Calame,
M.~Chiesa,
O.~Nicrosinii,
F.~Piccinini,
G.~Polesello,
N.~Valle\\
\emph{INFN Sezione di Pavia, via A. Bassi 6, 27100 Pavia, Italy}
}

%Italy, INFN Sezione di Perugia
\addauthor{
S.~Ajmal,
O. ~Panella\\
\emph{INFN Sezione di Perugia, Via A. Pascoli, 06123, Perugia, Italy}
}

%Italy, INFN Sezione di Pisa
\addauthor{
P. ~Azzurri,
D.~Barducci$^{12}$,
D.~Buttazzo,
A.~Dondarini$^{12}$,
A.~Korajac,
G.~Marino$^{12}$,
F.~Palla,
P.~Panci$^{12}$\\
\emph{INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy}
}

%Italy, INFN Sezione di Trieste
\addauthor{
D.~Marzocca$^{13}$\\
\emph{INFN Trieste, Via Valerio 2, 34127 Trieste, Italy}
}

%Italy, Milan University
\addauthor{
A.~Vicini\\
\emph{TIFLab, Universit\`a degli Studi di Milano, Via Celoria 16, 20133 Milano, Italy}
}

%Italy, Politecnico di Bari
\addauthor{
N.~De~Filippis$^{14}$,
F.M.~Procacci$^{14}$\\
\emph{Politecnico di Bari, Via Orabona 4, 70126 Bari, Italy}
}

%Italy, Scuola Normale Superiore
\addauthor{
Alberto Lusiani$^{15}$\\
\emph{Scuola Normale Superiore, Piazza dei Cavalieri 7, 56126 Pisa, Italy}
}

%Italy, Università degli Studi di Padova
\addauthor{
B.~Erdelyi$^{16}$,
R.~Gr\"ober$^{16}$,
A.~Rossia$^{16}$\\
\emph{Dipartimento di Fisica e Astronomia "G. Galilei", Universit\`a degli Studi di Padova, Via F. Marzolo 8, I-35131, Italy}
}

%Italy, Università di Pavia
\addauthor{
G.~Montagna$^{17}$,
F.~Ucci$^{17}$\\
\emph{Universit\`a di Pavia, 27100 Pavia, Italy}
}

%Italy, University of Udine
\addauthor{
M.~Cobal$^{18}$,
G.~Panizzo$^{18}$,
M.~Pinamonti$^{19}$,
L.~Pintucci$^{18}$,
L.~Toffolin$^{18}$\\
\emph{University of Udine, Via delle Scienze 206, Udine, Italy}
}

%Italy, Universit`a degli Studi di Roma la Sapienza
\addauthor{
M.~Bulliri\\
\emph{Universit`a degli Studi di Roma la Sapienza, Piazzale Aldo Moro 5, 00185, Roma, Italy}
}

%Italy, Universit`a degli Studi Roma Tre
\addauthor{
R.~Franceschini\\
\emph{Universit\`a degli Studi Roma Tre, Via della Vasca Navale 84, I-00146, Rome, Italy}
}

%Japan, High Energy Accelerator Research Organization
\addauthor{
D. ~Jeans,
J.~Nakajima\\
\emph{KEK, Tsukuba, Japan}
}

%Japan, Tokyo Gakugei University
\addauthor{
K.~Hidaka\\
\emph{Tokyo Gakugei University, Koganei, Tokyo 184-8501, Japan}
}

%Morocco, Cadi Ayyad University
\addauthor{
M.~Ouchemhou\\
\emph{Polydisciplinary Faculty, Laboratory of Fundamental and Applied Physics, Cadi Ayyad University, Sidi Bouzid, B.P. 4162, Safi, Morocco}
}

%Poland, AGH University of Krakow
\addauthor{
H.~Khanpour\\
\emph{AGH University, Faculty of Physics and Applied Computer Science, Al. Mickiewicza 30, 30-055 Krak\'ow, Poland}
}

%Poland, Institute of Nuclear Physics Polish Academy of Sciences
\addauthor{
M.~Skrzypek\\
\emph{The Henryk Niewodnicza\'nski
Institute of Nuclear Physics
Polish Academy of Sciences
ul. Radzikowskiego 152,
31-342 Krak\'ow, Poland}
}

%Poland, Jagiellonian University in Krakow
\addauthor{
A.~Price,
W.~P{\l}aczek,
A.~Si\'odmok\\
\emph{Faculty of Physics, Astronomy and Applied Computer Science, ul. Lojasiewicza 11, 30-348 Krak\'ow, Poland}
}

%Poland, University of Warsaw
\addauthor{
B.~Brudnowski,
J.~Kalinowski,
J.~Klamka,
K.~Mekala$^{20}$,
K.~Sakurai,
A.F.~\.Zarnecki,
K.~Zembaczy\'nski\\
\emph{Faculty of Physics, University of Warsaw, Warsaw, Poland}
}

%Portugal, Centro de Física Teórica de Partículas, Instituto Superior Técnico, Universidade de Lisboa
\addauthor{
J.~Hajer,
B.~Oliveira\\
\emph{Centro de F\'isica Te\'orica de Part\'iculas (CFTP), Instituto Superior T\'ecnico (IST), Universidade de Lisboa, 1049-001 Lisboa, Portugal}
}

%Portugal, Laboratório de Instrumentação e Física Experimental de Partículas
\addauthor{
N.F.~Castro$^{21}$,
G.~Chachamis$^{22}$\\
\emph{LIP -- Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas, Escola de Ci\`encias, Campus de Gualtar, Universidade do Minho, 4701-057 Braga, Portugal}
}

%%Russian Federation, Joint Institute for Nuclear Research
%\addauthor{
%A.~Nesterenko\\
%\emph{Joint Institute for Nuclear Research, Dubna, 141980, Russian Federation}
%}
%
%%Russian Federation, National Research Nuclear University MEPhI
%\addauthor{
%V. A.~Okorokov\\
%\emph{National Research Nuclear University MEPhI, Kashirskoe shosse 31, 115409 Moscow, Russian Federation}
%}

%Serbia, Vinca Institute of Nuclear Sciences
\addauthor{
I.~Bozovic$^{23}$,
G.~Kacarevic,
I.~Smiljanic,
I.~Vidakovic,
N.~Vukasinovic\\
\emph{Vin\v{c}a Institute of Nuclear Sciences, University of Belgrade, Belgrade, Serbia}
}

%Spain, Centro de Investigaciones  Energéticas, Medioambientales y Tecnológicas
\addauthor{
J.~Alcaraz Maestre$^{24}$,
M.~Cepeda$^{24}$,
M.C.~Fouz$^{24}$\\
\emph{Centro de Investigaciones  Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT)
Madrid, Spain}
}

%Spain, IFIC, CSIC-Universitat de València
\addauthor{
A.~Irles,
L.~Mantani,
V.A.~Mitsou,
M.~Moreno~Ll\'acer,
E.~Musumeci,
B.~Pattnaik,
M.A.~Sanchis,
M.~Vos\\
\emph{IFIC, CSIC-Universitat de Val\`encia, Valencia, Spain}
}

%Spain, Instituto de Física Teórica, CSIC-Universidad Autónoma de Madrid
\addauthor{
J.A.~Aguilar-Saavedra,
S.~Heinemeyer,
A.~Sabio Vera$^{25}$\\
\emph{Instituto de F\'isica Te\'orica, CSIC-Universidad Aut\'onoma de Madrid, Madrid, Spain}
}

%Spain, Instituto Galego de Física de Altas Enerxías (IGFAE), Universidade de Santiago de Compostela
\addauthor{
I.~Corredoira\\
\emph{Instituto Galego de F\'isica de Altas Enerx\'ias (IGFAE), Universidade de Santiago de Compostela
Santiago de Compostela, Spain}
}

%Spain, Universidad de Cordoba
\addauthor{
F.~Cornet-Gomez\\
\emph{Campus Universitario de Rabanales, Ctra. N-IVa, Km. 396. 14071, Cordoba, Spain}
}

%Spain, Universidad de Granada
\addauthor{
Mikael Chala,
Jorge de Blas\\
\emph{Departamento de F\'isica Te\'orica y del Cosmos, Universidad de Granada,
Campus de Fuentenueva, 18071 Granada, Spain}
}

%Sweden, KTH Royal Institute of Technology
\addauthor{
M.~Vande Voorde\\
\emph{Department of Physics, Royal Institute of Technology, Stockholm; Sweden}
}

%Sweden, Lund University
\addauthor{
T.~Sj\"ostrand\\
\emph{Department of Physics, Lund University, Lund, Sweden}
}

%Sweden, Uppsala University
\addauthor{
A.~Gall\'en,
R.~Gonzalez Suarez,
G.~Ripellino\\
\emph{Department of Physics and Astronomy, Uppsala University, L{\"a}gerhyggsv{\"a}gen 1, Uppsala, 752 37, Sweden}
}

%Switzerland, CERN
\addauthor{
J.~Aebischer,
M.~Al-Thakeel,
S.~Aumiller,
V.~Cairo,
J.M.~Carceller,
D.~d'Enterria,
J.~Davighi,
M.~Defranchis,
M.~Di Carlo,
F.~Erben,
B.~Francois,
G.~Ganis,
D.~Garcia,
G.~Guerrieri,
A.~J\"uttner,
S.~Kuberski,
A.~Mehta,
L.~Reichenbach$^{26}$,
A.~Sailer,
M.~Selvaggi,
J.~Smiesko,
A.~Tolosa-Delgado,
J.~T.~Tsang\\
\emph{CERN, Geneva, Switzerland}
}

%Switzerland, Eidgenössische Technische Hochschule Zürich
\addauthor{
S.~Thor\\
\emph{ETH Z\"{u}rich, 8092 Z\"{u}rich, Switzerland}
}

%Switzerland, Université de Genève
\addauthor{
T.~Critchley,
P.~Kontaxakis,
A.~Sfyrla\\
\emph{D\'epartement de Physique Nucl\'eaire et Corpusculaire (DPNC), Universit\'e de Gen\`eve, 1205 Gen\`eve, Switzerland}
}

%Switzerland, University of Basel
\addauthor{
S.~Antusch,
A.~Greljo\\
\emph{Department of Physics, University of Basel, 4056 Basel, Switzerland}
}

%Switzerland, University of Zurich
\addauthor{
M.~Bordone$^{27}$,
F.~Canelli,
A.~Ilg,
G.~Isidori,
B.~Kilminster,
T.H.~Kwok,
V.~Lukashenko,
A.~Macchiolo,
Z.~Polonsky\\
\emph{Physik-Institut, University of Zurich, 8057 Z\"urich, Switzerland}
}

%The Netherlands, Nikhef
\addauthor{
P.~Koppenburg,
J.~Rojo$^{28}$\\
\emph{Nikhef Theory Group, Science Park 105, 1098 XG Amsterdam, The Netherlands}
}

%The Netherlands, University of Amsterdam
\addauthor{
J.~Klari\'c$^{29}$\\
\emph{University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands}
}

%UK, University of Oxford
\addauthor{
P.N.~Burrows,
C.~Hays\\
\emph{Department of Physics, University of Oxford, Oxford OX1 5NZ, UK}
}

%United Kingdom, Imperial College London
\addauthor{
E.~Curtis,
A.-M.~Magnan,
N.~Wardle\\
\emph{The Blackett Laboratory, Imperial College, London SW7 2BW, United Kingdom}
}

%United Kingdom, University of Edinburgh
\addauthor{
C.~Leonidopoulos,
J.~ter Hoeve\\
\emph{University of Edinburgh, Edinburgh EH9 3FD, United Kingdom}
}

%United Kingdom, University of Glasgow
\addauthor{
C.~Englert,
M.~Miralles L\'opez,
J.~Nesbitt,
D.~Protopopescu,
S.~Renner,
A.~Robson,
Y.~Zhang\\
\emph{University of Glasgow, Glasgow G12 8QQ, Scotland, United Kingdom}
}

%United Kingdom, University of Manchester
\addauthor{
E.~Celada,
V.~Miralles,
A.~Pilkington,
M.~Thomas,
E.~Vryonidou\\
\emph{University of Manchester, Manchester M13 9PL, United Kingdom}
}

%United Kingom, Cavendish Laboratory, University of Cambridge
\addauthor{
J.~Hayward,
S.~Williams\\
\emph{Cavendish Laboratory, University of Cambridge, Cambridge CB3 0HE, United Kingom}
}

%USA, Baylor University
\addauthor{
B.F.L.~Ward\\
\emph{Baylor University, Waco, TX 76798-7316, USA}
}

%USA, Brookhaven National Laboratory
\addauthor{
H.~Abidi,
K.A.~Assamagan,
D.~Boye,
E.~Brost,
V.~Cavaliere,
A.E.~Connelly,
~C. L. Del Pio,
G.~Iakovidis,
A.~Li,
M.A.~Pleier,
A.~Sciandra,
S.~Snyder,
R.H.~Szafron,
A.~Tishelman-Charny,
I.~Veli\v{s}\v{c}ek\\
\emph{Brookhaven National Laboratory, Upton, NY 11973-5000, USA}
}

%USA, Brown University
\addauthor{
L.~Gouskos,
L.~Li\\
\emph{Brown University, 182 Hope Street, Providence, RI 02912, USA}
}

%USA, Jefferson Lab
\addauthor{
Z.~Yu\\
\emph{Theory Center, Jefferson Lab, Newport News, Virginia 23606, USA}
}

%USA, Johns Hopkins University
\addauthor{
A. ~Gritsan,
N.~Pinto\\
\emph{Johns Hopkins University, Baltimore, Maryland 21218, USA}
}

%USA, Massachusetts Institute of Technology
\addauthor{
J.~Eysermans\\
\emph{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
}

%USA, Michigan State University
\addauthor{
R.~Schwienhorst,
C.-P.~Yuan$^{30}$\\
\emph{Department of Physics and Astronomy, Michigan State University, East Lansing, Michigan 48824, USA}
}

%USA, Northeastern University
\addauthor{
M.~Larson,
L.~Skinnari\\
\emph{Northeastern University, Boston, Massachusetts 02115, USA}
}

%USA, Princeton University
\addauthor{
W.~Chung,
L. S.~Mandacar\'{u} Guerra\\
\emph{Princeton University, Princeton, New Jersey 08544, USA}
}

%USA, SLAC National Accelerator Laboratory
\addauthor{
D.~Ntounis,
C.~Vernieri\\
\emph{SLAC, 2575 Sand Hill Rd, Menlo Park, CA 94025, USA}
}

%USA, Texas Tech University
\addauthor{
V. ~Slokenbergs\\
\emph{Texas Tech University, Lubbock, Texas, 79409, USA}
}

%USA, University of California, Davis
\addauthor{
H.-C.~Cheng\\
\emph{University of California, One Shields Avenue, Davis, California, USA}
}

%USA, University of California, Santa Cruz
\addauthor{
W.~Altmannshofer\\
\emph{University of California, Santa Cruz, CA 95064, USA}
}

%USA, University of Cincinnati
\addauthor{
M.~Szewc$^{31}$\\
\emph{Department of Physics, University of Cincinnati, Cincinnati, Ohio 45221, USA}
}

%USA, University of Pittsburgh
\addauthor{
A.~Freitas\\
\emph{University of Pittsburgh, Pittsburgh, PA 15260, USA}
}

%USA, University of Wisconsin-Madison
\addauthor{
S.~Dasu,
A.~Mohammadi,
C.-H.~Nee\\
\emph{University of Wisconsin-Madison, Madison, WI 53706-1390, USA}
}


%%Russian Federation
\addauthor{
A.~Nesterenko\\
V. A.~Okorokov\\
\emph{Affiliated with an institute covered by a cooperation agreement with CERN}
}

\addauthor{
\begin{flushleft}
{$^{0}$}Also at: ARC Centre of Excellence for Dark Matter Particle Physics, Australia\\
{$^{1}$}Also at: Physik-Institut, University of Zurich, 8057 Z\"urich, Switzerland\\
{$^{2}$}Also at: Department of Physics, Simon Fraser University, University Drive W, Burnaby, Canada\\
{$^{3}$}Also at: China Center of Advanced Science and Technology, Beijing, China\\
{$^{4}$}Also at: Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), Sorbonne Universit\'e et CNRS, Paris\\
{$^{5}$}Also at: Weizmann Institute of Science, 234 Herzl Street, POB 26, Rehovot 7610001, Israel\\
{$^{6}$}Also at: LPCA, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand, France\\
{$^{7}$}Also at: Physics Department, Faculty of Sciences, Arak University, Arak\\
{$^{8}$}Also at: Department of Physics, Faculty of Science, Ferdowsi University of Mashhad, Mashhad, Iran\\
{$^{9}$}Also at: Department of Physics, Do\v{g}u\c{s} University, Dudullu-\"{U}mraniye, 34775 Istanbul, T\"urkiye\\
{$^{10}$}Also at: Dipartimento di Fisica, Università degli Studi di Milano, 20133 Milano, Italy\\
{$^{11}$}Also at: TIFLab, Università degli Studi di Milano, 20133 Milano, Italy\\
{$^{12}$}Also at: Universit\`a di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy\\
{$^{13}$}DM acknowledges support by the Italian Ministry of University and Research (MUR) via the PRIN project n. 20224JR28W.\\
{$^{14}$}Also at: INFN Sezione di Bari, Via Orbona 4, 70126 Bari, Italy\\
{$^{15}$}Also at: INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy\\
{$^{16}$}Also at: INFN Sezione di Padova, Via Marzolo 8, 35100 Padova, Italy\\
{$^{17}$}Also at: INFN Sezione di Pavia, via A. Bassi 6, 27100 Pavia, Italy\\
{$^{18}$}Also at: INFN Gruppo Collegato di Udine\\
{$^{19}$}Also at: INFN Trieste, Via Valerio 2, 34127 Trieste, Italy\\
{$^{20}$}Also at: DESY, Hamburg, Germany\\
{$^{21}$}Also at: Departamento de F\'{i}sica, Escola de Ci\^{e}ncias, Universidade do Minho, 4710-057 Braga, Portugal\\
{$^{22}$}Also at: LIP -- Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas, Lisboa, Portugal\\
{$^{23}$}Supported by Fund of Science RS, Grant IDEJE HIGHTONE-P\\
{$^{24}$}Grant PID2021-122134NB-C22 funded by MICIU/AEI/10.13039/501100011033\\
{$^{25}$}Also at: Universidad Autonoma de Madrid, E-28049 Madrid, Spain\\
{$^{26}$}Also at: University of Bonn, Physikalisches Institut, Nussallee 12, 53115 Bonn\\
{$^{27}$}Also at: CERN, Geneva, Switzerland\\
{$^{28}$}Also at: Department of Physics and Astronomy, Vrije Universiteit, NL-1081 HV Amsterdam, The Netherlands\\
{$^{29}$}Also at: University of Zagreb, Bijeni\v{c}ka c. 32, 10000 Zagreb, Croatia\\
{$^{30}$}Supported by the U.S. National Science Foundation under Grant No.~PHY-2310291.\\
{$^{31}$}MS acknowledges support in part by NSF grants OAC-2103889, OAC-2411215 and OAC-2417682 and by DOE grant DE-SC101977.
Also at International Center for Advanced Studies (ICAS), ICIFI and ECyT-UNSAM, 25 de Mayo y Francia, 1650 San Mart\'{i}n, Buenos Aires, Argentina\\
%{$^*$}Editors ({\ttfamily \href{mailto:ecfa-editors@cern.ch}{ecfa-editors@cern.ch}})
\end{flushleft}
}



==> ecfa_authors_p3_YR2format_250220.tex <==
% Author list for 'ECFA Higgs/top/electroweak Factory Study Report' in YR2 format
% automatically generated on 2025-02-20 at 14:02:42 UTC
% via https://www.ppe.gla.ac.uk

%Australia, Monash University
\addauthor{
J.~Altmann,
P.~Skands\\
\emph{Monash University, Wellington Road, Clayton VIC-3800, Australia}
}

%Australia, University of Adelaide
\addauthor{
A.~Desai$^{0}$\\
\emph{The University of Adelaide, Adelaide, SA 5005, Australia}
}

%Austria, Institute of High Energy Physics, Vienna
\addauthor{
W.~Mitaroff\\
\emph{Institute of High Energy Physics, Austrian Academy of Sciences, 1050 Vienna, Austria}
}

%Austria, University of Graz
\addauthor{
S.~Pl\"atzer$^{1}$\\
\emph{Institute of Physics, NAWI Graz, University of Graz, Universit\"atsplatz 5, 8010 Graz, Austria}
}

%Belgium, Ghent University
\addauthor{
D.~Dobur,
K.~Skovpen\\
\emph{Ghent University, Proeftuinstraat 86, 9000 Gent, Belgium}
}

%Belgium, Université catholique de Louvain
\addauthor{
M. ~Drewes,
G.~Durieux,
Y.~Georis,
Y.~Ma\\
\emph{Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, 1348 Louvain-la-Neuve, Belgium}
}

%Belgium, Vrije Universiteit Brussel
\addauthor{
A.~De Moor,
K.~Gautam$^{2}$,
E.~Ploerer$^{2}$,
M.~Tytgat\\
\emph{Inter-University Institute for High Energies, Vrije Universiteit Brussel,
Pleinlaan 2, 1050 Ixelles, Belgium}
}

%Brazil, Universidade do Estado do Rio de Janeiro
\addauthor{
K.~Mota~Amarilo\\
\emph{Universidade do Estado do Rio de Janeiro, Rio de Janeiro, Brazil}
}

%Canada, TRIUMF
\addauthor{
M.J.~Basso$^{3}$\\
\emph{TRIUMF, Wesbrook Mall, Vancouver, Canada}
}

%China, Fudan University
\addauthor{
J.~Gu\\
\emph{Department of Physics and Center for Field Theory and Particle Physics, Fudan University,
Shanghai 200438, China}
}

%China, Hefei University of Technology
\addauthor{
Y.~Zhang\\
\emph{School of Physics, Hefei University of Technology, Hefei 230601, China}
}

%China, Institute of High Energy Physics, Chinese Academy of Sciences
\addauthor{
X.-H.~Jiang$^{4}$,
Bin Yan\\
\emph{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
}

%China, Peking University
\addauthor{
X.-K. Wen\\
\emph{School of Physics, Peking University, Beijing 100871, China}
}

%China, Sun Yat-sen University
\addauthor{
J.~Liao\\
\emph{School of Physics, Sun Yat-sen University, Guangzhou, 510275, China}
}

%China, Sun Yat-sen University (Shenzhen)
\addauthor{
C.~Li\\
\emph{School of Science, Sun Yat-sen University (SYSU), Shenzhen, 518107, China}
}

%Croatia, Rudjer Boskovic Institute
\addauthor{
T.~Robens\\
\emph{Rudjer Boskovic Institute, Bijenicka cesta 54, 10000 Zagreb, Croatia}
}

%Denmark, Niels Bohr Institute, Copenhagen University
\addauthor{
M.~Dam\\
\emph{Niels Bohr Institute, Copenhagen University, Jagtvej 155, 2200 Copenhagen, Denmark}
}

%France, APC, Laboratoire AstroParticule et Cosmologie, Paris
\addauthor{
G.~Bernardi,
K.~Dewyspelaere,
A.~Maloizel,
G.~Marchiori\\
\emph{APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, Paris, France}
}

%France, Institut de Physique des 2 Infinis de Lyon IN2P3-CNRS/Université Claude Bernard Lyon 1
\addauthor{
S.~Gascon-Shotkin,
E.~Jourd'huy,
C.~Verollet,
J.~Xiao\\
\emph{Institut de Physique des 2 Infinis de Lyon IN2P3-CNRS, rue Enrico Fermi
69622 Villeurbanne Cedex, France}
}

%France, Institut Polytechnique des Sciences Avancées
\addauthor{
R.~Perez-Ramos$^{5}$\\
\emph{DRII-IPSA, 94200 Ivry-sur-Seine, France}
}

%France, Laboratoire de Physique de Clermont Auvergne, Université Clermont Auvergne, CNRS/IN2P3
\addauthor{
R.~Madar,
T.~Miralles,
S.~Monteil\\
\emph{LPCA, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand, France}
}

%France, Laboratoire de physique des 2 infinis Irène Joliot-Curie
\addauthor{
Y.~Amhis,
I.~Combes,
N.~Morange,
R.~P\"oschl,
M.~Reboud,
F.~Richard,
O.~Sumensari\\
\emph{IJCLab, Universit\'e Paris-Saclay, CNRS/IN2P3, 91405 Orsay, France}
}

%France, Laboratoire de Physique Théorique et Hautes Energies
\addauthor{
G.~Cacciapaglia\\
\emph{Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), Sorbonne Universit\'e et CNRS, 75252 Paris, France}
}

%France, Laboratoire Leprince-Ringuet
\addauthor{
V.~Balagura,
V.~Boudry,
J.-C.~Brient,
C.~Charlot,
C.~Ochando,
R.~Salerno,
Y.~Shi,
Y.~Sirois\\
\emph{Laboratoire Leprince-Ringuet, Ecole Polytechnique, 91128 Palaiseau, France}
}

%France, LAPP, Université Savoie Mont Blanc, CNRS/IN2P3, Annecy
\addauthor{
O.~Arnaez,
M.~Delmastro,
H.~Taibi,
Z.~Wu\\
\emph{LAPP, 9 Chem. de Bellevue, 74940 Annecy, France}
}

%Germany, Albert-Ludwigs-Universität Freiburg
\addauthor{
S.D.~Dittmaier,
M.~Gabelmann\\
\emph{Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany}
}

%Germany, CNRS Helmholtz Dark Matter Lab
\addauthor{
D.~Zerwas\\
\emph{DMLab, Deutsches Elektronen-Synchrotron DESY, CNRS/IN2P3, Hamburg, Germany}
}

%Germany, DESY Hamburg
\addauthor{
J.~Alimena,
M.~Berggren,
F.~Blekman$^{6}$,
B.~Bliewert,
J.~Braathen,
A.~Filipe Silva,
F.~Gaede,
C.~Grojean,
J.~List,
T.~Madlener,
A.~B.~Meyer,
M.T.~N\'u\~nez Pardo de Vera,
K.~Radchenko Serdula,
J.~Reuter,
F.~Sefkow,
J.~Torndal,
A.~Verduras Schaeidt,
G.~Weiglein\\
\emph{DESY, Hamburg, Germany}
}

%Germany, II. Physikalisches Institut, Georg-August-Universität Göttingen
\addauthor{
K.~K\"oneke\\
\emph{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"ottingen, G\"ottingen, Friedrich-Hund-Platz 1, 37077 G\"ottingen, Germany}
}

%Germany, Johannes Gutenberg Universität Mainz
\addauthor{
B.~Dudar,
F.~Yu\\
\emph{PRISMA+ Cluster of Excellence and Mainz Institute for Theoretical Physics, Johannes Gutenberg University, 55099 Mainz, Germany}
}

%Germany, Karlsruhe Institute of Technology
\addauthor{
S.~Alshamaily,
G.~Brodbek,
U.~Einhaus,
S.~Giappichini,
P.~Goldenzweig,
S.~Keilbach,
J.~Kieseler,
M.~Klute,
M.~Presilla,
F.~Simon,
A.~Wiedl,
X.~Zuo\\
\emph{Karlsruhe Institute of Technology, Karlsruhe, Germany}
}

%Germany, Max-Planck-Institut für Physik
\addauthor{
P.~Lo Chiatto$^{7}$\\
\emph{Max-Planck-Institut f{\"u}r Physik, Boltzmannstra{\ss}e 8, 85748 Garching bei M{\"u}nchen, Germany}
}

%Germany, Rheinische Friedrich-Wilhems-Universität Bonn
\addauthor{
P.~Bechtle,
M.~Vellasco\\
\emph{University of Bonn, Physikalisches Institut, Nussallee 12, 53115 Bonn, Germany}
}

%Germany, TU Dortmund University
\addauthor{
K.~Kr\"oninger,
L.~R\"ohrig$^{8}$\\
\emph{TU Dortmund University, Department of Physics, Otto-Hahn-Str. 4a, 44227 Dortmund, Germany}
}

%Germany, Universität Heidelberg
\addauthor{
H.~Bahl,
M.D.~Tat\\
\emph{Universit\"at Heidelberg, Heidelberg, Germany}
}

%Germany, University of Hamburg
\addauthor{
A.~Grohsjean,
J~Lahiri,
G.~Moortgat-Pick\\
\emph{University of Hamburg, Hamburg, Germany}
}

%Germany, University of Siegen
\addauthor{
W.~Kilian\\
\emph{Center for Particle Physics Siegen, Universit\"at Siegen, 57068 Siegen, Germany}
}

%India, Indian Institute of Technology Guwahati
\addauthor{
P.~Poulose\\
\emph{Indian Institute of Technology Guwahati, Assam 781039, India}
}

%India, The Institute of Mathematical Sciences
\addauthor{
J.~Dutta\\
\emph{The Institute of Mathematical Sciences, CIT Campus, Tharamani, Chennai, Tamil Nadu, 600113, India}
}

%Iran, Institute for Research in Fundamental Sciences
\addauthor{
M.~Mohammadi Najafabadi,
M.~Nourbakhsh,
S.~Tizchang$^{9}$\\
\emph{School of Particles and Accelerators, Institute for Research in Fundamental Sciences (IPM), Artesh Highway, Tehran 1956836681, Iran}
}

%Iran, Isfahan University of Technology
\addauthor{
Z.~Baharyioon,
A.~Jafari\\
\emph{Department of Physics, Isfahan University of Technology, Isfahan, 84156-83111, Iran}
}

%Iran, University of Tehran
\addauthor{
A.~Amiri$^{10}$,
K.~Azizi$^{11}$,
F.~Fatehi,
R.~Jafariseyedabad$^{10}$,
M.~Malekhosseini,
S.~Rostami\\
\emph{Department of Physics, University of Tehran, North Karegar Avenue, Tehran 14395-547, Iran}
}

%Ireland, Dublin Institute for Advanced Studies
\addauthor{
V.~Keus\\
\emph{Dublin Institute of Advanced Studies (DIAS), Dublin D04 C932, Ireland}
}

%Israel, Technion – Israel Institute of Technology
\addauthor{
Y.~Soreq\\
\emph{Physics Department, Technion - Israel Institute of Technology, Haifa 3200003, Israel}
}

%Italy, INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine
\addauthor{
M.~Cobal$^{12}$,
G.~Panizzo$^{12}$,
M.~Pinamonti$^{12}$,
L.~Pintucci$^{12}$,
L.~Toffolin$^{12}$\\
\emph{INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine, Via delle Scienze 206, Udine, Italy}
}

%Italy, INFN Laboratori Nazionali di Frascati
\addauthor{
E.~Bagnaschi,
F.~Mescia\\
\emph{INFN, Laboratori Nazionali di Frascati, Via E. Fermi 40, 00044 Frascati, Italy}
}

%Italy, INFN Sezione di Bologna
\addauthor{
G.L.~Alberghi,
L.~Bellagamba\\
\emph{INFN Sezione di Bologna, Viale Carlo Berti Pichat 6/2, 40127 Bologna, Italy}
}

%Italy, INFN Sezione di Firenze
\addauthor{
M.~Tammaro\\
\emph{INFN Sezione di Firenze, Via G. Sansone 1, 50019 Sesto Fiorentino, Italy}
}

%ITALY, INFN Sezione di Lecce
\addauthor{
E.G.~Gorini,
F.G.~Grancagnolo,
M.P.~Primavera\\
\emph{INFN Sezione di Lecce, Lecce, Italy}
}

%Italy, INFN Sezione di Milano
\addauthor{
A.~Andreazza$^{13}$,
C.~Meroni$^{13}$,
F.~Sabatini,
R.~Zanzottera$^{13}$,
M.~Zaro$^{14}$\\
\emph{INFN Sezione di Milano, Via Celoria 16, 20133 Milano, Italy}
}

%Italy, INFN Sezione di Padova
\addauthor{
P.~Azzi,
A.~De Vita,
N.~Selimovi\'c\\
\emph{INFN Sezione di Padova, Via Marzolo 8, 35131 Padova, Italy}
}

%Italy, INFN Sezione di Pavia
\addauthor{
C.~Carloni Calame,
M.~Chiesa,
O.~Nicrosinii,
F.~Piccinini,
G.~Polesello,
N.~Valle\\
\emph{INFN Sezione di Pavia, via A. Bassi 6, 27100 Pavia, Italy}
}

%Italy, INFN Sezione di Perugia
\addauthor{
S.~Ajmal,
O.~Panella\\
\emph{INFN Sezione di Perugia, Via A. Pascoli, 06123, Perugia, Italy}
}

%Italy, INFN Sezione di Pisa
\addauthor{
P.~Azzurri,
D.~Barducci$^{15}$,
D.~Buttazzo,
A.~Dondarini$^{15}$,
A.~Korajac,
G.~Marino$^{15}$,
F.~Palla,
P.~Panci$^{15}$\\
\emph{INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy}
}

%Italy, INFN Sezione di Trieste
\addauthor{
D.~Marzocca\\
\emph{INFN Trieste, Via Valerio 2, 34127 Trieste, Italy}
}

%Italy, Milan University
\addauthor{
A.~Vicini\\
\emph{TIFLab, Universit\`a degli Studi di Milano, Via Celoria 16, 20133 Milano, Italy}
}

%Italy, Politecnico di Bari
\addauthor{
N.~De~Filippis$^{16}$,
F.M.~Procacci$^{16}$\\
\emph{Politecnico di Bari, Via Orabona 4, 70126 Bari, Italy}
}

%Italy, Scuola Normale Superiore
\addauthor{
Alberto Lusiani$^{17}$\\
\emph{Scuola Normale Superiore, Piazza dei Cavalieri 7, 56126 Pisa, Italy}
}

%Italy, Università degli Studi di Padova
\addauthor{
B.A.~Erdelyi$^{18}$,
R.~Gr\"ober$^{18}$,
A.~Rossia$^{18}$\\
\emph{Dipartimento di Fisica e Astronomia "G. Galilei", Universit\`a degli Studi di Padova, 35131 Padova, Italy}
}

%Italy, Università degli Studi di Roma la Sapienza
\addauthor{
M.~Bulliri\\
\emph{Universit\`a degli Studi di Roma la Sapienza, Piazzale Aldo Moro 5, 00185 Rome, Italy}
}

%Italy, Università di Pavia
\addauthor{
G.~Montagna$^{19}$,
F.~Ucci$^{19}$\\
\emph{Universit\`a di Pavia, 27100 Pavia, Italy}
}

%Italy, Universit`a degli Studi Roma Tre
\addauthor{
R.~Franceschini$^{20}$\\
\emph{Universit\`a degli Studi Roma Tre, Via della Vasca Navale 84, 00146 Rome, Italy}
}

%Japan, High Energy Accelerator Research Organization
\addauthor{
K.~Fujii,
D.~Jeans,
J.~Nakajima\\
\emph{KEK, Tsukuba, Japan}
}

%Japan, Hokkaido University
\addauthor{
A.~Das\\
\emph{Hokkaido University, Sapporo 060-0810, Japan}
}

%Japan, Iwate University
\addauthor{
S.~Narita\\
\emph{Iwate University, Morioka, Iwate 020-8551, Japan}
}

%Japan, Shinshu University
\addauthor{
T.~Takeshita\\
\emph{Shinshu University, Matsumoto, Nagano, Japan}
}

%Japan, Tokyo Gakugei University
\addauthor{
K.~Hidaka\\
\emph{Tokyo Gakugei University, Koganei, Tokyo 184-8501, Japan}
}

%Morocco, Cadi Ayyad University
\addauthor{
M.~Ouchemhou\\
\emph{Polydisciplinary Faculty, Laboratory of Fundamental and Applied Physics, Cadi Ayyad University, Sidi Bouzid, B.P. 4162, Safi, Morocco}
}

%Poland, AGH University of Krakow
\addauthor{
H.~Khanpour\\
\emph{AGH University, Faculty of Physics and Applied Computer Science, Al. Mickiewicza 30, 30-055 Krak\'ow, Poland}
}

%Poland, Institute of Nuclear Physics Polish Academy of Sciences
\addauthor{
J.~Bhom,
P.~Bruckman,
M.~Chrzaszcz,
A.~Kaczmarska,
M.~Kucharczyk,
T.~Lesiak,
P.~Malecki,
M.~Skrzypek,
Z.~Was\\
\emph{The Henryk Niewodnicza\'nski
Institute of Nuclear Physics
Polish Academy of Sciences
ul. Radzikowskiego 152,
31-342 Krak\'ow, Poland}
}

%Poland, Jagiellonian University in Krakow
\addauthor{
A.~Price,
W.~P{\l}aczek,
A.~Si\'odmok\\
\emph{Faculty of Physics, Astronomy and Applied Computer Science, ul. Lojasiewicza 11, 30-348 Krak\'ow, Poland}
}

%Poland, University of Warsaw
\addauthor{
B.~Brudnowski,
J.~Kalinowski,
J.~Klamka,
K.~Mekala$^{21}$,
K.~Sakurai,
A.F.~\.Zarnecki,
K.~Zembaczy\'nski\\
\emph{Faculty of Physics, University of Warsaw, Warsaw, Poland}
}

%Portugal, Centro de Física Teórica de Partículas, Instituto Superior Técnico, Universidade de Lisboa
\addauthor{
J.~Hajer,
B.~Oliveira\\
\emph{Centro de F\'isica Te\'orica de Part\'iculas (CFTP), Instituto Superior T\'ecnico (IST), Universidade de Lisboa, 1049-001 Lisboa, Portugal}
}

%Portugal, Laboratório de Instrumentação e Física Experimental de Partículas
\addauthor{
N.F.~Castro$^{22}$,
G.~Chachamis$^{23}$\\
\emph{LIP -- Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas, Escola de Ci\`encias, Campus de Gualtar, Universidade do Minho, 4701-057 Braga, Portugal}
}

%%Russian Federation, Joint Institute for Nuclear Research
%\addauthor{
%A.~Nesterenko\\
%\emph{Joint Institute for Nuclear Research, Dubna, 141980, Russian Federation}
%}
%
%%Russian Federation, National Research Nuclear University MEPhI
%\addauthor{
%V. A.~Okorokov\\
%\emph{National Research Nuclear University MEPhI, Kashirskoe shosse 31, 115409 Moscow, Russian Federation}
%}

%Serbia, Vinca Institute of Nuclear Sciences
\addauthor{
I.~Bozovic$^{24}$,
G.~Kacarevic,
G.~Milutinovic-Dumbelovic,
I.~Smiljanic,
I.~Vidakovic,
N.~Vukasinovic\\
\emph{Vin\v{c}a Institute of Nuclear Sciences, University of Belgrade, Belgrade, Serbia}
}

%Spain, Centro de Investigaciones  Energéticas, Medioambientales y Tecnológicas
\addauthor{
J.~Alcaraz Maestre$^{25}$,
M.~Cepeda$^{26}$,
M.C.~Fouz$^{25}$\\
\emph{Centro de Investigaciones  Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT)
Madrid, Spain}
}

%Spain, IFIC, CSIC-Universitat de València
\addauthor{
J.~Fuster,
A.~Irles,
L.~Mantani,
J.P.~M\'arquez,
V.A.~Mitsou,
M.~Moreno~Ll\'acer,
E.~Musumeci,
B.~Pattnaik,
A.~Saibel,
M.A.~Sanchis,
M.~Vos,
J.~Zurita\\
\emph{IFIC, CSIC-Universitat de Val\`encia, Valencia, Spain}
}

%Spain, Instituto de Física de Cantabria
\addauthor{
A.~Ruiz~Jimeno\\
\emph{Instituto de F\'isica de Cantabria, Av de los Castros, 39005 Santander, Spain}
}

%Spain, Instituto de Física Teórica, CSIC-Universidad Autónoma de Madrid
\addauthor{
J.A.~Aguilar-Saavedra,
S.~Heinemeyer,
A.~Sabio Vera$^{27}$\\
\emph{Instituto de F\'isica Te\'orica, CSIC-Universidad Aut\'onoma de Madrid, Madrid, Spain}
}

%Spain, Instituto Galego de Física de Altas Enerxías (IGFAE), Universidade de Santiago de Compostela
\addauthor{
I.~Corredoira\\
\emph{Instituto Galego de F\'isica de Altas Enerx\'ias (IGFAE), Universidade de Santiago de Compostela
Santiago de Compostela, Spain}
}

%Spain, Universidad de Alcalá
\addauthor{
F.~G.~Celiberto$^{28}$\\
\emph{Alcal\'a de Henares, Madrid, E-28805, Spain}
}

%Spain, Universidad de Cordoba
\addauthor{
F.~Cornet-Gomez\\
\emph{Campus Universitario de Rabanales, Ctra. N-IVa, Km. 396. 14071, Cordoba, Spain}
}

%Spain, Universidad de Granada
\addauthor{
M.~Chala,
J.~de Blas\\
\emph{Departamento de F\'isica Te\'orica y del Cosmos, Universidad de Granada,
Campus de Fuentenueva, 18071 Granada, Spain}
}

%Sweden, KTH Royal Institute of Technology
\addauthor{
M.~Vande Voorde\\
\emph{Department of Physics, Royal Institute of Technology, Stockholm; Sweden}
}

%Sweden, Lund University
\addauthor{
T.~Sj\"ostrand\\
\emph{Department of Physics, Lund University, Lund, Sweden}
}

%Sweden, Uppsala University
\addauthor{
A.~Gall\'en,
R.~Gonzalez Suarez,
G.~Ripellino\\
\emph{Department of Physics and Astronomy, Uppsala University, L{\"a}gerhyggsv{\"a}gen 1, Uppsala, 752 37, Sweden}
}

%Switzerland, CERN
\addauthor{
M.~Al-Thakeel,
S.~Aumiller,
V.~Cairo,
J.~M.~Carceller,
C.~Cornella,
D.~d'Enterria,
J.~Davighi,
M.~M.~Defranchis,
M.~Di Carlo,
F.~Erben,
B.~Francois,
G.~Ganis,
D.~Garcia,
G.~Guerrieri,
A.~J\"uttner,
S.~Kuberski,
A.~Mehta,
L.~Reichenbach$^{29}$,
A.~Sailer,
S.~Sasikumar,
M.~Selvaggi,
J.~Smiesko,
A.~Tolosa-Delgado,
J.~T.~Tsang\\
\emph{CERN, Geneva, Switzerland}
}

%Switzerland, Eidgenössische Technische Hochschule Zürich
\addauthor{
S.~Thor\\
\emph{ETH Z\"{u}rich, 8092 Z\"{u}rich, Switzerland}
}

%Switzerland, Paul Scherrer Institute
\addauthor{
L.~Biermann,
M.~Spira\\
\emph{Paul Scherrer Institute
Particle Physics Theory Group LTP
Forschungsstrasse 111
CH-5232 Villigen PSI, Switzerland}
}

%Switzerland, Université de Genève
\addauthor{
T.~Critchley,
P.~Kontaxakis,
A.~Sfyrla\\
\emph{D\'epartement de Physique Nucl\'eaire et Corpusculaire (DPNC), Universit\'e de Gen\`eve, 1205 Gen\`eve, Switzerland}
}

%Switzerland, University of Basel
\addauthor{
S.~Antusch,
A.~Greljo\\
\emph{Department of Physics, University of Basel, 4056 Basel, Switzerland}
}

%Switzerland, University of Zurich
\addauthor{
M.~Bordone$^{30}$,
F.~Canelli,
A.~Ilg,
G.~Isidori,
B.~Kilminster,
T.H.~Kwok,
V.~Lukashenko,
A.~Macchiolo,
Z.~Polonsky\\
\emph{Physik-Institut, University of Zurich, 8057 Z\"urich, Switzerland}
}

%Türkiye, Bolu Abant Izzet Baysal University
\addauthor{
H.~Denizli,
A.~Senol\\
\emph{Department of Physics, Bolu Abant Izzet Baysal University, 14280, Bolu, T\"{u}rkiye}
}

%Türkiye, Institute of Accelerator Technologies (Ankara University)
\addauthor{
H.~Duran Yildiz\\
\emph{Institute of Accelerator Technologies, Ankara University, Ankara, T\"urkiye}
}

%The Netherlands, Nikhef
\addauthor{
P.~Koppenburg,
J.~Rojo$^{31}$\\
\emph{Nikhef, Science Park 105, 1098 XG Amsterdam, The Netherlands}
}

%The Netherlands, University of Amsterdam
\addauthor{
J.~Klari\'c$^{32}$,
V.~Plakkot$^{33}$\\
\emph{University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands}
}

%UK, University of Oxford
\addauthor{
P.N.~Burrows,
C.~Hays,
G.~Wilkinson\\
\emph{Department of Physics, University of Oxford, Oxford OX1 5NZ, UK}
}

%Ukraine, National Science Center ``Kharkiv Institute of Physics and Technology''
\addauthor{
E.~Bulyak\\
\emph{NSC KIPT, 1 Academichna Str. Kharkiv UA-61108, Ukraine}
}

%United Kingdom, Imperial College London
\addauthor{
E.~Curtis,
A.-M.~Magnan,
N.~Wardle\\
\emph{The Blackett Laboratory, Imperial College, London SW7 2BW, United Kingdom}
}

%United Kingdom, University of Edinburgh
\addauthor{
S.~Farrington,
C.~Leonidopoulos{$^*$},
J.~Silva,
J.~ter Hoeve\\
\emph{University of Edinburgh, Edinburgh EH9 3FD, United Kingdom}
}

%United Kingdom, University of Glasgow
\addauthor{
C.~Englert,
M.~Miralles L\'opez,
J.~Nesbitt,
D.~Protopopescu,
S.~Renner,
A.~Robson{$^*$},
Y.~Zhang\\
\emph{University of Glasgow, Glasgow G12 8QQ, Scotland, United Kingdom}
}

%United Kingdom, University of Manchester
\addauthor{
J.M.~Burridge,
E.~Celada,
A.J.~Costa,
V.~Miralles,
A.~Pilkington,
M.~Thomas,
E.~Vryonidou,
A.R.~Wiederhold\\
\emph{University of Manchester, Manchester M13 9PL, United Kingdom}
}

%United Kingom, Cavendish Laboratory, University of Cambridge
\addauthor{
J.~Hayward,
M.~Kenzie,
S.~Williams\\
\emph{Cavendish Laboratory, University of Cambridge, Cambridge CB3 0HE, United Kingom}
}

%USA, Baylor University
\addauthor{
B.F.L.~Ward\\
\emph{Baylor University, Waco, TX 76798-7316, USA}
}

%USA, Brookhaven National Laboratory
\addauthor{
H.~Abidi,
K.A.~Assamagan,
D.~Boye,
E.~Brost,
V.~Cavaliere,
A.E.~Connelly,
C.L.~Del Pio,
G.~Iakovidis,
A.~Li,
M.A.~Pleier,
A.~Sciandra,
S.~Snyder,
A.~Tishelman-Charny,
I.~Veli\v{s}\v{c}ek\\
\emph{Brookhaven National Laboratory, Upton, NY 11973-5000, USA}
}

%USA, Brown University
\addauthor{
L.~Gouskos,
L.~Li\\
\emph{Brown University, 182 Hope Street, Providence, RI 02912, USA}
}

%USA, Fermi National Accelerator Laboratory
\addauthor{
L.~Gray\\
\emph{Fermilab, PO Box 500, Batavia, IL 60510, USA}
}

%USA, Jefferson Lab
\addauthor{
Z.~Yu\\
\emph{Theory Center, Jefferson Lab, Newport News, Virginia 23606, USA}
}

%USA, Johns Hopkins University
\addauthor{
N.~Pinto$^{34}$\\
\emph{Johns Hopkins University, Baltimore, Maryland 21218, USA}
}

%USA, Massachusetts Institute of Technology
\addauthor{
J.~Eysermans\\
\emph{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
}

%USA, Michigan State University
\addauthor{
R.~Schwienhorst,
C.-P.~Yuan$^{35}$\\
\emph{Department of Physics and Astronomy, Michigan State University, East Lansing, Michigan 48824, USA}
}

%USA, Northeastern University
\addauthor{
M.~Larson,
L.~Skinnari\\
\emph{Northeastern University, Boston, Massachusetts 02115, USA}
}

%USA, Princeton University
\addauthor{
W.~Chung,
L. S.~Mandacar\'{u} Guerra\\
\emph{Princeton University, Princeton, New Jersey 08544, USA}
}

%USA, SLAC National Accelerator Laboratory
\addauthor{
D.~Ntounis,
C.~Vernieri\\
\emph{SLAC, 2575 Sand Hill Rd, Menlo Park, CA 94025, USA}
}

%USA, Stony Brook University
\addauthor{
V.~Dao\\
\emph{Stony Brook University, 100 Nicolls Rd, Stony Brook, NY 11794, USA}
}

%USA, Texas Tech University
\addauthor{
V.~Slokenbergs\\
\emph{Texas Tech University, Lubbock, Texas, 79409, USA}
}

%USA, University of Alabama
\addauthor{
N.~Okada\\
\emph{University of Alabama, Tuscaloosa, Alabama 35487, USA}
}

%USA, University of California, Davis
\addauthor{
H.-C.~Cheng\\
\emph{University of California, One Shields Avenue, Davis, California, USA}
}

%USA, University of California, Santa Cruz
\addauthor{
W.~Altmannshofer\\
\emph{University of California, Santa Cruz, CA 95064, USA}
}

%USA, University of Cincinnati
\addauthor{
M.~Szewc$^{36}$\\
\emph{Department of Physics, University of Cincinnati, Cincinnati, Ohio 45221, USA}
}

%USA, University of Kansas
\addauthor{
G.W.~Wilson\\
\emph{University of Kansas, Lawrence, KS 66045, USA}
}

%USA, University of Maryland-College Park
\addauthor{
S.~Airen\\
\emph{University of Maryland-College Park,
College Park, Maryland 20740, USA}
}

%USA, University of Pittsburgh
\addauthor{
A.~Freitas\\
\emph{University of Pittsburgh, Pittsburgh, PA 15260, USA}
}

%USA, University of Wisconsin-Madison
\addauthor{
S.~Dasu,
A.~Mohammadi,
C.-H.~Nee\\
\emph{University of Wisconsin-Madison, Madison, WI 53706-1390, USA}
}

%USA, Yale University
\addauthor{
T.~Lagouri\\
\emph{Yale University, New Haven CT, USA}
}

%%Russian Federation
\addauthor{
A.~Nesterenko{$^{37}$},\\
V.A.~Okorokov{$^{38}$}\\
\emph{Affiliated with an institute covered by a cooperation agreement with CERN}
}

\addauthor{
A.~V.~Gritsan{$^{39}$},\\
\emph{Affiliated with an institute covered by a cooperation agreement between the US DOE, US NSF, and CERN}
}

\addauthor{
\begin{flushleft}
{$^{0}$}Also at: ARC Centre of Excellence for Dark Matter Particle Physics, Australia\\
{$^{1}$}Also at: University of Vienna\\
{$^{2}$}Also at: Physik-Institut, University of Zurich, 8057 Z\"urich, Switzerland\\
{$^{3}$}Also at: Department of Physics, Simon Fraser University, University Drive W, Burnaby, Canada\\
{$^{4}$}Also at: China Center of Advanced Science and Technology, Beijing, China\\
{$^{5}$}Also at: Laboratoire de Physique Théorique et Hautes Energies (LPTHE), Sorbonne Université et CNRS, Paris\\
{$^{6}$}Also at: University of Hamburg, Hamburg, Germany\\
{$^{7}$}Also at: Weizmann Institute of Science, 234 Herzl Street, POB 26, Rehovot 7610001, Israel\\
{$^{8}$}Also at: LPCA, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand, France\\
{$^{9}$}Also at: Physics Department, Faculty of Sciences, Arak University, Arak\\
{$^{10}$}Also at: Department of Physics, Faculty of Science, Ferdowsi University of Mashhad, Mashhad, Iran\\
{$^{11}$}Also at: Department of Physics, Do\v{g}u\c{s} University, Dudullu-\"{U}mraniye, 34775 Istanbul, T\"urkiye\\
{$^{12}$}Also at: Dipartimento
PolitecniAlso at: co di Ingegneria e Architettura, Università di Udine, Udine\\
{$^{13}$}Also at: Dipartimento di Fisica, Università degli Studi di Milano, 20133 Milano, Italy\\
{$^{14}$}Also at: TIFLab, Università degli Studi di Milano, 20133 Milano, Italy\\
{$^{15}$}Also at: Universit\`a di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy\\
{$^{16}$}Also at: INFN Sezione di Bari, Via Orbona 4, 70126 Bari, Italy\\
{$^{17}$}Also at: INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy\\
{$^{18}$}Also at: INFN Sezione di Padova, Via Marzolo 8, 35131 Padova, Italy\\
{$^{19}$}Also at: INFN Sezione di Pavia, via A. Bassi 6, 27100 Pavia, Italy\\
{$^{20}$}Also at: INFN Sezione di Roma Tre, Via della Vasca Navale 84, 00146, Roma, Italy\\
{$^{21}$}Also at: DESY, Hamburg, Germany\\
{$^{22}$}Also at: Departamento de F\'{i}sica, Escola de Ci\^{e}ncias, Universidade do Minho, 4710-057 Braga, Portugal\\
{$^{23}$}Also at: LIP -- Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas, Lisboa, Portugal\\
{$^{24}$}Supported by Fund of Science RS, Grant IDEJE HIGHTONE-P\\
{$^{25}$}Grant PID2021-122134NB-C22 funded by MICIU/AEI/10.13039/501100011033\\
{$^{26}$}Grants PID2021-122134NB-C22 and CNS2023-144781, funded by MCIU/AEI/10.13039/501100011033 and by European Union NextGenerationEU/PRTR\\
{$^{27}$}Also at: Universidad Autonoma de Madrid, E-28049 Madrid, Spain\\
{$^{28}$}F.G.C. acknowledges support from the Atracci\'on de Talento Grant n. 2022-T1/TIC-24176 of the Comunidad Aut\'onoma de Madrid, Spain.\\
{$^{29}$}Also at: University of Bonn, Physikalisches Institut, Nussallee 12, 53115 Bonn\\
{$^{30}$}Also at: CERN, Geneva, Switzerland\\
{$^{31}$}Also at: Department of Physics and Astronomy, Vrije Universiteit, NL-1081 HV Amsterdam, The Netherlands\\
{$^{32}$}Also at: University of Zagreb, Bijeni\v{c}ka c. 32, 10000 Zagreb, Croatia\\
{$^{33}$}Also at: Nikhef, Science Park 105, 1098 XG Amsterdam, The Netherlands\\
{$^{34}$}NP acknowledges support in part by the US NSF grant PHY-2310072\\
{$^{35}$}Supported by the U.S. National Science Foundation under Grant No.~PHY-2310291.\\
{$^{36}$}MS acknowledges support in part by NSF grants OAC-2103889, OAC-2411215 and OAC-2417682 and by DOE grant DE-SC101977.
Also at International Center for Advanced Studies (ICAS), ICIFI and ECyT-UNSAM, 25 de Mayo y Francia, 1650 San Mart\'{i}n, Buenos Aires, Argentina\\
{$^{37}$} https://orcid.org/0000-0003-4747-699X\\
{$^{38}$} https://orcid.org/0000-0002-7162-5345\\
{$^{39}$} https://orcid.org/0000-0002-3545-7970\\
{$^*$}Editors 
\end{flushleft}
}



==> ecfa_authors_p3_YR2format_250224.tex <==
% Author list for 'ECFA Higgs/top/electroweak Factory Study Report' in YR2 format
% automatically generated on 2025-02-24 at 15:02:08 UTC
% via https://www.ppe.gla.ac.uk

%Australia, Monash University
\addauthor{
J.~Altmann,
P.~Skands\\
\emph{Monash University, Wellington Road, Clayton VIC-3800, Australia}
}

%Australia, University of Adelaide
\addauthor{
A.~Desai$^{0}$\\
\emph{The University of Adelaide, Adelaide, SA 5005, Australia}
}

%Austria, Institute of High Energy Physics, Vienna
\addauthor{
W.~Mitaroff\\
\emph{Institute of High Energy Physics, Austrian Academy of Sciences, 1050 Vienna, Austria}
}

%Austria, University of Graz
\addauthor{
S.~Pl\"atzer$^{1}$\\
\emph{Institute of Physics, NAWI Graz, University of Graz, Universit\"atsplatz 5, 8010 Graz, Austria}
}

%Belgium, Ghent University
\addauthor{
D.~Dobur,
K.~Skovpen\\
\emph{Ghent University, Proeftuinstraat 86, 9000 Gent, Belgium}
}

%Belgium, Université catholique de Louvain
\addauthor{
M. ~Drewes,
G.~Durieux,
Y.~Georis,
Y.~Ma\\
\emph{Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, 1348 Louvain-la-Neuve, Belgium}
}

%Belgium, Vrije Universiteit Brussel
\addauthor{
A.~De Moor,
K.~Gautam$^{2}$,
E.~Ploerer$^{2}$,
M.~Tytgat\\
\emph{Inter-University Institute for High Energies, Vrije Universiteit Brussel,
Pleinlaan 2, 1050 Ixelles, Belgium}
}

%Brazil, Universidade do Estado do Rio de Janeiro
\addauthor{
K.~Mota~Amarilo\\
\emph{Universidade do Estado do Rio de Janeiro, Rio de Janeiro, Brazil}
}

%Canada, TRIUMF
\addauthor{
M.J.~Basso$^{3}$\\
\emph{TRIUMF, Wesbrook Mall, Vancouver, Canada}
}

%China, Fudan University
\addauthor{
J.~Gu\\
\emph{Department of Physics and Center for Field Theory and Particle Physics, Fudan University,
Shanghai 200438, China}
}

%China, Hefei University of Technology
\addauthor{
Y.~Zhang\\
\emph{School of Physics, Hefei University of Technology, Hefei 230601, China}
}

%China, Institute of High Energy Physics, Chinese Academy of Sciences
\addauthor{
X.-H.~Jiang$^{4}$,
Bin Yan\\
\emph{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
}

%China, Peking University
\addauthor{
X.-K.~Wen\\
\emph{School of Physics, Peking University, Beijing 100871, China}
}

%China, Sun Yat-sen University
\addauthor{
J.~Liao\\
\emph{School of Physics, Sun Yat-sen University, Guangzhou, 510275, China}
}

%China, Sun Yat-sen University (Shenzhen)
\addauthor{
C.~Li\\
\emph{School of Science, Sun Yat-sen University (SYSU), Shenzhen, 518107, China}
}

%Croatia, Rudjer Boskovic Institute
\addauthor{
T.~Robens\\
\emph{Rudjer Boskovic Institute, Bijenicka cesta 54, 10000 Zagreb, Croatia}
}

%Denmark, Niels Bohr Institute, Copenhagen University
\addauthor{
M.~Dam\\
\emph{Niels Bohr Institute, Copenhagen University, Jagtvej 155, 2200 Copenhagen, Denmark}
}

%France, APC, Laboratoire AstroParticule et Cosmologie, Paris
\addauthor{
G.~Bernardi,
K.~Dewyspelaere,
A.~Maloizel,
G.~Marchiori\\
\emph{APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, Paris, France}
}

%France, Institut de Physique des 2 Infinis de Lyon IN2P3-CNRS/Université Claude Bernard Lyon 1
\addauthor{
S.~Gascon-Shotkin,
E.~Jourd'huy,
C.~Verollet,
J.~Xiao\\
\emph{Institut de Physique des 2 Infinis de Lyon IN2P3-CNRS, rue Enrico Fermi
69622 Villeurbanne, France}
}

%France, Institut Polytechnique des Sciences Avancées
\addauthor{
R.~Perez-Ramos$^{5}$\\
\emph{DRII-IPSA, 94200 Ivry-sur-Seine, France}
}

%France, Laboratoire de Physique de Clermont Auvergne, Université Clermont Auvergne, CNRS/IN2P3
\addauthor{
R.~Madar,
T.~Miralles,
S.~Monteil\\
\emph{LPCA, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand, France}
}

%France, Laboratoire de physique des 2 infinis Irène Joliot-Curie
\addauthor{
Y.~Amhis,
I.~Combes,
N.~Morange,
R.~P\"oschl,
M.~Reboud,
F.~Richard,
O.~Sumensari\\
\emph{IJCLab, Universit\'e Paris-Saclay, CNRS/IN2P3, 91405 Orsay, France}
}

%France, Laboratoire de Physique Théorique et Hautes Energies
\addauthor{
G.~Cacciapaglia\\
\emph{Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), Sorbonne Universit\'e et CNRS, 75252 Paris, France}
}

%France, Laboratoire Leprince-Ringuet
\addauthor{
V.~Balagura,
V.~Boudry,
J.-C.~Brient,
C.~Charlot,
C.~Ochando,
R.~Salerno,
Y.~Shi,
Y.~Sirois\\
\emph{Laboratoire Leprince-Ringuet, Ecole Polytechnique, 91128 Palaiseau, France}
}

%France, LAPP, Université Savoie Mont Blanc, CNRS/IN2P3, Annecy
\addauthor{
O.~Arnaez,
M.~Delmastro,
H.~Taibi,
Z.~Wu\\
\emph{LAPP, 9 Chem. de Bellevue, 74940 Annecy, France}
}

%Germany, Albert-Ludwigs-Universität Freiburg
\addauthor{
S.D.~Dittmaier,
M.~Gabelmann\\
\emph{Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany}
}

%Germany, CNRS Helmholtz Dark Matter Lab
\addauthor{
D.~Zerwas\\
\emph{DMLab, Deutsches Elektronen-Synchrotron DESY, CNRS/IN2P3, Hamburg, Germany}
}

%Germany, DESY Hamburg
\addauthor{
J.~Alimena,
M.~Berggren,
F.~Blekman$^{6}$,
B.~Bliewert,
J.~Braathen,
A.~Filipe Silva,
F.~Gaede,
C.~Grojean,
J.~List,
T.~Madlener,
A.~B.~Meyer,
M.T.~N\'u\~nez Pardo de Vera,
K.~Radchenko Serdula,
J.~Reuter,
F.~Sefkow,
J.~Torndal,
A.~Verduras Schaeidt,
G.~Weiglein\\
\emph{DESY, Hamburg, Germany}
}

%Germany, II. Physikalisches Institut, Georg-August-Universität Göttingen
\addauthor{
K.~K\"oneke\\
\emph{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"ottingen, G\"ottingen, Friedrich-Hund-Platz 1, 37077 G\"ottingen, Germany}
}

%Germany, Johannes Gutenberg Universität Mainz
\addauthor{
B.~Dudar,
F.~Yu\\
\emph{PRISMA+ Cluster of Excellence and Mainz Institute for Theoretical Physics, Johannes Gutenberg University, 55099 Mainz, Germany}
}

%Germany, Karlsruhe Institute of Technology
\addauthor{
S.~Alshamaily,
G.~Brodbek,
U.~Einhaus,
S.~Giappichini,
P.~Goldenzweig,
S.~Keilbach,
J.~Kieseler,
M.~Klute,
M.~Presilla,
F.~Simon,
A.~Wiedl,
X.~Zuo\\
\emph{Karlsruhe Institute of Technology, Karlsruhe, Germany}
}

%Germany, Max-Planck-Institut für Physik
\addauthor{
P.~Lo Chiatto$^{7}$\\
\emph{Max-Planck-Institut f{\"u}r Physik, Boltzmannstra{\ss}e 8, 85748 Garching bei M{\"u}nchen, Germany}
}

%Germany, Rheinische Friedrich-Wilhems-Universität Bonn
\addauthor{
P.~Bechtle,
M.~Vellasco\\
\emph{University of Bonn, Physikalisches Institut, Nussallee 12, 53115 Bonn, Germany}
}

%Germany, TU Dortmund University
\addauthor{
K.~Kr\"oninger,
L.~R\"ohrig$^{8}$\\
\emph{TU Dortmund University, Department of Physics, Otto-Hahn-Str. 4a, 44227 Dortmund, Germany}
}

%Germany, Universität Heidelberg
\addauthor{
H.~Bahl,
M.D.~Tat\\
\emph{Universit\"at Heidelberg, Heidelberg, Germany}
}

%Germany, University of Hamburg
\addauthor{
A.~Grohsjean,
J~Lahiri,
G.~Moortgat-Pick\\
\emph{University of Hamburg, Hamburg, Germany}
}

%Germany, University of Siegen
\addauthor{
W.~Kilian\\
\emph{Center for Particle Physics Siegen, Universit\"at Siegen, 57068 Siegen, Germany}
}

%India, Indian Institute of Technology Guwahati
\addauthor{
P.~Poulose\\
\emph{Indian Institute of Technology Guwahati, Assam 781039, India}
}

%India, The Institute of Mathematical Sciences
\addauthor{
J.~Dutta\\
\emph{The Institute of Mathematical Sciences, CIT Campus, Tharamani, Chennai, Tamil Nadu, 600113, India}
}

%Iran, Institute for Research in Fundamental Sciences
\addauthor{
M.~Mohammadi Najafabadi,
M.~Nourbakhsh,
S.~Tizchang$^{9}$\\
\emph{School of Particles and Accelerators, Institute for Research in Fundamental Sciences (IPM), Artesh Highway, Tehran 1956836681, Iran}
}

%Iran, Isfahan University of Technology
\addauthor{
Z.~Baharyioon,
A.~Jafari\\
\emph{Department of Physics, Isfahan University of Technology, Isfahan, 84156-83111, Iran}
}

%Iran, University of Tehran
\addauthor{
A.~Amiri$^{10}$,
K.~Azizi$^{11}$,
F.~Fatehi,
R.~Jafariseyedabad$^{10}$,
M.~Malekhosseini,
S.~Rostami\\
\emph{Department of Physics, University of Tehran, North Karegar Avenue, Tehran 14395-547, Iran}
}

%Ireland, Dublin Institute for Advanced Studies
\addauthor{
V.~Keus\\
\emph{Dublin Institute of Advanced Studies (DIAS), Dublin D04 C932, Ireland}
}

%Israel, Technion – Israel Institute of Technology
\addauthor{
Y.~Soreq\\
\emph{Physics Department, Technion - Israel Institute of Technology, Haifa 3200003, Israel}
}

%Italy, INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine
\addauthor{
M.~Cobal$^{12}$,
G.~Panizzo$^{12}$,
M.~Pinamonti$^{12}$,
L.~Pintucci$^{12}$,
L.~Toffolin$^{12}$\\
\emph{INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine, Via delle Scienze 206, Udine, Italy}
}

%Italy, INFN Laboratori Nazionali di Frascati
\addauthor{
E.~Bagnaschi,
F.~Mescia\\
\emph{INFN, Laboratori Nazionali di Frascati, Via E. Fermi 40, 00044 Frascati, Italy}
}

%Italy, INFN Sezione di Bologna
\addauthor{
G.L.~Alberghi,
L.~Bellagamba\\
\emph{INFN Sezione di Bologna, Viale Carlo Berti Pichat 6/2, 40127 Bologna, Italy}
}

%Italy, INFN Sezione di Firenze
\addauthor{
M.~Tammaro\\
\emph{INFN Sezione di Firenze, Via G. Sansone 1, 50019 Sesto Fiorentino, Italy}
}

%ITALY, INFN Sezione di Lecce
\addauthor{
E.G.~Gorini,
F.G.~Grancagnolo,
M.P.~Primavera\\
\emph{INFN Sezione di Lecce, Lecce, Italy}
}

%Italy, INFN Sezione di Milano
\addauthor{
A.~Andreazza$^{13}$,
C.~Meroni$^{13}$,
F.~Sabatini,
R.~Zanzottera$^{13}$,
M.~Zaro$^{14}$\\
\emph{INFN Sezione di Milano, Via Celoria 16, 20133 Milano, Italy}
}

%Italy, INFN Sezione di Padova
\addauthor{
P.~Azzi,
A.~De Vita,
N.~Selimovi\'c\\
\emph{INFN Sezione di Padova, Via Marzolo 8, 35131 Padova, Italy}
}

%Italy, INFN Sezione di Pavia
\addauthor{
C.~Carloni Calame,
M.~Chiesa,
O.~Nicrosinii,
F.~Piccinini,
G.~Polesello,
N.~Valle\\
\emph{INFN Sezione di Pavia, via A. Bassi 6, 27100 Pavia, Italy}
}

%Italy, INFN Sezione di Perugia
\addauthor{
S.~Ajmal,
O.~Panella\\
\emph{INFN Sezione di Perugia, Via A. Pascoli, 06123, Perugia, Italy}
}

%Italy, INFN Sezione di Pisa
\addauthor{
P.~Azzurri,
D.~Barducci$^{15}$,
D.~Buttazzo,
A.~Dondarini$^{15}$,
A.~Korajac,
G.~Marino$^{15}$,
F.~Palla,
P.~Panci$^{15}$\\
\emph{INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy}
}

%Italy, INFN Sezione di Trieste
\addauthor{
D.~Marzocca\\
\emph{INFN Trieste, Via Valerio 2, 34127 Trieste, Italy}
}

%Italy, Milan University
\addauthor{
A.~Vicini\\
\emph{TIFLab, Universit\`a degli Studi di Milano, Via Celoria 16, 20133 Milano, Italy}
}

%Italy, Politecnico di Bari
\addauthor{
N.~De~Filippis$^{16}$,
F.M.~Procacci$^{16}$\\
\emph{Politecnico di Bari, Via Orabona 4, 70126 Bari, Italy}
}

%Italy, Scuola Normale Superiore
\addauthor{
Alberto Lusiani$^{17}$\\
\emph{Scuola Normale Superiore, Piazza dei Cavalieri 7, 56126 Pisa, Italy}
}

%Italy, Università degli Studi di Padova
\addauthor{
B.A.~Erdelyi$^{18}$,
R.~Gr\"ober$^{18}$,
A.~Rossia$^{18}$\\
\emph{Dipartimento di Fisica e Astronomia "G. Galilei", Universit\`a degli Studi di Padova, 35131 Padova, Italy}
}

%Italy, Università degli Studi di Roma la Sapienza
\addauthor{
M.~Bulliri\\
\emph{Universit\`a degli Studi di Roma la Sapienza, Piazzale Aldo Moro 5, 00185 Rome, Italy}
}

%Italy, Università di Bologna
\addauthor{
M.~Al-Thakeel$^{19}$,
F.~Maltoni$^{20}$\\
\emph{Universit\`a di Bologna, 40126 Bologna, Italy}
}

%Italy, Università di Pavia
\addauthor{
G.~Montagna$^{21}$,
F.~Ucci$^{21}$\\
\emph{Universit\`a di Pavia, 27100 Pavia, Italy}
}

%Italy, Universit`a degli Studi Roma Tre
\addauthor{
R.~Franceschini$^{22}$\\
\emph{Universit\`a degli Studi Roma Tre, Via della Vasca Navale 84, 00146 Rome, Italy}
}

%Japan, High Energy Accelerator Research Organization
\addauthor{
K.~Fujii,
D.~Jeans,
J.~Nakajima\\
\emph{KEK, Tsukuba, Japan}
}

%Japan, Hokkaido University
\addauthor{
A.~Das\\
\emph{Hokkaido University, Sapporo 060-0810, Japan}
}

%Japan, Iwate University
\addauthor{
S.~Narita\\
\emph{Iwate University, Morioka, Iwate 020-8551, Japan}
}

%Japan, Shinshu University
\addauthor{
T.~Takeshita\\
\emph{Shinshu University, Matsumoto, Nagano, Japan}
}

%Japan, The University of Tokyo
\addauthor{
M.~Ishino,
T.~Mori,
T.~Murata,
W.~Ootani,
T.~Seino,
T.~Suehara,
R.~Tagami,
J.~Tian\\
\emph{The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, 113-0033 Tokyo, Japan}
}

%Japan, Tokyo Gakugei University
\addauthor{
K.~Hidaka\\
\emph{Tokyo Gakugei University, Koganei, Tokyo 184-8501, Japan}
}

%Morocco, Cadi Ayyad University
\addauthor{
M.~Ouchemhou\\
\emph{Polydisciplinary Faculty, Laboratory of Fundamental and Applied Physics, Cadi Ayyad University, Sidi Bouzid, B.P. 4162, Safi, Morocco}
}

%Poland, AGH University of Krakow
\addauthor{
H.~Khanpour\\
\emph{AGH University, Faculty of Physics and Applied Computer Science, Al. Mickiewicza 30, 30-055 Krak\'ow, Poland}
}

%Poland, Institute of Nuclear Physics Polish Academy of Sciences
\addauthor{
J.~Bhom,
P.~Bruckman,
M.~Chrzaszcz,
A.~Kaczmarska,
M.~Kucharczyk,
T.~Lesiak,
P.~Malecki,
M.~Skrzypek,
Z.~Was\\
\emph{The Henryk Niewodnicza\'nski
Institute of Nuclear Physics
Polish Academy of Sciences
ul. Radzikowskiego 152,
31-342 Krak\'ow, Poland}
}

%Poland, Jagiellonian University in Krakow
\addauthor{
A.~Price,
W.~P{\l}aczek,
A.~Si\'odmok\\
\emph{Faculty of Physics, Astronomy and Applied Computer Science, ul. Lojasiewicza 11, 30-348 Krak\'ow, Poland}
}

%Poland, University of Warsaw
\addauthor{
B.~Brudnowski,
J.~Kalinowski,
J.~Klamka,
K.~Mekala$^{23}$,
K.~Sakurai,
A.F.~\.Zarnecki,
K.~Zembaczy\'nski\\
\emph{Faculty of Physics, University of Warsaw, Warsaw, Poland}
}

%Portugal, Centro de Física Teórica de Partículas, Instituto Superior Técnico, Universidade de Lisboa
\addauthor{
J.~Hajer,
B.~Oliveira\\
\emph{Centro de F\'isica Te\'orica de Part\'iculas (CFTP), Instituto Superior T\'ecnico (IST), Universidade de Lisboa, 1049-001 Lisboa, Portugal}
}

%Portugal, Laboratório de Instrumentação e Física Experimental de Partículas
\addauthor{
N.F.~Castro$^{24}$,
G.~Chachamis$^{25}$\\
\emph{LIP -- Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas, Escola de Ci\`encias, Campus de Gualtar, Universidade do Minho, 4701-057 Braga, Portugal}
}

%%Russian Federation, Joint Institute for Nuclear Research
%\addauthor{
%A.~Nesterenko\\
%\emph{Joint Institute for Nuclear Research, Dubna, 141980, Russian Federation}
%}
%
%%Russian Federation, National Research Nuclear University MEPhI
%\addauthor{
%V. A.~Okorokov\\
%\emph{National Research Nuclear University MEPhI, Kashirskoe shosse 31, 115409 Moscow, Russian Federation}
%}

%Serbia, Vinca Institute of Nuclear Sciences
\addauthor{
I.~Bozovic$^{26}$,
G.~Kacarevic,
G.~Milutinovic-Dumbelovic,
I.~Smiljanic,
I.~Vidakovic,
N.~Vukasinovic\\
\emph{Vin\v{c}a Institute of Nuclear Sciences, University of Belgrade, Belgrade, Serbia}
}

%Spain, Centro de Investigaciones  Energéticas, Medioambientales y Tecnológicas
\addauthor{
J.~Alcaraz Maestre$^{27}$,
M.~Cepeda$^{28}$,
M.C.~Fouz$^{27}$\\
\emph{Centro de Investigaciones  Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT)
Madrid, Spain}
}

%Spain, IFIC, CSIC-Universitat de València
\addauthor{
J.~Fuster,
A.~Irles,
L.~Mantani,
J.P.~M\'arquez,
V.A.~Mitsou,
M.~Moreno~Ll\'acer,
E.~Musumeci,
B.~Pattnaik,
A.~Saibel,
M.A.~Sanchis,
M.~Vos,
J.~Zurita\\
\emph{IFIC, CSIC-Universitat de Val\`encia, Valencia, Spain}
}

%Spain, Instituto de Física de Cantabria
\addauthor{
A.~Ruiz~Jimeno\\
\emph{Instituto de F\'isica de Cantabria, Av de los Castros, 39005 Santander, Spain}
}

%Spain, Instituto de Física Teórica, CSIC-Universidad Autónoma de Madrid
\addauthor{
J.A.~Aguilar-Saavedra,
S.~Heinemeyer,
A.~Sabio Vera$^{29}$\\
\emph{Instituto de F\'isica Te\'orica, CSIC-Universidad Aut\'onoma de Madrid, Madrid, Spain}
}

%Spain, Instituto Galego de Física de Altas Enerxías (IGFAE), Universidade de Santiago de Compostela
\addauthor{
I.~Corredoira\\
\emph{Instituto Galego de F\'isica de Altas Enerx\'ias (IGFAE), Universidade de Santiago de Compostela
Santiago de Compostela, Spain}
}

%Spain, Universidad de Alcalá
\addauthor{
F.~G.~Celiberto$^{30}$\\
\emph{Alcal\'a de Henares, Madrid, E-28805, Spain}
}

%Spain, Universidad de Cordoba
\addauthor{
F.~Cornet-Gomez\\
\emph{Campus Universitario de Rabanales, Ctra. N-IVa, Km. 396. 14071, Cordoba, Spain}
}

%Spain, Universidad de Granada
\addauthor{
M.~Chala,
J.~de Blas\\
\emph{Departamento de F\'isica Te\'orica y del Cosmos, Universidad de Granada,
Campus de Fuentenueva, 18071 Granada, Spain}
}

%Sweden, KTH Royal Institute of Technology
\addauthor{
M.~Vande Voorde\\
\emph{Department of Physics, Royal Institute of Technology, Stockholm; Sweden}
}

%Sweden, Lund University
\addauthor{
T.~Sj\"ostrand\\
\emph{Department of Physics, Lund University, Lund, Sweden}
}

%Sweden, Uppsala University
\addauthor{
A.~Gall\'en,
R.~Gonzalez Suarez,
G.~Ripellino\\
\emph{Department of Physics and Astronomy, Uppsala University, L{\"a}gerhyggsv{\"a}gen 1, Uppsala, 752 37, Sweden}
}

%Switzerland, CERN
\addauthor{
M.~Al-Thakeel,
S.~Aumiller,
V.~Cairo,
J.~M.~Carceller,
C.~Cornella,
D.~d'Enterria,
J.~Davighi,
M.~M.~Defranchis,
M.~Di Carlo,
F.~Erben,
B.~Francois,
G.~Ganis,
D.~Garcia,
G.~Guerrieri,
A.~J\"uttner,
S.~Kuberski,
A.~Mehta,
L.~Reichenbach$^{31}$,
A.~Sailer,
S.~Sasikumar,
M.~Selvaggi,
J.~Smiesko,
A.~Tolosa-Delgado,
J.~T.~Tsang\\
\emph{CERN, Geneva, Switzerland}
}

%Switzerland, Eidgenössische Technische Hochschule Zürich
\addauthor{
S.~Thor\\
\emph{ETH Z\"{u}rich, 8092 Z\"{u}rich, Switzerland}
}

%Switzerland, Paul Scherrer Institute
\addauthor{
L.~Biermann,
M.~Spira\\
\emph{Paul Scherrer Institute
Particle Physics Theory Group LTP
Forschungsstrasse 111
5232 Villigen PSI, Switzerland}
}

%Switzerland, Université de Genève
\addauthor{
T.~Critchley,
P.~Kontaxakis,
A.~Sfyrla\\
\emph{D\'epartement de Physique Nucl\'eaire et Corpusculaire (DPNC), Universit\'e de Gen\`eve, 1205 Gen\`eve, Switzerland}
}

%Switzerland, University of Basel
\addauthor{
S.~Antusch,
A.~Greljo\\
\emph{Department of Physics, University of Basel, 4056 Basel, Switzerland}
}

%Switzerland, University of Zurich
\addauthor{
M.~Bordone$^{32}$,
F.~Canelli,
A.~Ilg,
G.~Isidori,
B.~Kilminster,
T.H.~Kwok,
V.~Lukashenko,
A.~Macchiolo,
Z.~Polonsky\\
\emph{Physik-Institut, University of Zurich, 8057 Z\"urich, Switzerland}
}

%T"urkiye, Bolu Abant Izzet Baysal University
\addauthor{
H.~Denizli,
A.~Senol\\
\emph{Department of Physics, Bolu Abant Izzet Baysal University, 14280 Bolu, T\"urkiye}
}

%T"urkiye, Institute of Accelerator Technologies (Ankara University)
\addauthor{
H.~Duran Yildiz\\
\emph{Institute of Accelerator Technologies, Ankara University, Ankara, T\"urkiye}
}

%The Netherlands, Nikhef
\addauthor{
P.~Koppenburg,
J.~Rojo$^{33}$\\
\emph{Nikhef, Science Park 105, 1098 XG Amsterdam, The Netherlands}
}

%The Netherlands, University of Amsterdam
\addauthor{
J.~Klari\'c$^{34}$,
V.~Plakkot$^{35}$\\
\emph{University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands}
}

%UK, University of Oxford
\addauthor{
P.N.~Burrows,
C.~Hays,
G.~Wilkinson\\
\emph{Department of Physics, University of Oxford, Oxford OX1 5NZ, UK}
}

%Ukraine, National Science Center ``Kharkiv Institute of Physics and Technology''
\addauthor{
E.~Bulyak\\
\emph{NSC KIPT, 1 Academichna Str. Kharkiv UA-61108, Ukraine}
}

%United Kingdom, Imperial College London
\addauthor{
E.~Curtis,
A.-M.~Magnan,
N.~Wardle\\
\emph{The Blackett Laboratory, Imperial College, London SW7 2BW, United Kingdom}
}

%United Kingdom, University of Edinburgh
\addauthor{
S.~Farrington,
C.~Leonidopoulos$^*$,
J.~Silva,
J.~ter Hoeve\\
\emph{University of Edinburgh, Edinburgh EH9 3FD, United Kingdom}
}

%United Kingdom, University of Glasgow
\addauthor{
C.~Englert,
M.~Miralles L\'opez,
J.~Nesbitt,
D.~Protopopescu,
S.~Renner,
A.~Robson$^*$,
Y.~Zhang\\
\emph{University of Glasgow, Glasgow G12 8QQ, Scotland, United Kingdom}
}

%United Kingdom, University of Manchester
\addauthor{
J.M.~Burridge,
E.~Celada,
A.J.~Costa,
V.~Miralles,
A.~Pilkington,
M.~Thomas,
E.~Vryonidou,
A.R.~Wiederhold\\
\emph{University of Manchester, Manchester M13 9PL, United Kingdom}
}

%United Kingom, Cavendish Laboratory, University of Cambridge
\addauthor{
J.~Hayward,
M.~Kenzie,
S.~Williams\\
\emph{Cavendish Laboratory, University of Cambridge, Cambridge CB3 0HE, United Kingom}
}

%USA, Baylor University
\addauthor{
B.F.L.~Ward\\
\emph{Baylor University, Waco, TX 76798-7316, USA}
}

%USA, Brookhaven National Laboratory
\addauthor{
H.~Abidi,
K.A.~Assamagan,
D.~Boye,
E.~Brost,
V.~Cavaliere,
A.E.~Connelly,
~C. L. Del Pio,
G.~Iakovidis,
A.~Li,
M.A.~Pleier,
A.~Sciandra,
S.~Snyder,
R.H.~Szafron,
A.~Tishelman-Charny,
I.~Veli\v{s}\v{c}ek\\
\emph{Brookhaven National Laboratory, Upton, NY 11973-5000, USA}
}

%USA, Brown University
\addauthor{
L.~Gouskos,
L.~Li\\
\emph{Brown University, 182 Hope Street, Providence, RI 02912, USA}
}

%USA, Fermi National Accelerator Laboratory
\addauthor{
L.~Gray\\
\emph{Fermilab, PO Box 500, Batavia, IL 60510, USA}
}

%USA, Jefferson Lab
\addauthor{
Z.~Yu\\
\emph{Theory Center, Jefferson Lab, Newport News, Virginia 23606, USA}
}

%USA, Johns Hopkins University
\addauthor{
N.~Pinto$^{36}$\\
\emph{Johns Hopkins University, Baltimore, Maryland 21218, USA}
}

%USA, Massachusetts Institute of Technology
\addauthor{
J.~Eysermans\\
\emph{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
}

%USA, Michigan State University
\addauthor{
R.~Schwienhorst,
C.-P.~Yuan$^{37}$\\
\emph{Department of Physics and Astronomy, Michigan State University, East Lansing, Michigan 48824, USA}
}

%USA, Northeastern University
\addauthor{
M.~Larson,
L.~Skinnari\\
\emph{Northeastern University, Boston, Massachusetts 02115, USA}
}

%USA, Princeton University
\addauthor{
W.~Chung,
L. S.~Mandacar\'{u} Guerra\\
\emph{Princeton University, Princeton, New Jersey 08544, USA}
}

%USA, SLAC National Accelerator Laboratory
\addauthor{
D.~Ntounis,
C.~Vernieri\\
\emph{SLAC, 2575 Sand Hill Rd, Menlo Park, CA 94025, USA}
}

%USA, Stony Brook University
\addauthor{
V.~Dao\\
\emph{Stony Brook University, 100 Nicolls Rd, Stony Brook, NY 11794, USA}
}

%USA, Texas Tech University
\addauthor{
V.~Slokenbergs\\
\emph{Texas Tech University, Lubbock, Texas, 79409, USA}
}

%USA, University of Alabama
\addauthor{
N.~Okada\\
\emph{University of Alabama, Tuscaloosa, Alabama 35487, USA}
}

%USA, University of California, Davis
\addauthor{
H.-C.~Cheng\\
\emph{University of California, One Shields Avenue, Davis, California, USA}
}

%USA, University of California, Santa Cruz
\addauthor{
W.~Altmannshofer\\
\emph{University of California, Santa Cruz, CA 95064, USA}
}

%USA, University of Cincinnati
\addauthor{
M.~Szewc$^{38}$\\
\emph{Department of Physics, University of Cincinnati, Cincinnati, Ohio 45221, USA}
}

%USA, University of Kansas
\addauthor{
G.W.~Wilson\\
\emph{University of Kansas, Lawrence, KS 66045, USA}
}

%USA, University of Maryland-College Park
\addauthor{
S.~Airen\\
\emph{University of Maryland-College Park,
College Park, Maryland 20740, USA}
}

%USA, University of Pittsburgh
\addauthor{
A.~Freitas\\
\emph{University of Pittsburgh, Pittsburgh, PA 15260, USA}
}

%USA, University of Wisconsin-Madison
\addauthor{
S.~Dasu,
A.~Mohammadi,
C.-H.~Nee\\
\emph{University of Wisconsin-Madison, Madison, WI 53706-1390, USA}
}

%USA, Yale University
\addauthor{
T.~Lagouri\\
\emph{Yale University, New Haven CT, USA}
}

%%Russian Federation
\addauthor{
A.~Nesterenko{$^{39}$},\\
V.A.~Okorokov{$^{40}$}\\
\emph{Affiliated with an institute covered by a cooperation agreement with CERN}
}

\addauthor{
A.~V.~Gritsan{$^{31}$},\\
\emph{Affiliated with an institute covered by a cooperation agreement between the US DOE, US NSF, and CERN}
}

\addauthor{
\begin{flushleft}
{$^{0}$}Also at ARC Centre of Excellence for Dark Matter Particle Physics, Australia\\
{$^{1}$}Also at University of Vienna\\
{$^{2}$}Also at Physik-Institut, University of Zurich, 8057 Z\"urich, Switzerland\\
{$^{3}$}Also at Department of Physics, Simon Fraser University, University Drive W, Burnaby, Canada\\
{$^{4}$}Also at China Center of Advanced Science and Technology, Beijing, China\\
{$^{5}$}Also at Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), Sorbonne Universit\'e et CNRS, Paris\\
{$^{6}$}Also at University of Hamburg, Hamburg, Germany\\
{$^{7}$}Also at Weizmann Institute of Science, 234 Herzl Street, POB 26, Rehovot 7610001, Israel\\
{$^{8}$}Also at LPCA, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand, France\\
{$^{9}$}Also at Physics Department, Faculty of Sciences, Arak University, Arak\\
{$^{10}$}Also at Department of Physics, Faculty of Science, Ferdowsi University of Mashhad, Mashhad, Iran\\
{$^{11}$}Also at Department of Physics, Do\v{g}u\c{s} University, Dudullu-\"{U}mraniye, 34775 Istanbul, T\"urkiye\\
{$^{12}$}Also at Dipartimento
PolitecniAlso at co di Ingegneria e Architettura, Università di Udine, Udine\\
{$^{13}$}Also at Dipartimento di Fisica, Università degli Studi di Milano, 20133 Milano, Italy\\
{$^{14}$}Also at TIFLab, Università degli Studi di Milano, 20133 Milano, Italy\\
{$^{15}$}Also at Universit\`a di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy\\
{$^{16}$}Also at INFN Sezione di Bari, Via Orbona 4, 70126 Bari, Italy\\
{$^{17}$}Also at INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy\\
{$^{18}$}Also at INFN Sezione di Padova, Via Marzolo 8, 35131 Padova, Italy\\
{$^{19}$}Also at INFN Sezione di Bologna, Viale Carlo Berti Pichat 6/2, 40127 Bologna, Italy\\
{$^{20}$}Also at Universit\'e catholique de Louvain\\
{$^{21}$}Also at INFN Sezione di Pavia, via A. Bassi 6, 27100 Pavia, Italy\\
{$^{22}$}Also at INFN Sezione di Roma Tre, Via della Vasca Navale 84, 00146 Rome, Italy\\
{$^{23}$}Also at DESY, Hamburg, Germany\\
{$^{24}$}Also at Departamento de F\'{i}sica, Escola de Ci\^{e}ncias, Universidade do Minho, 4710-057 Braga, Portugal\\
{$^{25}$}Also at LIP -- Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas, Lisboa, Portugal\\
{$^{26}$}Supported by Fund of Science RS, Grant IDEJE HIGHTONE-P\\
{$^{27}$}Grant PID2021-122134NB-C22 funded by MICIU/AEI/10.13039/501100011033\\
{$^{28}$}Grants PID2021-122134NB-C22 and CNS2023-144781, funded by MCIU/AEI/10.13039/501100011033 and by European Union NextGenerationEU/PRTR\\
{$^{29}$}Also at Universidad Autonoma de Madrid, E-28049 Madrid, Spain\\
{$^{30}$}F.G.C. acknowledges support from the Atracci\'on de Talento Grant n. 2022-T1/TIC-24176 of the Comunidad Aut\'onoma de Madrid, Spain.\\
{$^{31}$}Also at University of Bonn, Physikalisches Institut, Nussallee 12, 53115 Bonn\\
{$^{32}$}Also at CERN, Geneva, Switzerland\\
{$^{33}$}Also at Department of Physics and Astronomy, Vrije Universiteit, NL-1081 HV Amsterdam, The Netherlands\\
{$^{34}$}Also at University of Zagreb, Bijeni\v{c}ka c. 32, 10000 Zagreb, Croatia\\
{$^{35}$}Also at Nikhef, Science Park 105, 1098 XG Amsterdam, The Netherlands\\
{$^{36}$}NP acknowledges support in part by the US NSF grant PHY-2310072\\
{$^{37}$}Supported by the U.S. National Science Foundation under Grant No.~PHY-2310291.\\
{$^{38}$}MS acknowledges support in part by NSF grants OAC-2103889, OAC-2411215 and OAC-2417682 and by DOE grant DE-SC101977.
Also at International Center for Advanced Studies (ICAS), ICIFI and ECyT-UNSAM, 25 de Mayo y Francia, 1650 San Mart\'{i}n, Buenos Aires, Argentina\\
{$^{39}$} https://orcid.org/0000-0003-4747-699X\\
{$^{40}$} https://orcid.org/0000-0002-7162-5345\\
{$^{41}$} https://orcid.org/0000-0002-3545-7970\\
{$^*$}Editors
\end{flushleft}
}




==> ecfa_authors_p3_YR2format_250522.tex <==
% Author list for 'ECFA Higgs/top/electroweak Factory Study Report' in YR2 format
% automatically generated on 2025-05-22 at 10:05:06 Europe/London
% via https://www.ppe.gla.ac.uk
% 371 authors

%Australia, Monash University
\addauthor{
J.~Altmann,
P.~Skands\\
\emph{Monash University, Wellington Road, Clayton VIC-3800, Australia}
}

%Australia, University of Adelaide
\addauthor{
A.~Desai$^{0}$\\
\emph{The University of Adelaide, Adelaide, SA 5005, Australia}
}

%Austria, Institute of High Energy Physics, Vienna
\addauthor{
W.~Mitaroff\\
\emph{Institute of High Energy Physics, Austrian Academy of Sciences, 1050 Vienna, Austria}
}

%Austria, University of Graz
\addauthor{
S.~Pl\"atzer$^{1}$\\
\emph{Institute of Physics, NAWI Graz, University of Graz, Universit\"atsplatz 5, 8010 Graz, Austria}
}

%Belgium, Ghent University
\addauthor{
D.~Dobur,
K.~Skovpen\\
\emph{Ghent University, Proeftuinstraat 86, 9000 Gent, Belgium}
}

%Belgium, Université catholique de Louvain
\addauthor{
M. ~Drewes,
G.~Durieux,
Y.~Georis,
Y.~Ma\\
\emph{Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e catholique de Louvain, 1348 Louvain-la-Neuve, Belgium}
}

%Belgium, Vrije Universiteit Brussel
\addauthor{
A.~De Moor,
K.~Gautam$^{2}$,
E.~Ploerer$^{2}$,
M.~Tytgat\\
\emph{Inter-University Institute for High Energies, Vrije Universiteit Brussel,
Pleinlaan 2, 1050 Ixelles, Belgium}
}

%Brazil, Universidade do Estado do Rio de Janeiro
\addauthor{
K.~Mota~Amarilo\\
\emph{Universidade do Estado do Rio de Janeiro, Rio de Janeiro, Brazil}
}

%Canada, TRIUMF
\addauthor{
M.J.~Basso$^{3}$\\
\emph{TRIUMF, Wesbrook Mall, Vancouver, Canada}
}

%China, Fudan University
\addauthor{
J.~Gu\\
\emph{Department of Physics and Center for Field Theory and Particle Physics, Fudan University,
Shanghai 200438, China}
}

%China, Hefei University of Technology
\addauthor{
Y.~Zhang\\
\emph{School of Physics, Hefei University of Technology, Hefei 230601, China}
}

%China, Institute of High Energy Physics, Chinese Academy of Sciences
\addauthor{
X.-H.~Jiang$^{4}$,
M.~Ruan,
B.~Yan\\
\emph{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
}

%China, Peking University
\addauthor{
X.-K.~Wen\\
\emph{School of Physics, Peking University, Beijing 100871, China}
}

%China, Sun Yat-sen University
\addauthor{
J.~Liao\\
\emph{School of Physics, Sun Yat-sen University, Guangzhou, 510275, China}
}

%China, Sun Yat-sen University (Shenzhen)
\addauthor{
C.~Li\\
\emph{School of Science, Sun Yat-sen University (SYSU), Shenzhen, 518107, China}
}

%Croatia, Rudjer Boskovic Institute
\addauthor{
T.~Robens\\
\emph{Rudjer Boskovic Institute, Bijenicka cesta 54, 10000 Zagreb, Croatia}
}

%Denmark, Niels Bohr Institute, Copenhagen University
\addauthor{
M.~Dam\\
\emph{Niels Bohr Institute, Copenhagen University, Jagtvej 155, 2200 Copenhagen, Denmark}
}

%France, APC, Laboratoire AstroParticule et Cosmologie, Paris
\addauthor{
G.~Bernardi,
K.~Dewyspelaere,
A.~Maloizel,
G.~Marchiori\\
\emph{APC, Universit\'e Paris Cit\'e, CNRS/IN2P3, Paris, France}
}

%France, Institut de Physique des 2 Infinis de Lyon IN2P3-CNRS/Université Claude Bernard Lyon 1
\addauthor{
S.~Gascon-Shotkin,
E.~Jourd'huy,
C.~Verollet,
J.~Xiao\\
\emph{Institut de Physique des 2 Infinis de Lyon IN2P3-CNRS, rue Enrico Fermi
69622 Villeurbanne, France}
}

%France, Institut Polytechnique des Sciences Avancées
\addauthor{
R.~Perez-Ramos$^{5}$\\
\emph{DRII-IPSA, 94200 Ivry-sur-Seine, France}
}

%France, Laboratoire de Physique de Clermont Auvergne, Université Clermont Auvergne, CNRS/IN2P3
\addauthor{
R.~Madar,
T.~Miralles,
S.~Monteil\\
\emph{LPCA, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand, France}
}

%France, Laboratoire de physique des 2 infinis Irène Joliot-Curie
\addauthor{
Y.~Amhis,
I.~Combes,
N.~Morange,
R.~P\"oschl,
M.~Reboud,
F.~Richard,
O.~Sumensari\\
\emph{IJCLab, Universit\'e Paris-Saclay, CNRS/IN2P3, 91405 Orsay, France}
}

%France, Laboratoire de Physique Théorique et Hautes Energies
\addauthor{
G.~Cacciapaglia\\
\emph{Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), Sorbonne Universit\'e et CNRS, 75252 Paris, France}
}

%France, Laboratoire Leprince-Ringuet
\addauthor{
V.~Balagura,
V.~Boudry,
J.-C.~Brient,
C.~Charlot,
C.~Ochando,
R.~Salerno,
Y.~Shi,
Y.~Sirois\\
\emph{Laboratoire Leprince-Ringuet, Ecole Polytechnique, 91128 Palaiseau, France}
}

%France, LAPP, Université Savoie Mont Blanc, CNRS/IN2P3, Annecy
\addauthor{
O.~Arnaez,
M.~Delmastro,
H.~Taibi,
Z.~Wu\\
\emph{LAPP, 9 Chem. de Bellevue, 74940 Annecy, France}
}

%Germany, Albert-Ludwigs-Universität Freiburg
\addauthor{
S.D.~Dittmaier,
M.~Gabelmann\\
\emph{Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany}
}

%Germany, CNRS Helmholtz Dark Matter Lab
\addauthor{
D.~Zerwas\\
\emph{DMLab, Deutsches Elektronen-Synchrotron DESY, CNRS/IN2P3, Hamburg, Germany}
}

%Germany, DESY Hamburg
\addauthor{
J.~Alimena,
M.~Berggren,
F.~Blekman$^{6}$,
B.~Bliewert,
J.~Braathen,
A.~Filipe Silva,
F.~Gaede,
C.~Grojean,
J.~List,
T.~Madlener$^{7}$,
A.~B.~Meyer,
M.T.~N\'u\~nez Pardo de Vera,
K.~Radchenko Serdula,
J.~Reuter,
F.~Sefkow,
J.~Torndal,
A.~Verduras Schaeidt,
G.~Weiglein\\
\emph{DESY, Hamburg, Germany}
}

%Germany, II. Physikalisches Institut, Georg-August-Universität Göttingen
\addauthor{
K.~K\"oneke\\
\emph{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"ottingen, G\"ottingen, Friedrich-Hund-Platz 1, 37077 G\"ottingen, Germany}
}

%Germany, Johannes Gutenberg Universität Mainz
\addauthor{
B.~Dudar,
F.~Yu\\
\emph{PRISMA+ Cluster of Excellence and Mainz Institute for Theoretical Physics, Johannes Gutenberg University, 55099 Mainz, Germany}
}

%Germany, Karlsruhe Institute of Technology
\addauthor{
S.~Alshamaily,
G.~Brodbek,
U.~Einhaus,
S.~Giappichini,
P.~Goldenzweig,
S.~Keilbach,
J.~Kieseler,
M.~Klute,
M.~Presilla,
F.~Simon,
A.~Wiedl,
X.~Zuo\\
\emph{Karlsruhe Institute of Technology, Karlsruhe, Germany}
}

%Germany, Max-Planck-Institut für Physik
\addauthor{
P.~Lo Chiatto$^{8}$\\
\emph{Max-Planck-Institut f{\"u}r Physik, Boltzmannstra{\ss}e 8, 85748 Garching bei M{\"u}nchen, Germany}
}

%Germany, Rheinische Friedrich-Wilhems-Universität Bonn
\addauthor{
P.~Bechtle,
M.~Vellasco\\
\emph{University of Bonn, Physikalisches Institut, Nussallee 12, 53115 Bonn, Germany}
}

%Germany, TU Dortmund University
\addauthor{
K.~Kr\"oninger,
L.~R\"ohrig$^{9}$\\
\emph{TU Dortmund University, Department of Physics, Otto-Hahn-Str. 4a, 44227 Dortmund, Germany}
}

%Germany, Universität Heidelberg
\addauthor{
H.~Bahl,
M.D.~Tat\\
\emph{Universit\"at Heidelberg, Heidelberg, Germany}
}

%Germany, University of Hamburg
\addauthor{
A.~Grohsjean,
J~Lahiri,
G.~Moortgat-Pick\\
\emph{University of Hamburg, Hamburg, Germany}
}

%Germany, University of Siegen
\addauthor{
W.~Kilian\\
\emph{Center for Particle Physics Siegen, Universit\"at Siegen, 57068 Siegen, Germany}
}

%India, Indian Institute of Technology Guwahati
\addauthor{
P.~Poulose\\
\emph{Indian Institute of Technology Guwahati, Assam 781039, India}
}

%India, The Institute of Mathematical Sciences
\addauthor{
J.~Dutta\\
\emph{The Institute of Mathematical Sciences, CIT Campus, Tharamani, Chennai, Tamil Nadu, 600113, India}
}

%Iran, Institute for Research in Fundamental Sciences
\addauthor{
M.~Mohammadi Najafabadi,
M.~Nourbakhsh,
S.~Tizchang$^{10}$\\
\emph{School of Particles and Accelerators, Institute for Research in Fundamental Sciences (IPM), Artesh Highway, Tehran 1956836681, Iran}
}

%Iran, Isfahan University of Technology
\addauthor{
Z.~Baharyioon,
A.~Jafari\\
\emph{Department of Physics, Isfahan University of Technology, Isfahan, 84156-83111, Iran}
}

%Iran, University of Tehran
\addauthor{
A.~Amiri$^{11}$,
K.~Azizi$^{12}$,
F.~Fatehi,
R.~Jafariseyedabad$^{11}$,
M.~Malekhosseini,
S.~Rostami\\
\emph{Department of Physics, University of Tehran, North Karegar Avenue, Tehran 14395-547, Iran}
}

%Ireland, Dublin Institute for Advanced Studies
\addauthor{
V.~Keus\\
\emph{Dublin Institute of Advanced Studies (DIAS), Dublin D04 C932, Ireland}
}

%Israel, Technion – Israel Institute of Technology
\addauthor{
Y.~Soreq\\
\emph{Physics Department, Technion - Israel Institute of Technology, Haifa 3200003, Israel}
}

%Italy, INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine
\addauthor{
M.~Cobal$^{13}$,
G.~Panizzo$^{13}$,
M.~Pinamonti$^{13}$,
L.~Pintucci$^{13}$,
L.~Toffolin$^{13}$\\
\emph{INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine, Via delle Scienze 206, Udine, Italy}
}

%Italy, INFN Laboratori Nazionali di Frascati
\addauthor{
E.~Bagnaschi,
F.~Mescia\\
\emph{INFN, Laboratori Nazionali di Frascati, Via E. Fermi 40, 00044 Frascati, Italy}
}

%Italy, INFN Sezione di Bologna
\addauthor{
G.L.~Alberghi,
L.~Bellagamba\\
\emph{INFN Sezione di Bologna, Viale Carlo Berti Pichat 6/2, 40127 Bologna, Italy}
}

%Italy, INFN Sezione di Firenze
\addauthor{
M.~Tammaro\\
\emph{INFN Sezione di Firenze, Via G. Sansone 1, 50019 Sesto Fiorentino, Italy}
}

%Italy, INFN Sezione di Lecce
\addauthor{
E.G.~Gorini,
F.G.~Grancagnolo,
M.P.~Primavera\\
\emph{INFN Sezione di Lecce, Lecce, Italy}
}

%Italy, INFN Sezione di Milano
\addauthor{
A.~Andreazza$^{14}$,
C.~Meroni$^{14}$,
F.~Sabatini,
R.~Zanzottera$^{14}$,
M.~Zaro$^{15}$\\
\emph{INFN Sezione di Milano, Via Celoria 16, 20133 Milano, Italy}
}

%Italy, INFN Sezione di Padova
\addauthor{
P.~Azzi,
A.~De Vita,
N.~Selimovi\'c\\
\emph{INFN Sezione di Padova, Via Marzolo 8, 35131 Padova, Italy}
}

%Italy, INFN Sezione di Pavia
\addauthor{
C.~Carloni Calame,
M.~Chiesa,
O.~Nicrosinii,
F.~Piccinini,
G.~Polesello,
N.~Valle\\
\emph{INFN Sezione di Pavia, via A. Bassi 6, 27100 Pavia, Italy}
}

%Italy, INFN Sezione di Perugia
\addauthor{
S.~Ajmal,
O.~Panella\\
\emph{INFN Sezione di Perugia, Via A. Pascoli, 06123, Perugia, Italy}
}

%Italy, INFN Sezione di Pisa
\addauthor{
P.~Azzurri,
D.~Barducci$^{16}$,
D.~Buttazzo,
A.~Dondarini$^{16}$,
A.~Korajac,
G.~Marino$^{16}$,
F.~Palla,
P.~Panci$^{16}$\\
\emph{INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy}
}

%Italy, INFN Sezione di Trieste
\addauthor{
D.~Marzocca\\
\emph{INFN Trieste, Via Valerio 2, 34127 Trieste, Italy}
}

%Italy, Milan University
\addauthor{
A.~Vicini\\
\emph{TIFLab, Universit\`a degli Studi di Milano, Via Celoria 16, 20133 Milano, Italy}
}

%Italy, Politecnico di Bari
\addauthor{
N.~De~Filippis$^{17}$,
F.M.~Procacci$^{17}$\\
\emph{Politecnico di Bari, Via Orabona 4, 70126 Bari, Italy}
}

%Italy, Scuola Normale Superiore
\addauthor{
Alberto Lusiani$^{18}$\\
\emph{Scuola Normale Superiore, Piazza dei Cavalieri 7, 56126 Pisa, Italy}
}

%Italy, Università degli Studi di Padova
\addauthor{
B.A.~Erdelyi$^{19}$,
R.~Gr\"ober$^{19}$,
A.~Rossia$^{19}$\\
\emph{Dipartimento di Fisica e Astronomia "G. Galilei", Universit\`a degli Studi di Padova, 35131 Padova, Italy}
}

%Italy, Università degli Studi di Roma la Sapienza
\addauthor{
M.~Bulliri\\
\emph{Universit\`a degli Studi di Roma la Sapienza, Piazzale Aldo Moro 5, 00185 Rome, Italy}
}

%Italy, Università di Bologna
\addauthor{
M.~Al-Thakeel$^{20}$,
F.~Maltoni$^{21}$\\
\emph{Universit\`a di Bologna, 40126 Bologna, Italy}
}

%Italy, Università di Pavia
\addauthor{
G.~Montagna$^{22}$,
F.~Ucci$^{22}$\\
\emph{Universit\`a di Pavia, 27100 Pavia, Italy}
}

%Italy, Universit`a degli Studi Roma Tre
\addauthor{
R.~Franceschini$^{23}$\\
\emph{Universit\`a degli Studi Roma Tre, Via della Vasca Navale 84, 00146 Rome, Italy}
}

%Japan, High Energy Accelerator Research Organization
\addauthor{
K.~Fujii,
D.~Jeans,
J.~Nakajima\\
\emph{KEK, Tsukuba, Japan}
}

%Japan, Hokkaido University
\addauthor{
A.~Das\\
\emph{Hokkaido University, Sapporo 060-0810, Japan}
}

%Japan, Iwate University
\addauthor{
S.~Narita\\
\emph{Iwate University, Morioka, Iwate 020-8551, Japan}
}

%Japan, Shinshu University
\addauthor{
T.~Takeshita\\
\emph{Shinshu University, Matsumoto, Nagano, Japan}
}

%Japan, The University of Tokyo
\addauthor{
M.~Ishino,
T.~Mori,
T.~Murata,
W.~Ootani,
T.~Seino,
T.~Suehara,
R.~Tagami,
J.~Tian\\
\emph{The University of Tokyo, 7-3-1 Hongo, Bunkyo-ku, 113-0033 Tokyo, Japan}
}

%Japan, Tokyo Gakugei University
\addauthor{
K.~Hidaka\\
\emph{Tokyo Gakugei University, Koganei, Tokyo 184-8501, Japan}
}

%Morocco, Cadi Ayyad University
\addauthor{
M.~Ouchemhou\\
\emph{Polydisciplinary Faculty, Laboratory of Fundamental and Applied Physics, Cadi Ayyad University, Sidi Bouzid, B.P. 4162, Safi, Morocco}
}

%Poland, AGH University of Krakow
\addauthor{
H.~Khanpour\\
\emph{AGH University, Faculty of Physics and Applied Computer Science, Al. Mickiewicza 30, 30-055 Krak\'ow, Poland}
}

%Poland, Institute of Nuclear Physics Polish Academy of Sciences
\addauthor{
J.~Bhom,
P.~Bruckman,
M.~Chrzaszcz,
A.~Kaczmarska,
M.~Kucharczyk,
T.~Lesiak,
P.~Malecki,
M.~Skrzypek,
Z.~Was\\
\emph{The Henryk Niewodnicza\'nski
Institute of Nuclear Physics
Polish Academy of Sciences
ul. Radzikowskiego 152,
31-342 Krak\'ow, Poland}
}

%Poland, Jagiellonian University in Krakow
\addauthor{
A.~Price,
W.~P{\l}aczek,
A.~Si\'odmok$^{24}$\\
\emph{Faculty of Physics, Astronomy and Applied Computer Science, ul. Lojasiewicza 11, 30-348 Krak\'ow, Poland}
}

%Poland, University of Warsaw
\addauthor{
B.~Brudnowski$^{25}$,
J.~Kalinowski,
J.~Klamka$^{25}$,
K.~Mekala$^{26}$,
K.~Sakurai,
A.F.~\.Zarnecki$^{25}$,
K.~Zembaczy\'nski$^{25}$\\
\emph{Faculty of Physics, University of Warsaw, Warsaw, Poland}
}

%Portugal, Centro de Física Teórica de Partículas, Instituto Superior Técnico, Universidade de Lisboa
\addauthor{
J.~Hajer,
B.~Oliveira\\
\emph{Centro de F\'isica Te\'orica de Part\'iculas (CFTP), Instituto Superior T\'ecnico (IST), Universidade de Lisboa, 1049-001 Lisboa, Portugal}
}

%Portugal, Laboratório de Instrumentação e Física Experimental de Partículas
\addauthor{
N.F.~Castro$^{27}$,
G.~Chachamis$^{28}$\\
\emph{LIP -- Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas, Escola de Ci\`encias, Campus de Gualtar, Universidade do Minho, 4701-057 Braga, Portugal}
}

%%Russian Federation, Joint Institute for Nuclear Research
%\addauthor{
%A.~Nesterenko\\
%\emph{Joint Institute for Nuclear Research, Dubna, 141980, Russian Federation}
%}
%
%%Russian Federation, National Research Nuclear University MEPhI
%\addauthor{
%V. A.~Okorokov\\
%\emph{National Research Nuclear University MEPhI, Kashirskoe shosse 31, 115409 Moscow, Russian Federation}
%}

%Serbia, Vinca Institute of Nuclear Sciences
\addauthor{
I.~Bozovic$^{29}$,
G.~Kacarevic,
G.~Milutinovic-Dumbelovic,
I.~Smiljanic,
I.~Vidakovic,
N.~Vukasinovic\\
\emph{Vin\v{c}a Institute of Nuclear Sciences, University of Belgrade, Belgrade, Serbia}
}

%Spain, Centro de Investigaciones  Energéticas, Medioambientales y Tecnológicas
\addauthor{
J.~Alcaraz Maestre$^{30}$,
M.~Cepeda$^{31}$,
M.C.~Fouz$^{30}$\\
\emph{Centro de Investigaciones  Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT)
Madrid, Spain}
}

%Spain, IFIC, CSIC-Universitat de València
\addauthor{
J.~Fuster,
A.~Irles,
L.~Mantani,
J.P.~M\'arquez,
V.A.~Mitsou,
M.~Moreno~Ll\'acer,
E.~Musumeci,
B.~Pattnaik,
A.~Saibel,
M.A.~Sanchis,
M.~Vos,
J.~Zurita\\
\emph{IFIC, CSIC-Universitat de Val\`encia, Valencia, Spain}
}

%Spain, Instituto de Física de Cantabria
\addauthor{
A.~Ruiz~Jimeno\\
\emph{Instituto de F\'isica de Cantabria, Av de los Castros, 39005 Santander, Spain}
}

%Spain, Instituto de Física Teórica, CSIC-Universidad Autónoma de Madrid
\addauthor{
J.A.~Aguilar-Saavedra,
S.~Heinemeyer,
A.~Sabio Vera$^{32}$\\
\emph{Instituto de F\'isica Te\'orica, CSIC-Universidad Aut\'onoma de Madrid, Madrid, Spain}
}

%Spain, Instituto Galego de Física de Altas Enerxías (IGFAE), Universidade de Santiago de Compostela
\addauthor{
I.~Corredoira\\
\emph{Instituto Galego de F\'isica de Altas Enerx\'ias (IGFAE), Universidade de Santiago de Compostela
Santiago de Compostela, Spain}
}

%Spain, Universidad de Alcalá
\addauthor{
F.~G.~Celiberto$^{33}$\\
\emph{Alcal\'a de Henares, Madrid, E-28805, Spain}
}

%Spain, Universidad de Cordoba
\addauthor{
F.~Cornet-Gomez\\
\emph{Campus Universitario de Rabanales, Ctra. N-IVa, Km. 396. 14071, Cordoba, Spain}
}

%Spain, Universidad de Granada
\addauthor{
M.~Chala,
J.~de Blas$^{34}$\\
\emph{Departamento de F\'isica Te\'orica y del Cosmos, Universidad de Granada,
Campus de Fuentenueva, 18071 Granada, Spain}
}

%Sweden, KTH Royal Institute of Technology
\addauthor{
M.~Vande Voorde\\
\emph{Department of Physics, Royal Institute of Technology, Stockholm; Sweden}
}

%Sweden, Lund University
\addauthor{
T.~Sj\"ostrand\\
\emph{Department of Physics, Lund University, Lund, Sweden}
}

%Sweden, Uppsala University
\addauthor{
A.~Gall\'en,
R.~Gonzalez Suarez,
G.~Ripellino\\
\emph{Department of Physics and Astronomy, Uppsala University, L{\"a}gerhyggsv{\"a}gen 1, Uppsala, 752 37, Sweden}
}

%Switzerland, CERN
\addauthor{
S.~Aumiller,
V.~Cairo,
J.~M.~Carceller,
C.~Cornella,
D.~d'Enterria,
J.~Davighi,
M.~M.~Defranchis,
M.~Di Carlo,
F.~Erben,
B.~Francois,
G.~Ganis,
D.~Garcia,
G.~Guerrieri,
A.~J\"uttner,
S.~Kuberski,
A.~Mehta,
L.~Reichenbach$^{35}$,
A.~Sailer$^{7}$,
S.~Sasikumar,
M.~Selvaggi,
J.~Smiesko,
A.~Tolosa-Delgado,
J.~T.~Tsang\\
\emph{CERN, Geneva, Switzerland}
}

%Switzerland, Eidgenössische Technische Hochschule Zürich
\addauthor{
S.~Thor\\
\emph{ETH Z\"{u}rich, 8092 Z\"{u}rich, Switzerland}
}

%Switzerland, Paul Scherrer Institute
\addauthor{
L.~Biermann,
M.~Spira\\
\emph{Paul Scherrer Institute
Particle Physics Theory Group LTP
Forschungsstrasse 111
5232 Villigen PSI, Switzerland}
}

%Switzerland, Université de Genève
\addauthor{
T.~Critchley,
P.~Kontaxakis,
A.~Sfyrla\\
\emph{D\'epartement de Physique Nucl\'eaire et Corpusculaire (DPNC), Universit\'e de Gen\`eve, 1205 Gen\`eve, Switzerland}
}

%Switzerland, University of Basel
\addauthor{
S.~Antusch,
A.~Greljo\\
\emph{Department of Physics, University of Basel, 4056 Basel, Switzerland}
}

%Switzerland, University of Zurich
\addauthor{
M.~Bordone$^{36}$,
F.~Canelli,
A.~Ilg,
G.~Isidori,
B.~Kilminster,
T.H.~Kwok,
V.~Lukashenko,
A.~Macchiolo,
Z.~Polonsky\\
\emph{Physik-Institut, University of Zurich, 8057 Z\"urich, Switzerland}
}

%The Netherlands, Nikhef
\addauthor{
P.~Koppenburg,
J.~Rojo$^{37}$\\
\emph{Nikhef, Science Park 105, 1098 XG Amsterdam, The Netherlands}
}

%The Netherlands, University of Amsterdam
\addauthor{
J.~Klari\'c$^{38}$,
V.~Plakkot$^{39}$\\
\emph{University of Amsterdam, Science Park 904, 1098 XH Amsterdam, The Netherlands}
}

%T\"urkiye, Bolu Abant Izzet Baysal University
\addauthor{
H.~Denizli,
A.~Senol\\
\emph{Department of Physics, Bolu Abant Izzet Baysal University, 14280 Bolu, T\"urkiye}
}

%T\"urkiye, Institute of Accelerator Technologies (Ankara University)
\addauthor{
H.~Duran Yildiz\\
\emph{Institute of Accelerator Technologies, Ankara University, Ankara, T\"urkiye}
}

%UK, University of Oxford
\addauthor{
P.N.~Burrows,
C.~Hays,
G.~Wilkinson\\
\emph{Department of Physics, University of Oxford, Oxford OX1 5NZ, UK}
}

%Ukraine, National Science Center 'Kharkiv Institute of Physics and Technology'
\addauthor{
E.~Bulyak\\
\emph{NSC KIPT, 1 Academichna Str. Kharkiv UA-61108, Ukraine}
}

%United Kingdom, Imperial College London
\addauthor{
E.~Curtis,
A.-M.~Magnan,
N.~Wardle\\
\emph{The Blackett Laboratory, Imperial College, London SW7 2BW, United Kingdom}
}

%United Kingdom, University of Edinburgh
\addauthor{
S.~Farrington,
C.~Leonidopoulos$^*$,
J.~Silva,
J.~ter Hoeve\\
\emph{University of Edinburgh, Edinburgh EH9 3FD, United Kingdom}
}

%United Kingdom, University of Glasgow
\addauthor{
C.~Englert,
M.~Miralles L\'opez,
J.~Nesbitt,
D.~Protopopescu,
S.~Renner,
A.~Robson$^*$,
Y.~Zhang\\
\emph{University of Glasgow, Glasgow G12 8QQ, Scotland, United Kingdom}
}

%United Kingdom, University of Manchester
\addauthor{
J.M.~Burridge,
E.~Celada,
A.J.~Costa,
V.~Miralles,
A.~Pilkington,
M.~Thomas,
E.~Vryonidou,
A.R.~Wiederhold\\
\emph{University of Manchester, Manchester M13 9PL, United Kingdom}
}

%United Kingdom, University of Southampton
\addauthor{
K.~Mimasu\\
\emph{School of Physics and Astronomy, Highfield, Southampton S017 1BJ, United Kingdom}
}

%United Kingom, Cavendish Laboratory, University of Cambridge
\addauthor{
J.~Hayward,
M.~Kenzie,
S.~Williams\\
\emph{Cavendish Laboratory, University of Cambridge, Cambridge CB3 0HE, United Kingom}
}

%USA, Baylor University
\addauthor{
B.F.L.~Ward\\
\emph{Baylor University, Waco, TX 76798-7316, USA}
}

%USA, Brookhaven National Laboratory
\addauthor{
H.~Abidi,
K.A.~Assamagan,
D.~Boye,
E.~Brost,
V.~Cavaliere,
A.E.~Connelly,
~C. L. Del Pio,
G.~Iakovidis,
A.~Li,
M.A.~Pleier,
A.~Sciandra,
S.~Snyder,
R.H.~Szafron,
A.~Tishelman-Charny,
I.~Veli\v{s}\v{c}ek\\
\emph{Brookhaven National Laboratory, Upton, NY 11973-5000, USA}
}

%USA, Brown University
\addauthor{
L.~Gouskos,
L.~Li\\
\emph{Brown University, 182 Hope Street, Providence, RI 02912, USA}
}

%USA, Fermi National Accelerator Laboratory
\addauthor{
L.~Gray\\
\emph{Fermilab, PO Box 500, Batavia, IL 60510, USA}
}

%USA, Jefferson Lab
\addauthor{
Z.~Yu\\
\emph{Theory Center, Jefferson Lab, Newport News, Virginia 23606, USA}
}

%USA, Johns Hopkins University
\addauthor{
N.~Pinto$^{40}$\\
\emph{Johns Hopkins University, Baltimore, Maryland 21218, USA}
}

%USA, Massachusetts Institute of Technology
\addauthor{
J.~Eysermans\\
\emph{Massachusetts Institute of Technology, Cambridge, MA 02139, USA}
}

%USA, Michigan State University
\addauthor{
R.~Schwienhorst,
C.-P.~Yuan$^{41}$\\
\emph{Department of Physics and Astronomy, Michigan State University, East Lansing, Michigan 48824, USA}
}

%USA, Northeastern University
\addauthor{
M.~Larson,
L.~Skinnari\\
\emph{Northeastern University, Boston, Massachusetts 02115, USA}
}

%USA, Princeton University
\addauthor{
W.~Chung,
L. S.~Mandacar\'{u} Guerra\\
\emph{Princeton University, Princeton, New Jersey 08544, USA}
}

%USA, SLAC National Accelerator Laboratory
\addauthor{
D.~Ntounis,
A.~Schwartzman,
C.~Vernieri\\
\emph{SLAC, 2575 Sand Hill Rd, Menlo Park, CA 94025, USA}
}

%USA, Stony Brook University
\addauthor{
V.~Dao\\
\emph{Stony Brook University, 100 Nicolls Rd, Stony Brook, NY 11794, USA}
}

%USA, Texas Tech University
\addauthor{
V.~Slokenbergs\\
\emph{Texas Tech University, Lubbock, Texas, 79409, USA}
}

%USA, University of Alabama
\addauthor{
N.~Okada\\
\emph{University of Alabama, Tuscaloosa, Alabama 35487, USA}
}

%USA, University of California, Davis
\addauthor{
H.-C.~Cheng\\
\emph{University of California, One Shields Avenue, Davis, California, USA}
}

%USA, University of California, Santa Cruz
\addauthor{
W.~Altmannshofer\\
\emph{University of California, Santa Cruz, CA 95064, USA}
}

%USA, University of Cincinnati
\addauthor{
M.~Szewc$^{42}$\\
\emph{Department of Physics, University of Cincinnati, Cincinnati, Ohio 45221, USA}
}

%USA, University of Kansas
\addauthor{
G.W.~Wilson\\
\emph{University of Kansas, Lawrence, KS 66045, USA}
}

%USA, University of Maryland-College Park
\addauthor{
S.~Airen\\
\emph{University of Maryland-College Park,
College Park, Maryland 20740, USA}
}

%USA, University of Pittsburgh
\addauthor{
A.~Freitas\\
\emph{University of Pittsburgh, Pittsburgh, PA 15260, USA}
}

%USA, University of Wisconsin-Madison
\addauthor{
S.~Dasu,
A.~Mohammadi,
C.-H.~Nee\\
\emph{University of Wisconsin-Madison, Madison, WI 53706-1390, USA}
}

%USA, Yale University
\addauthor{
T.~Lagouri\\
\emph{Yale University, New Haven CT, USA}
}

%%Russian Federation
\addauthor{
A.~Nesterenko{$^{43}$},
V.A.~Okorokov{$^{44}$}\\
\emph{Affiliated with an institute covered by a cooperation agreement with CERN}
}

\addauthor{
A.~V.~Gritsan{$^{45}$},\\
\emph{Affiliated with an institute covered by a cooperation agreement between the US DOE, US NSF, and CERN}
}

\addauthor{
\begin{flushleft}
\small{
{$^{0}$}Also at ARC Centre of Excellence for Dark Matter Particle Physics, Australia\\
{$^{1}$}Also at Particle Physics, Faculty of Physics, University of Vienna, Boltzmanngasse 5, A-1090 Wien, Austria\\
{$^{2}$}Also at Physik-Institut, University of Zurich, 8057 Z\"urich, Switzerland\\
{$^{3}$}Also at Department of Physics, Simon Fraser University, University Drive W, Burnaby, Canada\\
{$^{4}$}Also at China Center of Advanced Science and Technology, Beijing, China; supported in part by the National Natural Science Foundation of China under grant No. 12342502.\\
{$^{5}$}Also at Laboratoire de Physique Th\'eorique et Hautes Energies (LPTHE), Sorbonne Universit\'e et CNRS, Paris\\
{$^{6}$}Also at University of Hamburg, Hamburg, Germany\\
{$^{7}$}Supported by the EU's Horizon 2020 Research and Innovation programme under Grant Agreement No 101004761\\
{$^{8}$}Also at Weizmann Institute of Science, 234 Herzl Street, POB 26, Rehovot 7610001, Israel\\
{$^{9}$}Also at LPCA, Universit\'e Clermont Auvergne, CNRS/IN2P3, Clermont-Ferrand, France\\
{$^{10}$}Also at Physics Department, Faculty of Sciences, Arak University, Arak, Iran\\
{$^{11}$}Also at Department of Physics, Faculty of Science, Ferdowsi University of Mashhad, Mashhad, Iran\\
{$^{12}$}Also at Department of Physics, Do\v{g}u\c{s} University, Dudullu-\"{U}mraniye, 34775 Istanbul, T\"urkiye\\
{$^{13}$}Also at Dipartimento Politecnico di Ingegneria e Architettura, Universit\`a di Udine, Udine\\
{$^{14}$}Also at Dipartimento di Fisica, Università degli Studi di Milano, 20133 Milano, Italy\\
{$^{15}$}Also at TIFLab, Università degli Studi di Milano, 20133 Milano, Italy\\
{$^{16}$}Also at Universit\`a di Pisa, Lungarno Pacinotti 43, 56126 Pisa, Italy\\
{$^{17}$}Also at INFN Sezione di Bari, Via Orbona 4, 70126 Bari, Italy\\
{$^{18}$}Also at INFN Sezione di Pisa, Largo Bruno Pontecorvo 3, 56127, Pisa, Italy\\
{$^{19}$}Also at INFN Sezione di Padova, Via Marzolo 8, 35131 Padova, Italy\\
{$^{20}$}Also at INFN Sezione di Bologna, Viale Carlo Berti Pichat 6/2, 40127 Bologna, Italy\\
{$^{21}$}Also at Universit\'e catholique de Louvain, 1348 Louvain-la-Neuve, Belgium\\
{$^{22}$}Also at INFN Sezione di Pavia, via A. Bassi 6, 27100 Pavia, Italy\\
{$^{23}$}Also at INFN Sezione di Roma Tre, Via della Vasca Navale 84, 00146 Rome, Italy\\
{$^{24}$}Supported by the National Science Centre, Poland, under awards 2023/50/A/ST2/00224 and 2019/34/E/ST2/00457\\
{$^{25}$}Supported by the National Science Centre, Poland, under the OPUS research project no. 2021/43/B/ST2/01778\\
{$^{26}$}Also at DESY Hamburg.  Supported by the National Science Centre, Poland, under the OPUS research project no. 2021/43/B/ST2/01778\\
{$^{27}$}Also at Departamento de F\'{i}sica, Escola de Ci\^{e}ncias, Universidade do Minho, 4710-057 Braga, Portugal\\
{$^{28}$}Also at LIP -- Laborat\'orio de Instrumenta\c{c}\~ao e F\'isica Experimental de Part\'iculas, Lisboa, Portugal\\
{$^{29}$}Supported by Fund of Science RS, Grant IDEJE HIGHTONE-P\\
{$^{30}$}Supported by Grant PID2021-122134NB-C22 funded by MICIU/AEI/10.13039/501100011033\\
{$^{31}$}Supported by Grants PID2021-122134NB-C22 and CNS2023-144781, funded by MCIU/AEI/10.13039/501100011033 and by European Union NextGenerationEU/PRTR\\
{$^{32}$}Also at Universidad Autonoma de Madrid, E-28049 Madrid, Spain\\
{$^{33}$}Supported by the Atracci\'on de Talento Grant n. 2022-T1/TIC-24176 of the Comunidad Aut\'onoma de Madrid, Spain\\
{$^{34}$}Partially funded by MICIU/AEI/10.13039/501100011033 and FEDER/UE (grant PID2022-139466NB-C21)\\
{$^{35}$}Also at University of Bonn, Physikalisches Institut, Nussallee 12, 53115 Bonn, Germany.  Supported by the Wolfgang Gentner Programme of the German Federal Ministry of Education and Research (grant no. 13E18CHA)\\
{$^{36}$}Also at CERN, Geneva, Switzerland\\
{$^{37}$}Also at Department of Physics and Astronomy, Vrije Universiteit, NL-1081 HV Amsterdam, The Netherlands\\
{$^{38}$}Also at University of Zagreb, Bijeni\v{c}ka c. 32, 10000 Zagreb, Croatia\\
{$^{39}$}Also at Nikhef, Science Park 105, 1098 XG Amsterdam, The Netherlands\\
{$^{40}$}Supported in part by the US NSF grant PHY-2310072\\
{$^{41}$}Supported by the U.S. National Science Foundation under Grant No.~PHY-2310291\\
{$^{42}$}Supported in part by NSF grants OAC-2103889, OAC-2411215 and OAC-2417682 and by DOE grant DE-SC101977; also at International Center for Advanced Studies (ICAS), ICIFI and ECyT-UNSAM, 25 de Mayo y Francia, 1650 San Mart\'{i}n, Buenos Aires, Argentina\\
{$^{43}$} https://orcid.org/0000-0003-4747-699X\\
{$^{44}$} https://orcid.org/0000-0002-7162-5345\\
{$^{45}$} https://orcid.org/0000-0002-3545-7970\\
{$^*$}Editors
}
\end{flushleft}
}



==> ecfa_coordsIAC.tex <==


\begin{center}
{\LARGE{ECFA Higgs, electroweak, and top factory study}}
\end{center}

\vspace*{5mm}

\begin{adjustwidth*}{1.3cm}{1.3cm}

The ECFA Higgs, electroweak, and top Factory Study ran between 2021 and 2025 as a broad effort across the experimental and theoretical particle physics communities, bringing together participants from many different proposed future collider projects.  Activities across three main working groups advanced the joint development of tools and analysis techniques, fostered new considerations of detector design and optimisation, and led to a new set of studies resulting in improved projected sensitivities across a wide physics programme. This report demonstrates the significant expansion in the state-of-the-art understanding of the physics potential of future \epem Higgs, electroweak, and top factories, and has been submitted as input to the 2025 European Strategy for Particle Physics Update.

\end{adjustwidth*}


\vspace*{15mm}


\begin{adjustwidth*}{1.3cm}{-1cm}
\noindent {\Large{Study Coordinators:}}

\begin{multicols}{2}
\noindent\textbf{WG1 Physics Performance}\\
Jorge de Blas (Granada)\\
Patrick Koppenburg (Nikhef)\\
Jenny List (DESY)\\
Fabio Maltoni (UC Louvain / Bologna)\\
\emph{Former coordinator:}\\ 
Juan Alcaraz Maestre (CIEMAT Madrid)

\vspace*{5mm}
\noindent\textbf{Chief Editors}\\
Christos Leonidopoulos (Edinburgh)\\
Aidan Robson (Glasgow)

\columnbreak
\noindent\textbf{WG2 Physics Analysis Methods}\\
Patrizia Azzi (INFN Padova)\\
Fulvio Piccinini (INFN Pavia)\\
Dirk Zerwas (IJCLab/DMLab)

\vspace*{5mm}
\noindent\textbf{WG3 Detector R\&D}\\
Mary Cruz Fouz (CIEMAT Madrid)\\
Giovanni Marchiori (APC Paris)\\
Felix Sefkow (DESY)
\end{multicols}

\vspace*{8mm}
\noindent {\Large{International Advisory Committee:}}

\begin{multicols}{2}
\noindent Jean-Claude Brient (Paris LLR)\\
Patricia Conde Muino (IST/LIP)\\
Didier Contardo (IN2P3)\\
Mogens Dam (Copenhagen NBI)\\
Juan Fuster (Valencia)\\
Jorgen D’Hondt (VU Brussel)\\
Christophe Grojean (DESY)\\
Patrick Janot (CERN)\\
Christos Leonidopoulos (Edinburgh)\\
Tadeusz Lesiak (Krakow)\\
Chiara Meroni (Milano)\\
Joachim Mnich (CERN)\\
Aleandro Nisati (Rome I)\\
Aidan Robson (Glasgow)\\
Frank Simon (KIT)\\
Paris Sphicas (Athens/CERN, Chair)\\
Steinar Stapnes (CERN)\\
Roberto Tenchini (Pisa)\\
Guy Wilkinson (Oxford)\\
Andrea Wulzer (Lausanne)\\
\end{multicols}
\noindent \emph{Former members:}\\
Alain Blondel (Geneva)\\
Karl Jakobs (Freiburg, former Chair)\\
Max Klein (Liverpool)

\end{adjustwidth*}

%\vspace*{7mm}
\clearpage
\noindent{\Large{Contributors:}}



==> sections/commontools/MovedFromWG1.tex <==
% \subsection{Reconstruction and simulation details moved here by the WG1 coordinators}
% {\color{red}PK: WG2 conveners, please move to where appropriate.}

% {\color{red} DZ: VcbVcsFT is to a large extent a duplication of the discussion of taggers in the reconstruction section, this could be mediated by referring to the reconstruction chapter in the physics section and providing the table as added value in the physics section}

% \input{sections/flavour/VcbVcsFT}

% {\color{red} DZ: the fragmentation section is too detailed to be integrated into \ref{sec:gen} and limited to a single implementation of a specfic process, IMHO better suited for \ref{sec:higgs}}
% \input{sections/higgs/HtoSS-frag}

% \input{sections/higgs/HtoSS-perf}

==> sections/higgs/cpinhzz.tex <==
\subsubsection*{Introduction}

\newcommand{\OHBtil}{\ensuremath{\widetilde{\mathcal{O}}_{\Phi\widetilde{B}}}\xspace}
\newcommand{\OHWtil}{\ensuremath{\widetilde{\mathcal{O}}_{\Phi\widetilde{W}}}\xspace}
\newcommand{\OHWtilB}{\ensuremath{\widetilde{\mathcal{O}}_{\Phi\widetilde{W}B}}\xspace}
\newcommand{\cHBtil}{\ensuremath{c_{\Phi\widetilde{B}}}\xspace}
\newcommand{\cHWtil}{\ensuremath{c_{\Phi\widetilde{W}}}\xspace}
\newcommand{\cHWtilB}{\ensuremath{c_{\Phi\widetilde{W}B}}\xspace}
\newcommand{\Zee}{\ensuremath{\PZ\to\Pe\Pe}\xspace}
\newcommand{\Zmm}{\ensuremath{\PZ\to\PGm\PGm}\xspace}

The established \CP violation in the Standard Model (SM) is insufficient to account for the matter dominance observed in the Universe, therefore searches for additional sources of \CP violation are well-motivated to connect the SM with paradigms of baryogenesis through new interactions. An effective field theory approach provides one framework for searching for \CP-violating effects in a motivated higher-dimensional operator deformation of the SM~\cite{Grzadkowski:2010es}.  Assuming that new physics at some high energy scale, $\Lambda$, provides additional sources of \CP violation, the effects at low energy scales can be expressed as operators in an effective Lagrangian:
$$\mathcal{L_{\text{SMEFT}}}\approx \mathcal{L}_{\text{SM}}^{(4)} + \sum_i\frac{c_i^{(6)}}{\Lambda^2}\mathcal{O}_i^{(6)}
+ \sum_i\frac{c_j^{(8)}}{\Lambda^4}\mathcal{O}_j^{(8)} + \dots,
$$
\noindent where $\mathcal{O}_i^{(6)}$ and $\mathcal{O}_j^{(8)}$ parametrize generic extensions of the SM at low energy. The leading subset of those operators that are \CP-odd and that affect $\PH\PV\PV$ interactions is: 
\begin{equation}
\label{eq:ops}
\OHBtil = \Phi^{\dagger}\Phi B^{\mu\nu}\Phi \widetilde{B}_{\mu\nu} \, , \;\; 
\OHWtil = \Phi^{\dagger}\Phi W^{i\,\mu\nu}\widetilde{W}^i_{\mu\nu} \, , \;\;
\text{and} \;\;
\OHWtilB = \Phi^{\dagger}\sigma^i \widetilde{W}^{i\,\mu\nu}B_{\mu\nu} \; .
\end{equation}
Considering only these dimension-6 operators, the scattering amplitude is:
$$|\mathcal{M}|^2 = |\mathcal{M}_{\text{SM}}|^2 + 2Re(\mathcal{M}^*_{\text{SM}}\mathcal{M}_{\text{d6}}) + |\mathcal{M}_{\text{d6}}|^2 \; .$$
The interference term $\mathcal{M}^*_{\text{SM}}\mathcal{M}_{\text{d6}}$ should be the leading correction to the SM, proportional to $1/\Lambda^2$, while other contributions are proportional to $1/\Lambda^4$.  The interference term is \CP-odd and produces asymmetries in \CP-odd observables, but integrates to zero for \CP-even observables. `Squared' dimension-6 interactions compete with dimension-8 interactions, but for the \CP-odd interactions listed above lead to \CP-even modifications. \CP-odd observables targeting the interference term can therefore be used to set genuinely \CP-sensitivity limits on the Wilson coefficients associated with these operators: \cHBtil, \cHWtil, and \cHWtilB .

\subsubsection*{Studies}
\label{sec:studies}
Studies are carried out using fast simulation.  Events are generated using \textsc{MadGraph5\_aMC@NLO}. 
\textsc{SMEFTSim 3.0} is used to include the anomalous interactions from the EFT operators.
Detector effects are modeled via \textsc{delphes} parameterizations.
SM events are simulated and normalisation factors applied to cover missing higher-order effects.  
Cross-checks on event yields are made with relevant LHC and future-collider studies.

In the first instance $\epem\to\PZ\PH$ events are studied at $\sqrt{s}=240$\,GeV with \Zee or \Zmm, and \Hbb, using the \textsc{IDEA} concept \textsc{delphes} card.  A simple kinematic selection is made following \cite{azzi2012prospectivestudieslep3cms}, plus two b-tags at the 85\% efficiency working point.  A data sample corresponding to 5\,\abinv of integrated luminosity is assumed.  

Sensitivities are studied both using angular observables directly, and neural-net (NN) based observables.  Traditional angular observables are those such as angles between decay planes, and the rapidity-ordered azimuthal angle between two objects, for example $\Delta\phi_{\ell\ell} = \phi_1 - \phi_2$ between the $\PZ$ decay leptons, where $y_1 > y_2$.
The NN-based analyses follow the approach of \cite{Bhardwaj:2021ujv} and \cite{PhysRevD.107.016008}.  
As the \CP asymmetries arise from the interference between SM and \CP-odd amplitudes, 
interference-only events are generated for each EFT operator.
These interference samples are split into constructive and destructive interference 
and the NN is trained to distinguish between the two samples.
A single observable is constructed from the NN classifications, i.e. 
$O_{NN}=P_+ - P_{-}$, 
such that a dedicated observable is optimised for each EFT operator.

\subsubsection*{Results}
It is enlighting to consider the performance of different genuinely \CP-sensitive observables such $\Delta\phi_{\ell\ell}$ in direct comparison against neural-net improved observables. We can expect good statistical control at future facilities, hence, there is the possibility to augment $\Delta\phi_{\ell\ell}$ with measures of momentum transfer to gain sensitivity. In particular, the invariant mass $m_{12}$ is motivated as an additional observable as the interference term swaps sign around the $\PZ$ pole in the electron final state. 

Figures \ref{fig:cpInHZZplots} (left) and (centre) show the expected event yields in the di-electron final state as a function of $\Delta\phi_{\ell\ell}$ and $O_{NN}$, respectively. The interference effects are enhanced relative to the SM prediction for the neural-net-based observable. Permutation feature importance techniques show that this enhancement is caused by a sign-flip in the interference spectrum around the $\PZ$ pole, as shown in Figure  \ref{fig:cpInHZZplots} (right). This feature is not observed in dimuon final states, indicating that interference between VH and VBF diagrams is the likely origin.

\begin{figure}
  \centering
  \includegraphics[width=0.31\textwidth]{figs/Higgs/cpInHZZ_fig_phi_ee}
  \includegraphics[width=0.32\textwidth]{figs/Higgs/cpInHZZ_fig_ONN}
  \includegraphics[width=0.35\textwidth]{figs/Higgs/deltaphiee_vs_mee.png}
  \caption{Sensitivity of \CP-sensitive observables for the $\OHWtilB$ operator: (left) event yield as a function of $\Delta\phi_{\ell\ell}$; (centre) event yield as a function of $O_{NN}$; (right) event yields as a function of $\Delta\phi_{\ell\ell}$ and $m_{\ell\ell}$.
  \label{fig:cpInHZZplots}}
\end{figure}

Constraints on the Wilson coefficients are derived using a profile likelihood test and are shown in \cref{table:cpInHZZresults}.  The procedure accounts for statistical fluctuations in the observable. Experimental systematic effects are not included, but these are expected to have a very small effect on on the measured asymmetries, as discussed/shown in \cite{PhysRevD.107.016008}. 
For the $\Delta\phi_{\ell\ell}$ observable, the constraints on the $\OHWtilB$ operator are weaker than the constraints obtained for the other operators. $\OHWtilB$ is known to be notoriously difficult to constrain (see e.g.~\cite{Bernlochner:2018opw}), whereas the hierarchy between $\OHWtil$ and $\OHBtil$ reflects the usual $U(1)_Y$ vs. $SU(2)_L$ coupling hierarchy. Additional kinematic information provides substantially tighter constraints. Going beyond simply exploiting 2d correlations, the neural network observable $O_{NN}$ distils the available \CP information into a highly sensitive measure of \CP violation. For $\OHWtil$, which is the only operator to affect the Higgs boson's interactions with the $\PW$ boson, the 2d $\Delta\phi_{\ell\ell}-m_{12}$ correlations formidably reflect the amplitude's \CP information.

\begin{table}[t!]
%\vspace*{5mm}
\centering{
\begin{tabular}{ l|c|c|c } 
Observable & \cHWtil/$\Lambda^2$ & \cHBtil/$\Lambda^2$ & \cHWtilB/$\Lambda^2$ \\ 
\hline
$\Delta\phi_{\ell\ell}$ & [-0.41, 0.41] & [-0.60, 0.60] & [-1.2, 1.2]\\
$\Delta\phi_{\ell\ell}$ vs $m_{12}$ & [-0.35, 0.35] & [-0.30, 0.30] & [-0.5, 0.5] \\
$O_{NN}$ & [-0.35, 0.35] & [-0.22, 0.22] & [-0.4,0.4] \\
\end{tabular}
}
\caption{Sensitivity to the interactions of \cref{eq:ops} from $\epem\to\PZ\PH$ events with \Zee or \Zmm, and \Hbb as described in \cref{sec:studies}, assuming 5\,\abinv of data.
\label{table:cpInHZZresults}}
\end{table}


==> sections/higgs/cpinhzz2.tex <==
%\subsubsection*{Introduction}
%
%\newcommand{\OHBtil}{\ensuremath{\widetilde{\mathcal{O}}_{\Phi\widetilde{B}}}\xspace}
%\newcommand{\OHWtil}{\ensuremath{\widetilde{\mathcal{O}}_{\Phi\widetilde{W}}}\xspace}
%\newcommand{\OHWtilB}{\ensuremath{\widetilde{\mathcal{O}}_{\Phi\widetilde{W}B}}\xspace}
%\newcommand{\cHBtil}{\ensuremath{c_{\Phi\widetilde{B}}}\xspace}
%\newcommand{\cHWtil}{\ensuremath{c_{\Phi\widetilde{W}}}\xspace}
%\newcommand{\cHWtilB}{\ensuremath{c_{\Phi\widetilde{W}B}}\xspace}
%\newcommand{\Zee}{\ensuremath{\PZ\to\Pe\Pe}\xspace}
%\newcommand{\Zmm}{\ensuremath{\PZ\to\PGm\PGm}\xspace}
%
%The established \CP violation in the Standard Model (SM) is insufficient to account for the matter dominance observed in the Universe, therefore searches for additional sources of \CP violation are well-motivated to connect the SM with paradigms of baryogenesis through new interactions. An effective field theory approach provides one framework for searching for \CP-violating effects in a motivated higher-dimensional operator deformation of the SM~\cite{Grzadkowski:2010es}.  Assuming that new physics at some high energy scale, $\Lambda$, provides additional sources of \CP violation, the effects at low energy scales can be expressed as operators in an effective Lagrangian:
%$$\mathcal{L_{\text{SMEFT}}}\approx \mathcal{L}_{\text{SM}}^{(4)} + \sum_i\frac{c_i^{(6)}}{\Lambda^2}\mathcal{O}_i^{(6)}
%+ \sum_i\frac{c_j^{(8)}}{\Lambda^4}\mathcal{O}_j^{(8)} + \dots,
%$$
%\noindent where $\mathcal{O}_i^{(6)}$ and $\mathcal{O}_j^{(8)}$ parametrise generic extensions of the SM at low energy. The leading subset of those operators that are \CP-odd and that affect $\PH\PV\PV$ interactions is: 
%\begin{equation}
%\label{eq:ops}
%\OHBtil = \Phi^{\dagger}\Phi B^{\mu\nu}\Phi \widetilde{B}_{\mu\nu} \, , \;\; 
%\OHWtil = \Phi^{\dagger}\Phi W^{i\,\mu\nu}\widetilde{W}^i_{\mu\nu} \, , \;\;
%\text{and} \;\;
%\OHWtilB = \Phi^{\dagger}\sigma^i \widetilde{W}^{i\,\mu\nu}B_{\mu\nu} \; .
%\end{equation}
%Considering only these dimension-6 operators, the scattering amplitude is:
%$$|\mathcal{M}|^2 = |\mathcal{M}_{\text{SM}}|^2 + 2Re(\mathcal{M}^*_{\text{SM}}\mathcal{M}_{\text{d6}}) + |\mathcal{M}_{\text{d6}}|^2 \; .$$
%The interference term $\mathcal{M}^*_{\text{SM}}\mathcal{M}_{\text{d6}}$ should be the leading correction to the SM, proportional to $1/\Lambda^2$, while other contributions are proportional to $1/\Lambda^4$.  The interference term is \CP-odd and produces asymmetries in \CP-odd observables, but integrates to zero for \CP-even observables. `Squared' dimension-6 interactions compete with dimension-8 interactions, but for the \CP-odd interactions listed above lead to \CP-even modifications. \CP-odd observables targeting the interference term can therefore be used to set genuinely \CP-sensitivity limits on the Wilson coefficients associated with these operators: \cHBtil, \cHWtil, and \cHWtilB .
%
%\subsubsection*{Studies}
%\label{sec:studies}
Further studies explore the extra sensitivity to \OHBtil, \OHWtil, and \OHWtilB, as defined in \cref{eq:ops}, that can be obtained using neural-net (NN) based observables over direct angular observables.

Studies are carried out using fast simulation.  Events are generated using \textsc{MadGraph5\_aMC@NLO}. 
\textsc{SMEFTSim 3.0} is used to include the anomalous interactions from the EFT operators.
Detector effects are modeled via \textsc{delphes} parametrisations.
SM events are simulated and normalisation factors applied to cover missing higher-order effects.  
Cross-checks on event yields are made with relevant LHC and future-collider studies.

In the first instance $\epem\to\PZ\PH$ events are studied at $\sqrt{s}=240$\,GeV with \Zee or \Zmm, and \Hbb, using the \textsc{IDEA} concept \textsc{delphes} card.  A simple kinematic selection is made following \cite{azzi2012prospectivestudieslep3cms}, plus two b-tags at the 85\% efficiency working point.  A data sample corresponding to 5\,\abinv of integrated luminosity is assumed.  

%Sensitivities are studied both using angular observables directly, and neural-net (NN) based observables.  
Traditional angular observables are those such as angles between decay planes, and the rapidity-ordered azimuthal angle between two objects, for example $\Delta\phi_{\ell\ell} = \phi_1 - \phi_2$ between the $\PZ$ decay leptons, where $y_1 > y_2$.
The NN-based analyses follow the approach of \cite{Bhardwaj:2021ujv} and \cite{PhysRevD.107.016008}.  
As the \CP asymmetries arise from the interference between SM and \CP-odd amplitudes, 
interference-only events are generated for each EFT operator.
These interference samples are split into constructive and destructive interference 
and the NN is trained to distinguish between the two samples.
A single observable is constructed from the NN classifications, i.e.\ 
$O_{NN}=P_+ - P_{-}$, 
such that a dedicated observable is optimised for each EFT operator.

%\subsubsection*{Results}
It is enlightening to consider the performance of different genuinely \CP-sensitive observables such $\Delta\phi_{\ell\ell}$ in direct comparison against neural-net improved observables. We can expect good statistical control at future facilities, hence, there is the possibility of augmenting $\Delta\phi_{\ell\ell}$ with measures of momentum transfer to gain sensitivity. In particular, the invariant mass $m_{12}$ is motivated as an additional observable as the interference term swaps sign around the $\PZ$ pole in the electron final state. 

Figures \ref{fig:cpInHZZplots} (left) and (centre) show the expected event yields in the di-electron final state as a function of $\Delta\phi_{\ell\ell}$ and $O_{NN}$, respectively. The interference effects are enhanced relative to the SM prediction for the neural-net-based observable. Permutation feature importance techniques show that this enhancement is caused by a sign-flip in the interference spectrum around the $\PZ$ pole, as shown in Figure  \ref{fig:cpInHZZplots} (right). This feature is not observed in dimuon final states, indicating that interference between VH and VBF diagrams is the likely origin.

\begin{figure}
  \centering
  \includegraphics[width=0.31\textwidth]{figs/Higgs/cpInHZZ_fig_phi_ee}
  \includegraphics[width=0.32\textwidth]{figs/Higgs/cpInHZZ_fig_ONN}
  \includegraphics[width=0.35\textwidth]{figs/Higgs/deltaphiee_vs_mee.png}
  \caption{Sensitivity of \CP-sensitive observables for the $\OHWtilB$ operator: (left) event yield as a function of $\Delta\phi_{\ell\ell}$; (centre) event yield as a function of $O_{NN}$; (right) event yields as a function of $\Delta\phi_{\ell\ell}$ and $m_{\ell\ell}$.
  \label{fig:cpInHZZplots}}
\end{figure}

Constraints on the Wilson coefficients are derived using a profile likelihood test and are shown in \cref{table:cpInHZZresults}.  The procedure accounts for statistical fluctuations in the observable. Experimental systematic effects are not included, but these are expected to have a very small effect on on the measured asymmetries, as discussed/shown in \cite{PhysRevD.107.016008}. 
For the $\Delta\phi_{\ell\ell}$ observable, the constraints on the $\OHWtilB$ operator are weaker than the constraints obtained for the other operators. $\OHWtilB$ is known to be notoriously difficult to constrain (see e.g.\ \cite{Bernlochner:2018opw}), whereas the hierarchy between $\OHWtil$ and $\OHBtil$ reflects the usual $U(1)_Y$ vs. $SU(2)_L$ coupling hierarchy. Additional kinematic information provides substantially tighter constraints. Going beyond simply exploiting 2d correlations, the neural network observable $O_{NN}$ distils the available \CP information into a highly sensitive measure of \CP violation. For $\OHWtil$, which is the only operator to affect the Higgs boson's interactions with the $\PW$ boson, the 2d $\Delta\phi_{\ell\ell}-m_{12}$ correlations formidably reflect the amplitude's \CP information.

\begin{table}[t!]
%\vspace*{5mm}
\centering{
\begin{tabular}{ l|c|c|c } 
Observable & \cHWtil/$\Lambda^2$ & \cHBtil/$\Lambda^2$ & \cHWtilB/$\Lambda^2$ \\ 
\hline
$\Delta\phi_{\ell\ell}$ & [-0.41, 0.41] & [-0.60, 0.60] & [-1.2, 1.2]\\
$\Delta\phi_{\ell\ell}$ vs $m_{12}$ & [-0.35, 0.35] & [-0.30, 0.30] & [-0.5, 0.5] \\
$O_{NN}$ & [-0.35, 0.35] & [-0.22, 0.22] & [-0.4,0.4] \\
\end{tabular}
}
\caption{Sensitivity to the interactions of \cref{eq:ops} from $\epem\to\PZ\PH$ events with \Zee or \Zmm, and \Hbb, assuming 5\,\abinv of data.
\label{table:cpInHZZresults}}
\end{table}

The initial studies indicate that all of the sensitivity comes from analysis of the $\PZ\to\ell\ell$ topology, hence the analysis is being extended to remove the requirement on a particular Higgs final state and treat it inclusively,   %Furthermore, we are extending the studies to higher centre-of-mass energies (including $\sqrt{s}=365$\,GeV) to examine the interplay between VBF and VH processes in more detail. 
while additional studies are examining the extra sensitivity available from longitudinal beam polarisation; results will be added in January.


==> sections/higgs/cptautau.tex <==
\label{sec:CPtau}
The spin state of the two tau leptons produced from the Higgs decay, $\PH \to \PGtm \PGtp$, is given by the maximally entangled 2-qubit \cite{Altakach:2022ywa,Fabbrichesi:2022ovb}
\begin{equation}
| \Psi_{H \to \PGt \PGt}(\delta) \rangle = \frac{1}{\sqrt{2}} \left( | +,- \rangle + e^{i 2 \delta} | -,+ \rangle \right)\,.
\label{eq:pure}
\end{equation}
where $\delta$ is the \CP-phase in the $\PH \PGt \PGt$ interaction $\propto \PH \bar \psi_{\PGt} (\cos \delta + i g_5 \sin \delta) \psi_{\PGt}$.
The spin correlation matrix is then given by
\begin{equation}
C_{ij} \equiv \langle \hat s^-_i \hat s^+_j \rangle,
~~~~
C = \begin{pmatrix}
\cos 2 \delta & \sin 2 \delta & 0  \\
-\sin 2 \delta & \cos 2 \delta  & 0  \\
0 & 0  & -1  \\
\end{pmatrix}\,.
\label{eq:Cmat}
\end{equation}
In this expression, $\hat s^\mp_i$ is the $i$-th component of the $\PGt^\mp$ spin.
The $i = 1,2,3$ component corresponds to the 
directions of the normalised vectors ($\mathbf r$, $\mathbf n$, $\mathbf k$) in the helicity basis, which is defined as follows: at the centre of mass frame of $\PGtp \PGtm$, $\mathbf{ k}$ is the direction of $\PGtm$.
The vector $\mathbf{ r}$ is on the plane spanned by $\mathbf{ k}$ and $\mathbf{ h}$, which is the motion of the Higgs in the $\PGtp \PGtm$ rest frame, and defined as $\mathbf{ r} \equiv (\mathbf{ h} - \mathbf{ k} \cos \theta)/\sin \theta$ with $\cos \theta \equiv \mathbf{ k} \cdot \mathbf{ h}$. Finally, $\mathbf{ n} \equiv \mathbf{ k} \times \mathbf{ r}$.

If the $C$-matrix is measured with good accuracy, one can use it to constrain the \CP-phase $\delta$. 
From Eq.\ \eqref{eq:Cmat} we see that
only the $rn$ part (i.e.\ the upper-left $2 \times 2$ part) of the $C$-matrix is sensitive to $\delta$. By comparing the measured $C$-matrix entries in the $rn$ part and the prediction in Eq.\ \eqref{eq:Cmat}, we construct the $\chi^2$ function as \cite{Altakach:2022ywa}
\begin{equation}
\chi^2(\delta) = \frac{ \left( C_{rr} - \cos 2 \delta \right)^2 }{ \sigma^2_{rr} } +  
\frac{ \left( C_{rn} - \sin 2 \delta \right)^2 }{ \sigma^2_{rn} } 
\,+\, \frac{ \left( C_{nn} - \cos 2 \delta \right)^2 }{ \sigma^2_{nn} } 
+ \frac{ \left( C_{nr} + \sin 2 \delta \right)^2 }{ \sigma^2_{nr} } \,,
\label{eq:chi2_delta}
\end{equation}
where $C_{ij}$ and $\sigma_{ij}$ are the central value and the standard deviation, respectively, obtained from the result of the quantum information measurement with the $\PGt^\pm \to \PGppm \PGn$ channel summarised in Table \label{tb:result_2} in section \ref{sec:tautau_ent}.
The goodness of fits is $\chi^2_\mathrm{ min}(\mathrm{ ILC})/\mathrm{ d.o.f.} = 0.93/3$ 
and
$\chi^2_\mathrm{ min}$(FCC-ee)/{d.o.f.} = 0.86/3,
where we used the benchmark collider parameters listed in 
Table \ref{tb:colliders}.





%
\begin{table}[t!]
\begin{center}
\begin{tabular}{r | c | c} 
 %\hline
  & ~~~ILC~~~ & ~~~FCC-ee~~~ \\ [0.5ex] 
 \hline 
 energy (GeV) & 250 & 240  \\ [0.5ex]
 %\hline
 luminosity (ab$^{-1}$) & 3 & 5  \\[0.5ex]
 %\hline
 beam resolution $e^+$ (\%) & 0.18 & $0.83 \times 10^{-4}$  \\[0.5ex]
beam resolution $e^-$ (\%) & 0.27  & $0.83 \times 10^{-4}$  
\\[0.5ex]
$\sigma(e^+ e^- \to HZ)$ (fb) & 240.1  & 240.3 
\\[0.5ex]
\# of signal ($\sigma \cdot \mathrm{ BR} \cdot L \cdot \epsilon$) & 385 & 663
%414  & 691 
\\[0.5ex]
\# of background ($\sigma \cdot \mathrm{ BR} \cdot L \cdot \epsilon$) & 20 & 36
\end{tabular}
\caption{Parameters for benchmark lepton colliders \cite{Baer:2013cma, FCC:2018evy}. Only the main background, $\Pep\Pem \to \PZ \PGtp \PGtm$, is considered, where $\PGtp \PGtm$ are produced from off-shell $\PZ/\gamma$. The numbers of signal and background reported here include the decay branching ratios and the efficiency of the event selection, $|m_{\mathrm{ recoil}} - m_{\PSH|} < 5$ GeV. \label{tb:colliders} }
\end{center}
\end{table}
%



\begin{figure}[t!]
    \centering
	\includegraphics[width=0.5\linewidth]{figs/Higgs/delCp_phase_FCCILC_with_IP}\,
	\caption{$\Delta \chi^2$ as a function of the \CP phase $\delta$ \cite{Altakach:2022ywa}.
	}
	\label{fig:chi2}
\end{figure}

The minimum of $\chi^2$ appears at the vicinity of three \CP-conserving points: $\delta = 0$, $\pm 180^{\circ}$ (\CP-even) and $\pm 90^{\circ}$ (\CP-odd).
Focusing on the minimum around $\delta = 0$,
the 1, 2 and 3 $\sigma$ regions of $\delta$
obtained from this analysis are listed in Table \ref{tb:cp}.
%
\begin{table}[t!]
\begin{center}
\begin{tabular}{ c | c | c } 
%\hline
~~~~CL~~~~ & ILC & FCC-ee \\ [0.5ex] 
\hline 
 68.3\,\% & $[-7.94^{\circ},6.20^{\circ}]$  & $[-5.17^{\circ}, 5.11^{\circ}]$ \\
 %\hline
 95.5\,\% & $[-10.89^{\circ},9.21^{\circ}]$  & $[-7.36^{\circ}, 7.31^{\circ}]$ \\
%\hline
 99.7\,\% & $[-13.84^{\circ},12.10^{\circ}]$  & $[-9.21^{\circ}, 9.21^{\circ}]$   \\
%\hline
\end{tabular}
\end{center}
\caption{Expected sensitivities on the \CP phase $\delta$ \cite{Altakach:2022ywa}.
\label{tb:cp}}
\end{table}
%
%
The analysis is based on $\Delta \chi^2(\delta) \equiv \chi^2(\delta) - \chi^2_\mathrm{ min}$, whose values around $\delta = 0$ are plotted in Fig.~\ref{fig:chi2}.
We note that the allowed windows are asymmetric. This is due to the statistical uncertainty of the 100 pseudo-experiments. 




We see that the resolution of $\delta$ obtained from this analysis is roughly $\sim 7.5^{\circ}$ (ILC) and $\sim 5^{\circ}$ (FCC-ee) at 1 $\sigma$ level.
These results should be compared with the resolutions 
obtained in the standard approach for the $\PH \to \PGtp \PGtm, \PGt^\pm \to \PGppm \PGn$ channel,
which exploits the angle $\varphi^\star$ 
\cite{Kramer:1993jn,Was:2002gv}
defined between the two planes, each spanned by the pair of momentum 3-vectors $(\vec{p}_{\PGpp}, \vec{p}_{\PGtp})$ and
$(\vec{p}_{\PGpm}, \vec{p}_{\PGtm})$ in the Higgs rest frame.
Using the same analysis described in section \ref{sec:tautau_ent} and the statistical method based on 100 pseudo-experiments,
we find the resolution of the \CP-phase 
with the $\varphi^\star$ method
is $6.4^{\circ}$ for FCC-ee.
This shows that the proposed method based on Eq.\ \eqref{eq:chi2_delta} is at least as good as the standard method with $\varphi^\star$.

In the literature, the $\PH \PGt \PGt$ \CP phase measurement at ILC using different tau decay modes
have also been explored \cite{Bower:2002zx,Desch:2003rw}.
The studies in \cite{Harnik:2013aja, Jeans:2018anq}
exploit the $\PGt^\pm \to \rho^\pm \PGn$ channel 
and suggest that the sensitivity can reach $\sim 4 ^{\circ}$,\footnote{Note, however, that these analyses do not include the effect of energy mismeasurement.}
which is in line with the expectations of first theoretical studies, i.e.,  $2.8^{\circ}$ \cite{Berge:2013jra}, including also other decay modes, e.g.\ $\PGt^\pm \to a^\pm \PGn$ and $\PGt^\pm \to \Plpm \PGn \PAGn$.
A recent study \cite{Chen:2017bff} using a likelihood analysis based on the Matrix-Element
claims that the \CP-phase can be measured in the accuracy of $2.9^{\circ}$ at the ILC.

At HL-LHC, the resolution of the $\PH \PGt\PGt$ \CP-phase measurement is expected to reach  
$\sim 11^{\circ}$ using the tau decay modes
$\PGt^\pm \to \PGppm \PGn$ \cite{Hagiwara:2016zqz}
and $\PGt^\pm \to \rho^\pm \PGn$ \cite{Harnik:2013aja}.
Combining comprehensive decay modes with the Matrix-Element likelihood method, the resolution may reach
$5.2^{\circ}$ \cite{Chen:2017nxp}.
On the other hand, however, ref.\ \cite{Askew:2015mda}
claims that the detector effect severely impacts on 
the performance of \CP measurements at HL-LHC
and the \CP phase hypothesis $\delta = 0$ can be distinguished from $\delta = 90^{\circ}$ %(with $L = 1$\,ab$^{-1}$,)
only at 95\,\% CL with $\PGt^\pm \to \PGppm \PGn$ channel.

\subsubsection*{Model independent \CP test}

Under the \CP conjugation, the $C$-matrix transforms as 
$C \xrightarrow{\CP} C^T$.
This fact can be used for a model-independent test for \CP violation.
To measure the asymmetry in the $C$-matrix, 
we define \cite{Altakach:2022ywa}
\begin{equation}
A = (C_{rn} - C_{nr})^2 + (C_{nk} - C_{kn})^2 + (C_{kr} - C_{rk})^2 \geq 0 \,.
\end{equation}
An experimental verification of $A \neq 0$ immediately confirms the violation of \CP. 

From the result summarised in Table \ref{tb:result_2} in section \ref{sec:tautau_ent}, $A$ is obtained as 
\begin{equation}
A \,=\,
\left\{
\begin{array}{ll}
0.168 \pm 0.131 &~~~\mathrm{ (ILC)}
\\
0.081 \pm 0.060 &~~~(\mathrm{ FCC}\text{-}\mathrm{ ee})
\end{array}
\right.
%\nonumber
\end{equation}
Here, the error corresponds to a 1\,$\sigma$ statistical uncertainty obtained from 100 pseudo-experiments. 
The result is consistent with 
the Standard Model (i.e.\ absence of \CP violation)
at $\sim 1\,\sigma$ level.

In the explicit model leading to \eqref{eq:Cmat},
we obtain $A = 4 \sin^2(2 \delta)$.
One can interpret the above model-independent result 
within this model and derive bounds on $\delta$.
In the domain around $\delta = 0$, the following limits are obtained at $1\,\sigma$ \cite{Altakach:2022ywa}
\begin{equation}
|\delta| <
\left\{
\begin{array}{l}
7.9^{\circ} ~~~\mathrm{ (ILC)}
\\
5.4^{\circ}~~~(\mathrm{ FCC}\text{-}\mathrm{ ee})
\end{array}
\right.\,,
%\nonumber
\end{equation}
consistently with the limits obtained in the $\chi^2$ analysis (see Table \ref{tb:cp}). 


==> sections/higgs/higgs_self.tex <==

\vspace*{.1cm}
\subsection{\focustopic Higgs self-coupling}
\label{sec:Hself}
\editor{Junping Tian, Jorge de Blas}


\subsubsection{Introduction}
%\footnote{{\it Editorial note:} The contents of this introduction are based, in part, on a submission summarizing Ref.\cite{Bechtle:2024acc}. These have been substantially edited and may not accurately reflect the opinions or the intended message of the authors in that document.}
{\bf \color{blue} [HL-LHC projections quoted in this introductory section will be replaced with the latest values from ATLAS/CMS, when available.]}

Many open questions of particle physics are related to the Higgs sector and, in particular, to the Higgs potential. 
%
In the SM, the form of the potential follows directly from the symmetries of the theory and the requirement of renormalizability,
%
\begin{equation}
V_{\rm SM}(\phi)=-\mu^2 \phi^\dagger \phi + \lambda (\phi^\dagger \phi)^2=\frac 12 m_{\PH}^2 \PH^2+\lambda_{\PH\PH\PH}\PH^3 + \frac 14\lambda_{\PH\PH\PH\PH} \PH^4 + \ldots~~~(\mu^2,~\lambda >0).
\label{eq:VSM}
\end{equation}
%
However, its key structural properties, determined by the signs of the quartic and quadratic terms, are decided ad-hoc to trigger Electroweak Symmetry Breaking (EWSB) and have a potential that is bounded from below, respectively. 
%While this is enough to describe EWSB, it does not explain why it happens, and it is reasonable to assume that some underlying new physics describes the true dynamics responsible of this phenomenon. 
%
%Therefore, new physics is required to explain the origin 
%and true dynamics responsible for EWSB.
This leaves open the question of whether there is underlying new physics that explains the origin and true dynamics of EWSB.
%
The Higgs potential also plays a role in determining how 
the electroweak phase transition (EWPT) in the early universe took place, and could be linked to possible explanations of the observed asymmetry between matter and anti-matter in the universe in terms of electroweak baryogenesis. 

After the Higgs boson discovery at the LHC, the values of all the terms in \cref{eq:VSM} are precisely determined in the SM, as they can be 
predicted in terms of the vacuum expectation value, $v$, (or, alternatively, the Fermi constant) and the Higgs boson mass: 
%
\begin{equation}
\mu^2=\frac 12 m_{\PH}^2,~~~~\lambda=\frac{\lambda_{\PH\PH\PH}}{v}=\lambda_{\PH\PH\PH\PH}=\frac{m_{\PH}^2}{2 v^2}.
\end{equation}
%
Therefore, the observation of a modification on the Higgs boson self-interactions with respect to these predictions 
would give evidence of the presence of new physics.
%(Furthermore, based on perturbative unitarity arguments, such observation would also set upper bounds on the scale where the SM needs to be completed
%~\cite{Chang:2019vez}.)
%



The actual form of the Higgs potential that is realised in nature and its physical origin are, however, largely unknown up to now. 
%
While the bilinear term proportional to $\PH^2$ is related to the measured value of $m_{\PH}$, and tells us about the potential around the electroweak (EW) minimum, 
understanding the shape of the potential away from that point requires an experimental determination of the  
Higgs boson three- and four- (and possibly higher) point self-couplings. 
The observable effects of these interactions have only been loosely constrained experimentally so far. 
In this regard, it is important to clarify that the Higgs boson self-coupling(s), like any other coupling, are not themselves physical observables, hence their determination is tied to the interpretation of an observable (e.g. the Higgs pair production cross section) within a given theory framework. Therefore, a fully model-independent measurement of a Higgs coupling is not possible as a matter of principle at any collider, and the choice of both an appropriate theory framework and the observables to be interpreted play a role in the sensitivity to the strength of the Higgs (self-)interactions. 
In this section, we focus our attention on the challenges surrounding the experimental determination, and theory interpretation, of the Higgs trilinear coupling $\lambda_{\PH\PH\PH}$, proportional to $\PH^3$, whose measurement will provide the next step in understanding the shape of the Higgs potential. The main probes 
used currently in LHC experiments as well as those possible at future $\epem$ colliders are briefly described in what follows, with the progress made in the latter being the core focus of the section.

{\bf \color{blue} [The HL-LHC numbers in the next paragraph will be updated when the latest values from ATLAS/CMS are available.]}
The existing constraints on $\lambda_{\PH\PH\PH}$ from the LHC have mainly been obtained from the searches for the Higgs pair production process, dominated by the gluon-fusion channel. 
Assuming that all other Higgs boson couplings besides $\lambda_{\PH\PH\PH}$ are fixed to their SM values, the current bounds on the di-Higgs production cross section from ATLAS and CMS can be translated into limits on the Higgs self-coupling, $-1\lesssim \kappa_\lambda \lesssim 7 $ at 95$\%$ C.L. , with $\kappa_\lambda\equiv \lambda_{\PH\PH\PH}/\lambda_{\PH\PH\PH}^\textrm{SM}$~\cite{ATLAS:2024ish,CMS:2022dwd}. 
%-------------------------------------------
%Looking at what would be possible with the high-luminosity upgrade of the LHC, 
%previous projections (for the combined integrated luminosity that is expected to be collected by ATLAS and CMS) suggested that an experimental uncertainty for $\lambda_{\PH\PH\PH}$ of about 50\% at the 68\% C.L.\ would be within the reach of the HL-LHC if the SM value is realised in nature~\cite{Cepeda:2019klc}.
%These have been revisited since then, to include the improvements from Run 2 analysis and those developed for Run 3, e.g. in $b$-tagging, and newer individual results~\cite{ATL-PHYS-PUB-2022-005,ATL-PHYS-PUB-2024-016} suggest significantly improved expectations, bringing the HL-LHC precision
%on $\kappa_\lambda$ to around X\% at the 68\% C.L. ~\cite{HLLHC_klambda2025}. 
%-------------------------------------------
These results will be significantly improved  with the high-luminosity upgrade of the LHC.  Assuming the SM value of $\lambda_{\PH\PH\PH}$ is realised in nature, current HL-LHC projections~\cite{HLLHC_klambda2025} give an expected 68$\%$ C.L. uncertainty for $\kappa_\lambda$ of $1 ^{+\sigma_+} _{-\sigma_-}$. Further improvements are also expected when all (single- and double-Higgs) production and decay channels are included, and when the extended acceptance of the HL-LHC detectors is taken into account.
%-------------------------------------------
 It should be noted that, in the gluon fusion channel, the leading-order one-loop diagram containing $\lambda_{\PH\PH\PH}$ and the top Yukawa coupling $y_t$ enters together with a box diagram involving the coupling factor $y_t^2$, see \cref{fig:HHxs_diagrams}. Because of the destructive interference between the contributions from these two diagrams, the total cross section for di-Higgs production changes very substantially, if $\lambda_{\PH\PH\PH}$ is varied around the SM value. This is illustrated in the top-left panel of \cref{fig:HHxs_kappalambda}, where the Higgs pair production cross section is shown as a function of $\lambda_{\PH\PH\PH}$ for the different production modes. In this regard, it should also be noted that 
 a change in $\lambda_{\PH\PH\PH}$ would not only affect the total cross section, but also the kinematic properties of the Higgs pairs, e.g. their invariant mass, and hence the signal acceptance and efficiency. This information can be used to mitigate the loss in statistical sensitivity due to the smaller cross section for moderately large values of $\lambda_{\PH\PH\PH}$, around the minimum in \cref{fig:HHxs_kappalambda}.
%{\bf \color{blue}[It would be good to add here a figure of $\kappa_\lambda$ HL-LHC, so it is easier to present things later.]}


%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\centering
  \includegraphics[width=0.9\textwidth]{./figs/Hself/HH-Feynman-all_v2.pdf}
%  %\end{center}
\caption{Diagrams contributing to the main Higgs pair-production production mechanism at hadron and $\epem$ colliders.\label{fig:HHxs_diagrams}}
\end{figure}
%
\begin{figure}[ht!]
\centering
%  %\begin{center}	
  \includegraphics[width=0.45\textwidth]{./figs/Hself/HH_LHC.png}
~
  \includegraphics[width=0.5\textwidth]{./figs/Hself/xsec_coupling_BSM.pdf}
~
  \includegraphics[width=0.5\textwidth]{./figs/Hself/CrossSectionPlot.pdf}
%  %\end{center}
\caption{Higgs pair-production cross section, as a function of $\lambda_{\PH\PH\PH}$, at the LHC~\cite{Frederix:2014hta} (top left) and $\epem$ colliders~\cite{DiMicco:2019ngk} (top right). 
All other interactions contributing to the processes are assumed to take their SM values. 
(Bottom) $\epem\to \PH\PH + X$ SM production cross section as a function of $\sqrt{s}$~\cite{DiMicco:2019ngk}.}
\label{fig:HHxs_kappalambda}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


While the existing bounds on $\lambda_{\PH\PH\PH}$ are rather weak, 
they can still probe so-far untested parameter regions of physics beyond the SM (BSM), in those scenarios where corrections to 
$\lambda_{\PH\PH\PH}$ are much larger than those to the interactions between
$\PH$ and the gauge bosons and fermions. 
Power counting arguments, both from an effective field theory perspective~\cite{Chang:2019vez,Falkowski:2019tft,Durieux:2022hbu} and in particular classes of models~\cite{Kanemura:2002vm,Durieux:2022hbu,Bahl:2022jnx,Bahl:2023eau},
suggest that such a hierarchy of corrections can indeed be generated by new physics at the tree,
1-loop and even 2-loop level. 
This is discussed and illustrated with some examples in \cref{sec:largeH3}. 
%
%Furthermore, a sizable upward shift in $\lambda_{\PH\PH\PH}$ is also motivated in scenarios giving rise to a strong first-order EWPT which is for instance required for electroweak baryogenesis~\cite{Sakharov:1967dj} and could also source a gravitational wave stochastic background detectable at the future space-based observatory LISA~\cite{Grojean:2006bp, Caprini:2015zlo}. 
Furthermore, a sizable upward shift in $\lambda_{\PH\PH\PH}$ is also motivated in scenarios giving rise to a strong first-order EWPT which is for instance required for electroweak baryogenesis~\cite{Sakharov:1967dj}. (A large value of $\lambda_{\PH\PH\PH}$ could therefore also have cosmological consequences, detectable as a gravitational wave stochastic background at the future space-based observatory LISA~\cite{Grojean:2006bp, Caprini:2015zlo}.)
A first-order electroweak phase transition can occur in many BSM theories proposed for several decades. These include singlet scalar extensions, triplet scalar extensions, two-Higgs doublet models, supersymmetric models, left-right symmetric models, Pati-Salam model, Georgi--Machacek model, Zee--Babu model, extended composite Higgs models, neutrino mass models and hidden sector models involving scalars, and others (see the extended list of references compiled in Ref.~\cite{Ramsey-Musolf:2024zex}). 
%
For a recent example in the case of the 2HDM see e.g. Ref.~\cite{Biekotter:2022kgf} , where the parameter region featuring a strong first-order EWPT and a potentially detectable gravitational wave signal at the future space-based observatory LISA is correlated with an enhancement of $\lambda_{\PH\PH\PH}$ compared to the SM value by about a factor of 2.
%
On the other hand, it is also important to note that large $\mathcal{O}(1)$ corrections to $\lambda_{\PH\PH\PH}$ are not expected to be obtained in the more natural models explaining electroweak symmetry breaking, like the minimal supersymmetry or composite Higgs models, without some tuning, and some special dynamical features are needed (discussed in \cref{sec:largeH3}) to generate large deviations of $\lambda_{\PH\PH\PH}$ and to remain compatible with all other experimental constraints (e.g. single-Higgs measurements or electroweak precision data). 
%Furthermore, a very significant upward shift in $\lambda_{\PH\PH\PH}$ is also motivated in many scenarios giving rise to a strong first-order EWPT which is required for electroweak baryogenesis; see e.g.\ \cite{Biekotter:2022kgf} for the case of the 2HDM, where the parameter region featuring a strong first-order EWPT and a potentially detectable gravitational wave signal at the future space-based observatory LISA is correlated with an enhancement of $\lambda_{\PH\PH\PH}$ compared to the SM value by about a factor of 2. %{[\bf add more references to other models?]}
%Conversely, models where $\lambda_{\PH\PH\PH}$ is suppressed by order one corrections with respect the SM are also possible~\cite{Noble:2007kk}.
%On the other hand, it is also important to note that large ${\cal O}(1)$ corrections to $\lambda_{\PH\PH\PH}$ are not expected to be obtained in the more natural models explaining electroweak symmetry breaking, like supersymmetry of composite Higgs models, without some tuning. 


At future colliders, information about $\lambda_{\PH\PH\PH}$ could be obtained in different and complementary ways. One approach relies on the energy reach, and is relevant for colliders whose centre-of-mass energy can go well past the $\PH\PH$ threshold, to the point where the cross section is large enough to produce Higgs pairs with enough statistical significance. %A second approach, based on the precision reach of different measurements, typically single Higgs processes, is the main source of information at low-energy Higgs factories.
Another method, accessible already at the HL-LHC and with the energies reachable by Higgs factories running at the $\PZ\PH$ and top-quark production thresholds, is based on the precision reach of different measurements, typically single Higgs processes.

%Starting with $\epem$ colliders with a CM energy of at least 500~GeV,  the Higgs pair production process $\epem \to Z\PH\PH$ can be measured. (This is also the case for the weak-boson fusion process $\epem \to \nu_e\bar\nu_e \PH\PH$, though this would benefit from much larger CM energies, around the TeV, see bottom panel in \cref{fig:HHxs_kappalambda}.) 
Starting with the Higgs pair-production approach, which is already in use at the LHC: at $\epem$ colliders a CM energy of at least 500~GeV would be needed to measure the $\epem \to \PZ\PH\PH$ process. 
(This is also the case for the weak-boson fusion process $\epem \to \nu_e\bar\nu_e \PH\PH$, though this would benefit from much larger CM energies, starting around 1 TeV; see bottom panel in \cref{fig:HHxs_kappalambda}.)
As will be discussed in \cref{sec:HHprod}, assuming the SM value of $\lambda_{\PH\PH\PH}$ is realised in nature,
a 550 GeV linear $\epem$ collider would obtain a determination of $\kappa_\lambda = 1 \pm 0.15$ ($15\%$), 
combining the results from the $\PZ\PH\PH$ and $\nu_e\bar\nu_e \PH\PH$ channels~\cite{JTianComb}. 
Furthermore, unlike the leading process at hadron colliders, 
in the $Z\PH\PH$ channel at a 550 GeV $\epem$ collider, assuming the $\PH\PH\PZ\PZ$ interaction is SM-like, the interference terms involving the $\lambda_{\PH\PH\PH}$ interaction contribute  
%the interference contribution in the $Z\PH\PH$ channel at a 550 GeV $\epem$ collider is 
constructively for $\kappa_\lambda>1$, leading to a growth in the cross section, as shown in the top-right panel of \cref{fig:HHxs_kappalambda}. As a result of this, if the value of $\lambda_{\PH\PH\PH}$ that is realised in nature is moderately larger than the SM prediction, $1\lesssim \kappa_\lambda \lesssim 4$ (see \cref{fig:HHxs_kappalambda}), 
the destructive interference in gluon-fusion will result in a degradation of the $\lambda_{\PH\PH\PH}$ determination at hadron colliders, whereas at $\epem$ colliders the accuracy would improve. 
As can be seen in \cref{fig:kappalambda}, 
the precision of the HL-LHC determination would change from $\kappa_\lambda = 1 \pm x$ ($X\%$) to $\kappa_\lambda = 2\pm y$ ($Y\%$)
(see, e.g. Ref.~\cite{ATL-PHYS-PUB-2024-016} for a recent projection from the ATLAS Collaboration illustrating this effect). 
% Changes for new projections?
%Despite this, and as can be seen in \cref{fig:kappalambda}, 
%the relative precision of the HL-LHC determination would remain similar,
%going from $\kappa_\lambda = 1 \pm x$ ($X\%$) to $\kappa_\lambda = 2\pm y$ ($Y\%$).
%In this same case, the determination of $\lambda_{\PH\PH\PH}$ at the ILC running at 550 GeV would improve to $\kappa_\lambda = 2 \pm 0.14$  ($7\%$), improving the HL-LHC result by a factor of 4.
%
On the other hand, in this same case, the determination of $\lambda_{\PH\PH\PH}$ at the ILC running at 550 GeV would improve to $\kappa_\lambda = 2 \pm 0.14$  ($7\%$), several times better than the one at the HL-LHC. 
%more than an order of magnitude better than the one at the HL-LHC. 
As mentioned above, such large values of $\kappa_\lambda$ would be favoured in scenarios giving rise to a strong first-order EWPT.\footnote{
Related to the possibility of measuring the Higgs pair production process and, aside from detecting possible enhancements in the value of $\kappa_\lambda$, we note here that in BSM scenarios with extra scalars, one typically finds additional triple Higgs couplings (THCs) involving also heavy Higgses that could be probed in $\epem \to \PH\PH +X$. Moreover, if the new scalars are sufficiently light, such couplings could be tested via a resonant contribution. The effects that such scenarios could have on $\epem \to Z\PH\PH$ is explored in \cref{sec:BSMHhh}, with special emphasis on the impact of loop corrections to these THCs. 
%{\bf [Reference to searches, where?]}
}
Conversely, from the same \cref{fig:kappalambda} one observes that the HL-LHC and $\epem$ sensitivity is very similar if $\lambda_{\PH\PH\PH}$ turns out to be relatively close to 0.
{\bf \color{blue} [The discussion in this paragraph will be updated when the HL-LHC projections for $\kappa_\lambda\not =1$ are available.]}
%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\centering
%  %\begin{center}	
  \includegraphics[width=0.7\textwidth]{./figs/Hself/lambda_ECFA25significanceILC550abs_2.pdf}
%  %\end{center}
\caption{Projected accuracies for $\lambda_{\PH\PH\PH}$ from Higgs pair production at the HL-LHC and a 550 GeV $\epem$ collider as a function of the actual value of $\lambda_{\PH\PH\PH}$ that is realised in nature. From the ILC study in~\cite{JL}.
See \cref{fig:KlambdaKi} for similar results from single-Higgs measurements.
{\bf \color{blue}[To be updated with the latest ATLAS/CMS HLLHC projections]}
}
\label{fig:kappalambda}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Below the threshold for Higgs pair production processes, %``low-energy'' $\epem$ Higgs factories 
future $\epem$ Higgs factories
are also sensitive to the effects of the Higgs self-coupling via its virtual loop %effects in other observables where the higher precision of the measurements can be used to compensate the loop suppression of such contributions. 
effects in precision observables. %where the higher precision of the measurements can be used to compensate the loop suppression of such contributions. 
Specifically, single Higgs observables, like the production cross section and branching ratios, receive one-loop contributions that depend on $\lambda_{\PH\PH\PH}$, while in the predictions for the electroweak precision observables at the Z~pole and for the W-boson mass $\lambda_{\PH\PH\PH}$ enters at the two-loop level. In particular, special attention has been paid to the determination
of the Higgs self-coupling from measurements of single-Higgs processes, where sub-percent precision would bring sensitivity to quantum effects of $\lambda_{\PH\PH\PH}$~\cite{McCullough:2013rea}. 
Thus, $\epem$ precision single-Higgs measurements open the possibility of testing $\lambda_{\PH\PH\PH}$ in a way that is complementary to Higgs pair production. 
For example, in single-Higgs processes $\lambda_{\PH\PH\PH}$ enters in diagrams with two off-shell and one on-shell Higgses, 
while in pair production, both at hadron and lepton colliders, $\lambda_{\PH\PH\PH}$ contributes in a diagram
where the situation is reversed, with one off-shell and two on-shell Higgses.
%
%Indeed, since both ways of extracting the self-coupling are model-dependent, 
%having two or more probes that can test new physics effects affecting the determination
%of the self-coupling in a different way (in this case, via on-shell and off-shell Higgs pair  
%
%and the new physics effects that can affect both, other than through modifications
%of the self-coupling are different, 
%
%in the sense the additional new physics entering that both processes
%is common while the one affecting the Higgs self-coupling is common. 
%
In general, the loop contributions involving $\lambda_{\PH\PH\PH}$ compete with larger lowest-order contributions, and with other loop contributions (e.g.\ a top-quark loop). The sensitivity to $\lambda_{\PH\PH\PH}$ via loop effects may also be more affected by the theoretical uncertainties induced by unknown higher-order contributions and by the experimental errors of the SM input parameters. 
The latter, however, are known or will be measured with a precision that suggests these parametric uncertainties are under control~\cite{Freitas:2019bre}, as will be discussed in \cref{sec:eeZH_H3}.

For the study of sensitivity to $\lambda_{\PH\PH\PH}$ in single Higgs processes, the possible deviations in the Higgs self-coupling with respect to the SM have been typically parametrised within the so-called SMEFT formalism, see \cref{sec:globalSMEFT}, truncated to dimension six.\footnote{This includes only effects of ${\cal O}(1/\Lambda^2)$ with $\Lambda$ the heavy scale acting as cutoff of the EFT. As is also shown in the results in \cref{sec:globalSMEFT}, the inclusion of effects of ${\cal O}(1/\Lambda^4)$ with the precision achievable at future colliders would seem to have only a small impact on the dimension-six results, suggesting the EFT expansion is well behaved.}   
%
The studies presented in Ref.~\cite{deBlas:2019rxi} (see Figure 11 in that reference) reported the sensitivity to $\lambda_{\PH\PH\PH}$ for different future colliders, assuming the SM value is realized in nature, i.e. $\kappa_{\lambda}=1$. Although these studies take into account the effect of projected SM theory uncertainties mentioned above and also illustrate some illuminating points about the interplay of different EFT contributions, they were restricted to the EFT calculations available at that time and, as we discuss below, recent EFT calculations of additional NLO effects could affect the $\lambda_{\PH\PH\PH}$ interpretation. 
%
For instance, in
an EFT analysis including only the 1-loop contributions from $\lambda_{\PH\PH\PH}$ as well as any possible contribution at leading-order, measurements at a single centre-of-mass energy show an approximate degeneracy, which can efficiently be lifted by performing measurements at a second $\sqrt{s}$~\cite{DiVita:2017vrr}.
With runs at \SI{240}{} and \SI{365}{\giga\electronvolt}, the FCC-ee would achieve the sensitivity pictured in \cref{fig:sensitivityH3CC}. 
 However, without any extra model assumptions, a consistent analysis in the EFT approach at next-to-leading order (NLO) requires the introduction of contributions from 
 all the operators that are relevant at that order. 
 %This introduces 
 %a large number of additional EFT contributions, in particular from $\epem\PQt\PAQt$ operators, which are currently poorly constrained, and could potentially reduce the precision in $\kappa_{\lambda}$.
 This introduces 
 a large number of additional EFT contributions, in particular from $\epem\PQt\PAQt$ operators, which are currently poorly constrained. This opens the possibility of testing also these new effects, though at the expense of potentially reducing the precision in $\kappa_{\lambda}$.
%
 For the main production process, $\epem \to \PZ\PH$, such NLO contributions have only been recently identified in Refs.~\cite{Asteriadis:2024qim,Asteriadis:2024xts}. 
Details on this calculation and its implications are discussed in \cref{sec:eeZH_NLO}. 
The study of the effect of these contributions in the determination of $\lambda_{\PH\PH\PH}$ and of the observables needed to constrain them 
will be the topic of future work.

\begin{figure}[h]\centering
\includegraphics[width=.5\textwidth]{./figs/Hself/fcc2dplot2}
\caption{$1\sigma$ sensitivity achievable on the trilinear self-coupling of the Higgs boson ($\delta \kappa_\lambda=\kappa_{\lambda}-1$, shown on the $x$ axis) with 240 and \SI{365}{\giga\electronvolt} runs at the FCC-ee.
Aside from the single Higgs coupling to the $Z$ boson ($\delta c_Z$, shown on the $y$ axis), 
26 additional Higgs and EW coupling modifications have been marginalised over to obtained the ellipses shown.
}
\label{fig:sensitivityH3CC}
\end{figure}

While the previous paragraphs and the different parts of this chapter focus on introducing/discussing aspects of the use of single- and double-Higgs measurements as probes of the Higgs boson self-coupling separately, it is important to remember that these are not to be considered as alternative probes but, as mentioned above, rather complementary ones. Indeed, since single- and double-Higgs processes are affected differently by new physics, 
a disagreement between a determination of $\kappa_\lambda$ from both methods with similar precision would evidence the presence of additional new effects, making clear the synergetic aspects of the two approaches. Therefore, as in any other of situation where a sign of new physics may be discovered in the data, 
having as many different types of observables as possible where one can test the new effect would help in characterising its origin.  

%-----------------------------------------------

\subsubsection{\texorpdfstring{Generating large corrections to the Higgs self-coupling in new physics models}{Generating large corrections to lambda(HHH) in BSM models}}\label{sec:largeH3}

As mentioned above, the dynamics and nature of the EWPT are closely connected to the Higgs self-coupling value. 
%-----------
%For instance, to obtain a strong first order phase transition, something that cannot be realised in the SM, 
%many Beyond-the-Standard-Model (BSM) theories require an order one deviation of $\lambda_{\PSh\PSh\PSh}$ from its SM prediction~\cite{Grojean:2004xa,Kanemura:2004ch,Noble:2007kk, Katz:2014bha, Huang:2016cjm}. 
%-----------
%For instance, if a strong first order phase transition is needed to explain the observed matter/anti-matter asymmetry, this is something that cannot be realised in the SM and would require new physics to obtain an order one deviation of $\lambda_{\PSh\PSh\PSh}$ from its SM value. 
%This can be predicted in many Beyond-the-Standard-Model (BSM) theories ~\cite{Grojean:2004xa,Kanemura:2004ch,Noble:2007kk, Katz:2014bha, Huang:2016cjm}. 
%-----------
%For instance, if a strong first order phase transition is needed to explain the observed matter/anti-matter asymmetry, this would require an order one deviation of $\lambda_{\PSh\PSh\PSh}$ from its SM value. 
%is something that cannot be realised in the SM and would require new physics to obtain an order one deviation of $\lambda_{\PSh\PSh\PSh}$ from its SM value. 
%This can be predicted in many Beyond-the-Standard-Model (BSM) theories ~\cite{Grojean:2004xa,Kanemura:2004ch,Noble:2007kk, Katz:2014bha, Huang:2016cjm}. 
%-----------
%As an example, the scenario of electroweak baryogenesis would require the EWPT to be of strong first order, which cannot be realised in the SM. In many Beyond-the-Standard-Model (BSM) theories, this is correlated with a deviation of $\lambda_{\PSh\PSh\PSh}$ from its SM prediction~\cite{Grojean:2004xa,Kanemura:2004ch,others}. 
%
For instance, if a strong first-order phase transition is needed to explain the observed matter/anti-matter asymmetry, this is something that cannot be realised in the SM but can be obtained in many BSM theories, typically in correlation with a large (order one) deviation of $\lambda_{\PSh\PSh\PSh}$ from its SM value~\cite{Grojean:2004xa,Kanemura:2004ch,Noble:2007kk, Katz:2014bha, Huang:2016cjm}. 



%Large deviations on the Higgs self-interactions can be predicted in many Beyond-the-Standard-Model (BSM) theories ~\cite{Grojean:2004xa,Kanemura:2004ch,Noble:2007kk, Katz:2014bha, Huang:2016cjm}. 
%However, given
Given the already tight constraints on the Higgs couplings to gauge bosons and heavy fermions, and their foreseen improvements at the (HL-)LHC, one can wonder if there is still room for possible large deviations in the Higgs self-couplings.  
In generic models of heavy decoupling new physics, the deviations in all Higgs couplings are expected to be roughly of the same order. For instance, in models that follow the {\it Strongly-Interacting Light Higgs} (SILH) power counting~\cite{Giudice:2007fh}, like composite Higgs or decoupling supersymmetric models, we expect 
%
\begin{equation}
\label{eq:k3SILH}
\delta \kappa_\lambda \sim \delta \kappa_V \sim \frac{v^2}{f^2},
\end{equation}
%
where the $f$ parameter is related to the typical coupling $g_\star$ and mass scale $m_\star$ of the new dynamics by $f \sim m_\star/g_\star$. (Similarly to $\kappa_\lambda$, we have introduced $\kappa_V$ as the Higgs coupling to vector bosons, normalized to the SM value.)
There are two main ways to depart from this relation: 
\begin{enumerate}
{\item enforcing a particular structure of the heavy new physics;}
{\item having non-decoupling/relatively light particles.}
\end{enumerate}
Even in the first class, the relation in \cref{eq:k3SILH} can be avoided in many ways and perturbativity arguments only give an upper bound on the ratio of the Higgs coupling deviations \cite{Durieux:2022hbu}:
%
\begin{equation}
\label{eq:ratio}
\left|  \frac{\delta \kappa_\lambda}{\delta \kappa_V}\right| \lesssim \mathrm{min} \left( \left(\frac{4\pi v}{m_{\PH}}\right)^2 , \frac{m_\star^2}{m_{\PH}^2} \right).
\end{equation}
%
However, among UV models with single particle extensions~\cite{deBlas:2017xtg}, only the one with a custodial electroweak quadruplet explicitly realises a parametric enhancement of the Higgs self-coupling deviation and gets close to saturate the bound in \cref{eq:ratio}, see \cref{fig:ParametricLargek3} (left). 
Another way to get parametrically large $\delta \kappa_\lambda$ is to rely on Goldstone bosons resulting from large charged spurion symmetry breaking, as in the Gegenbauer's Twin models~\cite{Durieux:2022sgm,Durieux:2022hbu}, as illustrated in the right panel of \cref{fig:ParametricLargek3}. Other dynamics that lead to large $\delta \kappa_\lambda$ include (i)  scenarios in which the Higgs is a generic bound state of a strongly coupled dynamics (i.e. not a Goldstone boson), (ii)  bosonic technicolour scenarios,  (iii)  Higgs-portal models.

\begin{figure} 
{\includegraphics[width=.47\textwidth]{./figs/Hself/CustodialEWQuadruplets.pdf}}
~~~~~{\includegraphics[width=.5\textwidth]{./figs/Hself/Gegenbauer.pdf}}
{\caption{(Left) Single-Higgs coupling and self-coupling deviations expected for a custodial electroweak quadruplet model, as a function of the heavy state coupling, $\lambda$, and mass, $M$. From Ref.~\cite{Durieux:2022hbu}. 
In the grey region, vacuum stability requires sizeable contributions from potential terms not included in the analysis. 
(Right) Ratio of self-coupling to $HVV$ corrections in the Gegenbauer's Twin model for several values of the charge of global symmetry breaking spurion. In the empty upper-left corner of the figure, the SM vacuum is no longer the global minimum of the potential and therefore becomes unstable. From Ref.~\cite{Durieux:2022hbu}.
In both figures, $\delta_{h^3}$ and $\delta_{VV}$ correspond to the quantities $\delta \kappa_\lambda$ and $\delta \kappa_V$ used in this report, respectively.
}\label{fig:ParametricLargek3}}
\end{figure}

Examples of the second class of models are models with extended scalar sectors because of large higher-order radiative corrections from the additional BSM scalars (which we generically denote $\Phi$)~\cite{Kanemura:2002vm,Kanemura:2004mg,Aoki:2012jj,Kanemura:2015fra,Kanemura:2015mxa,Arhrib:2015hoa,Kanemura:2016sos,Kanemura:2016lkz,He:2016sqr,Kanemura:2017wtm,Kanemura:2017wtm,Kanemura:2017gbi,Chiang:2018xpl,Basler:2018cwe,Senaha:2018xek,Braathen:2019pxr,Braathen:2019zoh,Kanemura:2019slf,Basler:2020nrq,Braathen:2020vwo,Bahl:2022jnx,Bahl:2022gqg,Bahl:2023eau,Aiko:2023xui,Basler:2024aaf}. 
%The corrections involving these BSM scalars, which we generically denote $\Phi$, 
These corrections are controlled by couplings of the general form $g_{\PH\PH\Phi\Phi}\propto(m_\Phi^2-\mathcal{M}^2)/v^2$, where $m_\Phi$ is the physical mass of the scalar $\Phi$, $\mathcal{M}$ is some mass scale controlling the decoupling of the BSM states, and $v$ is the SM vacuum expectation value. In scenarios where a splitting occurs between $\mathcal{M}$ and $m_\Phi$, the $g_{\PH\PH\Phi\Phi}$ couplings can grow rapidly and produce large BSM contributions to $\kappa_\lambda$. It should be emphasised that these loop effects involving BSM scalars and $g_{\PH\PH\Phi\Phi}$ couplings are not a perturbation of the tree-level trilinear Higgs coupling, but rather a new class of contributions only entering at the loop level. They can therefore become larger than the tree-level contribution, without being associated with a violation of perturbativity (this situation is analogous to that of loop-induced processes like e.g.\ $\PH\to\PGg\PGg$ or $\PH\to\PGg\PZ$). 

\begin{figure} 
{ \includegraphics[width=.47\textwidth]{./figs/Hself/benchmark_mAvskappalam.pdf}}
~~~{ \includegraphics[width=.45\textwidth]{./figs/Hself/benchmark_plane_2L.pdf}} 
{\caption{(Left) One- and two-loop predictions for $\kappa_\lambda$ as a function of $m_A=m_{H^\pm}$ in an aligned 2HDM scenario of Yukawa type I (see footnote~\ref{footnote:alignmentlimit}). The other BSM input parameters are chosen to be $M=m_H=\SI{600}{\giga\electronvolt}$ and $t_\beta=2$. 
(Right) Contour lines of $\kappa_\lambda$ (red) and $c_\text{eff}$ (blue), computed at two loops, in the $\{\mu_S,m_S\}$ parameter plane of the $Z_2$-SSM (with $\lambda_S=0$). The orange solid and dashed lines indicate the regions of parameter space probed by single-Higgs measurements at the HL-LHC (assuming SM-like central values) at the $1\sigma$ and $2\sigma$ levels respectively. 
}\label{fig:benchmark_masssplittingeffects}}
\end{figure}

The left panel of \cref{fig:benchmark_masssplittingeffects} presents an example of mass-splitting effects in $\kappa_\lambda$ up to the two-loop level in an aligned 2HDM~\cite{Bahl:2022jnx}. 
%
(In what follows, and for the rest of this subsection, we will slightly change the notation, using $\PSh$ to refer to the SM-like Higgs boson, to distinguish it from the other possible heavy Higgs bosons that appear, e.g. in 2HDM models, for which the notation $\PH, \PH^\pm$ is used.)
%
For the scenario considered here,\footnote{We refer the reader to Ref.~\cite{Braathen:2019zoh,Bahl:2022jnx} for details on our choices of conventions and notations for the CP-conserving 2HDM. $M$ is the BSM mass scale of the 2HDM (corresponding to the generic $\mathcal{M}$), $m_H,\ m_A,\ m_{H^\pm}$ are the masses of the BSM scalars, and $\alpha$ and $\beta$ are respectively the mixing angles in the CP-even sector and in the CP-odd and charged sectors. The alignment limit~\cite{Gunion:2002zf} means that the EW vacuum expectation value is aligned in field space with the detected Higgs boson $\PH$ of mass 125 GeV, and corresponds to $\alpha=\beta-\pi/2$ in terms of mixing angles. As a consequence of this limit, which has to be enforced in absence of any structural dynamics,
all couplings of $\PSh$ are SM-like at the tree level. \label{footnote:alignmentlimit}} with $M=m_H=\SI{600}{\giga\electronvolt}$, $m_A=m_{H^\pm}$ and $\tan\beta=2$, all relevant theoretical and experimental constraints have been verified. The comparison of the two-loop prediction for $\kappa_\lambda$ with recent experimental bounds on this coupling modifier~\cite{ATLAS:2022jtk} at the LHC allows excluding significant parts of the otherwise unconstrained parameter space of the model. For instance, in this specific scenario, the mass range $m_A=m_{H^\pm}\gtrsim \SI{900}{\giga\electronvolt}$ (or equivalently mass splittings $m_A-m_H\gtrsim\SI{300}{\giga\electronvolt}$) would lead to the two-loop prediction for $\kappa_\lambda$ to be larger than 7.2~\cite{ATLAS:2024ish} %, $\kappa_\lambda^{(2)}>6.3$ 
and is therefore excluded.  
%(while perturbative unitarity would only exclude $m_A=m_{H^\pm}\gtrsim \SI{1020}{\giga\electronvolt}$). 
Additionally, the mass range $m_A=m_{H^\pm}\gtrsim\SI{800}{\giga\electronvolt}$ of this scenario would be probed at the HL-LHC, as indicated in purple in the left panel of \cref{fig:benchmark_masssplittingeffects}. 
% The considered benchmark scenarios are defined in the figure caption as well as Refs.~\cite{Bahl:2022jnx,Bahl:2023eau}. 
%
Importantly, the mass-splitting effects shown in that same figure %\cref{fig:benchmark_masssplittingeffects} 
and the exclusions obtained with current LHC data, or expected with future colliders, are not restricted to the 2HDM, but have been found to occur in various BSM theories with additional scalars -- as can now be studied with the public tool \texttt{anyH3}~\cite{Bahl:2023eau}. 

The occurrence of large radiative corrections in $\lambda_{\PSh\PSh\PSh}$ raises the questions of how sizeable higher-order corrections to other Higgs properties involving $g_{\PSh\PSh\Phi\Phi}$ couplings can become, and where one would first observe a deviation from the SM predictions in these types of scenarios. Power counting arguments~\cite{Bahl:2024xyz} show that, in the limit of large $g_{\PSh\PSh\Phi\Phi}$ couplings, the leading one-loop BSM contributions to the trilinear Higgs coupling are of $\mathcal{O}(g_{\PSh\PSh\Phi\Phi}^2)$, while those in single-Higgs couplings grow at most linearly with $g_{\PSh\PSh\Phi\Phi}$. 

As a simple but illustrative example, we consider the $Z_2$-SSM,\footnote{We refer the reader to e.g.\ Ref.~\cite{Braathen:2020vwo} for an overview of the notations and conventions we employ in this work (we consider here the $N=1$ case of the $O(N)$-symmetric SSM of Ref.~\cite{Braathen:2020vwo}).} i.e.\ a real-singlet extension of the SM with an unbroken global $Z_2$ symmetry. Due to this symmetry, the BSM scalar $S$ does not mix with the detected Higgs boson at 125 GeV. Its mass takes the form $m_S^2=\mu_S^2+\lambda_{\PH\Phi}v^2$ where $\mu_S$ is the singlet Lagrangian mass term and $\lambda_{\PH\Phi}$ the portal quartic coupling between the singlet and the (SM-like) doublet. The coupling $\lambda_{\PH\Phi}$ plays in the $Z_2$-SSM the exact role of the generic $g_{\PSh\PSh\Phi\Phi}$ coupling in the discussion above. In this model, single-Higgs couplings $g_{\PSh XX}$, where $X$ can be a gauge boson or fermion, only receive BSM contributions via external-leg corrections --- there are no mixing effects at the tree level, and moreover vertex-type corrections do not appear because of the singlet nature of the BSM scalar and the unbroken $Z_2$ symmetry.  
% define ceff -> OK
This allows obtaining compact expressions for the single-Higgs coupling modifier $c_\text{eff}\equiv g_{\PSh XX}/g_{\PSh XX}^\text{SM}$ at one and two loops~\cite{Bahl:2024xyz}. 
%
In the right panel of \cref{fig:benchmark_masssplittingeffects}, we present contour lines for $\kappa_\lambda$(red) as well as the quantity $c_\text{eff}$ (blue), both computed at the two-loop order, in the $\{\mu_S,m_S\}$ parameter plane of the $Z_2$-SSM. As a conservative choice, we fix $\lambda_S=0$ in the plane; this cancels the effects from two-loop terms involving $\lambda_S$ in $\kappa_\lambda$ and $c_\text{eff}$ (we note that for these contributions, like for those involving only $g_{\PSh\PSh\Phi\Phi}$ couplings, the effects in $\kappa_\lambda$ have a higher scaling in powers of $\lambda_{\PH\Phi}$ than those in $c_\text{eff}$). We implemented the expected levels of accuracy on single-Higgs couplings at the HL-LHC as ``measurements'' (assuming SM-like central values) in \texttt{HiggsSignals}~\cite{Bahl:2022igd}, and orange lines in the left panel of  \cref{fig:benchmark_masssplittingeffects} correspond respectively to the $1\sigma$ (solid) and $2\sigma$ (dashed) exclusion ranges from HL-LHC measurements. 
The values indicated in each contour line for $\kappa_\lambda$ ($c_\text{eff}$) indicate the maximum (minimum) value of the parameter 
predicted in the region below the line.
Therefore, these lines provide information about the regions of the $Z_2$-SSM parameter space for which large corrections to $\kappa_\lambda$ can be obtained while those to $c_\text{eff}$ are small. 
As can be observed, comparing for instance the uppermost red and blue contour lines in the right panel of \cref{fig:benchmark_masssplittingeffects}, values of $\kappa_\lambda$ up to 1.5 could be obtained while corrections 
to $c_\text{eff}$ are kept below $0.5\%$.

Other examples where this hierarchy of corrections can be obtained from large radiative corrections include, for instance, the Inert Doublet Model (IDM), a variant of the 2HDM in which the second doublet is charged under an unbroken $\mathbb{Z}_2$ symmetry, see e.g. Refs.~\cite{Deshpande:1977rw,Barbieri:2006dq,Braathen:2019zoh,Aiko:2023nqj} for an overview of the model.
As in the above example for the $Z_2$-SSM, using the two-loop predictions for $\kappa_\lambda$ (from Refs.~\cite{Braathen:2019pxr,Braathen:2019zoh,Aiko:2023nqj}) and the one-loop BSM deviation in the $g_{\PSh\PZ\PZ}$ coupling, one can find regions of the IDM parameter space where large ${\cal O}(1)$ corrections of $\kappa_\lambda$ are predicted, while keeping the modifications of the Higgs couplings to vector bosons well below $1\%$. 

As we discuss next, the large values of $\lambda_{\PSh\PSh\PSh}$ discussed in this section
could be probed at O(10\%) at future \epem colliders operating at CM energies 
around \SI{500}{\giga\electronvolt}. 
Similarly, while corrections to single Higgs coupling can remain small in these models, 
deviations at the level of a few tens of percent in the value of $\kappa_\lambda$ would also 
induce effects at one-loop level in single-Higgs observables that could be tested 
at future \epem Higgs factories, as is explained in \cref{sec:eeZH_H3}.


%-----------------------------------------------


\subsubsection{\texorpdfstring{Progress in Higgs-pair production at $\epem$ colliders}{Progress in Higgs-pair production at e+ e- colliders}\label{sec:HHprod}}

Double Higgs production at $\Pep\Pem$ colliders with centre-of-mass energies $\sqrt{s} \geq$ \SI{500}{\giga\electronvolt} comprises both di-Higgs production from $\PW\PW$ fusion, $\PGn\PAGn\PH\PH$, dominant at centre-of-mass energies above \SI{1.2}{\tera\electronvolt} (see \cref{fig:HHxs_kappalambda}), as well as double Higgs-strahlung, $\PZ\PH\PH$, dominant at lower centre-of-mass energies. Both processes have been studied about $10$ years ago in detailed Geant4-based simulation of the ILD detector concept, considering the $\PH\PH \rightarrow  4\PQb$~\cite{Durig:2016jrs, Tian:2013} and $\PH\PH \rightarrow \PQb\PAQb\PW\PW^*$~\cite{Kurata:2013} final states.
For the SM value of the tri-linear Higgs self-coupling $\lambda_{\PH\PH\PH}$, the combination of the two channels yielded precisions of \SI{27}{\%} at \SI{500}{\giga\electronvolt} and \SI{10}{\%} when combining both centre-of-mass energies. A few years later, CLICdp studied the prospects at $\sqrt{s}=$\SI{1.4}{\tera\electronvolt} and \SI{3}{\tera\electronvolt}~\cite{Roloff:2019crr}, also in detailed Geant4-based simulation, reaching precisions down to $_{-\SI{7}{\%}}^{+\SI{11}{\%}}$, again assuming the SM value of $\lambda_{\PH\PH\PH}$. It should be noted that in particular for the $\PZ\PH\PH$  process, i.e.\ the measurements at around \SI{500}{\giga\electronvolt}, it has been shown explicitly that, for decoupling new physics, all other parameters entering the interpretation of the $\PZ\PH\PH$ cross-section will be determined with sufficient precision at a Higgs factory so that their impact on the extraction of $\lambda_{\PH\PH\PH}$ is negligible~\cite{Barklow:2017awn}. 
On the other hand, having relatively light new particle exchanges, e.g. in the last diagram in \cref{fig:HHxs_diagrams}, would still affect the interpretation of a possible effect in the data in terms of $\kappa_\lambda$. Being a tree-level exchange limits the type of possible new contributions, but additional observables/assumptions would still be needed to determine $\lambda_{\PH\PH\PH}$ separately from the 
additional new physics effects the process gives access to. (See, e.g. \cref{sec:BSMHhh} for the case of trilinear interactions of two Higgs bosons with an extra scalar.)

%\section{Update of the ILD Di-Higgs Analysis}

The  analysis of $\PZ\PH\PH$ production at \SI{500}{\giga\electronvolt} is being updated in detailed simulations of the ILD detector concept, covering the $\PH\PH \rightarrow \PQb\PAQb \PQb\PAQb$ and $\PZ \rightarrow$ $\PQq\PAQq$ / $\Pep\Pem$ / $\PGmp\PGmm$ / $\PGn\PAGn$ channels. While a full new analysis is ongoing, several key ingredients of the analysis have been updated to more modern analysis tools based on the MC production for the ILD Interim Design Report~\cite{ILDConceptGroup:2020sfq}. This concerns in particular the jet-flavour tagging, for which by an update from LCFIPlus~\cite{Suehara:2015ura} to a ParticleNet-based approach~\cite{Qu:2019gqs} so far a relative increase of the \PQb -tagging efficiency of 10\% at the same level of background rejection could be achieved on 6-jet events as shown in Figure~\ref{fig:anaimprove:flav}. Since the analysis requires at least three jets to be \PQb -tagged to reject $\PQt\PAQt$ and $\PZ\PZ\PH$ (with $\PZ \rightarrow$ $\PQc\PAQc$ /  $\PQs\PAQs$ / $\PQu\PAQu$ / $\PQd\PAQd$ ) backgrounds, the reduced inefficiency enters to the third power. The most signal-like $\PZ\PZ\PH$ background with at least one of the $\PZ \rightarrow \PQb\PAQb$ can only be rejected based on event kinematics. In this respect, an improvement of at least 10\% higher efficiency at same background level is expected from recent advances in correcting for semi-leptonic \PQb -decays and kinematic fitting~\cite{Einhaus:2022bnv}, as well as in using the full matrix elements for $\PZ\PH\PH$  and $\PZ\PZ\PH$. As example, Fig.~\ref{fig:anaimprove:kine} shows the improvement in the di-Higgs invariant mass reconstruction in the $\PZ \rightarrow \PGn\PAGn$ channel. For now, these two improvements will be propagated through the previous analysis~\cite{Durig:2016jrs}. In view of even significantly better flavour tagging tools reported in \cref{sec:com:flavourtagging} (see also e.g. Refs.~\cite{Bedeschi:2022rnj, Qu:2022mxj, Suehara:2024qoc}),  
%{\color{red} (for ECFA report replace by or add cross-ref to Sec \verb$\ref{sec:com:flavourtagging}$)}, 
as well as the potential expected from using machine-learning (ML) through-out the event selection, this is a quite conservative assumption. All numbers below have been scaled to the standard ILC running scenario~\cite{Barklow:2015tja}, i.e.\ \SI{4}{\per\atto\barn} with $P(\Pem,\Pep) = (\mp 80\%, \pm 30\%)$.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{.5\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/b_vs_uds_6j_zoom_2.pdf}
        \caption{}
        \label{fig:anaimprove:flav}    
    \end{subfigure}\hfill%
    \begin{subfigure}{.5\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/b_vs_c_6j_zoom_2.pdf}
        \caption{}
        %\label{fig:anaimprove:flav}    
    \end{subfigure}\hfill%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/mHH_nunu_before_2.pdf}
        \caption{}
        \label{fig:anaimprove:kine}    
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/mHH_nunu_after_2.pdf}
        \caption{}
        %\label{fig:anaimprove:kine}    
    \end{subfigure}%
    \caption{Reconstruction improvements considered in the updated $\PZ\PH\PH$ projection: (a), (b) \PQb -tagging efficiency (true positive rate) increases by about 10\% (relative) for the same background efficiency (false positive rate) at typical working points of the previous analysis (80\% \PQb -tagging efficiency with LCFIPlus) (c), (d) the resolution on the di-Higgs invariant mass improves by about a factor of two when the new semi-leptonic decay correction and kinematic fit are applied.}
    \label{fig:anaimprove}
\end{figure}

%The analysis concept follows Ref.~\cite{Durig:2016jrs}, capitalizing however on significant improvements in central high-level reconstruction tools like flavour tagging, kinematic fitting and overlay removal~\cite{Bliewert:2024} as well as on the usage of ML algorithms in the event selection. 
From this re-analysis of the channels studied in Ref.~\cite{Durig:2016jrs}, the obtained precision on the $\PZ\PH\PH$ production cross-section improves from the \SI{21.1}{\%} obtained in Ref.~\cite{Durig:2016jrs} to now \SI{16.0}{\%} 
for the SM case. 

In combination with the $\PH\PH \rightarrow \PQb\PAQb \PW\PW^*$ channel, the precision on the cross-section improves from the \SI{16.8}{\%} obtained in Ref.~\cite{Durig:2016jrs} to now \SI{12.8}{\%}, again for the SM case, while the corresponding precision on the self-coupling improves from \SI{26.6}{\%} to \SI{20.8}{\%}. By including $\PZ \rightarrow \PGtp\PGtm$, as well as $\PH\PH \rightarrow \PQb\PAQb \PGtp\PGtm$ and other modes well reconstructible in the $\Pep\Pem$ environment, the expected precision on the $\PZ\PH\PH$ cross-section improves further to \SI{11.2}{\%}, corresponding to a precision on a SM-like self-coupling value $\uplambda_{\mathrm{SM}}$ of \SI{18.1}{\%}.

One of the main limiting factors not yet addressed by novel algorithms is the jet clustering. Assuming that future developments, e.g.\ based on ML, will improve the di-jet mass resolution, we estimate that $\uplambda_{\mathrm{SM}}$ could be determined with a precision of \SI{15}{\%}. %Connected to this is the tagging of overlay particles, i.e.\ low $\pT$-hadrons from $\gamma\gamma$ interactions. Further improvements can be expected by going beyond the current treatment of overlay particles (clustering to beam jets), e.g. to multivariate or ML driven tools.

The analysis of the $\PW\PW$ fusion production has been investigated in Refs.~\cite{Tian:2013, Kurata:2013} at a centre-of-mass energy of \SI{1}{TeV}. At \SI{500}{GeV}, the separation of the $\PW\PW$ fusion contribution is still ongoing work and will be covered in future updates. If the $\PW\PW$ fusion cross-section at \SI{500}{GeV} could be constrained to the level of \SI{120}{\%} from the $\PH\PH \rightarrow \PQb\PAQb \PQb\PAQb$, translating to \SI{86}{\%} in combination with the other $\PH\PH$ decay modes. Combining the $\PW\PW$ fusion and $\PZ\PH\PH$ measurement would allow to constrain the SM value of $\uplambda_{\mathrm{SM}}$ to a precision of \SI{17}{\%} with current tools and \SI{14}{\%} when assuming improved jet clustering. 

The results summarised above have been extrapolated to other centre-of-mass energies. In particular, partial MC productions have been performed in full, Geant4-based simulation of ILD as well as using SGV~\cite{Berggren:2012ar} and centre-of-mass energies of \SI{550}{\giga\electronvolt} and \SI{600}{\giga\electronvolt}, showing that beyond the expected scaling with cross-section, both the flavour tag as well as the kinematic reconstruction profit from the higher boost of the produced bosons. This is true in particular for the jet clustering, which benefits from less confusion towards higher COM energies \cite{Torndal:2023mmr}.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{.5\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/HHH_ECM_CombinedGreen_new.pdf}
        \caption{}
        \label{fig:lambda:ZHH_WWfusion}    
    \end{subfigure}\hfill%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/dkala_abs_vs_kala_ILC550_ECFA25.pdf}
        \caption{}
        \label{fig:lambda:BSM}    
    \end{subfigure}%
    \caption{Projected precisions on the tri-linear Higgs self-coupling $\lambda_{\PH\PH\PH}$ for double Higgs-strahlung, di-Higgs production from $\PW\PW$ fusion, and their combination: (a) relative precision as a function of the centre-of-mass energy and (b) absolute uncertainty on the determination $\kappa_{\lambda}$ as a function of the value assumed to be realized in nature. }
    \label{fig:lambda}
\end{figure}

\Cref{fig:lambda:ZHH_WWfusion} shows the resulting evolution of the expected precision on $\uplambda$ with the centre-of-mass energy, for both production modes separately and for their combination. For instance at $\sqrt{s}=$\SI{550}{\giga\electronvolt}, the envisioned energy for C$^3$ as well as for a Linear Collider Facility at CERN, the expected combined precision on $\uplambda_{\mathrm{SM}}$ is \SI{15}{\%}, a substantial improvement over the \SI{26.6}{\%} of Ref.~\cite{Durig:2016jrs}.


Enlarging the scope to the BSM case, it is important to note that the two production modes play very complementary roles due to their very different interference patterns. This is illustrated in \cref{fig:lambda:BSM}, which shows the behaviour of the expected precision as a function of $\lambda_{\PH\PH\PH}/\lambda_{\PH\PH\PH}^{\mathrm{SM}}$ for the two production modes at $\sqrt{s}=$\SI{550}{\giga\electronvolt}. This shows that measurements of $\PZ\PH\PH$  production at centre-of-mass energies around \SI{500}{\giga\electronvolt} play a crucial role in pinning down the BSM behaviour of the tri-linear Higgs self-coupling.
%Furthermore, as we discuss in the next subsection, these types of measurements could also bring sensitivity to new contributions coming from genuine BSM triple Higgs couplings.

%-----------------------------------------------

\subsubsection{\texorpdfstring{Probing the Higgs self-coupling via single-Higgs processes}{Probing the Higgs self-coupling via single-Higgs processes}}\label{sec:eeZH_H3}

As emphasized in the introduction, the Higgs boson couplings cannot be directly measured, 
since they are not physical observables. 
Determinations of these quantities can only be obtained as a result of interpreting real observables, like cross sections, 
in a given theory framework. 
The measurements of single-Higgs processes that could be taken at any
of the future \epem Higgs factories, namely the inclusive cross section and rates for different decay channels of the Higgs boson, 
are typically interpreted in terms of single-Higgs couplings to the SM fermions and vector bosons, quantities that in the SM contribute
to these processes at tree level. But, clearly, owing to the quantum nature of these observables, such interpretation needs to 
be improved beyond this leading order approximation, as what these experiments measure are not single-Higgs couplings, but
combinations of such couplings and all the other interactions that enter in the process at the quantum level.

In the SM, the 1-loop corrections coming from the Higgs self-coupling to, e.g. the unpolarised $\epem \to \PZ\PH$ cross section at 240 GeV,  
are relatively small, increasing the LO cross section by $\sim1.5\%$. In the full set of NLO electroweak contributions, bosonic and fermionic corrections
partially cancel, so the total NLO correction amount to $\sim 3\%$. 
Furthermore, the NNLO from fermion loops are currently known to increase only the NLO result by $0.7\%$~\cite{Freitas:2023iyx}, and the uncertainty from missing bosonic electroweak corrections has been estimated to be less than $0.3\%$~\cite{Freitas:2023iyx}. Therefore, it is reasonable to expect 
that, with some moderate progress in the SM calculations, by the time of a future Higgs factory the SM uncertainty due to higher-order corrections will be further reduced and become much smaller than the leading $\lambda_{\PH\PH\PH}$ effects. Similarly, benefiting from future EW and Higgs measurements, parametric uncertainties from the EW input parameters are also expected to be very small, well below the experimental precision.~\footnote{
An estimate using the SM part of the calculation of \cite{Asteriadis:2024xts} gives an expected parametric uncertainty at FCC-ee well below $0.1\%$.
It is of particular relevance to improve the precision of the Higgs boson mass to around or below 20 MeV. See ~\cite{Freitas:2019bre} for estimates on the corresponding SM uncertainties on Higgs decay rates.}  

Thus, with an experimental precision at the per mille level in $\epem \to \PZ\PH$, it is clear that a future \epem Higgs factory would provide a clean test of the SM prediction for $\lambda_{\PH\PH\PH}$. 
The precision of such test, or the one on the determination of $\lambda_{\PH\PH\PH}$ if everything but this parameter is assumed to be SM-like, could be obtained parametrising the modifications of single-Higgs observables in terms of the following contribution to the Higgs potential
%
\begin{equation}
\Delta V(\PH)=(\kappa_\lambda -1) \frac 12 \frac{m_{\PH}^2}{v} \PH^3 .
\label{eq:VHgen}
\end{equation}
%
%Conversely, if everything but $\lambda_{\PH\PH\PH}$ turn out to be SM-like, a deviation from the SM expectations could be used to determine its actual value.
%
%But, again, 
In general, however,  
estimating the actual precision of the determination of $\lambda_{\PH\PH\PH}$ that would be possible from this (or any other) 
type of measurements is not something that can be addressed in a completely model-independent way. For instance,
different new particles could be exchanged virtually, e.g. in the EW loops, opening the possibility of testing 
many other new physics effects, but also requiring a commensurate number of other observables to identify the 
origin of a possible non-SM effect in the data as coming from $\kappa_\lambda\not =1$. 
As mentioned in the previous section, this can be addressed in a fairly general way for the case of decoupling new physics. 
The use of additional observables needed to constrain all the possible additional loop effects and extract $\lambda_{\PH\PH\PH}$ in this case is briefly discussed at the end of this chapter and is part of future work.
%~\footnote{This is not fundamentally different than the situation in Higgs pair production. In the case of single-Higgs measurements, different new particles could be exchanged virtually, e.g. in the EW loops, complicating the identification of the origin of a possible non-SM effect in the data as coming from $\kappa_\lambda\not =1$. Similarly, in $e^+ e^- \to \PZ\PH\PH$ relatively light new particles could be exchanged in the last diagram in \cref{fig:HHxs_diagrams}, introducing the same complication.
%In this last case, however, being a tree-level exchange limits the type of possible new contributions, simplifying the interpretation,  thus reducing the numbers of additional observables/assumptions needed to determine $\lambda_{\PH\PH\PH}$.
%

\Cref{eq:VHgen} could be used to extend the simplest Lagrangian description of 
%could be equivalent to the interpretation of 
the scenarios of the so-called $\kappa$ framework~\cite{LHCHiggsCrossSectionWorkingGroup:2012nn} 
considering only modifications of SM-like interactions to include corrections to the Higgs self-coupling,
%This could be considered as part of the following Lagrangian aplicable to models modifying mostly the SM Higgs interactions
%
\begin{equation}
\Delta {\cal L}=\Delta V(\PH) +  2 m_Z^2 \kappa_V \frac{\PH}{v}Z_\mu Z^\mu +  2 m_W^2 \kappa_V \frac{\PH}{v}W_\mu W^\mu - \sum_\psi m_\psi \overline{\psi}_L  \kappa_\psi \frac{\PH}{v} \psi_R +{\rm h.c.} ,
\label{eq:Lnonlinear}
\end{equation}
%
where we have assumed custodial symmetry. 
%This Lagrangian would provide a phenomenological parameterization of the effects of models modifying mostly the SM Higgs interactions.
%\begin{equation}
%{\cal L}=\frac 12 (\partial_\mu \PH)^2 - V(\PH) + \frac{v^2}{4} {\rm Tr}(D_\mu \Sigma^\dagger D^\mu \Sigma)\left[1+2 c_V \frac{\PH}{v} + c_{2V} \frac{\PH^2}{v^2}+\cdots\right] - \sum_\psi m_\psi \overline{\psi}_L \Sigma (1+ c_\psi \frac{h}{v} + \cdots)\psi_R +{\rm h.c.} ,
%\label{eq:Lnonlinear}
%\end{equation}
%
%where $\Sigma={\rm exp}(i\sigma_a \pi^a/v)$ is the matrix describing the longitudinal components of the $\PW$ and $\PZ$ gauge bosons, see e.g. \cite{Contino:2010mh}, and 
%-----
%which could be seen as a formulation of some of the scenarios considered in the so-called $\kappa$ framework~\cite{LHCHiggsCrossSectionWorkingGroup:2012nn}, extended with modifications on Higgs self-interactions, 
%and where we have assumed custodial symmetry.
%-----
%, and allowing the extension of the $\kappa$ description beyond leading order. 
A simple exercise performing a frequentist fit of \cref{eq:VHgen} and \cref{eq:Lnonlinear} to the expected precision of all the single-Higgs measurements at \epem colliders using two centre-of-mass energies, taking as an example FCC-ee at 240 and 365 GeV (from Ref.~\cite{deBlas:2022ofj}, updated to the FCC-ee baseline with 4 interaction points~\cite{FCC_feasibility_report}, see \cref{table:lumi:FCC} for the actual luminosities), would give the constraints on $\kappa_\lambda$ shown in \cref{fig:KlambdaKi}. In that figure we consider not only the possibility of $\kappa_\lambda=1$ but also use Asimov datasets generated with \cref{eq:VHgen} 
for different values of $\kappa_\lambda$. We use the theoretical expressions of Refs.~\cite{Degrassi:2016wml,DiVita:2017vrr} to describe the one-loop dependence of $\kappa_\lambda$, while the effects of the modifications of other Higgs couplings are kept at leading order. 
Since we are exploring values of $\kappa_\lambda \not =1$, in absence of precise estimates of the HL-LHC precision from Higgs pair production for such values we prefer not to include it in the combination. 
{\bf\color{blue} [The updated $\PH\PH$ projections from HL-LHC will be included in this example, when available.]}
The results are therefore an estimate of the standalone precision at \epem colliders using single-Higgs measurements at two energy points. 
As can be observed, with $\kappa_\lambda$ entering at the loop level, for moderate deviations from the SM value 
the change in the single Higgs cross sections is rather small and the absolute precision on $\kappa_\lambda$ 
does not change substantially. 

\begin{figure}[h]\centering
\includegraphics[width=.5\textwidth]{./figs/Hself/KappaLambdaHEFT_FCCee}
\caption{$1\sigma$ sensitivity on the trilinear self-coupling of the Higgs boson
achievable with the single-Higgs measurements at 240 and 365 GeV from FCC-ee. 
The results are obtained assuming different values of $\kappa_\lambda$ are realized in nature, and presented under two assumptions in the Lagrangian in \cref{eq:Lnonlinear}: (orange) all parameters are set to their SM values except for $\kappa_\lambda$; (blue) all couplings are considered as floating parameters and marginalized over to obtain the sensitivity to $\kappa_\lambda$. The lower panel shows the relative uncertainty.
}
\label{fig:KlambdaKi}
\end{figure}

%The Lagrangian in \cref{eq:Lnonlinear} is part of the so-called Higgs Effective Field Theory. 
To give precise meaning to the modifications in \cref{eq:Lnonlinear}, this must be embedded in a concrete model or in
a well-defined effective field theory. 
The projections available for $\kappa_\lambda$ from single-Higgs measurements in Refs.~\cite{DiVita:2017vrr,deBlas:2019rxi} were prepared in the so-called Standard Model Effective Field Theory (SMEFT).
%which also assumes that electroweak symmetry is linearly realized on the SM fields. 
We refer to \cref{sec:globalinterpretations} for a small description of the assumptions defining this framework
to describe the low-energy effects of decoupling new physics. 
Following the power-counting of the SMEFT, at the leading order in the EFT expansion --- a power series in $1/\Lambda$, with $\Lambda$ the cut-off of the EFT --- there are many more types of possible sources of BSM effects than those in \cref{eq:Lnonlinear}, including not only modifications of the SM Higgs properties, but also of the EW interactions and types of operators absent in the SM. 
While the large number of BSM effects provides a more general description of new physics scenarios, global analyses including different types of observables are required if one wants to individually constrain all the different directions in the EFT parameter space.
%In this regard, the fact that the SMEFT assumes that electroweak symmetry is linearly realized on the SM fields correlates some of the BSM effects 
%in different observables, and this makes close a global analysis at LO it relatively easy.
%and this makes it easier to perform global studies of different measurements to constrain all the different new physics interactions. 
%However, 
This is particularly relevant when going beyond tree level in the description of new physics effects, 
%going beyond, 
as needed for the determination of $\kappa_\lambda$ from single-Higgs couplings, 
as this increases the number of SMEFT operators that can enter in the analysis via their loop contributions. 
%and one need to make sure one has 
%brings the need to extend global analyses including 
%enough observables to properly interpret an eventual deviation 
%as coming from $\kappa_\lambda$.
The status of the NLO calculations required for this and steps needed to extend the results in Refs.~\cite{DiVita:2017vrr,deBlas:2019rxi} are described in the next section.

%While in \cref{eq:VHgen,eq:Lnonlinear} we considered arbitrary values for the different coefficients, the dimension-six formalism is more appropriate to describe relatively small BSM effects, corresponding to decoupling new physics, which is any case consistent with current phenomenological observations. 

It is important to note that, while these global analyses of the sensitivity to $\lambda_{\PH\PH\PH}$ in single-Higgs measurements performed within the EFT formalism depend on a large number of parameters that need to be constrained from data, a consequence of this is that the resulting $\lambda_{\PH\PH\PH}$-sensitivity is expected to be a conservative estimate of that which would be possible in actual models described by the EFT. 
Indeed, interpretations within specific models, which match into lower-dimensional slices of the EFT parameter space, add extra theory correlations between the different operators, reducing the %``freedom'',  and hence 
uncertainty that would be present should all these operators be independent degrees of freedom in the study. For a trivial example, a model predicting only a deviation of the Higgs self-coupling would match into the results of a SMEFT fit with only one operator to dimension six, $(\phi^\dagger \phi)^3$. For our purposes, this is equivalent to considering only the effect given by \cref{eq:VHgen}. As illustrated in the example in \cref{fig:KlambdaKi} with the improvement in the $\kappa_\lambda$ determination when this is the only degree of freedom in the fit (compare the orange band with the blue one, obtained including additional parameters), this model would be better constrained than in \cref{fig:sensitivityH3CC}, where one marginalizes over many other SMEFT parameters that would be zero in this particular scenario.
%, as these would be zero in the scenario of interest. 
 %Although it should be expected, given the nature of the EFT as an low approximation 
Finally, as in any other theory calculation, the level of agreement of the EFT fit results when matched to a model and that in the particular scenario will depend on the precision of the EFT theory calculations, both in the computation of observables as well as in the matching.\footnote{For example, it is well known that in some types of scenarios with extra scalar doublets it is important to include terms of dimension eight in the EFT expansion~\cite{Dawson:2022cmu}. See also \cite{Contino:2016jqw} for a more general discussion on the assessment of accuracy in the interpretation of the EFT description.} 
%For instance, and to give an extreme example, while clearly single or double Higgs observables at future $e^+ e^-$ colliders would be sensitive to a model introducing only very large deviations in $\kappa_\lambda$ from relatively light particles, that scenario may not be described accurately by the leading order dimension-6 SMEFT analysis of those observables. 
%For instance, and to give an extreme example, while clearly single or double Higgs observables at future $e^+ e^-$ colliders would be sensitive to a model introducing only a very large deviation in $\kappa_\lambda$ coming from the effects of relatively light particles, 
%the ``non-decoupling'' of such new physics effects due to the small gap between the particle masses and the scale of the observables may not be described accurately by the leading order dimension-6 SMEFT analysis.~\footnote{Note that, as long as the model is consistent with the EFT assumptions, this is not a limitation of the EFT description but of current calculations. 
%%The same failure would happen if the interpretation of single or double Higgs observables is done directly in the model including, e.g. its predictions for $\kappa_\lambda$ at 1-loop, but the large corrections enter at 2-loop, as in the case of some of the scenarios discussed in \cref{sec:largeH3}.
%}
% at the linear level, in the same way that any interpretation in terms of a given model would fail
 %extra theoretical uncertainties are needed for a interpretation in terms of such models. 
Continuing the effort of improving these interpretations to higher orders both in the EFT expansion as well as in perturbation theory, like the calculation described next, is therefore important to extend the range of applicability of current EFT results.
Conversely, this also highlights the need to, in the meantime, augment these interpretations with studies directly in terms of well-motivated models in those cases where they may not be described accurately in terms of current SMEFT calculations. 

\subsubsection{\texorpdfstring{$\epem \to \PZ\PH$ at NLO in the SMEFT}{e+ e- -> ZH at NLO in the SMEFT}}\label{sec:eeZH_NLO}

%We conclude this section discussing the progress on the theory side regarding the determination of $\lambda_{\PH\PH\PH}$ from single Higgs measurements, in particular in the context of EFT studies
%of new physics. 
%As mentioned above, sensitivity to the Higgs self-coupling in single Higgs processes comes from one-loop level contributions. The full structure of these NLO contributions depends on the particular theory framework used to interpret the measurements. 

We conclude this section discussing the progress on the theory side regarding the determination of $\lambda_{\PH\PH\PH}$ from single Higgs measurements, where the sensitivity to the Higgs self-coupling in single Higgs processes comes from one-loop level contributions, in the context of the SMEFT.  
%The full structure of these NLO contributions depends on the particular theory framework used to interpret the measurements. 
Within the SMEFT framework, the full set of NLO contributions from dimension-six operators %to the main Higgs production mechanism at low-energy Higgs factories, 
to $\epem \to \PZ\PH$ has recently been computed, first for operators involving the top quark~\cite{Asteriadis:2024qim} and then to the whole dimension-six basis~\cite{Asteriadis:2024xts}. A sample of such contributions is shown in \cref{fig:1loop}. From the point of view of the $\lambda_{\PH\PH\PH}$ SMEFT interpretation, 
these calculations open the possibility of extending previous studies in the direction of a model-independent interpretation within the assumptions of this EFT, see \cref{sec:globalSMEFT}.~\footnote{To achieve this, calculations of the NLO effects in other processes relevant for Higgs physics at $\epem$ are still missing, e.g.\ $\epem\to \nu\bar{\nu} \PH$ (via $W$ boson fusion).}

\begin{figure}
    \centering
    \includegraphics[height=69pt]{./figs/Hself/triag1.pdf}
    \includegraphics[height=69pt]{./figs/Hself/triag2.pdf}
    \includegraphics[height=69pt]{./figs/Hself/triag3.pdf}\\[8pt]
    \includegraphics[height=69pt]{./figs/Hself/box3.pdf}
    \includegraphics[height=69pt]{./figs/Hself/box2.pdf}
    \includegraphics[height=69pt]{./figs/Hself/box4.pdf}\\[8pt]
    \includegraphics[height=69pt]{./figs/Hself/4point1.pdf}
    \includegraphics[height=69pt]{./figs/Hself/4point2.pdf}
    \includegraphics[height=69pt]{./figs/Hself/4point3.pdf}
    \caption{
    %Sample virtual diagrams contributing to $\epem\rightarrow HZ$ at NLO in the dimension-6 SMEFT. We show contributions with one-loop vertex corrections (first row), planar and non-planar box diagrams (second row), and contributions with 4-point interactions (third row).
    }
    \caption{Example of 1-loop diagrams for contributions to the $\epem \to ZH$ cross section in the SMEFT.}\label{fig:1loop}
\end{figure}

Aside from the operators entering at LO, there are a total of 6 bosonic (4 of them CP violating), 9 two-fermion and 14 four-fermion dimension-six operators that contribute to $\epem \to \PZ\PH$ at NLO.
Of particular importance are the contributions of the top-quark operator mentioned before, e.g. $\epem \PQt\PAQt$ contact interactions, which are poorly constrained by current data but, as we will discuss below, will be measured at future \epem colliders. 
In this regard, and as in the case of the contributions from the Higgs self-coupling, 
considering modifications to top-quark interactions entering in other loop contributions to $\epem\to \PZ\PH$, runs at two centre-of-mass energies also provide complementary sensitivity and tight two-parameter constraints~\cite{Asteriadis:2024qim}, as shown in \cref{fig:top-operators}. 
Similarly, polarised beams can provide complementary information on different corrections, and help to separate the contributions of the Higgs self-coupling operator from those from top operators, as shown, e.g. in \cref{fig:top-operators-2}.
%The best way to constrain these additional effects, however, would be via a global study including additional observables with strong sensitivity to the new operators.


\begin{figure}[t]\centering
\includegraphics[width=0.35\textwidth]{./figs/Hself/CH_eu_1133}%
~~~~~~~~~~~~~~~~~~\includegraphics[width=0.35\textwidth]{./figs/Hself/CH_Cth}%
\caption{Left: Joint constraints on the trilinear Higgs self-coupling ($x$ axis) and on right-handed $\bar{e}e\bar{t}t$ operator ($y$ axis) from LEP, as well as \SI{240} and \SI{365}{\giga\electronvolt} runs.
Right: Similarly for the top-quark Yukawa operator ($y$ axis).
Figures reproduced from Ref.~\cite{Asteriadis:2024xts}.
}
\label{fig:top-operators}
\end{figure}
%
\begin{figure}[h]\centering
\includegraphics[width=0.35\textwidth]{./figs/Hself/Cfu33_Cphi}%
~~~~~~~~~~~~~~~~~~\includegraphics[width=0.35\textwidth]{./figs/Hself/Clq11133_Cphi}%
\caption{Left: contributions from modifications of the Higgs tri-linear coupling operator ($x$ axis) on the cross section $\epem \to \PZ\PH$ at \SI{240}{\giga\electronvolt}, correlated with those from $C_{\phi u}[3,3]$, which modify the $Zt\bar{t}$ vertex, and depending on the polarization of the $\epem$ system. Right: the same for the $\epem \PQt\PAQt$ operator with coefficient $C_{lq}^{(1)}[1,1,3,3]$ ($y$ axis).
Figures reproduced from Ref.~\cite{Asteriadis:2024qim}.
}
\label{fig:top-operators-2}
\end{figure}


%In a global study, these new NLO effects show that, in the single-Higgs analysis at NLO there would be a considerable amount of degeneracy.
The large number of different interactions entering at NLO would suggest that in the single-Higgs analysis at NLO there %would 
will be a considerable amount of degeneracy. 
%Thus, with 
With more operators simultaneously included, more observables need to be combined to constrain all directions 
in a global fit
and single out the potential new contributions to $\lambda_{\PH\PH\PH}$. 
%
In Higgsstrahlung production itself, angular distributions and radiative return to lower effective centre-of-mass energies could for instance be considered~\cite{talkecfa}.
%
Outside Higgs physics, the above-mentioned top interactions could be tested at the tree level in $\epem \to \PQt\PAQt$ at \SI{350}-\SI{365}{\giga\electronvolt}. Finally, some of the same top operators enter in Z-pole observables also at the loop-level, and a combined analysis exploiting the extreme high precision of the Tera-Z run could also help in a global analysis. 
The determination 
of $\lambda_{\PH\PH\PH}$ thus relies on %: (1) 
having precision measurements of a large enough number of observables to constrain any possible BSM effects in other contributions that enter in the calculations of the observables to the same order in perturbation theory as the leading contributions of $\lambda_{\PH\PH\PH}$.
%; (2) the precision of theory calculations and measurements of the inputs of the SM.\textbf{[JB: Already taken shown to have small effect]}
%

There is currently an ongoing effort to extend the $\lambda_{\PH\PH\PH}$ EFT determination from single-Higgs measurements, including these recent NLO effects, and other aspects related to this EFT interpretation. %These are discussed in \cref{sec:HprodH3}.

%The large dimensionality of the SMEFT analysis, especially when we move to studies including quantum corrections is sometimes used as an argument to question the potential of observables to obtain information about interactions entering only at the loop level. 

%While the large number of parameters presents indeed a technical complication, as it requre



%\subsubsection{Single-Higgs processes as probes of the Higgs self-coupling\label{sec:HprodH3}}
%\subsubsection{Progress in single-Higgs approach}
%\noindent Degeneracies at NLO SMEFT in $\PZ\PH$\\
%\noindent Differential cross-section measurements\\
%\noindent Results from New Global SMEFT Fit

% Extended SMEFT fit
% Determination of klambda different than SM (not in SMEFT)

%\textbf{[Results are hopefully available in January 2025, and discussed here]}. 
%------------------------------------------------------------------------





==> sections/higgs/hintro.tex <==
{\bf \color{blue} [The HL-LHC projections quoted in this chapter will be replaced with the latest values from ATLAS/CMS, when these are approved.]}

The Higgs boson that was first observed in 2012 by the ATLAS and CMS Collaborations with a mass of 125~\GeV~\cite{HIGG-2012-27,CMS-HIG-12-028} is the newest SM particle to be measured by experiments. It has been studied in detail at the LHC, and the upgraded experiments at the HL-LHC will provide further insight. This includes the LHCb experiment, which can provide additional constraints on Higgs-boson decays to a pair of bottom or charm quarks~\cite{LHCb:2013gxz}. 

The expected HL-LHC precision on the coupling between the Higgs boson and $\PZ$ bosons is 1.6\%, and goes up to about 7\% for the $\PH\PZ\PGg$ coupling~\cite{Dainese:2019rgk} (see \cref{fig:higgs:hllhccouplings}). However, these and other couplings are extracted under an assumption about the Higgs boson width, as the measurements combine production and decay processes.  Experiments at an $\epem$ collider can provide an absolute $\PH\PZ\PZ$ coupling determination with an inclusive measurement of the production cross section. This feature allows precise absolute determinations of many Higgs couplings at an $\epem$ collider, given  loose assumptions about the $\epem \to \PZ\PH$ process.  

There have been extensive studies on the sensitivity to many aspects of Higgs physics
for all of the major \epem\ Higgs factory options \cite{ILCInternationalDevelopmentTeam:2022izu,Abramowicz_2017,robson2018updatedclicluminositystaging,FCC:2018evy,CEPCPhysicsStudyGroup:2022uwl},
which have also been brought together in global fits,
for example those of Refs. \cite{DeBlas:2019qco,deBlas:2022ofj}. 
This report does not attempt to survey all of this previous work, 
but rather to summarize additional recent results that have been
developed in the context of the ECFA study, and submitted to it. 

\Cref{sec:ZHang} discusses studies of $\PZ\PH$ production and various interpretations, including \CP properties of the Higgs couplings.
%
An $\epem$ collider also allows measurements of the couplings of the Higgs boson to second-generation quarks, which are unattainable at the LHC if their values are of the order predicted by the SM. Even upper limits close to the SM value can be reached for the electron Yukawa 
at circular $\epem$ colliders running at $\sqrt{s}=125$~\GeV, via direct $s$-channel production $\epem\to\PH$, as described in \cref{sec:eYukawa} in the context of FCC-ee. The determination of the Higgs boson coupling to strange quarks will be challenging, and the extensive ongoing investigations into the prospects are described in \cref{sec:HtoSS}.

A key Higgs parameter is the strength of the trilinear Higgs boson coupling, $\lambda_{\PH\PH\PH}$, the measurement of which is frequently presented as the ratio of the observed value to the SM prediction, $\kappa_{\lambda}\equiv \lambda_{\PH\PH\PH}/\lambda_{\PH\PH\PH}^{\rm SM}$. At the HL-LHC, the latest combined extrapolation by the ATLAS and CMS Collaborations yields an expected uncertainty on $\kappa_{\lambda}$ of \textcolor{red}{ [--26\%,+29\%] } (see \cref{fig:higgs:hllhclambda}). %, while newer individual results suggest significantly improved expectations~\cite{ATL-PHYS-PUB-2022-005,ATL-PHYS-PUB-2024-016}.  
At $\epem$ centre-of-mass energies below about 500~\GeV, constraints of around 30\% can be obtained using precise $\epem \to \PZ\PH$ cross-section measurements, while above this energy the self-coupling can be determined to 20\% or better via Higgs pair production.  Details of the possible constraints are provided in \cref{sec:Hself}.

%The results in this chapter focus on updated and new Higgs boson studies since the %comprehensive Snowmass effort~\cite{Dawson:2022zbb}.

\begin{figure}[h!]  
    \begin{subfigure} {.4\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/Higgs/ATLAS_CMS_Higgs_couplings.pdf}
        \caption{}
        \label{fig:higgs:hllhccouplings}
    \end{subfigure}
    \quad
    \begin{subfigure}{.6\linewidth}  
        \centering
        \includegraphics[width=\linewidth]{figs/Higgs/ATLAS_CMS_Higgs_kappaL.pdf}         
        \caption{}
        \label{fig:higgs:hllhclambda}
        \end{subfigure}
    \caption{Expected precision of Higgs boson coupling measurements at the HL-LHC. The extrapolations were performed by the ATLAS and CMS Collaborations in 2022 as input to the Snowmass process~\cite{Dawson:2022zbb}. The expected precision of the Higgs boson coupling modifiers to other SM particles is shown on the left, while the Higgs boson self-coupling measurement projection is shown on the right. Reproduced from Ref.~\cite{Dainese:2019rgk}.}
\end{figure}


==> sections/higgs/hinv.tex <==

%\TODO{Needs introduction, significance of Hinv, and perhaps context of other sensitivities.  Keep or cut according to actual results.}

The SM predicts a small branching ratio ($\sim$ 0.1\%) for invisible decays of the Higgs boson (BR$(\PH\to\PZ\PZ^*\to\PGn\PAGn\PGn\PAGn)$).  However, new physics could significantly increase this; for example in frameworks such as the Higgs-Portal model, where dark matter interacts via couplings with the Higgs boson.  This section describes a new analysis assessing the sensitivity of an \epem collider to invisibly-decaying Higgs bosons.

The signal process, the Higgs-strahlung process with $\PH\to\mathrm{invisible}$ and $\PZ\to \PQq\PAQq$ is shown in Figure~\ref{fig:higgsstrahlung}. This channel promises the highest sensitivity due to its relatively large cross-section. The main background processes are 
$\Pep\Pem\to \PZ\PZ\to\PGn\PAGn\PQq\PAQq$ and $\Pep\Pem\to \PW\PW \to \Pl\PGn\PQq\PAQq$. In case of the signal with leptonically decaying $\PZ$ the background processes change accordingly.
\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{./figs/Higgs/higgsstrahlung.jpg}
\caption{Leading-order Feynman diagram of the Higgs-strahlung process.}
\label{fig:higgsstrahlung}
\end{figure}

We assume two centre-of-mass energies, $\sqrt{s}$ = \SI{250}{\giga\electronvolt} and \SI{500}{\giga\electronvolt}, and two beam polarisation configurations, (P\Pem, P\Pep) = ($\mp$ 0.8, $\pm$ 0.3).  Integrated luminosities of \SI{900}{\per\femto\barn} / \SI{1600}{\per\femto\barn} are assumed for both beam polarisation configurations at $\sqrt{s}$ = \SI{250}{\giga\electronvolt} / \SI{500}{\giga\electronvolt} based on the ILC running scenario~\cite{Fujii:2017vwa}.

We use the signal and background samples which have been generated in the context of the ILC Technical Design Report~\cite{Behnke:2013xla,ILC:2013jhg,Adolphsen:2013jya,Adolphsen:2013kya,Behnke:2013lya}. The beam energy spectrum includes the effects of beamstrahlung and the initial state radiation. The beam backgrounds from \PGg\PGg interactions are included in all signal and background processes. As the signal process, $\Pep\Pem\to \PQq\PAQq \PSH$ with $\PSH \to \PZ\PZ^\star\to \PGn\PAGn\PGn\PAGn$ is used adjusting BR(\PH $\to$ invisible) = 10\%. The background processes from \Pep\Pem interactions are categorized according to the number of final-state fermions and whether Higgs is included: two fermions (2f), four fermions (4f) and SM Higgs processes.

We perform the detector simulation with Mokka~\cite{MoradeFreitas:2002kj}/ DD4Hep~\cite{frank_markus_2018_1464634,}, a Geant4-based~\cite{GEANT4:2002zbu,} full
simulation, with the ILD detector model ILD\_o1\_v05 / ILD\_l5\_o1\_v02 for $\sqrt{s}$ = \SI{250}{\giga\electronvolt} / \SI{500}{\giga\electronvolt}. Events have been reconstructed using PandoraPFA~\cite{Thomson:2009rp} in the Gaudi framework~\cite{Barrand:2001ny} within the key4HEP stack.

The isolated lepton tagging is performed with IsolatedLeptonTagging processor~\cite{leptontagger} to remove (select) events which contain isolated leptons in case of the hadronic (leptonic) channel. We use the parameters summarized~\cite{Kato:2020pyl,} for IsolatedLeptonTagging, where ECAL is the energy deposit in the whole calorimeter system, p is the track momentum, EECAL / EHCAL is the energy deposit in the electromagnetic / hadron calorimeter system and Eyoke is the energy deposit in the Yoke system. A multivariate double cone method is used to require isolation and a cut on MVA output is applied.

After the isolated lepton tagging, the jet clustering is applied using the Durham algorithm~\cite{Moretti:1998qx} by the LCFIPlus processor~\cite{Suehara:2015ura} to force particles into two jets. At the same time, the beam background rejection with the rejection parameter $\alpha$ of 5.0 is performed at $\sqrt{s}$ = \SI{500}{\giga\electronvolt} to remove the beam backgrounds from \PGg\PGg interactions.

%After the event reconstruction step, an event selection is performed. As mentioned above, the branching ratio of \PH to invisible is assumed as 10\% for simplicity of event selection. The cut conditions and number of remaining events are listed in Table~\ref{tab:H2inv:cuts} where significance is defined as $N_S/\sqrt{N_S + N_B}$. And also t
The recoil mass distribution after event selection is shown in Figure~\ref{fig:recoil250} for $\sqrt{s}$ = \SI{250}{\giga\electronvolt} and Figure~\ref{fig:recoil500} for $\sqrt{s}$ = \SI{500}{\giga\electronvolt}.

%% results needed -- CH
%\begin{table}[h!]
%\centering
% \begin{tabular}{c| c c| c}
% \hline
% cut & signal (efficiency) & background (efficiency) & significance \\ [0.5ex]
% \hline
% no cut             & ??? & ??? & ??? \\
% $N_{\mathrm{lep}}$ & ??? & ??? & ??? \\
% \ldots             &  -- &  -- & ??? \\
% \hline
% \end{tabular}
% \caption{List of cuts for all scenarios {\color{red} Do we actually need this? -- NO!!   }}
%\label{tab:H2inv:cuts}
%\end{table}

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{./figs/Higgs/higgsstrahlung.jpg}
\includegraphics[width=0.45\textwidth]{./figs/Higgs/higgsstrahlung.jpg}
\caption{PLOT TO BE ADDED IN JANUARY  Recoil mass distribution after event selection at $\sqrt{s}$ = \SI{250}{\giga\electronvolt}. left: (P$_{\Pem}$, P$_{\Pep}$) = $(-0.8,+0.3)$, right: (P$_{\Pem}$, P$_{\Pep}$) = $(+0.8,-0.3)$.}
\label{fig:recoil250}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.45\textwidth]{./figs/Higgs/higgsstrahlung.jpg}
\includegraphics[width=0.45\textwidth]{./figs/Higgs/higgsstrahlung.jpg}
\caption{PLOT TO BE ADDED IN JANUARY   Recoil mass distribution after event selection at $\sqrt{s}$ = \SI{500}{\giga\electronvolt}. left: (P$_{\Pem}$, P$_{\Pep}$) = $(-0.8,+0.3)$, right: (P$_{\Pem}$, P$_{\Pep}$) = $(+0.8,-0.3)$.}
\label{fig:recoil500}
\end{figure}

After the event selection, we estimate 95\% C.L. upper limit on BR(H to invisible). First, we calculate significance from NS and NB for each bin of the recoil mass distribution after selection and combine them in all bins (Root Mean Square). Then, upper limit is calculated with combined significance using following formula:
\begin{equation}
    \mathrm{UL}_{95\%\mathrm{C.L.}} [\%]=\dfrac{10[\%]\times1.65}{\mathrm{significance}(\mathrm{BR}=10[\%])}
\end{equation}

The results are summarized in Table~\ref{tab:results250} for $\sqrt{s}$ = \SI{250}{\giga\electronvolt} and Table~\ref{tab:results500} for $\sqrt{s}$ = \SI{500}{\giga\electronvolt}.

\begin{table}[h!]
\centering
 \begin{tabular}{c| c c c}
 \hline
 Mode & $(-0.8,+0.3)$ & (+0.8, -0.3) & combined \\ [0.5ex]
 \hline
 $\PZ\to\PQq\PAQq$ & ??? & ??? & ??? \\
 $\PZ\to\Pl\PAl$   & ??? & ??? & ??? \\
 combined          &  -- &  -- & ??? \\
 \hline
 \end{tabular}
 \caption{95\% C.L. upper limit on BR(\PH $\to$invisible) for $\sqrt{s}$ = \SI{250}{\giga\electronvolt} TO BE ADDED IN JANUARY}
\label{tab:results250}
\end{table}

\begin{table}[h!]
\centering
 \begin{tabular}{c| c c c}
 \hline
 Mode & $(-0.8,+0.3)$ & (+0.8, -0.3) & combined \\ [0.5ex]
 \hline
 $\PZ\to\PQq\PAQq$ & ??? & ??? & ??? \\
 $\PZ\to\Pl\PAl$   & ??? & ??? & ??? \\
 combined          &  -- &  -- & ??? \\
 \hline
 \end{tabular}
 \caption{95\% C.L. UL on BR(\PH $\to$invisible) for $\sqrt{s}$ = \SI{500}{\giga\electronvolt}. TO BE ADDED IN JANUARY}
\label{tab:results500}\end{table}



==> sections/higgs/hmass.tex <==
\subsubsection*{Introduction}

The FCC-ee offers a unique opportunity to precisely measure the properties of the Higgs boson, using over $2\times 10^6$ events at a centre-of-mass energy \roots~=~240~\GeV~and an additional $4\times 10^5$ events at \roots~=~365~\GeV. A per mil level measurement of the total $\PZ\PH$ cross-section is essential for determining the absolute HZZ coupling, which is necessary to interpret other measurements including measurements done at hadron colliders. Determining the Higgs boson mass with a precision smaller than its width (4.1 MeV in the Standard Model) is necessary to either constrain or measure the electron Yukawa coupling via direct $\epem \rightarrow \PH$ production at \roots~=~125~\GeV. 

This summary investigates the $\PZ\PH$ production cross-section at both centre-of-mass energies, focusing on leptonic decays of the associated Z boson (electrons and muons), as well as the Higgs mass analysis obtained from the recoil distribution~\cite{eysermans_2024_a68b8-3mt57}. Results quoted are obtained from Monte Carlo events using the \whizard~+~\pythia event generator, interfaced with the fast simulation package Delphes. The IDEA detector with a crystal electromagnetic calorimeter is used as a reference detector. Furthermore, results are normalised to an integrated luminosity of \SI{10.8}{\per\atto\barn} and  \SI{3}{\per\atto\barn} for both \roots~=~240 and 365~\GeV~respectively. 

\subsubsection*{ZH cross-section}

\begin{figure}
  \begin{center}
    \includegraphics[width=0.5\linewidth]{figs/Higgs/recoil.pdf}
    \caption{Recoil mass distribution after all selections at \roots~=~240~\GeV.}
    \label{fig:recoil}
  \end{center}
\end{figure}

The $\PZ\PH$ cross-section analysis, performed in both $\PZ(\mumu$\PH$ and $\PZ(\epem$\PH$ final states, relies heavily on precise event selection to effectively suppress backgrounds from \ww, \PZ\PZ, and \PZ\PGg processes. To ensure independence from specific Higgs boson decay modes, the selection utilizes only the kinematic properties of the leptons. Events are selected by first identifying a pair of opposite-sign leptons, requiring at least one of the leptons to be isolated. The invariant mass of this lepton pair must be compatible with the Z boson mass ($86 < m_{\ell\ell} < 96~\GeV$), alongside specific requirements on the dilepton momentum ($20(50) < p_{\Pl\Pl} < 70(150)~\GeV$) at \roots~=~240(365)~\GeV~respectively. Lastly, the recoil of the dilepton system must be within the Higgs boson mass window of  $120 < m_{\text{rec}} < 140~\GeV$. The resulting recoil distribution after all selections is shown in Figure~\ref{fig:recoil} for the centre-of-mass energy of \roots~=~240~\GeV.

To further enhance sensitivity to the $\PZ\PH$ signal, the selected events are subjected to a Boosted Decision Tree (BDT), trained on the lepton-based input variables that maintain independence from specific Higgs boson decay modes. Additional variables based on the lepton angles are also included. The training is conducted separately for electron and muon events, as well as for both centre-of-mass energies. To retain the full statistical power of all selected events, the BDT output distribution is employed to extract the $\PZ\PH$ cross-section uncertainty through a binned maximum likelihood fit. At \roots~=~240~\GeV, the results show uncertainties of 0.76\% for the muon final state and 0.92\% for the electron final state, yielding a combined uncertainty of 0.58\%. At \roots~=~365~\GeV, the uncertainties are 1.91\% for the muon final state and 2.13\% for the electron final state, with a combined uncertainty of 1.42\%. Systematic uncertainties are found to be small compared to the statistical ones, and the total uncertainties are 0.59\% and 1.48\% at 240 and 365~GeV, respectively.

\subsubsection*{Higgs mass}

The Higgs mass is determined by reconstructing the recoil in both $\PZ(\mumu\PH$ and $\PZ(\epem\PH$ events, combined with precise knowledge of the centre-of-mass energy \roots. This analysis is performed exclusively at \roots~=~240~\GeV~, as the sensitivity at \roots~=~365~\GeV~is negligible due to lower statistics and poorer recoil resolution at the higher energy. The latter is primarily affected by the increased beam energy spread and larger initial-state radiation.

Starting from the baseline selection criteria for the cross-section analysis, an additional selection is applied using $\text{cos}(\theta_{\text{miss}}) < 0.98 $, with $\theta_{\text{miss}}$ the polar angle of the missing energy vector, to further reduce the $\PZ\PGg$ background. The remaining events are categorized based on the polar angles of the leptons: both central, one central and one forward, and both forward. This allows differentiation of the recoil resolutions, accounting for the varying material budget in different regions of the tracker. For each category, the recoil distribution is fitted using an analytic function comprising two Crystal Ball functions and a Gaussian. This procedure is repeated for off-peak samples ($\pm~50$~\MeV) relative to the nominal Higgs mass of 125~\GeV, with the backgrounds merged and modeled using a polynomial function.

A maximum likelihood fit is used to determine the Higgs mass sensitivity based on analytic shape models, yielding uncertainties of 3.92~\MeV~for the muon final state and 4.95~\MeV~for the electron final state, with a combined uncertainty of 3.07~\MeV. The electron channel shows slightly lower performance due to its poorer resolution and the presence of a small VBF contribution in the t-channel, which broadens the recoil distribution.

The primary systematic uncertainty arises from the centre-of-mass energy, conservatively estimated to be 2~\MeV~based on $\PZ\rightarrow \Pl\Pl$ radiative return events. When this uncertainty, along with other less significant uncertainties, is included in the likelihood fit, the Higgs mass uncertainties are 4.74~\MeV~for the muon final state and 5.68~\MeV~for the electron final state, with a combined uncertainty of 3.97~\MeV. The inclusion of systematic effects increases the overall uncertainty by 30\% compared to the statistical-only result.


\begin{table}[ht]
\centering
\begin{tabular}{llll}
\toprule
\textbf{Fit configuration}              & \textbf{\mumu} channel    & \textbf{\ee} channel  & combination  \\
\midrule
Nominal IDEA + crystal ECAL (2T field)  & 3.92 (4.74)               & 4.95 (5.68)           & 3.07 (3.97) \\ % OK
\midrule
IDEA + crystal ECAL with 3T field       & 3.22 (4.14)               & 4.11 (4.83)           & 2.54 (3.52) \\ % OK
\midrule
IDEA with silicon tracker (2T)          & 5.11 (5.73)               & 5.89 (6.42)           & 3.86 (4.55) \\ % OK
\midrule
Ideal resolution                        & 3.12 (3.95)               & 3.58 (4.52)           & 2.42 (3.40) \\ % OK
\bottomrule
\end{tabular}
\caption{Statistical uncertainty on the Higgs mass (MeV) for various detector configurations. The values in brackets represent the statistical+systematic uncertainties.}
\label{tab:mass:fit_results}
\end{table}

Table~\ref{tab:mass:fit_results} summarizes the results for various detector configurations. When the reconstructed muons and their uncertainties are substituted with generator-level kinematics, the total mass uncertainty -- dominated by selection requirements and backgrounds -- improves by 21\% for the statistical-only case and 14\% for the statistical plus systematic case. Increasing the magnetic field from 2T to 3T yields an improvement of 17\% (statistical only) and 11\% (statistical + systematic), although this improvement is ultimately limited by the beam energy spread, which becomes the dominant factor. Conversely, replacing the IDEA drift chamber with a heavier silicon tracker degrades the uncertainty by 26\% (statistical only) and 15\% (statistical + systematic).

\subsubsection*{Summary}

This note presents the expected results for the Higgs boson mass and the model-independent $\PZ\PH$ cross-section measurement with FCC-ee at \roots~=~240~GeV and \roots~=~365~GeV. Using di-muon and di-electron $\PZ\PH$ events, the $\PZ\PH$ cross-section can be measured with a relative precision of 0.59~\% at \roots~=~240 and 1.48~\% at \roots~=~365~\GeV. Using a similar event selection, the Higgs boson mass can be determined with an uncertainty of 3.97~MeV, including the dominant systematic uncertainty from the centre-of-mass energy.


==> sections/higgs/hself_V1.tex <==

\vspace*{.1cm}
\subsection{\focustopic Higgs self-coupling}
\label{sec:Hself}
\editor{Junping Tian, Jorge de Blas}

\subsubsection{Introduction}
%\footnote{{\it Editorial note:} The contents of this introduction are based, in part, on a submission summarizing Ref.\cite{Bechtle:2024acc}. These have been substantially edited and may not accurately reflect the opinions or the intended message of the authors in that document.}


Many open questions of particle physics are related to the Higgs sector and, in particular, to the Higgs potential.  
The Higgs potential gives rise to
electroweak symmetry breaking and plays a crucial role in determining how 
the electroweak phase transition (EWPT) in the early universe took place, as well as providing a possible explanation of the observed asymmetry between matter and anti-matter in the universe in terms of electroweak baryogenesis. However, the actual form of the Higgs potential that is realised in nature and its physical origin are largely unknown up to now. The Higgs potential receives contributions from the detected Higgs boson $\PH$ with a mass $m_{\PH}$ of about 125 GeV and from any additional scalar fields that could exist in nature, even if not detected so far. While the bilinear term proportional to $\PH^2$ is related to the measured value of $m_{\PH}$, and tells us about the potential around the electroweak (EW) minimum, 
accessing the trilinear Higgs coupling $\lambda_{\PH\PH\PH}$, proportional to $\PH^3$, is crucial to understanding the shape of the Higgs potential away from that point. 
However, the trilinear Higgs self-coupling, $\lambda_{\PH\PH\PH}$, and the quartic Higgs self-coupling, $\lambda_{\PH\PH\PH\PH}$, proportional to $\PH^4$, are only loosely constrained so far (and only weak bounds exist on contributions to the Higgs potential from additional fields).

It is important to clarify that the Higgs self-coupling(s), like any other coupling, are not themselves physical observables, hence their determination is tied to the interpretation of an observable (e.g. the Higgs pair production cross section) within a given theory framework. Therefore, a fully model-independent measurement of a Higgs coupling is impossible as a matter of principle at any future collider, and the choice of both theory framework and the observables to be interpreted can play a role in how easy is to measure $\lambda_{\PH\PH\PH}$. The main probes 
used currently in LHC experiments as well as those possible at future $\epem$ colliders are briefly described in what follows, with the progress made in the latter being the core focus of this section.

The existing constraints on $\lambda_{\PH\PH\PH}$ from the LHC have mainly been obtained from the searches for the Higgs pair production process, dominated by the gluon-fusion channel. %The current upper bound on the di-Higgs production cross section from ATLAS and CMS translates into an upper limit on $\lambda_{\PH\PH\PH}$ that is about 7 times larger than the (tree-level) SM value, assuming that all other Higgs couplings besides $\lambda_{\PH\PH\PH}$ are fixed to their SM values~\cite{ATLAS:2024ish,CMS:2022dwd}. (A lower limit can also be set.)
Assuming that all other Higgs couplings besides $\lambda_{\PH\PH\PH}$ are fixed to their SM values, the current bounds on the di-Higgs production cross section from ATLAS and CMS can be translated into limits on the Higgs self-coupling, $-1\lesssim \kappa_\lambda \lesssim 7 $ at 95$\%$ C.L. , with $\kappa_\lambda\equiv \lambda_{\PH\PH\PH}/\lambda_{\PH\PH\PH}^\textrm{SM}$~\cite{ATLAS:2024ish,CMS:2022dwd}. 
%
On the other hand, 
%The 
the current projections for the HL-LHC (for the combined integrated luminosity that is expected to be collected by ATLAS and CMS) yield an experimental uncertainty for $\lambda_{\PH\PH\PH}$ of about 50\% at the 68\% C.L.\ if the SM value is realised in nature~\cite{Cepeda:2019klc},
while newer individual results suggest significantly improved expectations~\cite{ATL-PHYS-PUB-2022-005,ATL-PHYS-PUB-2024-016}.%\textbf{[JB: To be updated for the next strategy with, apparently, a substantial improvement.]}
 It should be noted that, in the gluon fusion channel, the leading-order one-loop diagram containing $\lambda_{\PH\PH\PH}$ and the top Yukawa coupling $y_t$ enters together with a box diagram involving the coupling factor $y_t^2$ and, because of a large destructive interference between the contributions from these two diagrams, the total cross section for di-Higgs production changes very substantially, if $\lambda_{\PH\PH\PH}$ is varied around the SM value. This is illustrated in the left panel of \cref{fig:HHxs_kappalambda}, where the Higgs pair production cross section is shown as a function of $\lambda_{\PH\PH\PH}$ for the  different production modes.


%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\centering
%  %\begin{center}	
  \includegraphics[width=0.45\textwidth]{./figs/Hself/HH_LHC.png}
~
  \includegraphics[width=0.5\textwidth]{./figs/Hself/xsec_coupling_BSM.pdf}
%  %\end{center}
\caption{Higgs pair-production cross section, as a function of $\lambda_{\PH\PH\PH}$, at the LHC~\cite{Frederix:2014hta} (left) and $e^+ e^-$ colliders~\cite{DiMicco:2019ngk} (right).}
\label{fig:HHxs_kappalambda}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


While the existing bounds on $\lambda_{\PH\PH\PH}$ are rather weak, they nevertheless already probe so-far untested parameter regions of physics beyond the SM, 
in those scenarios where loop effects result in corrections to 
%Higgs self-couplings 
$\lambda_{\PH\PH\PH}$ that can be much larger, by more than two orders of magnitude, than to the couplings of $h$ to gauge bosons and fermions; see \cite{Kanemura:2002vm,Bahl:2022jnx,Bahl:2023eau} for investigations of extended Higgs sectors and \cite{Durieux:2022hbu} for SMEFT analyses. 
Some of these scenarios are discussed in \cref{sec:largeH3}. 
%
A very significant upward shift in $\lambda_{\PH\PH\PH}$ is also motivated in many scenarios giving rise to a strong first-order EWPT which is required for electroweak baryogenesis; see e.g.\ \cite{Biekotter:2022kgf} for the case of the 2HDM, where the parameter region featuring a strong first-order EWPT and a potentially detectable gravitational wave signal at the future space-based observatory LISA is correlated with an enhancement of $\lambda_{\PH\PH\PH}$ compared to the SM value by about a factor of 2.
%Conversely, models where $\lambda_{\PH\PH\PH}$ is suppressed by order one corrections with respect the SM are also possible~\cite{Noble:2007kk}.


At future $\epem$ colliders information about $\lambda_{\PH\PH\PH}$ could be obtained in different and complementary ways. The more ``traditional'' approach relies on the energy reach, and is relevant for colliders whose centre-of-mass energy can go well past the $\PZ\PH\PH$ threshold, to the point where the cross section is large enough to produce Higgs pairs with enough statistical significance. On the other hand, a second approach based on the precision reach of different measurements, typically single Higgs processes, is the main source of information at low-energy Higgs factories.


Starting with $\epem$ colliders with a CM energy of at least 500~GeV,  the Higgs pair production process $\epem \to Z\PH\PH$ can be measured. (This is also the case for the weak-boson fusion process $\epem \to \nu_e\bar\nu_e \PH\PH$, though this would benefit from much larger CM energies.) 
As will be discussed in ~\cref{sec:HHprod}, the projected accuracy at a 550 GeV linear $\epem$ collider is about 15\%, combining the results from the $Z\PH\PH$ and $\nu_e\bar\nu_e \PH\PH$ channels~\cite{JTianComb}. Furthermore, 
unlike the leading process at hadron colliders, the interference contribution in the $Z\PH\PH$ channel at a 550 GeV $\epem$ collider is constructive, as shown in the right-hand panel of \cref{fig:HHxs_kappalambda}. As a result of this, if the value of $\lambda_{\PH\PH\PH}$ that is realised in nature is actually larger than the SM prediction, the destructive interference in gluon-fusion will result in a degradation of the $\lambda_{\PH\PH\PH}$ determination at hadron colliders, whereas at $\epem$ the accuracy would improve. As can be seen in \cref{fig:kappalambda}, for $\kappa_\lambda = 2$ the precision of the HL-LHC determination would degrade to $\sim 84\%$ 
%{\it (such a degradation holds at any hadron collider and 
%has also been found 
(see, e.g.~\cite{ATL-PHYS-PUB-2024-016} for a recent projection from the ATLAS Collaboration illustrating this effect). 
On the other hand, in this same case, the determination of $\lambda_{\PH\PH\PH}$ at the ILC running at 550 GeV improves to $\sim 7\%$, more than an order of magnitude better than the one at the HL-LHC. 
As mentioned above, such large values of $\kappa_\lambda$ would be favoured in scenarios giving rise to a strong first-order EWPT. 
Furthermore, aside from possible enhancements in the value of $\kappa_\lambda$, 
in BSM scenarios with extra scalars, one typically finds additional triple Higgs couplings (THCs) involving also heavy Higgses. The measurements of the Higgs pair-production process could also bring sensitivity to THCs involving one of such BSM states which, if sufficiently light, could enter in the process via a resonant contribution. The effects that such scenarios could have on $\epem \to Z\PH\PH$ is explored in \cref{sec:BSMHhh}, with special emphasis on the impact of loop corrections to these THCs. 

%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht!]
\centering
%  %\begin{center}	
  \includegraphics[width=0.7\textwidth]{./figs/Hself/lambda_ECFA25significanceILC550abs_2.pdf}
%  %\end{center}
\caption{Projected accuracies for $\lambda_{\PH\PH\PH}$ at the HL-LHC and a 550 GeV $\epem$ collider as a function of the actual value of $\lambda_{\PH\PH\PH}$ that is realised in nature. From the ILC study in~\cite{JL}.}
\label{fig:kappalambda}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Below the threshold for Higgs pair production processes, ``low-energy'' $\epem$ Higgs factories can still be sensitive to the effects of the Higgs self-coupling, via its virtual loop effects in other observables, where the higher precision of the measurements can be used to (partially) compensate the loop suppression of such contributions. 
Specifically, the single Higgs observables receive one-loop contributions that depend on $\lambda_{\PH\PH\PH}$, while in the predictions for the electroweak precision observables at the Z~pole and for the W-boson mass $\lambda_{\PH\PH\PH}$ enters at the two-loop level. In particular, special attention has been paid to the determination
of the Higgs self-coupling from measurements of single-Higgs processes, where sub-percent precision could bring enough sensitivity to quantum effects of $\lambda_{\PH\PH\PH}$~\cite{McCullough:2013rea}. 
Thus, low-energy $\epem$ Higgs factories would bring the possibility of testing $\lambda_{\PH\PH\PH}$ in a way that is complementary to that from Higgs pair production.  
%
In general, the loop contributions involving $\lambda_{\PH\PH\PH}$ compete with larger lowest-order contributions, and with other loop contributions (e.g.\ a top-quark loop). The sensitivity to $\lambda_{\PH\PH\PH}$ via loop effects may also be more affected by the theoretical uncertainties induced by unknown higher-order contributions and by the experimental errors of the input parameters (in particular $\alpha_{\mathrm{em}}$, $\alpha_{\mathrm{s}}$, $m_t$, $m_b$, \ldots). 

For the study of sensitivity to $\lambda_{\PH\PH\PH}$ in single Higgs processes, the possible deviations in the Higgs self-coupling with respect to the SM have been typically parameterized within the so-called SMEFT formalism, see \cref{sec:globalSMEFT}, truncated to dimension six.\footnote{This includes only effects of ${\cal O}(1/\Lambda^2)$ with $\Lambda$ the heavy scale acting as cutoff of the EFT. As is also shown in the results in \cref{sec:globalSMEFT}, the inclusion of effects of ${\cal O}(1/\Lambda^4)$ with the precision achievable at future colliders would seem to have only a small impact on the dimension-six results, suggesting the EFT expansion is well behaved.}   
%
The studies presented in \cite{deBlas:2019rxi} (see Figure 11 in that reference) reported the sensitivity to $\lambda_{\PH\PH\PH}$ for different future colliders, assuming the SM value is realized in nature, i.e. $\kappa_{\lambda}=1$. Although these studies take into account the effect of projected SM theory uncertainties mentioned above and also illustrate some illuminating points about the interplay of different EFT contributions, they were restricted to the EFT calculations available at that time and, as we discuss below, recent EFT calculations of additional NLO effects could affect the $\lambda_{\PH\PH\PH}$ interpretation. 
%
For instance, in
an EFT analysis including only the 1-loop contributions from $\lambda_{\PH\PH\PH}$ as well as any possible contribution at leading-order, measurements at a single centre-of-mass energy show an approximate degeneracy, which can efficiently be lifted by performing measurements at a second $\sqrt{s}$~\cite{DiVita:2017vrr}.
With runs at \SI{240}{} and \SI{365}{\giga\electronvolt}, the FCC-ee would achieve the sensitivity pictured in \cref{fig:sensitivityH3CC}. 
 However, without any extra model assumptions, a consistent analysis in the EFT approach at next-to-leading order (NLO) requires introducing the contributions from 
 all the operators that contribute at that order. This introduces 
 a large number of additional EFT contributions, in particular from $\epem\PQt\PAQt$ operators, which are currently poorly constrained, and could potentially reduce the precision in $\kappa_{\lambda}$.
 %operators. 
 For the main production process $\epem \to \PZ\PH$ such NLO contributions have only been recently identified in~\cite{Asteriadis:2024qim,Asteriadis:2024xts}. 
Details on this calculation and its implications are discussed in \cref{sec:eeZH_NLO}
and
\cref{sec:HprodH3},
respectively.
%which close the contents of this chapter.


\begin{figure}[h]\centering
\includegraphics[width=.5\textwidth]{./figs/Hself/fcc2dplot2}
\caption{$1\sigma$ sensitivity achievable on the trilinear self-coupling of the Higgs (shown on the $x$ axis) with 240 and \SI{365}{\giga\electronvolt} runs at the FCC-ee.
Aside from the single Higgs coupling to the $Z$ boson (shown on the $y$ axis), %eighteen additional Higgs 
26 additional Higgs and EW coupling modifications have been marginalised over to obtained the ellipses shown.
%{\bf SH: why is $\Delta \chi^2 = 1$ is used in a 2-dim plot?}
}
\label{fig:sensitivityH3CC}
\end{figure}

%-----------------------------------------------

\subsubsection{\texorpdfstring{Generating large corrections to the Higgs self-coupling in new physics models}{Generating large corrections to lambda(HHH) in BSM models}}\label{sec:largeH3}
{\bf\color{blue} Notation for light Higgs here is inconsistent with the rest. Need to fix so light Higgs is still H, as in other parts of the higgs section. Use ${\cal H},~{\cal A}$ for the heavy ones? But figures use the wrong notation... For the moment I added a footnote to explain the change of ntoation}

As mentioned above, the Higgs self coupling is important for determining the dynamics and nature of the EW phase transition (EWPT). As an example, the scenario of electroweak baryogenesis would require the EWPT to be of strong first order, which cannot be realised in the SM. In many Beyond-the-Standard-Model (BSM) theories, this is correlated with a deviation of $\lambda_{\PSh\PSh\PSh}$ from its SM prediction~\cite{Kanemura:2004ch,Grojean:2004xa}.~\footnote{
In this section we use the notation $\PSh$ to refer to the SM-like Higgs boson, to distinguish it from the other possible heavy Higgs bosons that appear, e.g. in 2HDM models, for which the notation $\PH, \PH^\pm$ is used.} 
For instance, a strong first-order EWPT (SFOEWPT) in the Two-Higgs-Doublet Model (2HDM) would imply a value of $\kappa_\lambda \equiv \lambda_{\PSh\PSh\PSh}/\lambda^{\mathrm{SM, tree}}_{\PSh\PSh\PSh} \sim 2$~\cite{Biekotter:2022kgf}. 

Another interesting property of the trilinear Higgs coupling is that it can, in models with extended scalar sectors, deviate significantly from its SM prediction because of large higher-order radiative corrections from the additional BSM scalars (which we generically denote $\Phi$)~\cite{Kanemura:2002vm,Kanemura:2004mg,Aoki:2012jj,Kanemura:2015fra,Kanemura:2015mxa,Arhrib:2015hoa,Kanemura:2016sos,Kanemura:2016lkz,He:2016sqr,Kanemura:2017wtm,Kanemura:2017wtm,Kanemura:2017gbi,Chiang:2018xpl,Basler:2018cwe,Senaha:2018xek,Braathen:2019pxr,Braathen:2019zoh,Kanemura:2019slf,Basler:2020nrq,Braathen:2020vwo,Bahl:2022jnx,Bahl:2022gqg,Bahl:2023eau,Aiko:2023xui,Basler:2024aaf}. %The corrections involving these BSM scalars, which we generically denote $\Phi$, 
These corrections are controlled by couplings of the general form $g_{\PSh\PSh\Phi\Phi}\propto(m_\Phi^2-\mathcal{M}^2)/v^2$, where $m_\Phi$ is the physical mass of the scalar $\Phi$, $\mathcal{M}$ is some mass scale controlling the decoupling of the BSM states, and $v$ is the SM vacuum expectation value. In scenarios where a splitting occurs between $\mathcal{M}$ and $m_\Phi$, the $g_{\PSh\PSh\Phi\Phi}$ couplings can grow rapidly and produce large BSM contributions to $\kappa_\lambda$. It should be emphasised that these loop effects involving BSM scalars and $g_{\PSh\PSh\Phi\Phi}$ couplings are not a perturbation of the tree-level trilinear Higgs coupling, but rather a new class of contributions only entering at the loop level. They can therefore become larger than the tree-level contribution, without being associated with a violation of perturbativity (this situation is analogous to that of loop-induced processes like e.g.\ $\PSh\to\PGg\PGg$ or $\PSh\to\PGg\PZ$). 

\begin{figure} 
{ \includegraphics[width=.47\textwidth]{./figs/Hself/benchmark_mAvskappalam.pdf}}
~~~{ \includegraphics[width=.45\textwidth]{./figs/Hself/benchmark_plane_2L.pdf}} 
{\caption{(Left) One- and two-loop predictions for $\kappa_\lambda$ as a function of $m_A=m_{H^\pm}$ in an aligned 2HDM scenario of Yukawa type I (see footnote~\ref{footnote:alignmentlimit}). The other BSM input parameters are chosen to be $M=m_H=\SI{600}{\giga\electronvolt}$ and $t_\beta=2$. 
(Right) Contour lines of $\kappa_\lambda$ (red) and $c_\text{eff}$ (blue), computed at two loops, in the $\{\mu_S,m_S\}$ parameter plane of the $Z_2$-SSM (with $\lambda_S=0$). The orange solid and dashed lines indicate the regions of parameter space probed by single-Higgs measurements at the HL-LHC (assuming SM-like central values) at the $1\sigma$ and $2\sigma$ levels respectively. 
}\label{fig:benchmark_masssplittingeffects}}
\end{figure}

The left panel of \cref{fig:benchmark_masssplittingeffects} presents an example of mass-splitting effects in $\kappa_\lambda$ up to the two-loop level in an aligned 2HDM~\cite{Bahl:2022jnx}. 
For the scenario we consider,\footnote{We refer the reader to Ref.~\cite{Braathen:2019zoh,Bahl:2022jnx} for details on our choices of conventions and notations for the CP-conserving 2HDM. $M$ is the BSM mass scale of the 2HDM (corresponding to the generic $\mathcal{M}$), $m_H,\ m_A,\ m_{H^\pm}$ are the masses of the BSM scalars, and $\alpha$ and $\beta$ are respectively the mixing angles in the CP-even sector and in the CP-odd and charged sectors. The alignment limit~\cite{Gunion:2002zf} means that the EW vacuum expectation value is aligned in field space with the detected Higgs boson $\PH$ of mass 125 GeV, and corresponds to $\alpha=\beta-\pi/2$ in terms of mixing angles. As a consequence of this limit, all couplings of $\PH$ are SM-like at the tree level. \label{footnote:alignmentlimit}} with $M=m_H=\SI{600}{\giga\electronvolt}$, $m_A=m_{H^\pm}$ and $\tan\beta=2$, all relevant theoretical and experimental constraints have been verified. We find that the comparison of the two-loop prediction for $\kappa_\lambda$ with recent experimental bounds on this coupling modifier~\cite{ATLAS:2022jtk} at the LHC allows excluding significant parts of the otherwise unconstrained parameter space of the model; in this specific scenario, the mass range $m_A=m_{H^\pm}\gtrsim \SI{900}{\giga\electronvolt}$ (or equivalently mass splittings $m_A-m_H\gtrsim\SI{300}{\giga\electronvolt}$) would lead to the two-loop prediction for $\kappa_\lambda$ to be larger than 7.2~\cite{ATLAS:2024ish} %, $\kappa_\lambda^{(2)}>6.3$ 
and is therefore excluded (while perturbative unitarity would only exclude $m_A=m_{H^\pm}\gtrsim \SI{1020}{\giga\electronvolt}$). Additionally, the mass range $m_A=m_{H^\pm}\gtrsim\SI{800}{\giga\electronvolt}$ of this scenario would be probed at the HL-LHC, as indicated in purple in the left panel of \cref{fig:benchmark_masssplittingeffects}. % The considered benchmark scenarios are defined in the figure caption as well as Refs.~\cite{Bahl:2022jnx,Bahl:2023eau}. 
%
Importantly, the mass-splitting effects shown in that same figure %\cref{fig:benchmark_masssplittingeffects} 
and the exclusions obtained with current LHC data, or expected with future colliders, are not restricted to the 2HDM, but have been found to occur in various BSM theories with additional scalars -- as can now be studied with the public tool \texttt{anyH3}~\cite{Bahl:2023eau}. 

% power counting arguments
%The occurrence of large radiative corrections in $\lambda_{\PH\PH\PH}$ raises the questions of how sizeable higher-order corrections to other Higgs properties involving $g_{\PH\PH\Phi\Phi}$ couplings can become, and where one would first observe a deviation from the SM predictions in these types of scenarios. Power counting arguments~\cite{Bahl:2024xyz} show that, in the limit of large $g_{\PH\PH\Phi\Phi}$ couplings, the leading one-loop BSM contributions to the trilinear Higgs coupling are of $\mathcal{O}(g_{\PH\PH\Phi\Phi}^2)$, while those in single Higgs couplings grow at most linearly with $g_{\PH\PH\Phi\Phi}$. 
%Arguments from the point of view of effective field theories leading to similar conclusions on the relative magnitudes of BSM deviations in trilinear and single Higgs couplings can be found in~\cite{Durieux:2022hbu}. 

The occurrence of large radiative corrections in $\lambda_{\PSh\PSh\PSh}$ raises the questions of how sizeable higher-order corrections to other Higgs properties involving $g_{\PSh\PSh\Phi\Phi}$ couplings can become, and where one would first observe a deviation from the SM predictions in these types of scenarios. Power counting arguments~\cite{Bahl:2024xyz} show that, in the limit of large $g_{\PSh\PSh\Phi\Phi}$ couplings, the leading one-loop BSM contributions to the trilinear Higgs coupling are of $\mathcal{O}(g_{\PSh\PSh\Phi\Phi}^2)$, while those in single Higgs couplings grow at most linearly with $g_{\PSh\PSh\Phi\Phi}$. 
Arguments from the point of view of effective field theories leading to similar conclusions on the relative magnitudes of BSM deviations in trilinear and single Higgs couplings can be found in~\cite{Durieux:2022hbu}. 


% ------------------------------- New text: Jan 2025\\

%\begin{figure}
%{ \includegraphics[width=.47\textwidth]{./figs/Hself/Z2SSM_klam_vs_gHZZ.pdf}}
%~~~{ \includegraphics[width=.47\textwidth]{./figs/Hself/ECFA_IDM.pdf}} 
%{\caption{(Left) Scan results for the $Z_2$-SSM, shown in the plane of $\kappa_\lambda$ and $\delta g_{hZZ}$. The colour of the points indicates the order (one or two loops) at which these two quantities are computed, and is explained in the legend of the plot. The black dashed line corresponds to the expected $1\sigma$ accuracy of FCC-ee on the $\PSh\PZ\PZ$ coupling. 
%(Right) Scan results in the IDM, in the plane of $\kappa_\lambda^{(2)}$ (at two loops) and $\delta^{(1)}g_{hZZ}$ (at one loop). The points are grouped in hexagonal bins, and the colour of each of these bins represents the minimal BSM deviation among the points of the bin. The red solid line in the colour bar corresponds to the expected $1\sigma$ accuracy of FCC-ee on $\PSh\to\upgamma\upgamma$~\cite{FCCICHEP:2024}, while the horizontal and vertical lines are described in the legend and the text. 
%}\label{fig:benchmark_Z2SSM_scatter_IDM}}
%\end{figure}

%As a simple but illustrative example, we consider the $Z_2$-SSM,\footnote{We refer the reader to, e.g., Ref.~\cite{Braathen:2020vwo} for an overview of the notations and conventions we employ in this work (we consider here the $N=1$ case of the $O(N)$-symmetric SSM of Ref.~\cite{Braathen:2020vwo}).} i.e.\ a real-singlet extension of the SM with an unbroken global $Z_2$ symmetry. Due to this symmetry, the BSM scalar $S$ does not mix with the detected Higgs boson at 125 GeV. Its mass takes the form $m_S^2=\mu_S^2+\lambda_{H\Phi}v^2$ where $\mu_S$ is the singlet Lagrangian mass term and $\lambda_{H\Phi}$ the portal quartic coupling between the singlet and the (SM-like) doublet. The coupling $\lambda_{H\Phi}$ plays in the $Z_2$-SSM the exact role of the generic $g_{\PSh\PSh\Phi\Phi}$ coupling in the discussion in the previous section. In this model, single-Higgs couplings $g_{\PSh XX}$, where $X$ can be a gauge boson or fermion, only receive BSM contributions via external-leg corrections --- there are no mixing effects, and moreover vertex-type corrections do not appear because of the singlet nature of the BSM scalar and the unbroken $Z_2$ symmetry. This allows obtaining compact expressions for the single-Higgs coupling modifier $c_\text{eff}\equiv g_{\PSh XX}/g_{\PSh XX}^\text{SM}$ at one and two loops~\cite{Bahl:2024xyz}. 
%In the left panel of \cref{fig:benchmark_Z2SSM_scatter_IDM}, we present parameter scan results for the $Z_2$-SSM, in the plane of $\kappa_\lambda$ and the BSM deviation in the $g_{\PSh\PZ\PZ}$ coupling, $\delta g_{\PSh\PZ\PZ}$, calculated at the one- and two-loop level. One can see that large shifts in $\kappa_\lambda$ are possible, e.g.\ at two loops up to $\kappa_\lambda^{(2)} \approx 3 (2)$ for the case where one-loop (two-loop) corrections to the $g_{\PSh\PZ\PZ}$ coupling are taken into account, while the effect in $g_{\PSh\PZ\PZ}$ is below the $1\,\sigma$ sensitivity of the FCC-ee (derived from Ref.~\cite{FCCICHEP:2024}). 

%As a second example, we perform a parameter scan in the Inert Doublet Model (IDM), a variant of the 2HDM in which the second doublet is charged under an unbroken $\mathbb{Z}_2$ symmetry --- we refer the reader to e.g. Refs.~\cite{Deshpande:1977rw,Barbieri:2006dq,Braathen:2019zoh,Aiko:2023nqj} for an overview of the model. Similarly to the case of the $Z_2$-SSM, the masses of the BSM scalars $\Phi=H,\ A,\ H^\pm$ of the IDM take the form $m_\Phi^2=\mu_2^2 +\lambda_\Phi v^2$, with $\lambda_\Phi$ some combination of the Lagrangian quartic couplings and $\mu_2$ the BSM mass scale of the IDM. However, to the difference of the previous model, single Higgs couplings receive in the IDM genuine BSM vertex corrections, which we have here evaluated consistently at the one-loop level (with also leading two-loop corrections from Ref.~\cite{Aiko:2023nqj} included for the partial decay width of the Higgs to two photons).

%Our scan results in the IDM are shown in the right panel of ~\cref{fig:benchmark_Z2SSM_scatter_IDM}, with two-loop predictions for $\kappa_\lambda$ (from Refs.~\cite{Braathen:2019pxr,Braathen:2019zoh,Aiko:2023nqj}) on the horizontal axis and the one-loop BSM deviation in the $g_{\PSh\PZ\PZ}$ coupling on the vertical axis. For the latter, BSM vertex and external-leg corrections are included, with vanishing external momenta in order to obtain a quantity corresponding to $\kappa_Z$~\cite{LHCHiggsCrossSectionWorkingGroup:2012nn, LHCHiggsCrossSectionWorkingGroup:2013rie}. The colour of the hexagonal bins corresponds to the minimal BSM deviation in the Higgs partial decay width to two photons, evaluated at two loops, among the points within the bin --- this additional observable is relevant for the IDM, due to the presence of a charged BSM Higgs boson in the model. Vertical blue lines correspond to $20\%$ (dot-dashed) and $50\%$ (dotted) levels of accuracy on the determination of $\lambda_{\PH\PH\PH}$~(taking $\kappa_\lambda = 1$ as central value), while the red dotted horizontal corresponds to the $1\sigma$ precision expected for $g_{\PSh\PZ\PZ}$ at FCC-ee. Interestingly, we observe that a significant population of our scan points exhibit significant BSM deviations in $\kappa_\lambda$, with values up to $\kappa_\lambda\sim 2.8$, while maintaining $\delta^{(1)}g_{\PSh\PZ\PZ}$ below the $1\sigma$ line of FCC-ee. Meanwhile, for the majority of these points a measurement of $\Gamma(h\to\gamma\gamma)$ at the FCC-ee would also remain compatible with the SM up to the $1.5\sigma$ level. Finally, we have checked the impact of including both momentum dependence, as well as diagrams with an insertion of the modified value of $\kappa_\lambda$ (while these are formally of two-loop order, the question of their size becomes relevant for large $\kappa_\lambda$)  in the calculation of the $g_{\PSh\PZ\PZ}$ coupling. Importantly, we find for our IDM scan points that both effects lead overall to a reduction of the BSM deviation in $g_{\PSh\PZ\PZ}$ --- in other words, the results shown in the right panel of \cref{fig:benchmark_Z2SSM_scatter_IDM} constitute a conservative representation of the possible deviations in $\kappa_\lambda$ possible for IDM scenarios with BSM effects in $g_{\PSh\PZ\PZ}$ below the $1\sigma$ sensitivity of the FCC-ee. 

%------------------------------- New text: Jan 2025\\

%---------------------------------------OLD TEXT\\

As a simple but illustrative example, we consider the $Z_2$-SSM,\footnote{We refer the reader to e.g.\ Ref.~\cite{Braathen:2020vwo} for an overview of the notations and conventions we employ in this work (we consider here the $N=1$ case of the $O(N)$-symmetric SSM of Ref.~\cite{Braathen:2020vwo}).} i.e.\ a real-singlet extension of the SM with an unbroken global $Z_2$ symmetry. Due to this symmetry, the BSM scalar $S$ does not mix with the detected Higgs boson at 125 GeV. Its mass takes the form $m_S^2=\mu_S^2+\lambda_{\PSh\Phi}v^2$ where $\mu_S$ is the singlet Lagrangian mass term and $\lambda_{\PSh\Phi}$ the portal quartic coupling between the singlet and the (SM-like) doublet. The coupling $\lambda_{\PSh\Phi}$ plays in the $Z_2$-SSM the exact role of the generic $g_{\PSh\PSh\Phi\Phi}$ coupling in the discussion in the previous section. In this model, single-Higgs couplings $g_{\PSh XX}$, where $X$ can be a gauge boson or fermion, only receive BSM contributions via external-leg corrections --- there are no mixing effects at the tree level, and moreover vertex-type corrections do not appear because of the singlet nature of the BSM scalar and the unbroken $Z_2$ symmetry.  
% define ceff -> OK
This allows obtaining compact expressions for the single-Higgs coupling modifier $c_\text{eff}\equiv g_{\PSh XX}/g_{\PSh XX}^\text{SM}$ at one and two loops~\cite{Bahl:2024xyz}. % While for reasons of brevity we do not reproduce the expressions here, these will be provided in~\cite{Bahl:2024xyz}. 
%
%
% describe plot
In the right panel of \cref{fig:benchmark_masssplittingeffects}, we present contour lines for $\kappa_\lambda$(red) as well as the quantity $c_\text{eff}$ (blue), both computed at the two-loop order, in the $\{\mu_S,m_S\}$ parameter plane of the $Z_2$-SSM. As a conservative choice, we fix $\lambda_S=0$ in the plane; this cancels the effects from two-loop terms involving $\lambda_S$ in $\kappa_\lambda$ and $c_\text{eff}$ (we note that for these contributions, like for those involving only $g_{\PSh\PSh\Phi\Phi}$ couplings, the effects in $\kappa_\lambda$ have a higher scaling in powers of $\lambda_{\PSh\Phi}$ than those in $c_\text{eff}$). We implemented the expected levels of accuracy on single-Higgs couplings at the HL-LHC as ``measurements'' (assuming SM-like central values) in \texttt{HiggsSignals}~\cite{Bahl:2022igd}, and orange lines in \cref{fig:benchmark_masssplittingeffects} correspond respectively to the $1\sigma$ (solid) and $2\sigma$ (dashed) exclusion ranges from HL-LHC measurements. 

Comparing the contour lines for $\kappa_\lambda$ and $c_\text{eff}$ provides information about the regions of the $Z_2$-SSM parameter space for which measurements of the trilinear and single Higgs couplings, respectively, would have sensitivity. 
%ext-leg corrections in Z2SSM->indep of kinematics, so no info on BSM from differential measurements, etc. (same info in SM and BSM from differential information)
It is interesting to note that because in the $Z_2$-SSM BSM effects only enter single-Higgs couplings via (diagonal) external-leg corrections, they have no impact on the kinematics of the various processes that can be measured at $\Pep\Pem$ colliders (like, e.g.,  $\Pep\Pem\to\PZ\PSh$), so that differential measurements of such processes would not help to distinguish the $Z_2$-SSM from the SM. 
As can be observed from comparing the uppermost red and blue contour lines in the right panel of \cref{fig:benchmark_masssplittingeffects}, a measurement of $\lambda_{\PSh\PSh\PSh}$ to the $50\%$ accuracy level would probe a larger region of the parameter space of the $Z_2$-SSM (above the $\kappa_\lambda=1.5$ line) than measurements of single-Higgs couplings to the $0.5\%$ level (which would offer sensitivity to the region above the $c_\text{eff}=0.995$ line). Furthermore, compared with measurements of single Higgs couplings to $0.3\%$ 
%--- which is comparable to the expected accuracy on the $g_{\PH\PZ\PZ}$ coupling at low-energy Higgs factories ~\cite{Fujii:2017vwa,Bernardi:2024ecfa}
%the ILC~\cite{Fujii:2017vwa} or FCC-ee~\cite{Bernardi:2024ecfa} 
%--- 
a precision of 20\% on $\lambda_{\PSh\PSh\PSh}$ would be competitive for $\mu_S\gtrsim\SI{200}{\giga\electronvolt}$ or even more sensitive for $\mu_S\gtrsim\SI{300}{\giga\electronvolt}$. 
As we discuss next, such precision in $\lambda_{\PSh\PSh\PSh}$ is within the reach of future
\epem colliders operating at CM energies around \SI{500}{\giga\electronvolt}.

%------------------------------------OLD TEXT: END\\

%-----------------------------------------------


\subsubsection{\texorpdfstring{Progress in Higgs-pair production at $\epem$ colliders}{Progress in Higgs-pair production at e+ e- colliders}\label{sec:HHprod}}

Double Higgs production at $\Pep\Pem$ colliders with centre-of-mass energies $\sqrt{s} \geq$ \SI{500}{\giga\electronvolt} comprises both di-Higgs production from $\PW\PW$ fusion, $\PGn\PAGn\PH\PH$, dominant at centre-of-mass energies above \SI{1}{\tera\electronvolt}, as well as double Higgs-strahlung, $\PZ\PH\PH$, dominant at lower centre-of-mass energies. Both processes have been studied about $10$ years ago in detailed, Geant4-based simulation of the ILD detector concept, considering the $\PH\PH \rightarrow  4\PQb$~\cite{Durig:2016jrs, Tian:2013} and $\PH\PH \rightarrow \PQb\PAQb\PW\PW^*$~\cite{Kurata:2013} final states.
For the SM value of the tri-linear Higgs self-coupling $\lambda_{\PH\PH\PH}$, the combination of the two channels yielded precisions of \SI{27}{\%} at \SI{500}{\giga\electronvolt} and \SI{10}{\%} when combining both centre-of-mass energies. A few years later, CLICdp studied the prospects at $\sqrt{s}=$\SI{1.4}{\tera\electronvolt} and \SI{3}{\tera\electronvolt}~\cite{Roloff:2019crr}, also in detailed, Geant4-based simulation, reaching precisions down to \SI{8}{\%}, again assuming the SM value of $\lambda_{\PH\PH\PH}$. It should be noted that in particular for the $\PZ\PH\PH$  process, i.e.\ the measurements at around \SI{500}{\giga\electronvolt}, it has been shown explicitly that all other parameters entering the interpretation of the $\PZ\PH\PH$  cross-section will be determined sufficiently precise at a Higgs factory so that their impact on the extraction of $\lambda_{\PH\PH\PH}$ is negligible~\cite{Barklow:2017awn}.

%\section{Update of the ILD Di-Higgs Analysis}

The  analysis of \PZ\PH\PH production at \SI{500}{\giga\electronvolt} is being updated in detailed simulations of the ILD detector concept, covering the \PH\PH $\rightarrow$ \PQb\PAQb \PQb\PAQb and \PZ $\rightarrow$ \PQq\PAQq / \Pep\Pem / \PGmp\PGmm / \PGn\PAGn channels. While a full new analysis is ongoing, several key ingredients of the analysis have been updated to more modern analysis tools based on the MC production for the ILD Interim Design Report~\cite{ILDConceptGroup:2020sfq}. This concerns in particular the jet-flavour tagging, for which by an update from LCFIPlus~\cite{Suehara:2015ura} to a ParticleNet-based approach~\cite{CommonReco_FT_Meyer} so far a relative increase of the \PQb -tagging efficiency of 10\% at the same level of background rejection could be achieved on 6-jet events as shown in Figure~\ref{fig:anaimprove:flav}. Since the analysis requires at least three jets to be \PQb -tagged to reject \PQt\PAQt and \PZ\PZ\PH (with \PZ $\rightarrow$ \PQc\PAQc /  \PQs\PAQs / \PQu\PAQu / \PQd\PAQd ) backgrounds, the reduced inefficiency enters to the third power. The most signal-like \PZ\PZ\PH background with at least one of the \PZ $\rightarrow$ \PQb\PAQb can only be rejected based on event kinematics. In this respect, an improvement of at least 10\% higher efficiency at same background level is expected from recent advances in correcting for semi-leptonic \PQb -decays and kinematic fitting~\cite{Einhaus:2022bnv}, as well as in using the full matrix elements for \PZ\PH\PH  and \PZ\PZ\PH. As example, Fig.~\ref{fig:anaimprove:kine} shows the improvement in the di-Higgs invariant mass reconstruction in the \PZ $\rightarrow$ \PGn\PAGn channel. For now, these two improvements will be propagated through the previous analysis~\cite{Durig:2016jrs}. In view of even significantly better flavour tagging tools reported in \cref{sec:com:flavourtagging} (see also e.g. ~\cite{Bedeschi:2022rnj, Qu:2022mxj, Suehara:2024qoc}),  
%{\color{red} (for ECFA report replace by or add cross-ref to Sec \verb$\ref{sec:com:flavourtagging}$)}, 
as well as the potential expected from using machine-learning (ML) through-out the event selection, this is a quite conservative assumption. All numbers below have been scaled to the standard ILC running scenario~\cite{Barklow:2015tja}, i.e.\ \SI{4}{\per\atto\barn} with $P(\Pem,\Pep) = (\mp 80\%, \pm 30\%)$.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{.5\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/b_vs_uds_6j_zoom_2.pdf}
        \caption{}
        \label{fig:anaimprove:flav}    
    \end{subfigure}\hfill%
    \begin{subfigure}{.5\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/b_vs_c_6j_zoom_2.pdf}
        \caption{}
        \label{fig:anaimprove:flav}    
    \end{subfigure}\hfill%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/mHH_nunu_before_2.pdf}
        \caption{}
        \label{fig:anaimprove:kine}    
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/mHH_nunu_after_2.pdf}
        \caption{}
        \label{fig:anaimprove:kine}    
    \end{subfigure}%
    \caption{Reconstruction improvements considered in the updated \PZ\PH\PH projection: (a), (b) \PQb -tagging efficiency (true positive rate) increases by about 10\% (relative) for the same background efficiency (false positive rate) at typical working points of the previous analysis (80\% \PQb -tagging efficiency with LCFIPlus) (c), (d) the resolution on the di-Higgs invariant mass improves by about a factor of two when the new semi-leptonic decay correction and kinematic fit are applied.}
    \label{fig:anaimprove}
\end{figure}

%The analysis concept follows Ref.~\cite{Durig:2016jrs}, capitalizing however on significant improvements in central high-level reconstruction tools like flavour tagging, kinematic fitting and overlay removal~\cite{Bliewert:2024} as well as on the usage of ML algorithms in the event selection. 
From this re-analysis of the channels studied in~\cite{Durig:2016jrs}, the obtained precision on the \PZ\PH\PH production cross-section improves from the \SI{21.1}{\%} obtained in~\cite{Durig:2016jrs} to now \SI{16.0}{\%} 
for the SM case. 

In combination with the \PH\PH $\rightarrow$ \PQb\PAQb \PW\PW$^*$ channel, the precision on the cross-section improves from the \SI{16.8}{\%} obtained in~\cite{Durig:2016jrs} to now \SI{12.8}{\%}, again for the SM case, while the corresponding precision on the self-coupling reduces from \SI{26.6}{\%} to \SI{20.8}{\%}. By including \PZ $\rightarrow$ \PGtp\PGtm, as well as \PH\PH $\rightarrow$ \PQb\PAQb \PGtp\PGtm and other modes well reconstructible in the \Pep\Pem environment, the expected precision on the \PZ\PH\PH cross-section improves further to \SI{11.2}{\%}, corresponding to a precision on a SM-like self-coupling value $\uplambda_{\mathrm{SM}}$ of \SI{18.1}{\%}.

One of the main limiting factors not yet addressed by novel algorithms is the jet clustering. Assuming that future developments, e.g.\ based on ML, will improve the di-jet mass resolution, we estimate that $\uplambda_{\mathrm{SM}}$ could be determined with a precision of \SI{15}{\%}. %Connected to this is the tagging of overlay particles, i.e.\ low $p_T$-hadrons from $\gamma\gamma$ interactions. Further improvements can be expected by going beyond the current treatment of overlay particles (clustering to beam jets), e.g. to multivariate or ML driven tools.

The analysis of the \PW\PW fusion production has been investigated in Refs.~\cite{Tian:2013, Kurata:2013} at a centre-of-mass energy of \SI{1}{TeV}. At \SI{500}{GeV}, the separation of the \PW\PW fusion contribution is still ongoing work and will be covered in future updates. If the \PW\PW fusion cross-section at \SI{500}{GeV} could be constrained to the level \SI{120}{\%} from the \PH\PH $\rightarrow$ \PQb\PAQb \PQb\PAQb, translating to \SI{86}{\%} in combination with the other \PH\PH decay modes. Combining the \PW\PW fusion and  \PZ\PH\PH measurement would allow to constrain the SM value of $\uplambda_{\mathrm{SM}}$ to a precision of \SI{17}{\%} with current tools and \SI{14}{\%} when assuming improved jet clustering. 

The results summarised above have been extrapolated to other centre-of-mass energies. In particular, partial MC productions have been performed in full, Geant4-based simulation of ILD as well as using SGV~\cite{Berggren:2012ar} and centre-of-mass energies of \SI{550}{\giga\electronvolt} and \SI{600}{\giga\electronvolt}, showing that beyond the expected scaling with cross-section, both the flavour tag as well as the kinematic reconstruction profit from the higher boost of the produced bosons. This is true in particular for the jet clustering, which benefits from less confusion towards higher COM energies \cite{Torndal:2023mmr}.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{.5\textwidth}
    \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/HHH_ECM_Combined_new.pdf}
        \caption{}
        \label{fig:lambda:ZHH_WWfusion}    
    \end{subfigure}\hfill%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{figs/Hself/dkala_abs_vs_kala_ILC550_ECFA25.pdf}
        \caption{}
        \label{fig:lambda:BSM}    
    \end{subfigure}%
    \caption{Projected precisions on the tri-linear Higgs self-coupling $\lambda_{\PH\PH\PH}$ for double Higgs-strahlung, di-Higgs production from $\PW\PW$ fusion and their combination: (a) relative precision as a function of the centre-of-mass energy and (b) absolute uncertainty on $kappa_{\lambda}$ as a function of $kappa_{\lambda}$. }
    \label{fig:lambda}
\end{figure}

\Cref{fig:lambda:ZHH_WWfusion} shows the resulting evolution of the expected precision on $\uplambda$ with the centre-of-mass energy, for both production modes separately and for their combination. For instance at $\sqrt{s}=$\SI{550}{\giga\electronvolt}, the envisioned energy for C$^3$ as well as for a Linear Collider Facility at CERN, the expected combined precision on $\uplambda_{\mathrm{SM}}$ is \SI{15}{\%}, a substantial improvement over the \SI{26.6}{\%} of~\cite{Durig:2016jrs}.


Enlarging the scope to the BSM case, it is important to note that the two production modes play very complementary roles due to their very different interference patterns. This is illustrated in \cref{fig:lambda:BSM}, which shows the behaviour of the expected precision as a function of $\lambda_{\PH\PH\PH}/\lambda_{\PH\PH\PH}^{\mathrm{SM}}$ for the two production modes at $\sqrt{s}=$\SI{550}{\giga\electronvolt}, as well at $\sqrt{s}=$\SI{1}{\tera\electronvolt}. This shows that measurements of $\PZ\PH\PH$  production at centre-of-mass energies around \SI{500}{\giga\electronvolt} play a crucial role in pinning down the BSM behaviour of the tri-linear Higgs self-coupling.
Furthermore, as we discuss in the next subsection, these types of measurements could also bring sensitivity to new contributions coming from genuine BSM triple Higgs couplings.

%-----------------------------------------------


%------------------------------------------------------------------------
\subsubsection{\texorpdfstring{BSM triple Higgs couplings in double Higgs production at $\epem$ Colliders}{BSM Triple Higgs Couplings in double Higgs production at e+e- Colliders}}\label{sec:BSMHhh}

{\bf\color{blue} Notation for light Higgs here is inconsistent with the rest. This section, however, would be better in searched as it is not SM Higgs selfcoupling, but rather using HH production for BSM Higgses. I suggest moving this to section 8.2.5 inside the "Exotic Scalar Searches/Searhces in other production channels".}

In this section we investigate the impact of one-loop corrections to the triple Higgs couplings (THCs)
on di-Higgs production in models with 
extended Higgs sectors at high-energy $\epem$ colliders, and explore the experimental sensitivity to such (BSM) THCs.
We work in the framework of the CP-conserving 2-Higgs doublet model (2HDM)~\cite{Branco:2011iw} and 
focus on the double Higgs-strahlung process, \ie $\epem\to \PSh\PSh\PZ$, with $\PSh$ being the 
Higgs boson discovered at the LHC.  
The process involves two THCs, which are the $\PSh$ self-coupling $\lambda_{\PSh\PSh\PSh}$ (or alternatively its ratio to
the SM prediction,  $\kappa_\lambda$), and the coupling $\lambda_{\PSh\PSh\PH}$, which enters through a resonant diagram mediated by 
the heavy Higgs boson $\PH$. 

Our calculation captures the leading EW corrections by including the predictions of the involved THCs at the one-loop
level, which can become very large in the 2HDM as has been shown in \cite{Kanemura:2002vm}.
We compute the one-loop corrections to $\lambda_{\PSh\PSh\PSh}$ and $\lambda_{\PSh\PSh\PH}$ using the Coleman-Weinberg effective potential, as implemented in the code \texttt{BSMPT}~\cite{Basler:2018cwe,Basler:2020nrq,Basler:2024aaf}.
We furthermore compare our results to those of a fully diagrammatic computation of the one-loop corrections to $\lambda_{\PSh\PSh\PSh}$ using the code \texttt{anyH3}~\cite{Bahl:2023eau}.
This allows us to estimate the importance of the finite-momentum effects in the one-loop corrections to $\lambda_{\PSh\PSh\PH}$.


To summarize the (preliminary) results of our work, we focus on a particular point in the 2HDM %, named BP1, 
with the following input parameters:
$
    m_{\PH}=\bar m = 300\ \GeV,\  m_{\PSA} = m_{\PSHpm}=650\ \GeV,\  \tan\beta=12,\  c_{\beta-\alpha}=0.12,
$
where we follow the same notation for the 2HDM input parameters as in~\cite{Arco:2020ucn}.
This point is allowed by the present constraints as described in~\cite{Muhlleitner:2020wwk}.
This leads to the following tree-level and one-loop THCs:
$
    \kappa_{\lambda}^{(0)} = 0.95,\ \kappa_{\lambda}^{(1)} = 4.69, \ \lambda_{\PSh\PSh\PH}^{(0)} = 0.02, \ \lambda_{\PSh\PSh\PH}^{(1)} = 0.21,
$
as given by the effective potential computation.

\Cref{fig:BP1} shows the differential distribution of the cross section w.r.t.\ the 
invariant di-Higgs mass $m_{\PSh\PSh}$ for the above input parameters.
The blue lines include the one-loop values of $\kappa_{\lambda}$ and $\lambda_{\PSh\PSh\PH}$ from the effective potential, the dashed red lines include the fully diagrammatic prediction for $\kappa_{\lambda}^{(1)}$, the yellow lines show the 2HDM tree-level prediction and the dotted black lines show the SM tree-level prediction.
Our cross section predictions are obtained with the tree-level formulas of~\cite{Djouadi:1999gv,Muhlleitner:2000jj} (adapted to the 2HDM), including the one-loop corrected THCs.
The right axis of the plots shows the expected final 4$\PQb$-jet events $\bar N_{4\PQb\PZ}$ after applying detection cuts as described in \cite{Arco:2021bvf}.
We assume the projected ILC operating scenario with a centre-of-mass energy of $\sqrt{s}=500\ \GeV$
~\cite{Barklow:2015tja} with an integrated luminosity of 1.6\ \abinv and a beam polarization of 
$P_{e^-} = -80\%$ and $P_{e^+} = +30\%$.
We furthermore include an experimental uncertainty due to the future detector resolution by implementing a Gaussian smearing in the cross section distributions, as described in \cite{Arco:2022lai}. 
The upper left, upper right, lower left and lower right plot assumes no uncertainty and a 2\%, 5\% and 10\% uncertainty, respectively.


First we comment on the one-loop effects of $\kappa_{\lambda}$.
The tree-level prediction yields a prediction very close to the SM value, since we are very close to the alignment limit ($c_{\beta-\alpha}=0$).
On the contrary, the large one-loop corrections for $\kappa_{\lambda}$ lead to an enhancement of the non-resonant contributions to the cross section, due to the constructive interference of the $\lambda_{\PSh\PSh\PSh}$ diagram with the other non-resonant contributions.
These large values of $\lambda_{\PSh\PSh\PSh}$ at the one-loop level can be realized in the 2HDM (and in other models with extended Higgs sectors) with heavy Higgs bosons with a mass splitting between them.
We can also conclude that the finite-momentum effects in the one-loop corrections to $\kappa_{\lambda}$, see the red dashed line,
are minor, since they imply only a 5\% deviation in the total cross section prediction.
Therefore, the use of one-loop corrected THCs obtained from the effective potential provides a good approximation for the one-loop scalar corrections to the di-Higgs production.

We now turn to the effect of the one-loop corrections of $\lambda_{\PSh\PSh\PH}$, which enters the cross section 
through a resonant diagram mediated by the heavy Higgs boson $\PH$.
For our benchmark point, the resonance peak is expected at $m_{\PSh\PSh} = m_{\PH} = 300\ \GeV$, as it can be seen in all plots in \cref{fig:BP1}.
As an estimate of the relevance of the $\PH$ resonance peak, and therefore the possible access to the coupling $\lambda_{\PSh\PSh\PH}$, we compute the statistical significance $Z$ of the resonance peak.
We perform a profile likelihood ratio test between the no-resonance hypothesis (\ie with $\lambda_{\PSh\PSh\PH}=0$, corresponding to the dot-dashed lines in \cref{fig:BP1}) and the complete prediction with the $\PH$ peak, as described in~\cite{Cowan:2010js}.
For our considered point, the statistical significances containing the one-loop corrected THCs, $Z^{(1)}$, are larger than the ones from the tree-level distributions, $Z^{(0)}$. Both values are given in each plot.
This is due to the fact that for our benchmark point the tree-level prediction for $\lambda_{\PSh\PSh\PH}$ is very close to zero, while the one-loop correction increases the value of this coupling to a much larger value of 0.2, which makes the $\PH$ resonance peak more prominent.

We also find that the smearing of the cross section distributions has a relevant effect on the significance of the $\PH$ resonance peak.
A large experimental uncertainty in the cross section distributions (or in other words, large smearing values) makes the $\PH$ resonance peak less prominent and sharp, leading to a smaller significance, as can be inferred from the given $Z$ values.
We therefore conclude that the experimental resolution of the $m_{\PSh\PSh}$ distributions will be crucial for the determination of $\lambda_{\PSh\PSh\PH}$ from the $\PH$ resonance peak.
 
In conclusion, our study shows that one-loop corrections to THCs in models with extended Higgs sectors significantly affect the di-Higgs production cross section. 
These corrections can lead to a substantial enhancement of the cross section, even in the alignment limit. Therefore, it is crucial to include them in any accurate phenomenological analysis.

Finally, we provide a list of some open questions that should be addressed in future work:
1) How relevant can the remaining one-loop corrections be for the $\PSh\PSh$ production, especially from the $\PH\PZ\PZ$ vertex?
2) What is the expected experimental resolution on the $m_{\PSh\PSh}$ distributions?
3) What would be the effect of the experimental backgrounds and how would this affect the access to the BSM THCs?
4) How relevant could the finite momentum effects be for the loop-corrected $\lambda_{\PSh\PSh\PH}$ coupling?

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{./figs/Hself/plotinvmass-BPlahhH-1-sqrts500-HwidthNLO-smeared.pdf}
        \caption{Differential distribution of the cross section w.r.t.~to $m_{\PSh\PSh}$ for the considered input parameters at $\sqrt{s}=500\ \GeV$ for different smearing assumptions. }
    \label{fig:BP1}
\end{figure}

%-----------------------------------------------

\subsubsection{\texorpdfstring{Higgs self-coupling in single-Higgs processes: $\epem \to \PZ\PH$ at NLO in the SMEFT}{e+ e- -> ZH at NLO in the SMEFT}}\label{sec:eeZH_NLO}

We conclude this section discussing the progress on the theory side regarding the determination of $\lambda_{\PH\PH\PH}$ from single Higgs measurements, in particular in the context of EFT studies
of new physics. 
As mentioned above, sensitivity to the Higgs self-coupling in single Higgs processes comes from one-loop level contributions. The full structure of these NLO contributions depends on the particular theory framework used to interpret the measurements. Within the SMEFT framework, the full set of contributions from dimension-six operators to the main Higgs production mechanism at low-energy Higgs factories, $\epem \to \PZ\PH$, has recently been computed, first for operators involving the top quark~\cite{Asteriadis:2024qim} and then to the whole dimension-six basis~\cite{Asteriadis:2024xts}. A sample of such contributions is shown in \cref{fig:1loop}. From the point of view of the $\lambda_{\PH\PH\PH}$ SMEFT interpretation, 
these calculations open the possibility of extending previous studies in the direction of a model-independent interpretation within the assumptions of this EFT, see \cref{sec:globalSMEFT}.~\footnote{To achieve this, calculations of the NLO effects in other processes relevant for Higgs physics at $\epem$ are still missing, e.g.\ $\epem\to \nu\bar{\nu} \PH$ (via $W$ boson fusion).}

\begin{figure}
    \centering
    \includegraphics[height=69pt]{./figs/Hself/triag1.pdf}
    \includegraphics[height=69pt]{./figs/Hself/triag2.pdf}
    \includegraphics[height=69pt]{./figs/Hself/triag3.pdf}\\[8pt]
    \includegraphics[height=69pt]{./figs/Hself/box3.pdf}
    \includegraphics[height=69pt]{./figs/Hself/box2.pdf}
    \includegraphics[height=69pt]{./figs/Hself/box4.pdf}\\[8pt]
    \includegraphics[height=69pt]{./figs/Hself/4point1.pdf}
    \includegraphics[height=69pt]{./figs/Hself/4point2.pdf}
    \includegraphics[height=69pt]{./figs/Hself/4point3.pdf}
    \caption{
    %Sample virtual diagrams contributing to $\epem\rightarrow HZ$ at NLO in the dimension-6 SMEFT. We show contributions with one-loop vertex corrections (first row), planar and non-planar box diagrams (second row), and contributions with 4-point interactions (third row).
    }
    \caption{Example of 1-loop diagrams for contributions to the $\epem \to ZH$ cross section in the SMEFT.}\label{fig:1loop}
\end{figure}

Aside from the operators entering at LO, there are a total of 6 bosonic (4 of them CP violating), 9 two-fermion and 14 four-fermion dimension-six operators that contribute to $\epem \to \PZ\PH$ at NLO.
Of particular importance are the contributions of the top-quark operator mentioned before, e.g. $\epem \PQt\PAQt$ contact interactions, which are currently poorly constrained. 
In this regard, and as in the case of the contributions from the Higgs self-coupling, 
considering modifications to top-quark interactions entering in other loop contributions to $\epem\to \PZ\PH$, runs at two centre-of-mass energies also provide complementary sensitivity and tight two-parameter constraints~\cite{Asteriadis:2024qim}, as shown in \cref{fig:top-operators}. 
Similarly, polarized beams can provide complementary information on different corrections, and help to separate the contributions of the Higgs self-coupling operator from those from top operators, as shown, e.g. in \cref{fig:top-operators-2}.


\begin{figure}[t]\centering
\includegraphics[width=0.35\textwidth]{./figs/Hself/CH_eu_1133}%
~~~~~~~~~~~~~~~~~~\includegraphics[width=0.35\textwidth]{./figs/Hself/CH_Cth}%
\caption{Left: Joint constraints on the trilinear Higgs self-coupling ($x$ axis) and on right-handed $\bar{e}e\bar{t}t$ operator ($y$ axis) from LEP, as well as \SI{240} and \SI{365}{\giga\electronvolt} runs.
Right: Similarly for the top-quark Yukawa operator ($y$ axis).
Figures reproduced from~\cite{Asteriadis:2024xts}.
}
\label{fig:top-operators}
\end{figure}
%
\begin{figure}[h]\centering
\includegraphics[width=0.35\textwidth]{./figs/Hself/Cfu33_Cphi}%
~~~~~~~~~~~~~~~~~~\includegraphics[width=0.35\textwidth]{./figs/Hself/Clq11133_Cphi}%
\caption{Left: contributions from modifications of the Higgs tri-linear coupling operator ($x$ axis) on the cross section $e^+ e^- \to \PSZ\PH$ at \SI{240}{\giga\electronvolt}, correlated with those from $C_{\phi u}[3,3]$, which modify the $Zt\bar{t}$ vertex, and depending on the polarization of the $e^+ e^-$ system. Right: the same the $\epem \PQt\PAQt$ operator with coefficient $C_{lq}^{(1)}[1,1,3,3]$ ($y$ axis).
Figures reproduced from~\cite{Asteriadis:2024qim}.
}
\label{fig:top-operators-2}
\end{figure}


%In a global study, these new NLO effects show that, in the single-Higgs analysis at NLO there would be a considerable amount of degeneracy.
The large number of different interactions entering at NLO would suggest that in the single-Higgs analysis at NLO there %would 
will be a considerable amount of degeneracy. 
%Thus, with 
With more operators simultaneously included, more observables would need to be combined to constrain all directions 
in a global fit
and single out the potential new contributions to $\lambda_{\PH\PH\PH}$. 
%
In Higgsstrahlung production itself, angular distributions and radiative return to lower effective centre-of-mass energies could for instance be considered~\cite{talkecfa}.
%
Outside Higgs physics, the above-mentioned top interactions could be tested at the tree level in $\epem \to \PQt\PAQt$ at \SI{350}-\SI{365}{\giga\electronvolt}. Finally, some of the same top operators enter in Z-pole observables also at the loop-level, and a combined analysis exploiting the extreme high precision of the Tera-Z run could also help in a global analysis. 
The determination 
of $\lambda_{\PH\PH\PH}$ thus relies on %: (1) 
having precision measurements of a large enough number of observables to constrain any possible BSM effects in other contributions that enter in the calculations of the observables to the same order in perturbation theory as the leading contributions of $\lambda_{\PH\PH\PH}$.
%; (2) the precision of theory calculations and measurements of the inputs of the SM.\textbf{[JB: Already taken shown to have small effect]}
%

There is currently an ongoing effort to extend the $\lambda_{\PH\PH\PH}$ EFT determination from single-Higgs measurements, including these recent NLO effects, and other aspects related to this EFT interpretation. These are discussed in \cref{sec:HprodH3}.


\subsubsection{Single-Higgs processes as probes of the Higgs self-coupling\label{sec:HprodH3}}
%\subsubsection{Progress in single-Higgs approach}
%\noindent Degeneracies at NLO SMEFT in $\PZ\PH$\\
%\noindent Differential cross-section measurements\\
%\noindent Results from New Global SMEFT Fit

% Extended SMEFT fit
% Determination of klambda different than SM (not in SMEFT)

\textbf{[Results are hopefully available in January 2025, and discussed here]}. 
%------------------------------------------------------------------------





==> sections/higgs/htautau.tex <==
\subsubsection*{Introduction}

A cornerstone of the FCC-ee program is the investigation of Higgs boson properties \cite{FCC:2018byv}, mainly in the \SI{240}{\giga\electronvolt} operation stage with an integrated luminosity of $\mathcal{L}_{int}$=\SI{10.8}{\per\atto\barn}.
The $\PH\to\PGtp\PGtm$ process, in particular, benefits from the clean collision environment and can be measured with excellent precision. 
This study explores the prospective sensitivity of the $\Pep\Pem\to\zhsm$, $\PH\to\PGtp\PGtm$ cross section measurement at FCC-ee.
The CP property of the $\PH\PGt\PGt$ coupling also falls into the scope of interest of this study. 

\subsubsection*{Cross-section measurement}

Both signal and background processes have been simulated in the Monte Carlo event generator for high-energy physics \Whizard v. 3.0.3 \cite{Kilian:2007gr,Moretti:2001zz} with a parameterization of initial state radiation. Subsequently, Pythia6 \cite{Sjostrand:2006za} was used to handle hadronisation as well as tau decays, and Delphes v. 3.5.1pre05 \cite{deFavereau:2013fsa} simulated the response of IDEA detector~\cite{IDEA1} designed for FCC-ee \cite{FCC:2018evy}.  
Jet reconstruction is handled by FastJet \cite{Cacciari:1402449} using the \epem inclusive generalized $k_t$ algorithm with the jet-radius parameter equal to $R=0.5$ and a cut on the merging scale of ${\pt}_{j}$>\SI{2}{\giga\electronvolt}. 

The algorithm used in this analysis to reconstruct taus is based on the initial individuation of jets in the event. The four-vector of the taus, along with the charge and mass, is based on the jet constituents spatially close to the leading charged pion, for jets not containing leptons. Reconstructed taus need to have a mass smaller than \SI{3}{\giga\electronvolt} and the number of charged pions and photons in the candidates is then used to infer the decay mode. 
Leptonic taus decays are identified by looking directly at the isolated leptons in the event. The visible part of the four-momentum of the Higgs boson can then be reconstructed from the taus' four-momenta.

We divide our analysis based on the decays of the \PZ ($\PZ\to\Pl\Pl$ with $\Pl=\Pe,\PGm$, $\PZ\to\PQq\PQq$ with $\PQq=\PQu, \PQd, \PQs, \PQc, \PQb$, and $\PZ\to\PGn\PGn$) and Higgs boson ($\PH\to\PGt_{\Pl}\PGt_{\Pl}$, $\PH\to\PGt_{\Pl}\PGt_h$, and $\PH\to\PGt_h\PGt_h$ where $\PGt_{\Pl}$ and $\PGt_h$ denote leptonic and hadronic tau decays). After the basic event selection to define the categories, we have optimized cuts on the reconstructed objects and event observables in each category to enhance the signal-to-background ratio. The details can be found in \cref{tab:KIT-Htautau-cuts}. 

Parallel to this cut-based event selection, we have also trained a boosted decision tree (BDT) classifier in each of the categories except for the leptonic \PZ decays.
Every BDT has a size of 200 trees and a depth of two. For $\PZ\to \PQq\PQq$ the BDT has been trained and then applied on events with \SI{100}<$M_\text{collinear}$<\SI{150}{\giga\electronvolt}, while for $\PZ\to\PGn\PGn$ the events passed the cut $E^\text{miss}$>\SI{100}{\giga\electronvolt}. \cref{fig:KIT-Htautau-ROC} shows the ROC curves for each of the trainings and an example of the BDT score.

\begin{table}[h]
\centering
    \begin{tabular}{|c|c|c|}
    \hline
    $\PZ\to\Pl\Pl$ Selection  & $\PZ\to \PQq\PQq$ Selection & $\PZ\to \PGn\PGn$ Selection \\ \hline \hline
    \multicolumn{2}{|c|}{\SI{100}<$M_\text{collinear}$<\SI{150}{\giga\electronvolt}} &  \multirow{2}{*}{$E^\text{miss}$>\SI{100}{\giga\electronvolt}}\\ 
    \cline{1-2}
    \multicolumn{2}{|c|}{\SI{115}<$M_\text{recoil}$<\SI{160}{\giga\electronvolt}} & \\ \hline
    \multicolumn{2}{|c|}{$E^\text{miss}$>\SI{10}{\giga\electronvolt}} & \multirow{2}{*}{$|\Delta\phi_{\PGt\PGt}|$<\SI{3}} \\ 
    \cline{1-2}
    \SI{70}<\mass\PZ<\SI{100}{\giga\electronvolt}\; & \SI{80}<\mass\PZ<\SI{95}{\giga\electronvolt} & \\ \hline
    \multicolumn{3}{|c|}{$\Delta R_{\PGt\PGt}$>\SI{2}} \\ \hline
    \multicolumn{3}{|c|}{$\cos\theta_{\PGt\PGt}$<\SI{0}} \\ \hline
    \multicolumn{3}{|c|}{$|\cos{\theta^\text{miss}}|$<\SI{0.98}} \\ \hline
    \end{tabular}
    \caption{Table of subsequent cuts applied on the signal and background events in each category.}
    \label{tab:KIT-Htautau-cuts}
\end{table}

\begin{figure}[h]
    \begin{subfigure}[h]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/Higgs/RecoZ_mass.pdf}
        \subcaption{$\PZ\to\Pl\Pl$, $\PH\to\PGt_{\Pl}\PGt_{\Pl}$.}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/Higgs/Recoil.pdf}
        \subcaption{$\PZ\to\Pl\Pl$, $\PH\to\PGt_{\Pl}\PGt_h$.}
    \end{subfigure}
    \begin{subfigure}[h]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/Higgs/Collinear_mass.pdf}
        \subcaption{$\PZ\to\PQq\PQq$, $\PH\to\PGt_h\PGt_h$.}
    \end{subfigure}
    \caption{Some reconstructed variables for some of the categories studied. All signal and background samples are shown, having passed the full set of cuts listed in Tab. \ref{tab:KIT-Htautau-cuts}.}
    \label{fig:KIT-Htautau-plots_ll_zmass}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[h]{0.29\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/Higgs/BDT_ROC.pdf}
    \end{subfigure}
    \begin{subfigure}[h]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/Higgs/BDT_score.pdf}
    \end{subfigure}
    \caption{ROC curves for each of the BDT trainings and corresponding AUC value in the left plot. On the right, distribution of the BDT score for $\PZ\to\PQq\PQq$, $\PH\to\PGt_h\PGt_h$.}
    \label{fig:KIT-Htautau-ROC}
\end{figure}

The cross-section measurement has been extracted with the CMS Combine tool \cite{CMS:2024onh} using binned maximum-likelihood fits. 
With the cut-based analysis, the recoil mass distribution for the $\PZ\to\Pl\Pl$ and $\PZ\to \PQq\PQq$ categories are used in the fit, while for the $\PZ\to\PGn\PGn$ category the visible mass was fitted. 
In categories where the BDT training is available, an alternative fit is also performed directly on the BDT outpus instead of the mass variables.
%We allow the yields of all processes to float without prior constrain. Statistical uncertainties in the model are handled automatically by the software using the technique Barlow-Beeston-lite \cite{Barlow:1993dm}. 
Combining all categories of \PZ and Higgs decays with the cut-based strategy, the relative uncertainty on $\sigma_{\zhsm}\times\mathcal{B}$($\PH\to\PGtp\PGtm$) is found to be $\pm$ 1.23\%. By updaing the cut-based fit results with the BDT-based ones, where available, the combined relative uncertainty of the cross section measurement improved to $\pm$ 1.07\%.

\subsubsection*{CP measurement}
\begin{comment}
\subsection{Interpretation of the measurement in an Effective Field Theory framework}

%The \zhsm distributions could be sensitive to BSM contributions in the $\PGt\PGt$ Higgs-decay channel within an EFT scenario. 
The EFT framework is indeed able to parameterize potential BSM effects as anomalous higher-dimensional operators added to the SM Lagrangian:
%to encapsulate the effects of BSM physics at higher scales:
\begin{equation}
    \mathcal{L}_{\mathrm{EFT}}=\mathcal{L}_{\mathrm{SM}}+\sum_d \sum_i \frac{c_i^{(d)}}{\Lambda^{d-4}} \mathcal{O}_i^{(d)}, 
\end{equation}
with $d>4$. The parameters $c_i^{(d)}$ are called Wilson coefficients and are introduced by their corresponding operators $\mathcal{O}_i^{(d)}$ of dimension $d$. The parameter $\Lambda$ sets the scale of the BSM physics.

In a lepton and baryon number conserving scenario, only even dimensions are permitted and, retaining the series to the first order in the perturbative expansion, the cross-section of a process in respect to the SM value is given by:
\begin{equation}
    \sigma_{\mathrm{SM}+\mathrm{EFT}} \propto\left|\mathcal{M}_{\mathrm{SM}}+\sum_i \frac{c_i}{\Lambda^{2}} \mathcal{M}_{i} \right| = |\mathcal{M}_{\text{SM}}|^2 + 2 \sum_{i} \frac{c_i}{\Lambda^2} \mathcal{R}(\mathcal{M}_{\text{SM}}^* \mathcal{M}_i) + \sum_{i,j} \frac{c_i c_j}{\Lambda^4} \mathcal{R}(\mathcal{M}_i^* \mathcal{M}_j).
\end{equation}
\end{comment}

We introduce CP-violation within the Effective Field Theory (EFT) framework since the measurement of the Higgs boson couplings to fermions is expected to yield higher sensitivity and be more model-independent in this case, with CP-odd terms of the same order as the CP-even terms of the SM and not suppressed by powers of the energy scale. In the Warsaw basis in SMEFT, the dimension-6 operators that describe CP violation in the couplings between the Higgs boson and the tau leptons include $\mathcal{O}_{eH} = (H^\dagger H) (\bar{L}_L \tilde{H} e_R) + \text{h.c.}
$.
In this Yukawa operator, $L_L$ represents the left-handed lepton doublet, $e_R$ is the right-handed lepton, $H$ is the Higgs doublet, and $\tilde{H}$ is the conjugate Higgs doublet. The effective Yukawa coupling may have an imaginary part, indicating CP violation.

Angular distributions in \zhsm production can be used to increase sensitivity to both CP-even and CP-odd interactions of the Higgs boson. 
%They are defined on the decay and production planes in the appropriate frames. However, not all angles can always be defined due to missing information about the Z decay plane in the $Z\to\nu\nu$ channel where only $\theta_2$ is accessible. 
Other angular variables can be defined as usual between the four-momenta vectors of the Z and Higgs decay products. In any case, the definition of the angles related to the tauon four-momenta strongly depends on its precise reconstruction.

\subsubsection*{Conclusions}

In this document, we have presented an analysis of $\PH\to\PGtp\PGtm$ properties with \zhsm events at $\sqrt{s}=$\SI{240}{\giga\electronvolt} at the FCC-ee with $\mathcal{L}_{int}=$\SI{10.8}{\per\atto\barn}. In particular, we obtained the relative uncertainty expected at FCC-ee for $\sigma_{\zhsm}\times\mathcal{B}$($\PH\to\PGtp\PGtm$).

The second goal of this analysis is the study of CP violation contributions in the $\PH\to\PGtp\PGtm$ vertex in the same signal processes, by introducing this effect in the SM via EFT operators. This work is still ongoing and we expect to have preliminary results in the next few months.


==> sections/higgs/hvventangle.tex <==
{\color{red} PK: Just saw that \cite{Aguilar-Saavedra:2024jkj} is out. Not sure if it's the same thing.}

Angular momentum in the decay $\PH \to \PV_1 \PV_2$ of the Higgs boson into two weak bosons (which we consider as distinguishable) is fully determined by the tripartite density operator $\rho_{L S_1 S_2}$ involving the orbital angular momentum and the  spins of the two bosons. In particular, this operator can be used to determine the entanglement between any two parties of the $L S_1 S_2$ system. The SM predicts a large entanglement in most cases. Using as entanglement measure the negativity $N$~\cite{Plenio:2007zz}, one has for $\PH \to \PZ \PZ$ decays
\begin{align}
& L-(S_1 S_2) :\quad N = 0.757 \,, && L-S_1 :\quad N = 0.105 \,, \notag \\
& S_1-(L S_2) :\quad N = 0.998 \,, && L-S_2 :\quad N = 0.105 \,, \notag \\
& S_2-(L S_1) :\quad N = 0.998 \,, && S_1 - S_2 :\quad N = 0.843 \,,
\end{align}
with similar values for $\PH \to \PW \PW$~\cite{Aguilar-Saavedra:2024whi}. The numbers in the left side correspond to the entanglement between one subsystem and the rest; with all of them being non-zero, the system is said to have genuine tripartite entanglement. The numbers in the right side correspond to the entanglement between two parties when the degrees of freedom of the third one are integrated out. The entanglement, as well as the possible violation of Bell inequalities, can be determined from angular distributions of the decay products.

Angular distributions in the decay $\PH \to \PV_1 \PV_2$  can be parametrised either using a fixed reference system $(\hat x, \hat y, \hat z)$, or a moving one $(\hat r, \hat n, \hat k)$, where $\hat k$ is taken in the direction of one of the decay products in the Higgs rest frame. The former, referred to as `canonical basis', is the convenient one to express $\rho_{L S_1 S_2}$. The latter, also known as `helicity basis', is very useful for measurements, because the orbital angular momentum component in the direction of motion vanishes, which greatly simplifies the description. For example, there are 18 non-zero decay amplitudes in the canonical basis, while in the helicity basis the number is reduced to only three quantities $a_{\lambda_1 \lambda_2}$, with $(\lambda_1,\lambda_2) = (1,1)$, $(-1,-1)$ or $(0,0)$. These amplitudes in general depend on the off-shell boson mass $m_{V^*}$.

In the helicity basis the four-dimensional angular distribution is~\cite{Aguilar-Saavedra:2022wam,Aguilar-Saavedra:2022mpg}
\begin{equation}
\frac{1}{\sigma}\frac{d\sigma}{d\Omega_1d\Omega_2} = \frac{1}{(4\pi)^2}\left[ 1 +a_{lm}^1 Y_l^m(\theta_1, \phi_1) + a_{lm}^2 Y_l^m(\theta_2, \phi_2)    + c_{l_1 m_1 l_2 m_2}  Y_{l_1}^{m_1}(\theta_1, \phi_1)Y_{l_2}^{m_2}(\theta_2, \phi_2)  \right] \,,
\label{ec:dist4D}
\end{equation}
where $\Omega_1 = (\theta_1, \phi_1)$, $\Omega_2 = (\theta_2,\phi_2)$ are the angles that determine the orientation of the spin analysers $\Pf_1$, $\Pf_2$ for the two bosons $\PV_1$, $\PV_2$ in their respective rest frame, and $Y_l^m$ are the usual spherical harmonics. 
This angular distribution can be considered either differentially as a function of $m_{V^*}$, or integrated over this variable. In either case, its determination requires a full reconstruction of the final state, because the momenta of $\Pf_{1,2}$ have to be boosted to the rest frame of the decaying bosons. 

At the tree level, the coefficients $a_{lm}^{1,2}$ and $c_{l_1 m_1 l_2 m_2}$ are related to the elements of the spin-density operator $\rho_{S_1 S_2}$ in the helicity basis, which can be expanded in a basis of irreducible tensor operators $T^l_m$ as
\begin{eqnarray}
\rho_{S_1 S_2} & = & \frac{1}{9}\left[
\mathbf{1}_3 \otimes \mathbf{1}_3 + A^1_{lm} \, T^l_{m} \otimes \mathbf{1}_3 + A^2_{lm} \, \mathbf{1}_3 \otimes T^l_{m}  + C_{l_1 m_1 l_2 m_2} \, T^{l_1}_{m_1} \otimes T^{l_2}_{m_2}
\right] \,.
\label{ec:rhoAC}
\end{eqnarray}
The relation is $a_{lm}^1 = A_{lm}^1 B_l^1$, $a_{lm}^2 = A_{lm}^2 B_l^2$, $c_{l_1 m_1 l_2 m_2} = B_{l_1}^1 B_{l_2}^2 C_{l_1 m_1 l_2 m_2}$, with constants $B_l^i$ that represent the spin analysing power of the fermions $\Pf_i$, $i = 1,2$. For decay into charged leptons one has $B_1 = - \sqrt{2 \pi} \eta_\ell$, $B_2 = \sqrt{2\pi/5}$, with $\eta_\ell = \pm 1 $ for $\PW^\mp$ (taking as spin analyser the charged lepton) and $\eta_\ell \simeq 0.13$ for $\PZ$ (taking as spin analyser the negative lepton). Next-to-leading order (NLO) effects have been studied for $\PH \to \PZ \PZ$~\cite{Grossi:2024jae}. For terms with $l = 2$ the corrections with respect to the leading order are quite small, whereas for spin correlation terms $c_{1 m_1 1 m_2}$, which are suppressed by a small $\eta_\ell^2 \simeq 0.01$ factor, NLO corrections are at the 10\% level.

The statistics of Higgs bosons expected at a future $\Pep \Pem$ collider is one order of magnitude smaller than at LHC Run 3, and two orders of magnitude smaller than at the HL-LHC. Still, lepton colliders can explore decay modes that have large backgrounds in hadron collisions. Among them, the semileptonic decay modes
\begin{itemize}
\item $\PH \to \PW \PW \to \Pl \PGn \PQq \PAQq$
\item $\PH \to \PZ \PZ \to \Plp \Plm \PQq \PAQq$
\end{itemize}
are specially promising, though sensitivity studies are not yer available. The discrimination between quarks and anti-quarks, necessary for the direct measurement of the parameters of the distribution (\ref{ec:dist4D}), may be circumvented by assuming \CP conservation in the decay. In such scenario, the three helicity amplitudes for $\PH \to \PV_1 \PV_2$ (which depend on $m_{V^*}$) can be determined from a binned measurement of the parameters $a_{20}^{1,2}$ in Eq.~(\ref{ec:dist4D}), namely
\begin{equation}
a_{11} = a_{-1-1} = \left[ \frac{1}{4} + \frac{1}{2 \sqrt 2} \frac{a_{20}^i}{B_2^i} \right]^{1/2}  \qquad
a_{00} = - \left[ \frac{1}{2} - \frac{1}{\sqrt 2} \frac{a_{20}^i}{B_2^i} \right]^{1/2} \,.
\end{equation}
The parameters $a_{20}^i$ multiply spherical harmonics $Y_2^0(\theta,\phi)$ that are even in $\cos \theta$, therefore their experimental determination does not rely on the identification of quarks versus anti-quarks. Once the helicity amplitudes are measured, the density operator $\rho_{L S_1 S_2}$ can be determined in a model-independent fashion. A study for the $\PZ \PZ \to 4\Pl$ channel has shown that even despite the need of a (coarse) binning on $m_{V^*}$, there is a great statistical gain when determining the parameters of the density operators by using this method~\cite{Aguilar-Saavedra:2024whi}. 

Concerning the rest of decay modes, the fully-hadronic ones seem difficult due to the combinatorics required to properly identify the quarks resulting from each boson decay. The fully-leptonic final state $\PW^+ \PW^- \to \Plp \PGn \, \Plm \PGn$ is more favourable than in hadron collisions~\cite{Barr:2021zcp} but still the number of kinematical constraints (five, for the missing energy and on-shell conditions for $\PH$ and one $\PW$ boson) is smaller then the number of unknowns (six, for the two neutrino momenta) and the final state cannot be uniquely reconstructed. The possibility of a kinematical reconstruction via a likelihood fit or a multivariate method remains to be explored.


==> sections/higgs/hwidth.tex <==
\subsubsection*{Introduction}
\label{sec:HiggsWidth:Into}

The measurement of the Higgs boson's natural width, \GH, holds significant importance as any deviation from the Standard Model (SM) prediction could indicate the presence of new physics, such as the decay of the Higgs boson into previously unknown particles. According to the Standard Model, the Higgs boson's natural width is predicted to be approximately 4.1 MeV, a value too small for direct measurement. As a result, indirect methods have been employed at the Large Hadron Collider (LHC), utilizing the differing dependencies of on-shell and off-shell Higgs production on the particle's width \cite{ATLAS:2023dnm,CMS:2022ley}. Such techniques often make hefty theoretical assumptions, including the universality of the Higgs boson's on-shell and off-shell couplings to vector bosons.

In contrast, the Future Circular Collider-electron-positron (FCC-ee) \cite{asmaaabada_2019_fccee} offers a unique opportunity to measure the inclusive production cross-section of the $\PZ\PH$ process without presuming specific Higgs boson decay modes. This approach enables the determination of the absolute coupling between the Higgs and $\PZ$ bosons. Combining this measurement with data on the $\PZ\PH, \PH\to \PZ\PZ^*$ process, along with the $\PH\to \PZ\PZ^*$ branching ratio, allows for the calculation of the total Higgs boson width without any additional theoretical assumptions:
\begin{equation}
    \GH \propto \frac{\sigma_{\PZ\PH}^{2}}{\sigma_{\PZ\PH,\PH(\PZ\PZ^*)}}.
\end{equation}
Assuming that the $\PZ\PH$ production cross-section and the $\PZ\PH$, $\PH\to \PZ\PZ^*$ measurements uncertainties have close-to-no correlation, the uncertainty on the Higgs width measurement can be decomposed as:
\begin{equation}
    \frac{\delta\GH}{\GH} \propto \sqrt{\left(2\frac{\delta\sigma_{\PZ\PH}}{\sigma_{\PZ\PH}}\right)^{2} + \left(\frac{\delta\sigma_{\PZ\PH,\PH(\PZ\PZ^*)}}{\sigma_{\PZ\PH,\PH(\PZ\PZ^*)}}\right)^{2} }.
\end{equation}
Considering only statistical uncertainties, a 0.3\% relative uncertainty on the inclusive $\PZ\PH$ production cross-section can be achieved at the FCC-ee using leptonic $\PZ$ tagging. As it will be shown below, the relative uncertainties on the measurement of \GH\ will therefore be dominated by the precision on the determination of the $\PZ\PH/\PH\to \PZ\PZ^*$ cross-section.

A sensitivity study for the $\PZ\PH/\PH\to \PZ\PZ^*$ process measurement at the FCC-ee, with a center-of-mass energy of 240 GeV, has been conducted \cite{morange_2023_ysabc-wm427,HindTaibi2024,}. This study considered various final states, including those with either two or four leptons resulting from the decay of $\PZ$ bosons. Targeted event selections were focused on $\PZ\PH$ events where $\PZ$ bosons decay into electron-positron, muon-antimuon, neutrino-antineutrino, or quark-antiquark pairs. Post-selection, the contribution from vector-boson-fusion are minor and categorized as background. The study utilized fast simulation techniques for particle propagation and interaction with detector materials, incorporating parametrised efficiencies and resolutions. An assumed integrated luminosity of \SI{5}{\per\atto\barn}, equivalent to three years of operation with two detectors at distinct interaction points, was used for this analysis.

The provided information represents only a concise overview of the analysis. Detailed findings and methodologies will be outlined in the forthcoming FCC-ee feasibility study and a dedicated article currently under preparation.


\subsubsection*{Event samples}
\label{sec:HiggsWidth:Samples}


The studies are based on Monte Carlo event samples of the main signal and background processes, generated at $\ee$ center-of-mass energies of 240 GeV and normalised using their theoretical cross-sections to the target integrated luminosity of \SI{5}{\per\atto\barn}. The beam energy and the size of the interaction point are smeared according to the expected beam energy spread and size of the FCC-ee luminous region.

The \whizard generator \cite{Kilian:2007gr,Moretti:2001zz} has been used to produce signal events, where a Higgs boson is produced together with an \ee, \mm, \vv, $\PGt^+\PGt^-$ or \qq\ pair. The PYTHIA 8 generator \cite{Sjostrand:2014zea} has been used for the production of the main background event samples considered in this analysis: $\ee \to \PWp\PWm$ and $\ee \to \PZ\PZ$.

The generated events are passed through a parametric simulation of the detector response implemented in DELPHES \cite{deFavereau:2013fsa}. The reconstruction efficiencies and resolutions for various particle hypotheses are those expected for the IDEA detector with a crystal electromagnetic calorimeter upstream of a dual-readout fiber calorimeter. Lepton misidentification is assumed to be negligible. The kinematic properties of the jets are assumed to be determined from those of the constituents via a particle-flow algorithm.



\subsubsection*{Analysis strategy, event selection and categorisation}
\label{sec:HiggsWidth:Analysis}

Two analyses are performed in parallel: one considers final states with 2 leptons\footnote{In the following, the term ``lepton'' will be used to identify electrons or muons, while $\PGt$ leptons are excluded from the definition.}, along with either 2 quarks generating hadronic jets and 2 neutrinos, or 4 hadronic jets; and another considers final states with 4 leptons and either 2 quarks generating hadronic jets or 2 neutrinos. The presence of on-shell $\PZ$ bosons in the final state is sought by selecting events with an opposite-sign, same-flavour lepton pair with invariant mass close to that of the $\PZ$ boson, or using a looser selection when a leptonic off-shell $\PZ$ is considered in the 4-lepton case. Only the most sensitive combinations are considered. All analyses cluster the reconstructed particles, excluding the $\PZ$ boson decay products, using the exclusive $k_t$ Durham algorithm \cite{CATANI1991432,Cacciari:2011ma}. The particles are clustered into two or four jets depending on the considered topology. A selection on the event missing energy characterises events with a $\PZ$ boson decaying into neutrinos.

The signal is contaminated by non-resonant ($\ee \to \PWp\PWm$ and $\ee \to \PZ\PZ$) and resonant (mostly $\PH \to \PWp\PWm$, $\PH\to\PGt^+\PGt^-$) backgrounds. Dedicated selections are deployed to reduce specific backgrounds affecting some of the considered topologies, such as a selection on the recoil mass to distinguish between $\PZ$ bosons from $\PZ\PH$ production and those from Higgs decay, or a selection on the properties of a photon in the event to reduce $\PH \to \PZ \PGg$ contamination. The selections are designed to allow categorization of events targeting a given final state into orthogonal categories.

Dedicated Boosted Decision Tree (BDT) discriminants, trained on the kinematical properties of the objects in the final states for signal and backgrounds, are additionally used to increase the sensitivity of the 2-lepton analysis. Some of the final states, when relevant, split the event classes into subcategories with different signal-to-background ratios to enhance the sensitivity of the measurement and better constrain the backgrounds. Each of the studied analysis region selects tens to hundreds of $\PZ\PH,\HZZ$ signal events; this translates in a large final statistical component to the expected total uncertainty. A 10\% systematic uncertainty on the main non-resonant backgrounds is considered when performing the maximum-likelihood fits to the selected candidates, as well as a 5\% uncertainty on some resonant backgrounds (e.g. $\PH \to \PWp\PWm$) when relevant.



\subsubsection*{Results}
\label{sec:HiggsWidth:Results}


The results for each analysis are determined by a binned, maximum-likelihood fit to the distribution of a quantity that discriminates between the signals and the background. The chosen quantity for the fit in each considered channel is tabulated in Table~\ref{tab:ZHHZZ_results}, alongside the channel signal-to-background ratio and measurement sensitivity. Each channel is labelled according to the target decay of each $\PZ$ boson in the final state: $\PZ_1$ refers to the $\PZ$ boson produced in association with the Higgs boson, $\PZ_2$ is the on-shell $\PZ$ boson from the \HZZ\ decay, and $\PZ_3$ the off-shell $\PZ^*$ boson.

\begin{table}[!t]
  \centering
  \begin{tabular}{ccccccc}
    \hline \hline
    \multicolumn{3}{c}{Channel} & \multicolumn{2}{c}{Signal-over-background} & \multicolumn{2}{c}{Sensitivity} \\    
    $\PZ_1$ & $\PZ_2$ & $\PZ_3$ & $S/B$ & $S/\sqrt{B}$ & fit quantity & $\mu_{\PZ\PH, \PH\to \PZ\PZ^*}$ \\
    \hline
    $\LL$ & $\vv$ & $\jj$ & 1.06 & 12  & BDT discriminant        & 1 $\pm$ 0.074      \\
    $\LL$ & $\jj$ & $\vv$ & 0.30 & 4.6 & BDT discriminant        & 1 $\pm$ 0.107      \\
    $\vv$ & $\LL$ & $\jj$ & 0.55 & 9   & BDT discriminant        & 1 $\pm$ 0.069      \\
    $\LL$ & $\jj$ & $\jj$ & 0.04 & 4.6 & BDT discriminant        & 1 $\pm$ 0.124      \\
    \hline
    $\LL$ & $\LL$ & $\jj$ & 1.5  & 7.9 & $m^{\mbox{rec}}_{\LL_1}$ & $1\substack{+0.193 \\-0.176}$ \\
    $\LL$ & $\jj$ & $\LL$ & 0.95 & 6.2 & $m_{\jj+\LL_3}$          & $1\substack{+0.193 \\-0.174}$ \\
    $\jj$ & $\LL$ & $\LL$ & 3.1  & 11  & $m_{\LL_2+\LL_3}$        & $1\substack{+0.187 \\-0.168}$ \\           
    $\vv$ & $\LL$ & $\LL$ & 0.75 & 2.9 & $m_{\LL_2+\LL_3}$        & $1\substack{+0.394 \\-0.329}$ \\
    \hline
    \hline
  \end{tabular}
  \caption{Signal-over-background ratios, quantity used in the maximum likelihood fit, and expected sensitivity to the the $\ee \to \PZ\PH, \HZZ$ cross-section of the channels discussed in this study. $\PZ_1$ refers to the $\PZ$ boson produced in association with the Higgs boson, $\PZ_2$ is the on-shell $\PZ$ boson from the \HZZ\ decay, $\PZ_3$ the off-shell $\PZ^*$ boson. $S$ is the number of signal events and $B$ is the total number of background events. The details of the variable entering the BDT discriminants of the 2-lepton channels are found in Ref.~\cite{morange_2023_ysabc-wm427}. $m^{\mbox{rec}}_{\LL_1}$ is the recoil mass against the dilepton system of $\PZ_1$; all other variables refer to the invariant mass of system formed by objects listed in the subscript.}
  \label{tab:ZHHZZ_results}
\end{table}

The combination of the three most sensitive 2-lepton channels ($\LL\vv\jj$, $\LL\jj\vv$, $\vv\LL\jj$) leads to a precision of 4.6\%. The inclusion of the $\LL\jj\jj$ channel improves the overall sensitivity to 4.3\%. The combination of the 4-lepton channels considered in the second analysis leads to a precision of about 10\%; their naive combination with the 2-lepton channels results in an overall sensitivity of 4\%.

\subsubsection*{Conclusions}
\label{sec:HiggsWidth:Conclusions}

With an integrated luminosity of 5 ab$^{-1}$ in \epem collisions at $\sqrt{s} = 240$ GeV, collected by two detectors over three years of data-taking, FCC-ee could measure the natural width of the Higgs boson with a precision of approximately 4\%. Considering the new nominal FCC-ee luminosity of 7.5 ab$^{-1}$, the achievable precision would improve to around 3.3\%. This value represents an upper limit: further improvement could be possible through more advanced analysis techniques or by including additional final states, such as those targeting $\PGtp\PGtm$ topologies with dedicated $\PGt$-identification algorithms. A similar measurement of VBF \HZZ\ production at $\sqrt{s} = 365$ GeV could also be performed and combined to further enhance sensitivity. With all these improvements, a precision of 1--2\% could potentially be attainable, though further studies are required for a more definitive quantitative estimate.




==> sections/higgs/hzzclic.tex <==
As an energy-staged e$^+$e$^-$ collider, the Compact Linear Collider (CLIC) can provide a comprehensive physics program of measurements in the Higgs sector \cite{robson2018updatedclicluminositystaging} including \CP-even Higgs couplings to Z bosons ($g_{\PH\PZ\PZ}$). Most BSM models predict Higgs couplings to electroweak (EW) bosons to deviate from the Standard Model predictions at the order of a percent \cite{Barklow:2018}. As discussed in \cite{robson2020clichiggscouplingprospects}, a global fit to data from all energy stages allows extraction of the Higgs couplings with the required precision. Three independent individual measurements of $\text{BR}(\PH\to \PZ\PZ^*)$ as the observable for $g_{\PH\PZ\PZ}$ determination are discussed in \cite{Abramowicz_2017} and \cite{Vukasinovic:2022}, at CLIC center-of-mass energies: 350 GeV, 1.4 TeV and 3 TeV. In the full simulation of realistic experimental measurements, assuming integrated luminosities of 1 ab$^{-1}$, 1.5 ab$^{-1}$ and 5 ab$^{-1}$, respectively, the product of the Higgs production cross-section $\sigma$ and $\text{BR}(\PH\to \PZ\PZ^*)$ is measured corresponding to the number of selected signal events. The signal is chosen in $\PZ\PZ^*$ semileptonic final state, due to the smaller irreducible background than in the hadronic final state. In Higgsstrahlung at 350 GeV CLIC, primary $Z$ is assumed to decay hadronically. 

The event selection is based on identification of exactly two isolated leptons per event while the remaining Particle Flow Objects \cite{Thomson:2013} are clustered into four (two) jets. Isolation criteria are based on kinematic observables in the event: energy and impact parameter of a particle, ratio of particle's energy deposition in calorimeters and track vs. cone energy around the isolated lepton candidate. Multivariate analysis (MVA) \cite{hoecker:2009tmvatoolkitmultivariate} is applied to further suppress background on the basis of kinematic and event-shape variables.

Relative statistical precision $\delta$ is obtained as inverse of the statistical significance $S$, where $S = N_{S}/ \sqrt{N_{S}+N_{B}}$ for the selected numbers of signal $N_{S}$ and background $N_{B}$ events. Obtained statistical precision is further scaled to $\delta_{\mathrm{projected}}$ assuming the integrated luminosities foreseen in the current CLIC staging scenario with the electron beam polarisation of 80\%. Obtained and projected results are given in Table \ref{table:hzz_clic}. 

 \begin{table}[!h]      
\centering
\vspace{.5cm}
\begin{tabular}{ |p{2.7cm}|p{2.7cm}|p{2.7cm}| } 
%\begin{tabular}{ |c|c|c| } 
 \hline
% \multicolumn{3}{|c|} %$\text{BR}(\PH\to \PZ\PZ^*)$    & $\delta$   & $\delta_{projected}$  \\
\hfil $\text{BR}(\PH\to \PZ\PZ^*)$ & \hfil $\delta$ & \hfil $\delta_\text{projected}$ \\
\hline
\hfil 350 GeV & \hfil 20\% & \hfil 20\% \\ 
\hfil 1.4 TeV & \hfil 5.6\% & \hfil 3.4\% \\
\hfil 3 TeV & \hfil 3.0\% & \hfil 2.4\% \\
\hline
\end{tabular}
\caption{\label{table:hzz_clic}Statistical precision $\delta$ of $\text{BR}(\PH\to \PZ\PZ^*)$ from the fully simulated measurements and projected precision $\delta_\text{projected}$ obtained by scaling to the scenario with 80\% polarised electron beam and updated integrated luminosities (1 ab$^{-1}$ at 350 GeV, 2.5 ab$^{-1}$ at 1.4(5) TeV and 5 ab$^{-1}$ at 3 TeV).}
\end{table}

It is clear that a high-energy operation of an \epem collider is reaching a percent level relative statistical precision already in a stand-alone measurement. As discussed in \cite{Barklow:2018}, optimized global fits can provide a permille precision for Higgs to EW bosons \CP-even couplings including $g_{\PH\PZ\PZ}$.



==> sections/higgs/hzzcpfcc.tex <==
\subsubsection*{Introduction}

% \subsection{Motivation}
The search for \CP violation is an important research direction of future experiments in particle physics. 
\CP violation is one of the requirements for baryogenesis, and the SM mechanism is believed to be insufficient 
for generating the observed predominance of baryon matter over antimatter on a cosmological scale. 
The electron-positron colliders have unique features for testing \CP violation in the Higgs boson interactions. 
 While running in electron-positron collision mode at a centre-of-mass energy of \SI{240}{\giga\electronvolt}, 
the Future Circular Collider is expected to produce on the order of $10^6$ events of the Higgsstrahlung 
process $\Pep\Pem\to\PZ\PH$. Studying the kinematic distributions in this process allows for the probing 
of \CP-violation at the $\PH\PZ\PZ$ vertex. Figure~\ref{fig:angles} shows the relevant angular distributions.

In the Snowmass-2013 and Snowmass-2022 studies~\cite{Gritsan:2022php}, a benchmark parameter 
was established for the \CP-odd contribution based on production-invariant decay process:
%%%%%%%%%%%%%%%%%%%%%%%
\begin{eqnarray}
f_{\CP}^{\PH\PX}\equiv
\frac{\Gamma^{\CP\mathrm{-odd}}_{\PH\to \PX}
}{\Gamma^{\CP\mathrm{-odd}}_{\PH\to \PX}
+\Gamma^{\CP\mathrm{-even}}_{\PH\to \PX}}
\,,
\label{eq:fCP} 
\end{eqnarray}
%%%%%%%%%%%%%%%%%%%%%%%
where the partial decay $\PH\to \PX$ width is calculated with either the $\CP$-odd or $\CP$-even part of the amplitude. 
In the case of the $\PH\PZ\PZ$ vertex, which is the focus of this note, 
the reference decay is $\PH\rightarrow \PZ\PZ\rightarrow 2\Pe2\PGm$.
%The fractional \CP-odd coupling of the $\PH$ boson to two $\PZ$ bosons can 
% be defined as $$f^{\PH\PZ\PZ}_{\CP} = \frac{|a^{\PH\PZ\PZ}_3|^2}{\Sigma |a^{\PH\PZ\PZ}_i|^2(\sigma^{\PH\PZ\PZ}_i/\sigma^{\PH\PZ\PZ}_3)}$$
%
%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[b!]
    \centering
    \includegraphics[width=0.32\linewidth]{figs/Higgs/cos_1.pdf}
    \includegraphics[width=0.32\linewidth]{figs/Higgs/cos_2.pdf}
    \includegraphics[width=0.32\linewidth]{figs/Higgs/phi.pdf}
    \caption{Reconstructed angular distributions in the process $\epem \rightarrow  \PZ\PH \rightarrow  \mumu \PX$ and its backgrounds.
    The maximum \CP violation is apparent in the asymmetry produced by a 50\% mixture of \CP-odd and \CP-even contributions (green).}
    \label{fig:angles}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%
%
% In the first-order $q^2-$expansion of the effective Lagrangian from which the above expression is derived, the $a_i$ can be treated as  constants corresponding to dimension-six operators. In particular, $a_3$ characterises the strength of \CP-odd interactions at the $\PH\PZ\PZ$ vertex. The values $\sigma_i$ correspond to the effective cross section of the $\PH\to\PZ\PZ$ decay process with $a_i =1$ and $a_{j\neq i} = 0$. This definition of the \CP-sensitive parameter is convenient as systematic uncertainties on the individual $|a_i|$'s cancel in the ratio. 
%\subsection{Targeted Signals and Dominant Backgrounds}

The targeted signal process in this analysis is $\Pep\Pem\to\PZ\PH$. 
Four final states for the $\PZ$ are considered: $\PZ\to\Pep\Pem, \PGmp\PGmm$ (leptonic channels), 
and $\PQq\PAQq, \PQb\PAQb$ (hadronic channels), where 
$\PQq\PAQq$ refers to $\PQu\PAQu, \PQd\PAQd, \PQs\PAQs, \PQc\PAQc$. 
The $\PH$ boson is allowed to decay inclusively and is not reconstructed. 
Because the centre-of-mass energy ($\sqrt{s}$) of each event is precisely known, 
the four-momentum of the $\PH$ boson can be reconstructed using total four-momentum 
conservation with the knowledge of the reconstructed four-momentum of the $\PZ$. 
In the leptonic channels, the dominant backgrounds considered are 
$\Pep\Pem\to\PWp\PWm, \Pep\Pem\to\PZ\PZ,\Pep\Pem\to\PGmp\PGmm$ and $\Pep\Pem\to\PGtp\PGtm$. 
In the hadronic channels, the dominant backgrounds are $\Pep\Pem\to\PZ\PZ$ and $\Pep\Pem\to\PQq\PAQq$ 
(in the case of the latter background, $\PQq = \PQu, \PQd, \PQs, \PQc, \PQb$). 
The $\Pep\Pem\to\PWp\PWm$ background dominates the $\PZ\to\PQq\PAQq$ channel, 
but is suppressed in the $\PZ\to\PQb\PAQb$ channel.

\subsubsection*{Monte Carlo simulation, event selection, and the likelihood fit}

Signal Monte Carlo (MC) samples are generated using WHIZARD %\cite{Kilian:2011vkz} 
with parton showering done in PYTHIA6. % \cite{Sjostrand:2006qrn}. 
Background samples are generated and showered using \pythiaeight. % \cite{Sjostrand:2015oiw}. 
Reconstruction and detector simulation are performed by the fast simulation program DELPHES. 
%\cite{deFavereau:2014ald}. 
The concept detector simulated is the Innovative Detector for Electron-positron Accelerators (IDEA). 
Matrix-element re-weighting is performed by the MELA package.
% \cite{Gao:2010xkx, Bolognesi:2012hxo, Chen:2013elb}. 
Transition probabilities calculated from generator-level kinematic observables are used to re-weight the simulated, 
SM distributions to ones where the interaction at the $\PH\PZ\PZ$ vertex is fully \CP-odd 
or a mixture of \CP-even and \CP-odd. 

%\section{Analysis Strategy}
%\subsection{Preselection}

A set of preselection requirements is applied for each channel. In the leptonic channels, only events containing 
at least 2 leptons of opposite charge are selected. Both of these leptons are required to have momentum with 
a magnitude greater than \SI{20}{\giga\electronvolt}, which minimizes the noise from soft radiative processes. 
At least one lepton is required to be relatively isolated from the rest of the products of the event. 
In the hadronic channels, preselection requires that events have no more than two charged leptons. 
Any charged lepton entering the analysis is required to have momentum < \SI{20}{\giga\electronvolt}. 
Following these requirements, all reconstructed particles in the event are exclusively clustered to four 
jets by the Durham-$k_t$ algorithm
 % \cite{Catani:1991mxc} 
used in the FASTJET clustering program.

 % \cite{Cacciari:2012nja}. 
% This is done as, on average, four jets are expected per event. 
% Each jet is assigned a score ranging from [0,1] for in flavors Q (\PQu or \PQd), S, C, B, and G. 
% The combination of jets that minimizes the expression 
% $\chi^2 = 0.8(m_{\PZ} - m_{dijet})^2 - 0.2(m_{\PH} - m_{recoil})^2$ 
% is selected as the $\PZ$ candidate. It is enforced that the two selected jets have 
% maximum scores corresponding to the same flavor. 
The $\PZ\to ff$ difermion system that minimizes the expression $\chi^2 = 0.6(m_{\PZ} - m_{ff})^2 - 0.4(m_{\PH} - m_{recoil})^2$ 
is selected as the candidate for the~$\PZ$.
% (where $m_{\PZ/\PH}$ = the pole mass of the $\PZ/\PH$). 

%The hadronic channels are split between $\PZ\to\PQq\PAQq$ and $\PZ\to\PQb\PAQb$ 
% using the sum of the B-scores for each jet. If the jets have a sum of B-scores $\geq 1.7$, 
% the event is categorized as $\PZ\to\PQb\PAQb$. Otherwise, the event is categorized as $\PZ\to\PQq\PAQq$.

%\subsection{Kinematic Selection}
%\label{3.2}

A set of kinematic  requirements is applies in the leptonic channels:
on the invariant mass of the selected dilepton system $86 < m_\text{dilepton} < 96$;
on the three-momentum of the dilepton system $45 < p_\text{dilepton} < 55$;
on the recoil mass $124 < m_\text{recoil} < 127$;
on the cosine of the missing momentum $|\cos{\theta_\text{miss}}| < 0.98$;
and on the angle between the momentum of the $\PZ$ and the momentum of one of its decay products $|\cos{\theta_{2}}| < 0.99$.
 A looser set of requirements is applied on the same observables in the hadronic analysis.  
 An additional requirement on a visible energy $>$ \SI{150}{\giga\electronvolt} is applied. 
 %This  removes backgrounds of the type $\PZ\PH\to\PZ\to\PGnl\PAGnl,\PH\to\PX$. 

%\subsection{Template Fits}

Two optimal observables are computed using the matrix element technique: 
$D_{0^-}$, which is sensitive to the pure \CP-odd contribution, and 
$D_{\CP}$, which corresponds to the interference between the \CP-even and \CP-odd components. 
Three templates characterise the signal parameterization using MC simulation that,
together with the background, is incorporated into the likelihood model with a free parameter $f^{\PH\PZ\PZ}_{\CP}$.
The expected rates of events are normalized to the 10.8\,ab$^{-1}$ of data collected at $E_{\epem}=240$\,GeV.
\Cref{fig:scan} shows the expected constraints on $f^{\PH\PZ\PZ}_{\CP}$ at FCC-ee,
based on 10.8\,ab$^{-1}$ of data collected at $E_{\epem}=240$\,GeV.
The combined constraint is $f^{\PH\PZ\PZ}_{\CP}=\pm2.5\times10^{-5}$, which is
$\pm 5.5\times10^{-5}$ with $\PZ\rightarrow\Pep\Pem$ and  $\pm 4.6\times10^{-5}$ with $\PZ\rightarrow\PGmp\PGmm$.

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\linewidth]{figs/Higgs/leptonic_10800_lumiscan.pdf}
    \caption{The expected likelihood scans of $f^{\PH\PZ\PZ}_{\CP}$ with two $\PZ\to ff$ channels
    at FCC-ee, based on 10.8\,ab$^{-1}$ of data collected at $E_{\epem}=240$\,GeV.}
    \label{fig:scan}
\end{figure}

\subsubsection*{Summary}

This note presents the expected results for constraints on \CP-violating contributions 
in the Higgsstrahlung process at FCC-ee, based on 10.8\,ab$^{-1}$ of data collected at $E_{\epem}=240$\,GeV.
In the leptonic $\PZ$ boson channel, an expectation of $f^{\PH\PZ\PZ}_{\CP}=\pm2.5\times10^{-5}$ is projected. 
The hadronic $\PZ$ boson channel is anticipated to provide further improvements, with results expected soon.
Our results are similar to those obtained in the Snowmass-2022 studies~\cite{Gritsan:2022php}, 
when adjusted for the same luminosity, but they are more dependable due to the comprehensive detector studies conducted.


==> sections/higgs/hzzcppol.tex <==
The Higgs to $\PZ$ boson interaction can be expressed by the following effective Lagrangian \cite{Artoisenet:2013puc}:
 \begin{equation}
         \mathcal{L}_\text{EFF}=c_\text{SM} \,\PZ_\mu \PZ^\mu \PH -  \frac{{c}_{\PH\PZ\PZ}}{v}\PZ_{\mu\nu}{\PZ}^{\mu\nu}\PH -  \frac{\tilde{c}_{\PH\PZ\PZ}}{v}\PZ_{\mu\nu}\tilde{\PZ}^{\mu\nu}\PH, \label{eq:effl2}
                    \end{equation}
where $\tilde{c}_{\PH\PZ\PZ}$ denotes the loop-induced \CP-odd coupling, and can be parametrised by the mixing angle $\tilde{c}_{\PH\PZ\PZ}\propto\sin\xi_{\CP}$. 
Concerning the polarization of the initial electron and positron beams, one defines a projection operator, which is given by:
\begin{equation}
\small
    \frac{1}{2}(1 - \boldsymbol{P}\cdot \boldsymbol{\sigma}) =\frac{1}{2}(\delta_{\lambda\lambda'}-P^a\sigma^a_{\lambda\lambda'}) = \frac{1}{2}\begin{pmatrix}
        1- P_3& P_1- iP_2\\
        P_1 + iP_2& 1+P_3
    \end{pmatrix} = \frac{1}{2}\begin{pmatrix}
                1-f\cos\theta_P& f\sin\theta_P e^{-i\phi_P}\\
                f\sin\theta_P e^{i\phi_P}&  1+f\cos\theta_P
            \end{pmatrix},
    \label{eq:polmat}
\end{equation}
where $f$ is the polarization fraction. The Higgs-strahlung $\epem \rightarrow \PZ\PH$ is the dominant Higgs production process at \epem collider. By taking the polarization of the initial beams into account, the spin-density matrix of the Higgs-strahlung $\rho_{\lambda_r \lambda_u}$ can be derived. Eventually, we can obtain the spin-density matrix by applying the Bouchiat-Michel formula \cite{Bouchiat:1958yui}, and the spin density matrix is given by
\begin{equation}
                    % \begin{split}
                {\rho}=
                (1-P_-^3P_+^3)A+(P_-^3-P_+^3)B^+\sum_{mn}^{1,2}P_-^m P_+^n C_{mn}.
                % \end{split}
\end{equation}

Furthermore, we introduced the \CP-odd operator for the $\PH\PZ\PZ$ interaction of Eq.~\eqref{eq:effl2}, and obtain the following form of the total amplitude squared:
\begin{equation}
            \begin{split}
                    |\mathcal{M}|^2 &=(1-P_-^3P_+^3)( \cos^2\xi_{\CP}\,\mathcal{A}_\text{\CP-even} + {\sin2\xi_{\CP}\,\mathcal{A}_\text{\CP-odd}} + \sin^2\xi_{\CP}\,\widetilde{\mathcal{A}}_\text{\CP-even})\\
                    &+(P_-^3-P_+^3)(\cos^2\xi_{\CP}\,\mathcal{B}_\text{\CP-even} + {\sin2\xi_{\CP}\,\mathcal{B}_\text{\CP-odd}} + \sin^2\xi_{\CP}\,\widetilde{\mathcal{B}}_\text{\CP-even})\\
                    &+\sum_{mn}^{1,2}P_-^m P_+^n\left(\cos^2\xi_{\CP}\,\mathcal{C}^{mn}_\text{\CP-even} + {\sin2\xi_{\CP}\,\mathcal{C}^{mn}_\text{\CP-odd}} + \sin^2\xi_{\CP}\,\widetilde{\mathcal{C}}^{mn}_\text{\CP-even} \right).
            \end{split}
            \label{eq:ampsqbsm}
            \end{equation}
Note, that the \CP-invariant parts with $\cos^2\xi_{\CP}$ and $\sin^2\xi_{\CP}$ are both \CP-conserving, while the \CP-mixing terms with $\sin2\xi_{\CP}$ violate the \CP symmetry. 

Particularly, the \CP-violating terms $\mathcal{A}_\text{\CP-odd}$, $\mathcal{B}_\text{\CP-odd}$ and  $\mathcal{C}^{mn}_\text{\CP-odd}$ can be extracted by the triple-products, which are given by
            \begin{align}
                &\mathcal{A}_\text{\CP-odd}, \mathcal{B}_\text{\CP-odd}\propto \epsilon_{\mu\nu\alpha\beta} [p_{e^-}^\mu p^\nu_{e^+} p^\alpha_{\PGmp} p^\beta_{\PGmm}]\propto (\vec{p}_{\PGmp}\times \vec{p}_{\PGmm})\cdot \vec{p}_{e^-}, \\
                &\mathcal{C}^{mn}_\text{\CP-odd} \propto \epsilon_{\mu\nu\rho\sigma}[({p}_{e^-} +{p}_{e^+})^\mu p_{\PGmp}^\nu p_{\PGmm}^\rho s_{e^-}^\sigma ]\propto(\vec{p}_{\PGmp}\times\vec{p}_{\PGmm})\cdot \vec{s}_{e^-}.
            \end{align}
The triple-product is the azimuthal-angle difference between the $\PGmp\PGmm$ plane and the spin of the electron. Therefore, defining the orientation of the azimuthal plane by fixing the direction of electron transverse polarization, the $C^{\text{\CP-mix}}_{mn}$ depends directly on the azimuthal angle of $\phi_{\PGmm}$ (see Fig.~\ref{fig:coord}).

\begin{figure}[h]
    \centering
    \tikzstyle{every node}=[scale=2]
\begin{tikzpicture}[line width=1pt,scale=2]
\draw [-stealth](-1,0) -- (0,0);
\draw [-stealth](0,0) -- (0.7,0.7);
\draw [stealth-](0,0) -- (1,0);
\draw [-stealth](0,0) -- (-0.7,-0.7);
\draw[thin, ] (0.2,0) arc (0:-135:0.2);
\node [scale=0.3] at (0.1, -0.3) {$\theta_{\PH}$};
\node [scale=0.3] at (-0.8, -0.8) {$\PH$};
\node [scale=0.3] at (-1, -0.1) {$\Pem$};
\node [scale=0.3] at (1, -0.1) {$\Pep$};
\node [scale=0.3] at (0.3, 0.4) {$\PZ$};
\draw [-stealth](0.7,0.7) -- (0.9,1.1);
\draw [-stealth](0.7,0.7) -- (1.1,0.9);
\draw [dotted] (0.7, 0.7) -- (0.35, 0);
\draw[thin, ] (0.5,0) arc (0:63.4:0.15);
\node [scale=0.3] at (0.6, 0.1) {$\theta_{\PGmm}$};
\node [scale=0.3] at (1, 1.2) {$\PGmm$};
\node [scale=0.3] at (1.2, 1) {$\PGmp$};


\draw[help lines, ->] (0, -1.5) --(0,1.5);
\draw[help lines, ->] (-1.5, 0) --(1.5, 0);
\node[scale = 0.5] at (1.4, -0.2) {$\frac{\Vec{p}_{e^-}}{|\Vec{p}_{e^-}|}$};
\node[scale = 0.5] at (0, 1.8) {$\frac{\vec{s}_{e^-}}{|\vec{s}_{e^-}|}$};

%\draw [stealth-stealth](0,-2) -- (1,-2);
\end{tikzpicture}~~~~~~\begin{tikzpicture}[line width=1pt,scale=2]
\draw [-stealth](0,0) -- (-0.7,0.7);
\draw [-stealth](0,0) -- (0.7,-0.7);
\draw[thin, ] (0.2,0) arc (0:315:0.2);
\node [scale=0.3] at (0.2, 0.2) {$\phi_{\PH}$};
\node [scale=0.3] at (0.8, -0.8) {$\PH$};
\node [scale=0.3] at (-0.3, 0.4) {$\PZ$};
\draw [-stealth](-0.7,0.7) -- (-0.6,0.9);
\draw [-stealth](-0.7,0.7) -- (-0.8,0.5);
\draw [dotted] (-0.7, 0.7) -- (-1.05, 0);
\draw[thin, ] (-0.9,0) arc (0:63.4:0.15);
\node [scale=0.3] at (-0.8, 0.1) {$\phi_{\PGmm}$};
\node [scale=0.3] at (-0.5, 1.0) {$\PGmm$};
\node [scale=0.3] at (-0.9, 0.5) {$\PGmp$};

\draw [dotted] (-0.7, 0.7) -- (-1.0,1.0);
\draw[thin, ] (-0.67, 0.8) arc (63.4:135:0.1);
\node [scale=0.3] at (-0.75, 0.95) {$\Delta\phi$};

\draw[help lines, ->] (0, -1.5) --(0,1.5);
\draw[help lines, ->] (-1.5, 0) --(1.5, 0);
\node[scale = 0.5] at (1.4, -0.2) {$\frac{\Vec{s}_{e^-}\times\Vec{p}_{e^-}}{|\Vec{s}_{e^-}\times\Vec{p}_{e^-}|}$};
\node[scale = 0.5] at (0, 1.8) {$\frac{\vec{s}_{e^-}}{|\vec{s}_{e^-}|}$};

%\draw [stealth-stealth](0,-2) -- (1,-2);
\end{tikzpicture}
    \caption{The coordinate system in the laboratory frame for the $\epem \rightarrow \PH \PGmp \PGmm$ process with initial beams polarisation.}
    \label{fig:coord}
\end{figure}

Regarding the triple products in the \CP-odd amplitude terms, one can define two \CP-odd observables 
\begin{equation}
    \mathcal{O}^T_{\CP} = \cos_{\theta_{\PH}} \sin 2 \phi_{\PGmm},~~~~\mathcal{O}^{UL}_{\CP} = \cos\Delta\phi.
\end{equation}
Hence, we can define the asymmetries by the \CP-odd observables:
\begin{equation}
        \mathcal{A}_{\CP} = \frac{1}{\sigma_\text{tot}} \int\operatorname{sgn}(\mathcal{O}_{\CP}){d\sigma} = \frac{N(\mathcal{O}_{\CP}<0)-N(\mathcal{O}_{\CP}>0)}{N(\mathcal{O}_{\CP}<0)+N(\mathcal{O}_{\CP}>0)},
            \label{eq:asyN}
\end{equation}
where $N$ denotes the corresponding number of events. 
Since the SM is \CP conserving for the neutral current, the SM background for this asymmetry is negligible. However, the number of events fluctuates statistically leading to the uncertainty of this asymmetry, which is based on a binomial distribution and given by $\Delta\mathcal{A}_{\CP} = \sqrt{\frac{1-\mathcal{A}_{\CP}^2}{N_\mathrm{tot}}}$.

In principle, both observables $\mathcal{O}^T_{\CP}$ and $\mathcal{O}^{UL}_{\CP}$ are sensitive to the \CP-violation. The observable $\mathcal{O}^{UL}_{\CP}$ can be always measured for any initial polarisation states. However, the $\mathcal{O}^T_{\CP}$ can only be measured when initial beams are transversely polarised. Consequently, one can combine the observables $\mathcal{O}^T_{\CP}$ and $\mathcal{O}^{UL}_{\CP}$ to improve the sensitivity to \CP-violation, when the transverse polarisation of electron-positron beams are imposed. Therefore, we can simply combine the two observables by \cite{Li:2024mxw}
\begin{equation}
    \chi^2 = \left(\frac{\mathcal{A}^T_{\CP}}{\Delta\mathcal{A}^T_{\CP}}\right)^2 +\left(\frac{\mathcal{A}^{UL}_{\CP}}{\Delta\mathcal{A}^{UL}_{\CP}}\right)^2.
\end{equation}
On the other hand, one can only measure $\mathcal{O}^{UL}_{\CP}$ when the initial beams are longitudinally polarised, while the longitudinally polarisation can enhance the total cross-section.

In general, the polarisation can be helpful to improve the sensitivity to \CP-violation. The longitudinally polarisation can enhance the total cross-section and suppress the statistical uncertainties. The transverse polarisation can offer an additional observable, and combining the two observables would also improve the precision of \CP-violating coupling.

==> sections/higgs/ilccphvv.tex <==
Although a purely \CP-odd state for the Higgs boson is already excluded by the ATLAS and CMS experiments \cite{ATLAS:hzz, CMS:Chatrchyan_2013}, there is a possibility that the Higgs boson is a \CP violating mixture of states with opposite \CP parities. This possibility is discussed in \cite{vukasinovic:2024}, assuming Higgs boson production in $ZZ$-fusion, at 1 TeV ILC, with unpolarised beams. With the full reconstruction of Standard Model background and fast reconstruction of the signal, simulating 8 ab$^{-1}$ of data collected with the ILD detector \cite{ILDConceptGroup:2020sfq}, it is shown that the \CP mixing angle between scalar and pseudoscalar states can be measured with the statistical uncertainty of 3.8 mrad at 68\% CL, corresponding to $f_{\CP} = 1.44 \cdot 10^{-5}$, for the pure scalar state. This is the first result on sensitivity of an $e^{+}e^{-}$ collider to measure $f_{\CP}$ in the Higgs production vertex in vector boson fusion (VBF). Since the study does not assume any particular ILC polarisation scheme, it is a very generic to any (linear) $e^{+}e^{-}$ collider capable to operate at around 1 TeV center-of-mass energy.

The study hypothesized that the 125 GeV Higgs mass eigenstate (\Ph) is a mixture of \CP-even (\PH) and \CP-odd (\PSA) states: $\Ph = \PH \cdot \cos\Psi_{\CP} + \PSA \cdot \sin\Psi_{\CP}$, violating \CP symmetry through non-zero mixing angle $\Psi_{\CP}$. One of the most sensitive observables to $\Psi_{\CP}$ is the angle $\Delta\Phi$ between scattering planes. The dependence of $\Delta\Phi$ distribution minimum to $\Psi_{\CP}$ is determined empirically,  where the position of $\Delta\Phi$ minimum shifts to larger values for increasing positive values of $\Psi_{\CP}$ (and similarly to smaller $\Delta\Phi$ values for negative decreasing mixing angle). The shift for positive mixing angles is illustrated in Fig.~\ref{fig:hzz_angles}.  Position of the minimum of $\Delta\Phi$ distribution can be determined from the reconstructed data by a local fit with the function $f(\Delta\Phi) = A + B \cdot \cos(a \cdot \Delta\Phi - b)$ where A, B, a and b are free parameters of the fit. From the principle of the first derivative, the ratio b/a determines the minimum of $\Delta\Phi$ distribution. For $\Psi_{\CP}$ values up to 200 mrad, dependence of $(b/a)/\Psi_{\CP}$ on true (generated) mixing angle is to a good approximation linear with coefficients $k$ and $m$ determining a slope and a constant term, respectively. Above 200 mrad, the $\chi^2$ of the fit with $f (\Delta\Phi)$ significantly deteriorates. Knowing the parameters $k$ and $m$ from simulation, $\Psi_{\CP}$ values can be determined by solving the quadratic equation: $k \cdot \Psi^{2}_{\CP} + m \cdot \Psi_{\CP} - (b/a) = 0$. From the fit to a single pseudo-experiment, assuming 8 ab$^{-1}$ of data, one can measure $\Psi_{\CP}$\,= (2.4 $\pm$ 4.0) \,mrad. In order to estimate the statistical dispersion of results, 2000 pseudo-experiments are repeated each with 8 ab$^{-1}$ of data. The dispersion of the results assuming a pure scalar state is found to be 3.8 mrad at 68\% CL, as illustrated in Fig.~\ref{fig:hzz_pseudoexp}, corresponding to the absolute statistical uncertainty of the measurement. 

\begin{figure}[h!]  
    \begin{subfigure} {.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/fi_uglovi_mrad_2.pdf}
        \caption{}
        \label{fig:hzz_angles}
    \end{subfigure}
    \quad
    \begin{subfigure}{.5\linewidth}  
        \includegraphics[width=\linewidth]{figs/psi_pseudoexp_new.pdf}
        \caption{}
        \label{fig:hzz_pseudoexp}
    \end{subfigure}
    \caption{ (a) $\Delta\Phi$ distribution for different mixing angles ($\Psi_{\CP}$) illustrating the shift of the $\Delta\Phi$ minimum for non-zero values of $\Psi_{\CP}$. (b) Statistical dissipation of measured $\Psi_{\CP}$ values ($\Psi_{\mathrm{exp}}$) w.r.t. the true ones ($\Psi_{\mathrm{true}}$).}
\end{figure}

To interpret the obtained precision of measurement of the mixing angle in terms of sensitivity to the \CP-odd amplitude $f_{\CP}$, the framework described in \cite{gritsan:2022snowmass} is assumed, that is that $f_{\CP}$ will vary from zero as $\sin^{2}(\Delta(\Psi_{\CP}))$ for the pure scalar state, where $\Delta(\Psi_{\CP})$ is the absolute statistical uncertainty of the mixing angle measurement. The sensitivity of $\Psi_{\CP}$ measurement to $f_{\CP} \sim 10^{-5}$ illustrates the potential of a TeV linear collider to probe Higgs \CP-odd component in VBF Higgs production channels.



==> sections/higgs/tau_entanglement.tex <==
The prospects of quantum information measurement with $\PH \to \PGtm\PGtp$ at future lepton colliders have been studied in Refs.~\cite{Altakach:2022ywa, Ma:2023yvd, Fabbrichesi:2024wcd}.
In this section, we briefly describe the analysis and results presented in \cite{Altakach:2022ywa}.

The spin state of the two tau leptons from the Higgs decay is given by Eq.\ \eqref{eq:pure}.
Assuming the structure of the spin correlation matrix, $C$, in Eq.\ \eqref{eq:Cmat}, the \textit{concurrence} \cite{Hill:1997pfa,Wootters:1997id}, a measure of entanglement, is given by
\begin{equation}
{\cal C}[\rho] = \text{max} \left[ 0,\, \frac{D_{+} + C_{kk} - 1}{2},\,
\frac{D_{-} - C_{kk} - 1}{2} 
\right]
\label{eq:crho_tau}
\end{equation}
with $D_{\pm} \equiv \sqrt{(C_{rn} \pm C_{nr})^2 + (C_{rr} \mp C_{nn})^2}$.
The concurrence is a non-negative function of the spin density operator, $\rho$, and vanishes for all separable (nonentangled) states.
${\cal C}[\rho]$ takes the maximum value 1 for maximally entangled states.
In fact, for the spin state of the tau pair in $\PH \to \PGtm\PGtp$, we have ${\cal C}[\rho] = 1$.

It has been known that maximally entangled 2-qubit states maximally violate Bell inequalities \cite{Bell:1964kc}.  
The CHSH inequality \cite{Clauser:1969ny}, one of the Bell inequalities, is particularly useful.
This is a statement about the combination of spin correlations defined by 
\begin{equation}
R_\text{CHSH} = \frac{1}{2} \left| 
\bra \hat s^A_a \hat s^B_b \ket
- \bra \hat s^A_a \hat s^B_{b'} \ket
+ \bra \hat s^A_{a'} \hat s^B_{b} \ket
+ \bra \hat s^A_{a'} \hat s^B_{b'} \ket
\right|\,,
\label{eq:R}
\end{equation}
where $\hat s^I_i$ ($I = A,B$, $i=a,b$) is the spin $i$-component of particle $I$.
Alice, the observer of particle $A$, has two possible spin measurement axes, $a$ and $a'$, while Bob, the observer of particle $B$, has measurement axes $b$ and  $b'$.
It has been shown that for all Hidden Local Variable (HLV) theories and Quantum Mechanical (QM) theories 
\begin{equation}
R_\text{CHSH} \le \left\lbrace
\begin{array}{ll}
1 &  (\mathrm{HLV} \text{~\cite{Clauser:1969ny}})\\
\sqrt{2} &  (\mathrm{QM} \text{~\cite{Tsirelson}})
\end{array}
\right.
\end{equation}
for all sets of measurement axes $a, a', b$ and $b'$.
Observation of $R_\text{CHSH} > 1$ ($\sqrt{2}$) would, therefore, falsify Hidden Local Variable theories (Quantum Mechanical theories).   
The tau pair from $\PH \to \PGtm\PGtp$ saturate the quantum bound: $R_\text{CHSH}^\text{max} = \sqrt{2}$, where the maximum is taken over all sets of measurement axes. 

Suppose that at the rest frame of $\tau^{-}$ the tau spin is polarised into $\mathbf{s}$ direction ($|\mathbf{ s}| = 1$).  
The $\tau^{-}$ decays into a decay mode, $f$, producing a detectable particle $d$.  
The conditional probability that the particle $d$ takes the direction $\mathbf{u}$ ($|\mathbf{ u}| = 1$) when the $\PGtm$ spin is polarised in $\mathbf{ s}$ direction is given by \cite{Bullock:1992yt}
\begin{equation}
P(\mathbf{ u}|\mathbf{ s}) \, = \, 1 + \alpha_{f,d} \,   \mathbf{ s} \cdot \mathbf{ u}\,,
\label{eq:prob}
\end{equation}
with the normalisation $\int \frac{d \Omega}{4 \pi} P(\mathbf{ u}|\mathbf{ s}) = 1$,
where $\alpha_{f,d} \in [-1, 1]$ is called the spin analyzing power.
For the CP counterpart, $(f,d) \xleftrightarrow{\text{CP}} (\bar f, \bar d)$, $\alpha_{\bar f, \bar d} = - \alpha_{f, d}$.

We denote the $\PGtp$ polarisation by $\mathbf{ \bar s}$ ($|\mathbf{ \bar s}| = 1$). 
The direction of its decay product, $d'$, measured at the rest frame of the $\PGtp$, is represented by a unit vector $\mathbf{ \bar u}$.
We want to relate the spin correlation $\bra \mathbf{ s} \otimes \mathbf{ \bar s} \ket$
with the angular correlation $\bra \mathbf{ u} \otimes \mathbf{ \bar u} \ket$ since the latter is measureable. 
Using the probability distribution \eqref{eq:prob}, one can derive \cite{Altakach:2022ywa}
\begin{equation}
C_{ab} \,=\, \bra s_a \bar s_b \ket \,=\, \frac{9}{\alpha_{f,d} \alpha_{f',d'}} \bra u_a \bar u
_b \ket  \,,
\label{eq:angle-to-spin}
\end{equation}
where $u_a \equiv \mathbf{ u} \cdot \mathbf{ a}$, $\bar s_b \equiv \mathbf{ \bar s} \cdot \mathbf{ b}$, etc.\ are the components with respect to arbitrary unit vectors $\mathbf{ a}$ and $\mathbf{ b}$.
Using this relation, one can compute both the concurrence ${\cal C}[\rho]$ (Eq.\ \eqref{eq:crho_tau}) and the CHSH variable $R_\text{CHSH}$ (Eq.\ \eqref{eq:R}) from the angular correlation observables $\bra u_a \bar u_b \ket$. 
In $\PH \to \PGtm\PGtp$, the set of four measurement axes ($\mathbf{ a}_*$, $\mathbf{ a'}_*$, $\mathbf{ b}_*$, $\mathbf{ b'}_*$) that maximises $R_\text{CHSH}$ is obtained as \cite{Altakach:2022ywa}
\begin{equation}
%&&~~~~~~~~~~~~
\mathbf{ a}_* = \mathbf{ r},~~~\mathbf{ a'}_* = \mathbf{ n}, 
%\nonumber \\
%&&
~~~
\mathbf{ b}_* = \frac{1}{\sqrt{2}} \left( \mathbf{ n} + \mathbf{ r} \right),~~~
\mathbf{ b'}_* = \frac{1}{\sqrt{2}} \left( \mathbf{ n} - \mathbf{ r} \right)\,,
\label{eq:max_abab}
\end{equation}
where $\mathbf{ r}$ and $\mathbf{ n}$ are the two axes in the helicity basis defined in section \ref{sec:CPtau}.
In the following analysis, we fix the measurement axes as above and denote the CHSH variable obtained for those axes by $R_\mathrm{ CHSH}^*$.
The axes of the helicity basis ($\mathbf{ r}, \mathbf{ n}, \mathbf{ k}$) will be used to define the spin correlation matrix $C$.

\paragraph{Analysis}

We demonstrate the quantum information measurement in $\PH \to \PGtm\PGtp$ at future lepton colliders, assuming two collider settings, ILC and FCC-ee, listed in Table \ref{tb:colliders} in section \ref{sec:CPtau}.
In the analysis we focus on $\PGtpm \to \PGppm \PGn$ channel, where the spin analysing power is maximum, $\alpha_{f,d} = 1$ for $f = \PGtm \to \PGpm \PGn$ and $d = \PGpm$.
At lepton colliders, the Higgs is produced via the associated production $\epem \to \PZ \PH$.
From the total initial momentum, $P_\text{in}^\mu = (\sqrt{s}, 0, 0, 0)$ and the reconstructed $\PZ$ momentum, $p_{\PZ}^\mu$,
the Higgs momentum four-vector, $p_{\PH}^\mu$, can be obtained as $p_{\PH}^\mu = P_\text{in}^\mu - p_{\PZ}^\mu$.
The distribution of the recoil mass, $m_\text{recoil} = \sqrt{(P_\text{in} - p_{\PZ})^2}$,
therefore sharply peaks at the Higgs mass in the signal.
By selecting events that fall within a narrow window, $|m_\text{recoil} - m_{\PH}| < 5$ GeV, one can achieve background/signal $\sim 0.05$ with a signal efficiency of $93\%$ and $96\%$ for the ILC and FCC-ee, respectively.  


We generate signal and background events with {\texttt{MadGraph5\_aMC@NLO}}
\cite{Alwall:2014hca} at leading order in the Standard Model, i.e.~$(\kappa, \delta) = (1,0)$.
We employ the {\texttt{TauDecay}} package for $\tau$ decays~\cite{Hagiwara:2012vz}.
The beam energies are smeared according to the parameters in Table \ref{tb:colliders}.
All $Z$-boson decay modes without neutrinos and taus, $Z \to x \bar x$ with $x \bar x = q \bar q$, $e^+ e^-$, $\PGmp \PGmm$,
are included in the analysis.
The expected signal events,
[$\epem \to \PH\PZ$, $Z \to x \bar x$, $\PH \to \PGtp \PGtm$, $\PGtpm \to \PGn\PGppm$],
produced at the ILC and FCC-ee are 414 and 691, respectively.
At the ILC and (FCC-ee), after imposing the requirement, 
$|m_\text{recoil} - m_{\PH}| < 5$ GeV,
385 (663) signal events survive.
We estimated that 20 (36) background events contribute
to this phase-space region. 
We perform 100 pseudo-experiments for each benchmark collider and estimate the statistical uncertainties on the measurements.


On the right-hand-side of Eq.\ \eqref{eq:angle-to-spin},
the direction $u_a$ ($\bar u_b$) is measured at the rest frame of the respective mother tau lepton $\PGtm$ ($\PGtp$).
This means that in order to measure the spin correlation, it is crucial to reconstruct the $\PGtm$ and $\PGtp$ rest frames accurately.   
This requires the precise reconstruction of two neutrino momenta.  
For six unknown neutrino momentum components, there are two mass-shell constraints: $m_\tau^2 = (p_{\PGnGt} + p_{\PGpm})^2$ and $m_\tau^2 = (p_{\PAGnGt} + p_{\PGpp})^2$,
and four conditions from the energy-momentum conservation:
$(P_\text{in} - p_{\PZ})^\mu = (p_{\PGnGt} + p_{\PGpm} + p_{\PAGnGt} + p_{\PGpp})^\mu$.
By solving those six constraints for the six unknowns, an event can be fully reconstructed up to twofold solutions: $i_s = 1,2$. 
The exact method has been developed in \cite{Altakach:2022ywa} by adopting the formalism outlined in \cite{Harland-Lang:2011mlc, Harland-Lang:2012zen, Harland-Lang:2013wxa}.

To take into account the energy mismeasurement, 
we smear the energies of all visible particles in the final state as
%\begin{equation}
$E^\text{true} \,\to\, E^\text{obs} = (1 + \sigma_E \cdot \omega) \cdot E^\text{true}$
%\end{equation}
with the energy resolution $\sigma_E = 0.03$ \cite{FCC:2018evy, Behnke:2013lya}
for both ILC and FCC-ee,
where $\omega$ is a random number drawn from the normal distribution. 

The biggest experimental challenge in the $\PH \to \PGtm\PGtp$ channel is that $\tau$s are heavily boosted because $m_\tau \ll m_{\PH}$.
This means that going back to the rest frame of $\PGtm$ and $\PGtp$, one has to apply large boosts.  
Small reconstruction errors in the lab frame are amplified by the large boosts in the tau rest frame, which often spoil the measurement.  
In fact, it has been demonstrated that entanglement and CHSH violation cannot be observed in the simple kinematical method described above \cite{Altakach:2022ywa}. 

To overcome this problem and refine the accuracy of the reconstruction, we include the impact parameter information. 
Since tau leptons are marginally long-lived, $c \tau = 87.11$ $\mu$m \cite{Workman:2022ynf}, and highly boosted, one can observe a mismatch between the interaction point and the origin of the $\PGppm$ in $\PGtpm \to \PGn\PGppm$.
The impact parameter $\vec{b}_\pm$ is the minimal displacement of the extrapolated $\PGppm$ trajectory from the interaction point. 
The magnitude of the impact parameter $|\vec b_{\pm}|$ follows an exponentially falling distribution with the mean $|\vec b_{\pm}| \sim 100 \, \mu$m for $E_{\PGtpm} \sim m_{\PH}/2$,
which is significantly larger than the experimental resolutions \cite{Behnke:2013lya}.
In our numerical simulation, 
we take constant values 
$\sigma_{b_T} = 2 \, \mu$m (transverse)
and $\sigma_{b_z} = 5 \, \mu$m (longitudinal) 
for the impact parameter resolutions,
although the actual resolutions are 
functions of the track momentum and
the polar angle $\theta^*$ from the beam direction.
The above modeling with the constant parameters gives a reasonable approximation for
the track momentum $\sim 100$ GeV
and $\theta^* \gtrsim 20^\circ$ 
as can be seen in Figure II-3.10 in ref.\ 
\cite{Behnke:2013lya}.


If all quantities are accurately measured, the impact parameter, ${\vec{b}_\pm}$, from the $\PGtpm \to \PGn\PGppm$ decay,
is related to the directions of $\taup$ and $\pip$
and their angle $\Theta_\pm$ by \cite{Hagiwara:2016zqz}
\begin{equation}
\vec b_{\pm} \,=\, |\vec b_{\pm}| \cdot \left[ \mathbf{ e}_{\taupm}  \cdot \sin^{-1} \Theta_{\pm} 
\,-\, \mathbf{ e}_{\pipm} \cdot \tan^{-1} \Theta_{\pm}   \right]
\,\equiv\, \vec b_{\pm}^{\text{reco}} \left( \mathbf{ e}_{\taupm} \right)
\,,
\label{eq:b}
\end{equation}
where $\mathbf{ e}_{\taupm}$ and $\mathbf{ e}_{\pipm}$ 
are the unit vectors pointing to the directions of $\tau^{\pm}$ and $\pi^{\pm}$, respectively, and $\cos \Theta_{\pm} \equiv (\mathbf{ e}_{\taupm} \cdot \mathbf{ e}_{\pipm})$.
In the second line, we defined a 3-vector function
$\vec b_{\pm}^{\text{reco}} \left( \mathbf{ e}_{\taupm}  \right)$ and emphasised its dependence on $\mathbf{ e}_{\taupm}$.

We use this information to curb the effects of energy mismeasurement.
First, we shift the energy of a visible particle $\alpha$ ($\alpha = \PGppm, x, \bar x$) from the observed value as
%\begin{equation}
$E^\text{obs}_{\alpha} \to E_{\alpha}(\delta_\alpha) = (1 + \sigma_E \cdot \delta_\alpha) \cdot E_{\alpha}^\text{obs}$\,,
%\end{equation}
where $\delta_\alpha$ is a nuisance parameter characterising the amount of the shift with respect to the energy resolution $\sigma_E$.
Using these shifted energies, we solve the kinematical constraints, as outlined in \cite{Altakach:2022ywa}, and obtain the tau directions as functions of the nuisance parameters, $\mathbf{ e}^{i_s}_{\taupm}( \pmb{\delta} )$, up to twofold solutions, $i_s = 1,2$,
where $\pmb{\delta} = \{ \delta_{\PGpp}, \delta_{\PGpm}, \delta_x, \delta_{\bar x} \}$.
Based on the mismatch between the {\textit{observed}}
and {\textit{reconstructed}} impact parameters,
%\begin{equation}
$\vec \Delta^{i_s}_{b_\pm}( \pmb{\delta} ) 
\,\equiv\, 
\vec b_\pm - \vec b_\pm^\text{reco} \left( \mathbf{ e}^{i_s}_{\taup} ( \pmb{\delta} )
\right)$\,,
%\end{equation}
we define a contribution to the log-likelihood for a solution $i_s$ as
%\begin{equation}
$L^{i_s}(\pmb{ \delta }) \,=\, L^{i_s}_{+}(\pmb{ \delta }) + L^{i_s}_{-}(\pmb{ \delta })$
%\end{equation}
with
\begin{equation}
L^{i_s}_{\pm}(\pmb{\delta}) \,=\, \frac{ [\Delta^{i_s}_{b_\pm}( \pmb{\delta} )]_x^2 + [\Delta^{i_s}_{b_\pm}( \pmb{\delta} )]_y^2 }{ \sigma^2_{b_T} } \,+\,
\frac{ [\Delta^{i_s}_{b_\pm}( \pmb{\delta} )]_z^2 }{ \sigma^2_{b_z} }\,.
\end{equation}
The total log-likelihood function is then defined as
\begin{equation}
L(\pmb{\delta}) \,=\, \text{min} \left[ L^1( \pmb{\delta} ), L^2( \pmb{\delta} ) \right] \,+\, \delta_{\PGpp}^2\,+\, \delta_{\PGpm}^2\,+\, \delta_{x}
^2\,+\, \delta_{\bar x}^2 \,.
\end{equation}

The log-likelihood function, $L(\pmb{ \delta })$, is to  be minimised over the nuisance parameters, $\pmb{ \delta }$.
We denote the location of the minimum by $\pmb{ \delta}^* $.
We define ``the most likely'' solution $i_*$ as the solution that gives the smaller $L^{i_s}$, i.e.\
$
L^{i_*}( \pmb{ \delta}^* ) \,=\,
\text{min} \left[ L^1( \pmb{ \delta}^*), L^2(\pmb{ \delta}^*) \right]\,.
$
Our best guess for the tau lepton momenta is, therefore, given by 
%\begin{equation}
$p_{\taupm}^* = p^{i_*}_{\taupm}(\pmb{ \delta}^* )$\,.
%\end{equation}
We use $p_{\taupm}^*$ in the quantum property measurements. 


%\onecolumngrid
\begin{table*}[t!]
\begin{center}
\begin{tabular}{|c || c |} 
 \hline
  & ~~~ILC~~~ \\ 
 \hline \hline
 $C_{ij}$ & 
 $\begin{pmatrix} 
 0.830 \pm 0.176 & 0.020 \pm 0.146 & -0.019 \pm 0.159 \\
 -0.034 \pm 0.160 & 0.981 \pm 0.1527 & -0.029 \pm 0.156 \\
 -0.001\pm 0.158 & -0.021 \pm 0.155 & -0.729\pm 0.140
 \end{pmatrix}$
  \\ 
 \hline
 ${\cal C}[\rho]$  & $0.778\pm 0.126$   \\
 \hline
 $R_\text{CHSH}^*$ & $1.103 \pm 0.163$  \\
 \hline
\end{tabular}
%
\vspace{3mm}
~\\
~\\
%
\begin{tabular}{|c || c |} 
 \hline
  & ~~~FCC-ee~~~ \\ 
 \hline \hline
 $C_{ij}$ & 
 $\begin{pmatrix} 
 0.925 \pm 0.109 & -0.011 \pm 0.110 & 0.038 \pm 0.095 \\
 -0.009 \pm 0.110  & 0.929 \pm 0.113  & 0.001 \pm 0.115  \\
 -0.026 \pm 0.122  & -0.019 \pm 0.110  & -0.879 \pm 0.098  
 \end{pmatrix}$
  \\ 
 \hline
 ${\cal C}[\rho]$  & $0.871 \pm 0.084$   \\
 \hline
 $R_\text{CHSH}^*$ & $1.276 \pm 0.094$  \\
 \hline
\end{tabular}
%
%
\end{center}
\caption{Result of quantum property measurements with a log-likelihood method incorporating the impact parameter information.
\label{tb:result_2}}
\end{table*}
%


In Table \ref{tb:result_2} we show the result of our quantum information measurements. 
We see that for both ILC and FCC-ee the components of the $C$-matrix are correctly measured.  
The concurrence ${\cal C}[\rho]$
is also measured with good accuracy. 
and the formation of entanglement is observed at
more than 5\,$\sigma$.
Observation of CSHS violation is the most challenging one since it is the strongest quantum correlation.
As can be seen in the last line in Table \ref{tb:result_2},
the violation of the CHSH inequality is confirmed at the FCC-ee at $\sim 3\,\sigma$ level,
while $R^{*}_\text{CHSH} > 1$ is not observed at the ILC beyond the statistical uncertainty.
The superior performance of FCC-ee is attributed to the fact that the beam energy resolution of FCC-ee is much better than ILC.
The precise knowledge of the initial state momentum is crucial to reconstruct the rest frame of $\PGtpm$ accurately.


==> sections/higgs/zhang.tex <==

%\subsubsection{\CP-even coupling studies}
$\PZ\PH$ production and decay provides sensitivity to Higgs-boson properties and couplings, and can be used to test fundamental principles of quantum mechanics.  The $\PZ\PH$ cross-section is affected by modifications to the Higgs-boson mass, width, or self-coupling.  Prospects for cross-section measurements have recently been investigated for the FCC-ee, and sensitivity to Higgs-boson properties have been determined.  Results are presented in Sections ~\ref{sec:HiggsMass} and~\ref{sec:HiggsWidth}.  
The $\PZ\PH$ cross-section is also affected by \CP-even modifications to the $\PH\PZ\PZ$ coupling.  The sensitivity of a dedicated measurement of this coupling at CLIC using the $\PH\to \PZ\PZ$ decay is described in Section~\ref{sec:HZZCLIC}.  

\CP-odd modifications to the $\PH\PZ\PZ$ coupling affect the angular distributions of the final-state fermions from the $\PZ$-boson decay.  A sensitivity study at the FCC-ee using a matrix-element-based observable is described in Sec.~\ref{sec:HZZCPFCC}, and a separate study investigating neural-network-based observables is presented in Sec.~\ref{sec:HZZCP}.  The potential for improving \CP sensitivity using polarized beams is discussed in Sec.~\ref{sec:hzzcppol}.  Finally, the potential for probing the \CP properties of HVV couplings at a $\sqrt{s}=1$ TeV ILC is described in Sec.~\ref{sec:HVVCPILC}.

The primary programme of $\epem \to \PZ\PH$ production is to measure the Higgs-boson couplings to unrivalled precision.  There are ongoing studies to improve estimates of the $\PH\tau\tau$ coupling sensitivity at the FCC (Sec.~\ref{sec:Htautau}), and there has been a recent estimate of the \CP sensitivity to this coupling (Sec.~\ref{sec:HtautauCP}).  These decays can also be used to demonstrate quantum entanglement in the Higgs-boson decay, as discussed in Sec.~\ref{sec:Httentangle}.  Quantum entanglement tests can also be performed using $\PH \to \PV\PV$ decays (Sec.~\ref{sec:HVVentangle}).

\subsubsection{\texorpdfstring{Higgs boson mass and model-independent $\PZ\PH$ cross-section at FCC-ee}{Higgs boson mass and model-independent ZH cross-section at FCC-ee}}
\label{sec:HiggsMass}
\editor{Jan Eysermans - abstract 67}
\input{./sections/higgs/hmass.tex}

\subsubsection{\texorpdfstring{Higgs boson width from the $\PZ\PH, \PH \to \PZ\PZ^*$ cross section measurement at the FCC-ee}{Higgs boson width from the ZH, H -> ZZ* cross section measurement at the FCC-ee}}
\label{sec:HiggsWidth}
\editor{Nicolas Morange - abstract 95}
\input{./sections/higgs/hwidth.tex}

\subsubsection{\texorpdfstring{$\PH\to\PZ\PZ$ coupling sensitivity at CLIC}{H->ZZ coupling sensitivity at CLIC}}
\label{sec:HZZCLIC}
\editor{Ivanka Bozovic - abstract 6}
\input{./sections/higgs/hzzclic.tex}

%\subsubsection*{$\PH\to\PZ\PZ$ coupling sensitivity to angular observables}
%\author{Jiayin Gu}

%\subsubsection{\CP-odd coupling studies}

\subsubsection{\texorpdfstring{$\PH\PZ\PZ$ \CP studies at the FCC}{HZZ CP studies at FCC-ee}}
\label{sec:HZZCPFCC}
\editors{Andrei Gritsan, Nicholas Pinto, Valdis Slokenbergs - abstract 84}
\input{sections/higgs/hzzcpfcc.tex}

\subsubsection{\texorpdfstring{Improving $\PH\PZ\PZ$ \CP constraints with neural-network-based observables}{Improving HZZ CP constraints with neural-network-based observables}}
\label{sec:HZZCP}
\editor{Aidan Robson - abstract 74}
\input{sections/higgs/cpinhzz.tex}

\subsubsection{\texorpdfstring{\CP tests with polarised beams}{CP tests with polarised beams}}
\label{sec:hzzcppol}
\editor{Cheng Li - abstract 66}
\input{sections/higgs/hzzcppol.tex}

\subsubsection{\texorpdfstring{$\PH\PV\PV$ \CP studies at the ILC with $\sqrt{s}=1$~TeV}{HVV CP studies at the ILC with sqrt(s)=1 TeV}}
\label{sec:HVVCPILC}
\editor{Ivanka Bozovic - abstract 3}
\input{./sections/higgs/ilccphvv.tex}

\subsubsection{\texorpdfstring{$\PH\to\PGt\PGt$ coupling sensitivity at FCC-ee}{H->tau tau coupling sensitivity at FCC-ee}}
\label{sec:Htautau}
\editor{Sofia Giappichini - abstract 46}
\input{./sections/higgs/htautau.tex}

\subsubsection{\texorpdfstring{\CP studies in $\PH\to\PGt\PGt$}{CP studies in H->tau tau}}
\label{sec:HtautauCP}
\editor{Kazuki Sakurai}
\input{./sections/higgs/cptautau.tex}

\subsubsection{\texorpdfstring{Entanglement in $\PH\to\PGt\PGt$}{Entanglement in H->tau tau}}
\label{sec:Httentangle}
\editor{Kazuki Sakurai}
\input{./sections/higgs/tau_entanglement.tex}

\subsubsection{\texorpdfstring{Entanglement in $\PH\to\PV\PV$}{Entanglement in H->VV}}
\label{sec:HVVentangle}
\editor{Juan Antonio Aguilar Saavedra}
\input{./sections/higgs/hvventangle.tex}

%\subsubsection{Models of \CP violation in the Higgs sector}
%\editor{Gudrid Moortgat-Pick}


==> sections/introduction/formatting.tex <==
\section*{Document formatting convention requests \textcolor{red}{--- everyone please read!}}

\subsection*{Particle symbols}
\noindent For particles, please use the \texttt{heppennames2} package (included).

\noindent For example:
\begin{itemize}[nosep]
\item $\PQt\PAQt$ is \verb+$\PQt\PAQt$+ (which also has the local alias \verb+\ttbar+)
\item $\PH\to\PQb\PAQb$ is \verb+$\PH\to\PQb\PAQb$+ (which also has the local alias \verb+\Hbb+)
\end{itemize}
Please feel free to add other useful aliases to the relevant section of \texttt{ECFAreport\_definitions.sty}.

\subsection*{Units}
\noindent For units, please use the \texttt{siunitx} package.

\noindent For example:
\begin{itemize}[nosep]
\item \SI{3.1}{\per\atto\barn} is \verb+\SI{3.1}{\per\atto\barn}+
\item \SI{3.45d-4}{\micro\metre} is \verb+\SI{3.45d-4}{\micro\metre}+
\item \SI{13}{\giga\electronvolt} is \verb+\SI{13}{\giga\electronvolt}+
\end{itemize}

\subsection*{References}
\noindent
suggestion by Dirk:
Please use the \texttt{cleveref} package via the commands \texttt{\textbackslash cref} command which takes care of Fig. or Figure in an automatic way. Capitalize 
the c at the beginning of a sentence etc \texttt{\textbackslash Cref}

\subsection*{Captions}
Captions for figures and tables are put at the bottom.

\subsection*{Paper References}
\noindent Please use the \texttt{\textbackslash cite} commands, and \texttt{\textbackslash biber},
For example \verb+\cite{deBlas:2024bmz}+ \cite{deBlas:2024bmz}.


==> sections/introduction/physicslandscape.tex <==
\subsection{Physics Landscape Overview}





==> sections/searches/srch-det/srch-det.tex <==
\subsubsection{Key detector design issues}



==> sections/searches/srch-hdec/srch-hdec.tex <==
\subsubsection{Exotic Higgs boson decays (including invisible)}


\begin{itemize}
    \item     Gen. level: https://arxiv.org/abs/1612.09284 
    \item     $H\to 4\tau $: https://arxiv.org/abs/2110.13225 
    \item    $H\to inv$:
\begin{itemize}
       \item ILD: https://arxiv.org/abs/2002.12048  to be reexamined
       \item SiD: https://arxiv.org/abs/2203.08330 
       \item CLIC: https://arxiv.org/abs/2002.06034 
\end{itemize}
\end{itemize}



==> sections/searches/srch-polar/srch-polar.tex <==
\subsubsection{Role of polarization}



==> sections/searches/srch-syst/srch-syst.tex <==
\subsubsection{Key challenges in systematics}




==> sections/searches/srch-zdec/srch-zdec.tex <==


